The OPTX Project I: The Flux and Redshift Catalogs for the CLANS, CLASXS, and CDF-N fields

We present the redshift catalogs for the X-ray sources detected in the Chandra Deep Field North (CDF-N), the Chandra Large Area Synoptic X-ray Survey (CLASXS), and the Chandra Lockman Area North Survey (CLANS). The catalogs for the CDF-N and CLASXS fields include redshifts from previous work, while the redshifts for the CLANS field are all new. For fluxes above 10^-14 ergs cm^-2 s^-1 (2-8 keV) we have redshifts for 76% of the sources. We extend the redshift information for the full sample using photometric redshifts. The goal of the OPTX Project is to use these three surveys, which are among the most spectroscopically complete surveys to date, to analyze the effect of spectral type on the shape and evolution of the X-ray luminosity functions and to compare the optical spectral types with the X-ray spectral properties. We also present the CLANS X-ray catalog. The nine ACIS-I fields cover a solid angle of ~0.6 square degrees and reach fluxes of 7x10^-16 ergs cm^-2 s^-1 (0.5-2 keV) and 3.5x10^-15 ergs cm^-2 s^-1 (2-8 keV). We find a total of 761 X-ray point sources. Additionally, we present the optical and infrared photometric catalog for the CLANS X-ray sources, as well as updated optical and infrared photometric catalogs for the X-ray sources in the CLASXS and CDF-N fields. The CLANS and CLASXS surveys bridge the gap between the ultradeep pencil-beam surveys, such as the CDFs, and the shallower, very large-area surveys. As a result, they probe the X-ray sources that contribute the bulk of the 2-8 keV X-ray background and cover the flux range of the observed break in the logN-logS distribution. We construct differential number counts for each individual field and for the full sample.

==> tab11.tex <==
\begin{table}
\begin{scriptsize}
\caption{CLANS Optical/IR Counterparts Catalog}
\label{CLANSopt table}
\begin{tabular}{ccccccccccccccc}
\tableline\tableline
    \#&       RA&      DEC&   $g'$&   $r'$&   $i'$&   $z'$&   $J$&   $H$&   $K$&$3.6~\mu$m& $24~\mu$m&z$_{spec}$&z$_{phot}$& class\\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)& (10)&(11) & (12) & (13) & (14) & (15) \\
\tableline
     1&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
     2&  160.642&   59.176& 23.04& 22.40& 21.91& 21.78& 21.02& 19.80&-99.00& 19.50&-99.00&     1.43& -3.00&    4\\
     3&  160.642&   59.169& 25.43& 25.04& 24.40& 23.71& 22.53& 21.93&-99.00&-99.00&-99.00&    -1.00&  1.35&   -1\\
     4&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
     5&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.87&-99.00&    -1.00&-99.00&   -1\\
     6&  160.669&   59.254& 25.30& 24.36& 23.18& 22.31& 21.37& 20.91&-99.00& 20.57&-99.00&    -1.00&  0.95&   -1\\
     7&  160.672&   59.208& 23.27& 21.69& 20.42& 19.96& 19.51& 18.92&-99.00& 18.82&-99.00&    -1.00&  0.55&   -1\\
     8&  160.673&   59.233&-99.00&-99.00&-99.00&-99.00& 22.19& 21.66&-99.00& 20.27& 17.96&    -1.00&-99.00&   -1\\
     9&  160.676&   59.224& 24.22& 23.12& 22.08& 21.68& 21.25& 20.63&-99.00&-99.00&-99.00&     0.72& -3.00&    3\\
    10&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    11&  160.700&   59.252& 24.67& 24.08& 23.28& 22.58& 22.15& 21.56&-99.00& 20.94&-99.00&    -1.00&  0.55&   -1\\
    12&  160.711&   59.212&-99.00&-99.00& 23.46& 23.14& 23.31&-99.00&-99.00&-99.00&-99.00&     2.71& -3.00&    4\\
    13&  160.714&   59.200& 21.58& 21.28& 20.52& 20.20& 19.96& 19.54&-99.00& 18.89& 16.77&     0.78& -3.00&    4\\
    14&  160.716&   59.192& 22.42& 21.41& 20.43& 20.07& 19.67& 19.10&-99.00& 19.10&-99.00&    -1.00&  0.55&   -1\\
    15&  160.722&   59.173& 22.60& 21.26& 20.17& 19.78& 19.22& 18.56&-99.00& 18.18& 15.99&     0.57& -3.00&    1\\
    16&  160.726&   59.151&-99.00& 25.02& 24.12& 23.23& 22.61&-99.00&-99.00& 20.99&-99.00&     0.00&  1.05&  -99\\
    17&  160.727&   59.170&-99.00& 24.64& 24.55&-99.00&-99.00& 21.49&-99.00& 19.75& 17.03&     2.50& -3.00&    3\\
    18&  160.733&   59.074& 21.73& 21.31& 21.01& 20.53& 19.91& 19.60&-99.00& 18.08& 16.62&     2.76& -3.00&    4\\
    19&  160.737&   58.959& 23.00& 22.74& 22.26& 21.89& 21.59& 21.10&-99.00& 20.57&-99.00&    -1.00&  0.25&   -1\\
    20&  160.738&   59.239& 23.03& 22.80& 22.34& 22.07& 20.77& 20.40&-99.00& 19.23& 17.49&     1.54& -3.00&    1\\
    21&  160.744&   59.161& 24.58& 23.96& 23.00& 22.08& 21.07& 20.61&-99.00& 19.52&-99.00&    -1.00&  1.25&   -1\\
    22&  160.761&   59.219& 24.69& 23.45& 22.31& 21.52& 20.64& 20.00&-99.00& 19.56&-99.00&     1.02& -3.00&    1\\
    23&  160.765&   58.955& 21.94& 20.54& 19.56& 19.12& 18.65& 18.14&-99.00& 17.64& 14.68&    -1.00&  0.55&   -1\\
    24&  160.768&   59.109& 20.39& 19.48& 19.12& 18.79& 18.46& 18.33&-99.00& 18.58& 16.25&     0.33& -3.00&    3\\
    25&  160.771&   59.031& 24.18& 23.70& 23.08& 22.59& 21.90& 22.10&-99.00& 21.34&-99.00&    -1.00&-99.00&   -1\\
    26&  160.774&   58.947& 17.55& 17.14& 16.92& 16.74& 16.60& 16.35&-99.00& 17.19& 15.53&     0.05& -3.00&    1\\
    27&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.62&-99.00&     0.00&-99.00&  -99\\
    28&  160.779&   59.214& 25.33&-99.00& 24.15& 23.77& 22.34&-99.00&-99.00& 20.58&-99.00&    -1.00&  1.35&   -1\\
    29&  160.782&   59.202& 23.56& 23.28& 22.84& 22.70& 21.66& 21.10&-99.00& 19.71& 16.91&     0.00&  1.55&  -99\\
    30&  160.784&   59.056& 21.74& 21.12& 21.26& 20.91& 20.33& 20.59&-99.00& 19.58& 17.35&     0.95& -3.00&    4\\
    31&  160.787&   59.203& 22.91& 21.56& 20.61& 20.21& 19.72& 19.10&-99.00& 18.85& 16.90&    -1.00&  0.55&   -1\\
    32&  160.792&   59.281& 23.85& 23.29& 22.66& 21.90& 21.21& 20.54&-99.00& 19.87&-99.00&    -1.00&  0.95&   -1\\
    33&  160.793&   58.988& 24.13& 23.95& 23.42& 22.98& 21.78& 21.56&-99.00& 20.47& 17.41&     1.44& -3.00&    3\\
    34&  160.797&   59.191& 23.24& 23.09& 22.76& 22.69& 21.84&-99.00&-99.00& 20.71&-99.00&    -1.00&-99.00&   -1\\
    35&  160.799&   59.104& 24.76& 24.30& 23.56& 23.00& 21.45& 21.03&-99.00& 19.89&-99.00&    -1.00&  1.65&   -1\\
    36&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
    37&  160.805&   59.173& 24.51& 23.22& 22.35& 21.97& 21.80& 21.89&-99.00&-99.00&-99.00&    -1.00&  0.15&   -1\\
    38&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.38& 17.69&    -1.00&-99.00&   -1\\
    39&  160.810&   59.165&-99.00&-99.00&-99.00&-99.00& 20.18& 19.90&-99.00& 19.27&-99.00&     0.82& -3.00&    1\\
    40&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
    41&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.55&-99.00&    -1.00&-99.00&   -1\\
    42&  160.819&   59.185& 22.21& 21.90& 21.66& 21.39& 21.52& 21.35&-99.00& 21.32&-99.00&     0.00&  0.25&  -99\\
    43&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    44&  160.826&   59.174& 21.41& 21.23& 21.07& 20.89& 21.11& 21.02&-99.00& 20.16&-99.00&    -1.00&  1.75&   -1\\
    45&  160.827&   59.001& 23.58& 23.87& 23.48& 23.15& 22.68&-99.00&-99.00& 21.64&-99.00&     2.48& -3.00&    4\\
    46&  160.833&   59.144& 23.96& 22.87& 22.38& 21.79& 21.13& 20.91&-99.00& 19.44&-99.00&     1.27& -3.00&    3\\
    47&  160.834&   58.838& 21.08& 21.02& 21.00& 20.82& 20.75& 20.75&-99.00& 20.41& 18.31&    -1.00&  2.65&   -1\\
    48&  160.835&   59.072& 19.10& 18.35& 17.96& 17.74& 17.60& 17.62& 17.92& 18.84&-99.00&    -2.00&-99.00&   -2\\
    49&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.40&-99.00&    -1.00&-99.00&   -1\\
    50&  160.836&   58.939& 20.51& 19.09& 18.50& 18.20& 17.77& 17.59& 17.32& 17.96&-99.00&     0.35& -3.00&    0\\
    51&  160.837&   58.897& 23.04& 22.95& 22.66& 22.41& 21.42& 21.15&-99.00& 20.21&-99.00&    -1.00&  0.85&   -1\\
    52&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    53&  160.838&   59.032& 21.93& 21.33& 21.60& 21.15& 20.94& 20.49& 20.05& 19.53& 17.12&     1.44& -3.00&    4\\
    54&  160.839&   59.162& 21.04& 20.28& 19.64& 19.37& 19.13& 18.93& 19.14& 18.30& 15.46&     0.41& -3.00&    4\\
    55&  160.841&   59.119& 23.57& 23.17& 22.79& 22.57& 21.76& 21.59&-99.00& 20.13&-99.00&     0.00&  0.55&  -99\\
    56&  160.841&   59.215& 20.92& 20.34& 19.76& 19.47& 19.23& 18.96& 18.44& 18.30& 16.52&     0.68& -3.00&    4\\
    57&  160.842&   58.822& 21.77& 21.29& 20.71& 20.27& 19.89& 19.77&-99.00& 18.89& 17.12&    -1.00&  0.75&   -1\\
    58&  160.842&   59.114& 25.54& 25.09& 23.87& 23.06& 21.62& 21.08&-99.00& 20.28&-99.00&     0.00&  1.55&  -99\\
    59&  160.845&   58.999& 21.78& 21.86& 21.51& 21.46& 21.67& 21.10&-99.00& 20.49&-99.00&     1.72& -3.00&    4\\
    60&  160.846&   59.271&-99.00& 22.88& 22.59& 22.62& 22.15& 22.06&-99.00& 20.77&-99.00&     0.00&  0.35&  -99\\
    61&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    62&  160.848&   58.880&-99.00& 24.30& 23.74& 23.98&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    63&  160.852&   59.166&-99.00& 25.17& 23.92& 22.79& 21.99& 21.80&-99.00& 21.02&-99.00&    -1.00&  1.15&   -1\\
    64&  160.854&   59.286& 22.12& 21.38& 20.40& 19.70& 19.35& 19.03& 18.45& 17.98& 16.44&     1.07& -3.00&    1\\
    65&  160.862&   58.917& 22.99& 22.91& 22.83& 22.91&-99.00&-99.00&-99.00&-99.00&-99.00&     3.15& -3.00&    3\\
    66&  160.864&   59.093& 25.27& 24.84& 24.00& 23.39& 22.38&-99.00&-99.00& 20.80&-99.00&     1.30& -3.00&    1\\
    67&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.73&-99.00&     0.00&-99.00&  -99\\
    68&  160.882&   58.877& 25.04& 24.46& 23.86& 23.32& 21.66& 21.12& 20.54& 19.52& 17.61&     0.00&  1.35&  -99\\
    69&  160.884&   59.061& 22.83& 22.21& 21.65& 21.35& 21.02& 20.71& 20.87& 20.59&-99.00&     0.51& -3.00&    3\\
    70&  160.885&   58.901& 22.82& 22.50& 22.14& 21.53& 21.06& 20.92& 20.19& 19.86&-99.00&     1.00& -3.00&    3\\
    71&  160.886&   58.974& 21.97& 21.58& 21.31& 20.93& 20.42& 20.37& 19.96& 19.53& 17.26&     1.00& -3.00&    1\\
    72&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
    73&  160.886&   58.920&-99.00& 24.94& 24.94&-99.00&-99.00&-99.00&-99.00& 21.42&-99.00&     0.00&  0.95&  -99\\
    74&  160.888&   58.848& 23.35& 22.61& 22.63& 22.26& 21.80&-99.00&-99.00& 20.32&-99.00&     1.38& -3.00&    4\\
    75&  160.889&   58.828& 24.74& 23.93&-99.00&-99.00& 20.43& 20.19& 19.48& 18.87&-99.00&     0.75& -3.00&    0\\
    76&  160.892&   59.025& 23.85& 22.92& 21.93& 21.19& 20.60& 20.52& 20.19& 19.60&-99.00&     0.95& -3.00&    1\\
    77&  160.893&   58.938& 25.18& 24.40& 25.11& 24.40&-99.00&-99.00&-99.00&-99.00&-99.00&     1.29& -3.00&    4\\
    78&  160.897&   59.275&-99.00& 22.67& 21.72& 21.32& 20.72& 20.47& 20.11& 19.58&-99.00&     0.83& -3.00&    1\\
    79&  160.898&   58.973& 24.17& 23.10& 22.03& 21.18& 20.46& 20.27& 19.65& 18.86&-99.00&    -1.00&  1.15&   -1\\
    80&  160.899&   58.978& 24.07& 23.41&-99.00& 21.97& 20.92& 20.68& 19.88& 18.90& 17.24&     1.30& -3.00&    1\\
    81&  160.898&   58.880&-99.00&-99.00&-99.00&-99.00& 16.92& 16.83& 16.46& 17.04& 16.00&     0.23& -3.00&    3\\
    82&  160.901&   59.289& 25.36& 24.55& 23.52& 22.76& 21.37& 21.03& 20.55& 19.93&-99.00&     0.00&  1.65&  -99\\
    83&  160.901&   59.044& 22.36& 22.13& 21.38& 20.97& 20.40& 20.25& 19.81& 19.71&-99.00&     0.85& -3.00&    3\\
    84&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
    85&  160.909&   58.847&-99.00&-99.00&-99.00& 23.48&-99.00&-99.00&-99.00& 20.62&-99.00&    -1.00&-99.00&   -1\\
    86&  160.914&   59.034& 22.91& 21.48& 20.66& 20.25& 19.71& 19.31& 18.98& 18.94& 17.49&     0.52& -3.00&    3\\
    87&  160.914&   58.883& 24.92& 24.59& 23.98& 23.52& 22.21& 21.55&-99.00& 20.67& 18.12&    -1.00&  1.25&   -1\\
    88&  160.918&   59.051& 24.91& 24.35& 23.37& 22.44& 21.27& 20.90& 20.20& 19.42&-99.00&     1.34& -3.00&    1\\
    89&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.99&-99.00&     0.00&-99.00&  -99\\
    90&  160.922&   59.006& 25.48& 24.94& 24.70& 23.96& 22.21& 21.78& 21.05& 21.16&-99.00&    -1.00&  1.55&   -1\\
    91&  160.923&   59.282& 17.41& 17.09& 16.95& 16.80& 16.84& 16.82& 17.04& 17.60& 16.37&     0.03& -3.00&    1\\
    92&  160.923&   59.215& 24.94& 24.12& 23.19& 22.62& 21.53& 20.92& 20.63& 19.85&-99.00&    -1.00&  1.25&   -1\\
    93&  160.923&   59.299& 22.11& 21.92& 21.42& 21.20& 21.46& 21.63& 20.77& 19.80& 17.49&     1.92& -3.00&    4\\
    94&  160.928&   58.892& 23.18& 22.04& 21.14& 20.75& 20.24& 20.02& 19.59&-99.00&-99.00&     0.61& -3.00&    0\\
    95&  160.929&   58.892& 24.04& 23.53& 22.80& 22.17& 20.89& 20.46& 19.96& 19.09& 18.03&    -1.00&  1.55&   -1\\
    96&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.79&-99.00&     0.00&-99.00&  -99\\
    97&  160.930&   59.133& 23.13& 21.89& 20.53& 20.06& 19.48& 19.09& 18.68& 18.75&-99.00&    -1.00&  0.65&   -1\\
    98&  160.930&   58.927& 20.27& 19.59& 19.13& 18.83& 18.56& 18.38& 17.77& 17.48& 15.62&     0.47& -3.00&    4\\
    99&  160.932&   58.852& 23.75& 22.61& 21.42& 20.96& 20.34& 20.03& 19.58& 19.46&-99.00&     0.78& -3.00&    1\\
   100&  160.933&   59.238& 24.00& 22.67& 21.53& 21.10& 20.53& 20.11& 19.76& 19.82&-99.00&     0.68& -3.00&    1\\
   101&  160.932&   58.837& 21.88& 21.46& 21.40& 21.13& 20.96& 21.10& 20.94& 20.64&-99.00&     1.41& -3.00&    4\\
   102&  160.933&   59.141& 22.34& 20.72& 20.17& 19.83& 19.46& 19.25& 18.94& 19.24&-99.00&     0.45& -3.00&    3\\
   103&  160.939&   58.918&-99.00& 22.47& 22.06& 21.95& 21.51& 21.64& 21.40& 21.18&-99.00&     3.61& -3.00&    4\\
   104&  160.946&   58.965&-99.00&-99.00&-99.00&-99.00& 23.01&-99.00&-99.00& 21.98&-99.00&     0.00&-99.00&  -99\\
   105&  160.948&   58.709& 24.08& 23.96& 23.78& 23.55&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.45&   -1\\
   106&  160.949&   59.156& 25.30& 25.19& 25.12& 24.35& 22.76&-99.00&-99.00& 21.17&-99.00&    -1.00&  1.45&   -1\\
   107&  160.954&   58.928& 24.42& 24.30& 24.10& 23.74&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   108&  160.960&   58.670& 23.03& 22.93& 22.93& 22.79& 22.55& 21.56&-99.00& 21.25&-99.00&    -1.00&  0.25&   -1\\
   109&  160.962&   58.676&-99.00&-99.00&-99.00&-99.00& 15.55& 15.29& 15.81& 16.77&-99.00&    -2.00&-99.00&   -2\\
   110&  160.964&   58.956& 22.53& 22.23& 22.21& 21.71& 21.58& 21.29& 20.83& 20.08& 17.13&     2.59& -3.00&    4\\
   111&  160.964&   58.929& 22.21& 20.42& 19.77& 19.55& 19.19& 19.06& 18.52& 18.50& 17.21&     0.60& -3.00&    3\\
   112&  160.964&   58.827&-99.00&-99.00&-99.00&-99.00&-99.00& 21.89&-99.00& 20.87&-99.00&    -1.00&-99.00&   -1\\
   113&  160.966&   58.832& 24.39& 23.22& 22.17& 21.96& 21.57& 21.29& 20.89& 20.24& 16.61&     0.61& -3.00&    3\\
   114&  160.972&   59.289& 21.00& 20.77& 20.75& 20.76& 20.50& 20.69& 20.86& 20.41&-99.00&     2.72& -3.00&    4\\
   115&  160.973&   58.757& 24.14& 23.17& 22.30& 21.73& 21.00& 20.76& 20.41& 19.77& 18.11&     0.45& -3.00&    3\\
   116&  160.973&   58.888& 23.58& 22.84& 22.49& 22.50& 21.96& 21.96& 20.79& 20.13&-99.00&     0.56& -3.00&    3\\
   117&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.93&-99.00&     0.00&-99.00&  -99\\
   118&  160.975&   58.679& 24.60& 24.01& 23.94& 23.04&-99.00&-99.00&-99.00& 21.29&-99.00&     0.00&  0.35&  -99\\
   119&  160.979&   58.984&-99.00&-99.00& 21.79& 21.34& 20.83& 20.74& 20.24& 19.63& 16.69&     0.35& -3.00&    3\\
   120&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.74&-99.00&    -1.00&-99.00&   -1\\
   121&  160.980&   59.052& 20.31& 19.75& 20.16& 19.85& 20.08& 19.77& 19.57& 18.85& 17.24&     1.30& -3.00&    4\\
   122&  160.981&   59.017& 20.40& 19.26& 18.80& 18.44& 18.09& 17.87& 17.58& 18.02& 17.52&     0.41& -3.00&    0\\
   123&  160.983&   58.742& 22.43& 21.73& 20.83& 20.53& 20.29& 19.90& 19.76& 19.61&-99.00&     0.70& -3.00&    1\\
   124&  160.987&   58.918& 24.70& 24.75& 23.81& 23.66& 22.34&-99.00&-99.00& 21.55&-99.00&     0.00&  1.25&  -99\\
   125&  160.989&   58.825& 23.32& 22.75& 22.56& 22.66& 22.22& 22.21&-99.00&-99.00&-99.00&     3.49& -3.00&    4\\
   126&  160.991&   58.864& 23.43& 22.61& 21.53& 21.07& 20.54& 20.30& 19.91& 19.53& 17.36&     0.77& -3.00&    3\\
   127&  161.000&   58.794&-99.00& 24.82& 23.61& 22.57& 21.87& 21.17& 20.68& 20.22&-99.00&     1.52& -3.00&    1\\
   128&  161.002&   58.979& 23.52& 22.60& 21.63& 21.14& 20.85& 20.76& 20.09& 19.97&-99.00&     0.68& -3.00&    3\\
   129&  161.003&   58.869& 23.43& 22.58& 21.54& 21.10& 20.53& 20.28& 19.90& 19.07&-99.00&     0.78& -3.00&    1\\
   130&  161.003&   59.114& 24.90& 24.62& 24.25& 24.06& 22.55&-99.00&-99.00& 21.39&-99.00&     0.00&  1.95&  -99\\
   131&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.36&-99.00&     0.00&-99.00&  -99\\
   132&  161.006&   58.995& 21.40& 20.18& 19.65& 19.28& 18.83& 18.55& 18.18& 18.69& 17.18&     0.41& -3.00&    3\\
   133&  161.008&   58.875& 24.88& 24.18& 23.13& 22.33& 20.70& 20.35& 19.98& 19.58&-99.00&     1.08& -3.00&    1\\
   134&  161.016&   58.984& 22.90& 22.23& 21.70& 21.08& 20.43& 20.35& 19.66& 19.23& 17.62&     1.02& -3.00&    4\\
   135&  161.017&   59.026& 21.16& 20.71& 20.60& 20.38& 20.20& 20.03& 19.68& 19.06& 17.47&     1.22& -3.00&    4\\
   136&  161.017&   59.045& 19.59& 19.50& 19.22& 19.10& 18.89& 18.57& 18.33& 17.64& 16.20&     0.52& -3.00&    4\\
   137&  161.018&   59.150& 23.87& 22.66& 21.49& 21.06& 20.50& 20.28& 19.88& 19.96&-99.00&     0.65& -3.00&    0\\
   138&  161.018&   59.297&-99.00&-99.00&-99.00&-99.00& 21.70& 21.44& 20.89& 20.10& 17.63&    -1.00&-99.00&   -1\\
   139&  161.021&   58.985& 23.65& 22.35& 20.94& 20.37& 19.84& 19.43& 18.88& 18.62& 16.95&    -1.00&  0.65&   -1\\
   140&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.36&-99.00&     0.00&-99.00&  -99\\
   141&  161.021&   58.893& 24.55& 23.66& 22.63& 22.12& 21.56& 21.30& 20.99& 20.72&-99.00&     0.00&  0.65&  -99\\
   142&  161.024&   59.090& 21.21& 20.95& 20.52& 20.48& 20.14& 20.00& 19.78& 19.48& 18.34&     0.51& -3.00&    4\\
   143&  161.026&   58.987& 22.10& 21.60& 21.66& 21.24& 20.93& 20.66& 20.68& 19.84& 17.49&     3.64& -3.00&    4\\
   144&  161.027&   58.665& 23.52& 23.51& 23.18& 22.85& 21.92& 20.87&-99.00& 19.63& 16.59&     2.42& -3.00&    3\\
   145&  161.027&   59.035& 21.73& 20.99& 20.62& 20.17& 19.88& 19.39& 19.08& 19.03&-99.00&     0.45& -3.00&    4\\
   146&  161.028&   58.859&-99.00& 25.18& 24.60&-99.00&-99.00&-99.00&-99.00& 20.56& 17.44&     3.96& -3.00&    3\\
   147&  161.029&   59.160& 23.97& 23.51& 22.62& 22.28& 21.42& 21.06& 20.40& 19.79&-99.00&     1.19& -3.00&    4\\
   148&  161.030&   58.937& 19.93& 19.80& 19.65& 19.48& 19.72& 19.79& 19.61& 18.63& 16.37&    -1.00&-99.00&   -1\\
   149&  161.031&   58.944& 23.94& 22.85& 21.68& 21.17& 20.63& 20.32& 20.14& 20.00&-99.00&    -1.00&  0.65&   -1\\
   150&  161.032&   58.670&-99.00&-99.00&-99.00&-99.00& 21.90&-99.00&-99.00& 20.01&-99.00&     0.00&-99.00&  -99\\
   151&  161.033&   58.744& 21.68& 20.40& 19.67& 19.41& 18.84& 18.35& 17.88& 16.92& 14.38&     0.56& -3.00&    4\\
   152&  161.034&   58.991& 23.07& 22.91& 22.35& 22.13& 21.65& 21.41&-99.00&-99.00&-99.00&     2.00& -3.00&    3\\
   153&  161.039&   59.001& 23.40& 22.68& 21.74& 21.03& 20.25& 19.91& 19.64& 19.15&-99.00&     1.02& -3.00&    3\\
   154&  161.042&   58.873& 23.64& 23.59& 23.45& 23.30& 22.51& 21.75& 20.81& 19.43& 15.07&     0.00&-99.00&  -99\\
   155&  161.041&   58.980&-99.00&-99.00&-99.00&-99.00& 22.06& 21.69&-99.00& 20.38&-99.00&    -1.00&-99.00&   -1\\
   156&  161.046&   58.907& 24.57& 24.23& 24.14& 23.61&-99.00& 20.97& 20.48& 20.04&-99.00&     0.00&-99.00&  -99\\
   157&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.79&-99.00&     0.00&-99.00&  -99\\
   158&  161.048&   59.108&-99.00&-99.00& 22.34& 21.81& 21.31& 21.43& 20.61&-99.00&-99.00&     1.06& -3.00&    1\\
   159&  161.049&   58.886& 25.00& 24.62& 23.69& 23.48& 22.20& 21.62& 21.15& 20.80&-99.00&     0.00&  1.15&  -99\\
   160&  161.051&   58.916&-99.00&-99.00&-99.00& 20.50& 19.85& 19.66& 19.41& 17.82& 17.13&     0.78& -3.00&    3\\
   161&  161.050&   58.942& 24.45& 23.99& 23.83& 23.85&-99.00&-99.00&-99.00& 21.68&-99.00&    -1.00&  0.15&   -1\\
   162&  161.051&   58.825& 22.00& 21.53& 21.29& 21.03& 20.86& 20.70& 20.55& 20.32&-99.00&    -1.00&  0.35&   -1\\
   163&  161.052&   58.539& 22.63& 22.33& 21.95& 21.31& 20.58& 20.37&-99.00& 19.54&-99.00&    -1.00&  1.35&   -1\\
   164&  161.053&   59.275&-99.00& 22.51& 21.61& 21.12& 20.81& 20.50& 20.26& 20.30&-99.00&     0.76& -3.00&    3\\
   165&  161.054&   59.225& 22.56& 22.06& 21.70& 21.17& 20.62& 20.08& 19.71& 19.16& 17.71&     1.11& -3.00&    4\\
   166&  161.054&   58.877& 25.10& 24.75& 24.17& 24.07&-99.00&-99.00&-99.00& 21.32&-99.00&     0.00&-99.00&  -99\\
   167&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     1.07& -3.00&    1\\
   168&  161.058&   58.927&-99.00&-99.00&-99.00& 23.35&-99.00&-99.00&-99.00& 21.37& 17.36&     1.07& -3.00&    1\\
   169&  161.059&   59.138& 25.01& 24.21& 23.57& 22.90& 22.08& 21.26& 21.53& 21.12&-99.00&     0.00&  0.55&  -99\\
   170&  161.065&   58.721& 19.31& 18.44& 17.99& 17.75& 17.34& 16.97& 16.97& 17.65& 16.26&     0.23& -3.00&    3\\
   171&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.04&-99.00&    -1.00&-99.00&   -1\\
   172&  161.066&   59.017& 20.40& 20.13& 19.95& 19.95& 19.98& 19.75& 19.89& 19.13& 17.37&     1.58& -3.00&    4\\
   173&  161.070&   58.913& 24.41&-99.00& 21.99& 21.44& 20.71& 20.49& 20.30& 19.41&-99.00&     0.00&  0.65&  -99\\
   174&  161.071&   58.910& 19.14& 18.22& 17.80& 17.49& 17.21& 17.10& 17.06& 17.71&-99.00&     0.12& -3.00&    0\\
   175&  161.071&   59.005&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.25& 20.90&-99.00&     0.00&-99.00&  -99\\
   176&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   177&  161.073&   58.692& 23.26& 22.55& 22.28& 21.90& 21.61& 21.00&-99.00& 20.10& 18.07&     2.66& -3.00&    4\\
   178&  161.076&   59.112& 23.12& 22.81& 22.51& 21.95&-99.00& 21.17&-99.00&-99.00&-99.00&     2.33& -3.00&    4\\
   179&  161.077&   58.575& 23.78& 23.66& 23.43& 23.04& 22.34&-99.00&-99.00& 20.90&-99.00&    -1.00&  0.15&   -1\\
   180&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   181&  161.082&   58.940& 20.80& 20.30& 20.02& 19.93& 19.97& 20.00& 20.56& 20.48&-99.00&     0.21& -3.00&    1\\
   182&  161.085&   58.663& 25.33& 24.94& 23.77& 23.03& 21.76& 20.84&-99.00& 19.87& 16.74&     0.00&-99.00&  -99\\
   183&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.51&-99.00&     0.00&-99.00&  -99\\
   184&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   185&  161.089&   58.906&-99.00&-99.00&-99.00&-99.00& 22.10&-99.00& 21.21& 20.29& 18.02&     0.00&-99.00&  -99\\
   186&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.51&-99.00&    -1.00&-99.00&   -1\\
   187&  161.092&   59.135& 25.12&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   188&  161.095&   59.218& 22.41& 21.65& 21.01& 20.65& 19.59& 19.66& 19.15& 18.52& 16.10&     0.95& -3.00&    3\\
   189&  161.096&   59.297& 23.78& 22.49& 21.43& 21.05& 20.55& 20.33& 19.90& 19.79&-99.00&     0.62& -3.00&    3\\
   190&  161.099&   58.892& 24.77& 24.23& 23.54& 22.87& 21.55& 21.29& 21.15& 20.16&-99.00&     2.32& -3.00&    1\\
   191&  161.100&   58.748&-99.00&-99.00&-99.00&-99.00& 22.02& 21.88& 21.37& 21.21&-99.00&     0.00&-99.00&  -99\\
   192&  161.101&   58.775&-99.00& 22.27& 22.11& 21.82& 21.85& 21.39& 21.21& 21.81&-99.00&     2.44& -3.00&    3\\
   193&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.84&-99.00&    -1.00&-99.00&   -1\\
   194&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   195&  161.105&   58.782& 23.34& 22.53& 21.33& 20.80& 20.09& 19.72& 19.48& 19.07& 17.98&     0.95& -3.00&    1\\
   196&  161.106&   58.779& 24.85& 24.41& 23.81& 23.76& 21.85& 21.62& 20.92& 19.94&-99.00&     0.00&  1.75&  -99\\
   197&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   198&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   199&  161.109&   58.673&-99.00&-99.00& 24.18& 23.44& 22.36& 21.45&-99.00& 19.90& 17.46&     0.00&  1.15&  -99\\
   200&  161.115&   58.984& 21.70& 21.42& 20.88& 20.62& 20.13& 19.88& 19.55& 19.17& 16.99&     0.81& -3.00&    1\\
   201&  161.117&   59.235& 25.58& 24.36& 23.66& 23.44&-99.00& 22.38&-99.00& 20.91&-99.00&    -5.00&  0.55&  -99\\
   202&  161.118&   59.261&-99.00&-99.00&-99.00& 21.56& 20.76& 20.54& 20.00& 19.27&-99.00&     0.36& -3.00&    1\\
   203&  161.120&   58.909& 21.76& 22.22& 21.70& 22.01& 21.99&-99.00&-99.00&-99.00&-99.00&     2.53& -3.00&    3\\
   204&  161.120&   58.855& 21.70& 21.92& 21.54& 21.40& 21.27& 21.29& 21.08& 20.57&-99.00&     2.07& -3.00&    4\\
   205&  161.124&   59.260& 22.53& 21.94& 21.70& 21.53& 20.92& 20.83& 20.63& 19.73&-99.00&     1.00& -3.00&    4\\
   206&  161.126&   58.706&-99.00&-99.00&-99.00&-99.00& 21.54& 20.97&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   207&  161.127&   58.575& 23.72& 23.06& 22.18& 21.40& 20.72& 20.56&-99.00& 19.52&-99.00&    -1.00&  1.05&   -1\\
   208&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.89&-99.00&     0.00&-99.00&  -99\\
   209&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   210&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.27&-99.00&    -1.00&-99.00&   -1\\
   211&  161.131&   59.094& 21.07& 20.57& 20.56& 20.38& 20.49& 19.85& 19.96& 19.10& 16.05&     1.30& -3.00&    4\\
   212&  161.131&   58.894& 23.69& 23.07& 22.16& 21.62& 20.99& 20.52& 20.18& 20.03&-99.00&     0.95& -3.00&    1\\
   213&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   214&  161.134&   59.083& 23.15& 22.92& 22.47& 22.20& 21.33& 21.19& 20.90& 19.62& 16.43&     1.56& -3.00&    4\\
   215&  161.135&   59.174& 24.94& 24.79& 24.38& 24.34&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.15&   -1\\
   216&  161.138&   58.980& 21.19& 20.95& 20.85& 20.61& 20.05& 20.10& 19.72& 19.05& 16.40&     1.01& -3.00&    3\\
   217&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   218&  161.143&   58.728& 24.26&-99.00& 24.02& 23.86&-99.00&-99.00&-99.00& 21.06&-99.00&    -1.00&  0.35&   -1\\
   219&  161.143&   59.206& 23.62& 22.89& 23.15& 23.06& 22.18&-99.00&-99.00& 21.63&-99.00&     0.00&-99.00&  -99\\
   220&  161.145&   58.822& 23.37& 23.22& 22.82& 22.43& 22.05&-99.00&-99.00& 21.02&-99.00&     0.00&  2.05&  -99\\
   221&  161.146&   58.767&-99.00& 20.78& 20.73& 20.33& 20.09& 19.86& 19.64& 19.01& 17.90&     0.00&  0.65&  -99\\
   222&  161.149&   59.006& 24.17& 23.90& 23.42& 22.85& 22.07& 21.56&-99.00& 21.31&-99.00&     0.00&  1.35&  -99\\
   223&  161.151&   58.814& 21.21& 20.94& 20.56& 20.19& 19.90& 19.78& 19.37& 18.90& 16.98&     0.79& -3.00&    4\\
   224&  161.152&   58.784& 21.51& 21.46& 21.25& 21.36& 21.25& 20.74& 20.83& 20.17&-99.00&    -1.00&  1.25&   -1\\
   225&  161.155&   58.700& 24.75& 24.10& 23.74& 23.34&-99.00& 21.50&-99.00& 21.04&-99.00&    -1.00&-99.00&   -1\\
   226&  161.156&   58.885& 24.56& 23.67& 22.86& 22.30& 21.56& 21.07& 20.77& 19.88& 16.86&     0.00&  1.05&  -99\\
   227&  161.160&   58.984&-99.00&-99.00& 25.24& 24.21&-99.00& 21.62&-99.00& 20.72&-99.00&    -1.00&  1.75&   -1\\
   228&  161.160&   59.264&-99.00&-99.00&-99.00& 13.27& 13.62& 13.25& 13.04& 13.92& 17.79&    -2.00&-99.00&   -2\\
   229&  161.161&   59.218& 22.79& 22.06& 22.09& 21.71& 21.39& 20.77& 20.42& 19.86& 17.46&     1.45& -3.00&    4\\
   230&  161.161&   58.673&-99.00&-99.00& 24.95& 23.74& 22.04&-99.00&-99.00& 21.11&-99.00&     0.00&  1.55&  -99\\
   231&  161.161&   58.610& 24.37& 23.38& 22.31& 21.73& 21.20& 21.00&-99.00& 20.39&-99.00&    -1.00&  0.65&   -1\\
   232&  161.161&   58.749& 25.71& 24.52& 23.78& 23.22& 21.58& 21.05& 20.88& 19.71& 17.94&     0.00&  1.45&  -99\\
   233&  161.165&   59.228& 21.68& 21.22& 20.78& 20.36& 19.99& 19.72& 19.28& 18.52& 17.52&     0.90& -3.00&    4\\
   234&  161.170&   58.773&-99.00& 23.06& 22.02& 21.39& 20.66& 20.23& 19.71& 19.58&-99.00&     0.00&  0.75&  -99\\
   235&  161.171&   58.568& 24.71& 23.93&-99.00& 22.82& 21.95& 21.17&-99.00& 20.29&-99.00&    -1.00&  0.95&   -1\\
   236&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   237&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.67&-99.00&     0.00&-99.00&  -99\\
   238&  161.174&   58.922& 24.98& 24.74& 23.55& 22.81& 21.67& 21.37& 20.70& 20.21&-99.00&    -1.00&  1.55&   -1\\
   239&  161.175&   59.050& 22.59& 22.82& 22.26& 22.20& 21.68& 21.62& 21.02& 20.22& 17.62&     2.08& -3.00&    4\\
   240&  161.177&   59.044& 26.13& 24.47& 23.58& 22.97& 22.10& 21.60&-99.00& 21.28&-99.00&     0.00&  0.85&  -99\\
   241&  161.179&   59.294&-99.00&-99.00& 24.71& 23.63& 21.67& 21.17& 20.83& 20.10&-99.00&    -1.00&  1.45&   -1\\
   242&  161.178&   59.322& 21.94& 22.08& 21.46& 21.68& 21.23& 20.93& 20.56& 20.15&-99.00&     1.69& -3.00&    4\\
   243&  161.181&   59.285&-99.00&-99.00& 23.99& 23.62& 21.27& 21.23& 20.59& 20.26&-99.00&     0.00&  2.25&  -99\\
   244&  161.186&   58.661& 22.27& 21.35& 20.74& 20.30& 19.86& 19.42&-99.00& 18.59& 16.63&     0.42& -3.00&    1\\
   245&  161.187&   59.048& 22.06& 20.80& 19.96& 19.66& 19.21& 18.82& 18.61& 18.63&-99.00&     0.68& -3.00&    1\\
   246&  161.189&   58.902& 21.66& 21.34& 21.35& 21.12& 20.69& 20.44& 20.21& 19.72&-99.00&     1.06& -3.00&    4\\
   247&  161.191&   59.346& 25.17& 24.42& 23.56& 22.67&-99.00& 21.53& 20.55&-99.00&-99.00&     1.30& -3.00&    1\\
   248&  161.192&   58.744& 23.11& 22.94& 22.63& 22.74& 22.56&-99.00&-99.00& 21.77&-99.00&     0.00&  1.15&  -99\\
   249&  161.193&   58.825& 23.84& 22.95& 22.52& 21.99& 21.21& 21.02& 20.61& 19.91& 18.02&     0.00&  2.15&  -99\\
   250&  161.200&   59.173& 24.02& 23.47& 22.95& 22.31& 21.83& 20.92& 20.66& 20.09&-99.00&     1.28& -3.00&    1\\
   251&  161.202&   59.108& 22.12& 21.29& 21.36& 20.92& 20.38& 19.86& 19.38& 18.55& 17.58&    -1.00&  0.65&   -1\\
   252&  161.204&   58.790& 23.79& 22.58& 22.10& 21.63& 21.31& 21.47& 20.67& 20.18&-99.00&     0.00&  0.35&  -99\\
   253&  161.204&   59.169& 23.60& 22.98& 22.84& 22.43& 22.01& 21.29& 21.08& 20.69&-99.00&    -1.00&  0.15&   -1\\
   254&  161.204&   58.648& 24.03& 22.97&-99.00& 22.01& 22.08&-99.00&-99.00& 21.36&-99.00&     0.44& -3.00&    0\\
   255&  161.214&   59.330& 20.57& 19.70& 19.26& 18.95& 18.68& 18.50& 18.17& 17.81& 15.42&     0.46& -3.00&    4\\
   256&  161.216&   58.912& 21.92& 21.57& 21.57& 21.45& 21.12& 20.86& 20.54& 20.16&-99.00&     1.33& -3.00&    4\\
   257&  161.216&   58.754& 24.17& 23.37& 22.19& 21.59& 20.93& 20.50& 20.03& 19.51&-99.00&     0.95& -3.00&    1\\
   258&  161.217&   59.222& 25.17& 24.98& 24.31& 24.30& 22.49& 21.85& 21.28& 20.90&-99.00&     0.00&-99.00&  -99\\
   259&  161.218&   59.238& 22.96& 22.85& 22.71& 22.78& 22.53&-99.00&-99.00& 21.61&-99.00&     2.92& -3.00&    4\\
   260&  161.219&   59.052& 24.61& 23.43& 22.14& 21.61& 20.73& 20.40& 20.03& 19.70&-99.00&     0.91& -3.00&    3\\
   261&  161.219&   58.725&-99.00& 23.24&-99.00& 23.03&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   262&  161.220&   59.109& 24.15& 22.50& 20.84& 20.30& 19.77& 19.31& 18.86& 18.76&-99.00&     0.69& -3.00&    3\\
   263&  161.221&   58.915& 24.73& 24.78& 24.17& 23.69&-99.00&-99.00& 21.12& 19.40& 16.43&     0.00&  1.15&  -99\\
   264&  161.227&   59.132&-99.00&-99.00&-99.00&-99.00& 20.73& 20.21& 19.86& 19.47& 18.27&     0.58& -3.00&    1\\
   265&  161.227&   59.077& 22.75& 22.19& 21.35& 20.70& 20.10& 19.75& 19.47& 18.56& 16.87&     0.95& -3.00&    3\\
   266&  161.229&   59.359& 19.59& 19.14& 19.27& 19.14& 19.35& 18.94& 19.02& 18.19& 15.57&     1.29& -3.00&    4\\
   267&  161.229&   59.086&-99.00&-99.00&-99.00&-99.00& 17.93& 17.65& 17.34& 17.68& 17.68&     0.45& -3.00&    0\\
   268&  161.232&   58.930& 23.40& 21.88& 21.07& 20.69& 20.01& 19.89& 19.38& 19.60&-99.00&     0.48& -3.00&    0\\
   269&  161.231&   58.764&-99.00& 22.26& 21.20& 20.55& 19.99& 19.78& 19.13& 18.80& 17.08&     0.98& -3.00&    1\\
   270&  161.236&   58.924& 21.65& 21.42& 21.18& 20.97& 20.53& 20.23& 20.01& 19.17& 18.17&     1.04& -3.00&    4\\
   271&  161.239&   59.207& 25.63& 24.69& 24.02& 23.63& 21.76& 21.29& 20.85& 20.13&-99.00&    -1.00&  1.75&   -1\\
   272&  161.239&   58.682& 24.43& 24.17& 23.56& 23.25&-99.00&-99.00&-99.00& 20.64& 18.23&     0.00&  0.55&  -99\\
   273&  161.240&   58.560& 23.77&-99.00& 22.48& 22.10& 21.47&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.75&   -1\\
   274&  161.242&   59.209& 23.76& 23.38& 22.68& 22.09& 21.04& 20.59& 20.56& 19.69&-99.00&     1.43& -3.00&    1\\
   275&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   276&  161.253&   59.231& 23.69& 23.52& 22.91& 22.54& 21.83& 21.22& 21.34& 19.82& 16.74&     0.00&-99.00&  -99\\
   277&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.38&-99.00&     0.00&-99.00&  -99\\
   278&  161.263&   58.787& 21.10& 20.93& 20.82& 20.79& 20.73& 20.51& 20.64& 19.70&-99.00&     1.58& -3.00&    4\\
   279&  161.264&   59.212& 22.17& 22.07& 21.83& 21.44& 20.48& 20.86& 20.41& 19.58&-99.00&     0.87& -3.00&    4\\
   280&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.57&-99.00&     0.00&-99.00&  -99\\
   281&  161.264&   58.778&-99.00&-99.00&-99.00&-99.00& 22.37& 21.44& 21.30&-99.00&-99.00&     0.00&-99.00&  -99\\
   282&  161.265&   58.853& 24.13& 23.02& 21.75& 20.94& 20.16& 20.10& 19.64& 18.69&-99.00&     1.02& -3.00&    0\\
   283&  161.270&   59.216& 24.77& 24.20& 23.53& 22.98& 21.63& 21.59& 21.39& 20.82&-99.00&     1.53& -3.00&    3\\
   284&  161.271&   58.996& 21.97& 21.30& 20.60& 20.42& 19.79& 19.50& 19.03& 19.18& 15.54&     0.21& -3.00&    1\\
   285&  161.272&   58.977& 20.68& 19.62& 19.12& 18.83& 18.36& 18.18& 17.93& 18.50&-99.00&     0.24& -3.00&    1\\
   286&  161.275&   59.357& 23.87& 22.63& 21.40& 20.93& 20.38& 20.26& 19.82& 19.34&-99.00&     0.76& -3.00&    3\\
   287&  161.275&   58.773&-99.00& 22.67& 22.00& 21.26& 20.62& 20.28& 19.81& 19.15& 17.48&     1.16& -3.00&    1\\
   288&  161.276&   58.665& 25.06& 26.72& 24.13& 25.58&-99.00&-99.00&-99.00& 20.69&-99.00&     0.80& -3.00&    3\\
   289&  161.279&   58.608& 18.17& 17.38& 16.96& 16.63& 16.29& 16.20&-99.00&-99.00& 16.95&     0.12& -3.00&    3\\
   290&  161.279&   58.664& 25.60& 24.51& 23.16& 22.38& 20.98& 20.82&-99.00& 19.41& 17.02&    -1.00&  1.85&   -1\\
   291&  161.280&   58.806& 24.13& 24.36& 24.22& 23.88&-99.00&-99.00&-99.00& 21.73&-99.00&     2.53& -3.00&    3\\
   292&  161.281&   59.286& 24.57& 24.56& 24.21& 23.83&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&  0.55&  -99\\
   293&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -5.00&-99.00&  -99\\
   294&  161.283&   59.074& 24.98& 25.12& 24.83& 24.32&-99.00& 21.75&-99.00& 21.09&-99.00&     0.00&-99.00&  -99\\
   295&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   296&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   297&  161.293&   59.053& 24.59& 23.71& 22.62& 22.15& 21.84& 21.04& 20.65& 20.30&-99.00&     0.91& -3.00&    1\\
   298&  161.297&   59.274&-99.00& 19.23& 19.05& 18.88& 19.11& 19.14& 19.00& 18.47& 16.41&     1.79& -3.00&    4\\
   299&  161.298&   59.177& 24.92& 23.75& 23.40& 22.73& 21.82& 21.20& 21.11& 20.19&-99.00&     1.30& -3.00&    4\\
   300&  161.303&   59.036& 22.70& 22.23& 22.23& 21.64& 21.01& 20.97& 20.81& 20.05&-99.00&     1.01& -3.00&    4\\
   301&  161.304&   59.057& 24.39& 23.99& 23.48& 22.78&-99.00& 21.61& 21.42& 20.29&-99.00&     2.07& -3.00&    4\\
   302&  161.307&   58.682& 22.63& 20.86& 19.82& 19.41& 18.80& 18.50& 18.08& 18.26&-99.00&     0.58& -3.00&    3\\
   303&  161.310&   59.200& 22.50& 22.22& 22.04& 21.81& 21.62&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.25&   -1\\
   304&  161.310&   58.824& 22.37& 21.89& 21.11& 20.60& 20.09& 19.65& 19.44& 19.04& 17.75&     0.68& -3.00&    3\\
   305&  161.316&   59.319&-99.00&-99.00& 24.48& 23.83&-99.00&-99.00&-99.00& 20.91&-99.00&    -1.00&  1.15&   -1\\
   306&  161.317&   59.385& 22.12& 20.85& 20.38& 19.62&-99.00& 19.04& 18.57& 18.86& 14.78&    -1.00&  0.65&   -1\\
   307&  161.318&   59.315& 23.03& 22.47& 21.79& 21.31& 20.46& 20.34& 19.82& 19.45&-99.00&     1.00& -3.00&    4\\
   308&  161.318&   59.092&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.83& 19.58&-99.00&     0.00&-99.00&  -99\\
   309&  161.318&   59.193& 22.88& 22.20& 22.08& 21.59& 21.07& 20.74& 20.34& 19.62& 17.30&     1.30& -3.00&    4\\
   310&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.48&-99.00&     0.00&-99.00&  -99\\
   311&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   312&  161.324&   59.201& 23.94& 23.18& 22.42& 21.67& 21.03& 20.73& 20.23& 19.75&-99.00&     1.06& -3.00&    1\\
   313&  161.324&   59.115& 21.69& 21.62& 21.57& 21.10& 21.35& 20.99& 20.68& 20.89&-99.00&     2.23& -3.00&    4\\
   314&  161.328&   59.119&-99.00&-99.00&-99.00& 20.92& 20.77& 20.38& 20.29& 20.36&-99.00&     0.49& -3.00&    4\\
   315&  161.329&   58.744& 25.17& 23.62& 22.34& 21.51& 20.60& 20.19& 19.69& 18.89&-99.00&    -1.00&  1.25&   -1\\
   316&  161.329&   59.174& 24.43& 24.17& 23.47& 23.34& 22.22& 21.44& 21.47& 20.19&-99.00&     0.00&  0.85&  -99\\
   317&  161.330&   59.175& 23.14& 22.84& 22.37& 21.92& 21.30& 20.81& 20.80& 20.01&-99.00&    -1.00&  0.55&   -1\\
   318&  161.330&   58.721& 25.13& 24.27& 23.17& 22.36& 21.60& 21.08& 20.75& 20.21&-99.00&    -1.00&  1.15&   -1\\
   319&  161.335&   59.214& 23.27& 22.95& 22.76& 22.55& 21.35& 21.09& 20.99& 20.28&-99.00&    -1.00&  1.15&   -1\\
   320&  161.339&   59.185& 25.17& 23.25& 21.84& 20.99& 20.42& 19.86& 19.58& 19.37&-99.00&     0.90& -3.00&    3\\
   321&  161.342&   58.941& 25.66& 25.74&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   322&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.50& 17.84&     0.00&-99.00&  -99\\
   323&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.15&-99.00&     0.00&-99.00&  -99\\
   324&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   325&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   326&  161.352&   59.118&-99.00& 12.63&-99.00& 12.05& 12.62& 12.89& 12.19& 13.09& 17.45&    -2.00&-99.00&   -2\\
   327&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.36& 17.89&     0.00&-99.00&  -99\\
   328&  161.355&   58.717&-99.00& 23.61&-99.00& 22.14& 21.73& 21.04& 19.63& 18.95&-99.00&    -1.00&  0.85&   -1\\
   329&  161.362&   59.226& 24.89& 23.62& 22.36& 21.66& 20.86& 20.35& 20.04& 19.53&-99.00&     0.85& -3.00&    3\\
   330&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     1.30& -3.00&    1\\
   331&  161.368&   59.224& 25.00& 23.69& 22.79& 22.34& 21.71& 21.02& 20.91& 19.97& 15.65&    -1.00&  0.55&   -1\\
   332&  161.367&   59.167&-99.00&-99.00&-99.00&-99.00& 21.33& 21.03& 20.73& 20.56&-99.00&     0.00&-99.00&  -99\\
   333&  161.368&   58.614& 22.57& 22.07& 21.74& 21.45& 21.32& 21.88&-99.00& 20.59& 17.63&     2.14& -3.00&    4\\
   334&  161.372&   59.191&-99.00&-99.00& 24.05& 22.95& 21.68& 21.30& 20.65& 19.98&-99.00&     0.00&  1.95&  -99\\
   335&  161.373&   58.742&-99.00&-99.00& 24.77& 24.18&-99.00&-99.00&-99.00& 21.18&-99.00&     0.00&  1.05&  -99\\
   336&  161.376&   58.877& 22.70& 22.71& 21.90& 21.92& 21.40&-99.00& 20.96& 20.34&-99.00&     1.93& -3.00&    4\\
   337&  161.376&   58.921& 24.60& 24.39& 23.70& 23.58&-99.00&-99.00& 21.23& 20.14& 17.87&     1.01& -3.00&    1\\
   338&  161.378&   58.660& 22.57& 22.46& 22.19& 21.95& 21.48& 21.17&-99.00& 20.65&-99.00&     1.81& -3.00&    4\\
   339&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.24&-99.00&     0.00&-99.00&  -99\\
   340&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   341&  161.385&   59.232& 21.08& 21.05& 21.05& 20.91& 20.45& 20.36& 20.22& 20.00& 17.67&     2.66& -3.00&    4\\
   342&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   343&  161.387&   58.777&-99.00& 24.29& 23.26& 22.69& 21.67& 21.29& 20.18& 20.18& 18.02&     0.00&  1.45&  -99\\
   344&  161.389&   59.220& 23.45& 23.22& 23.14& 22.59&-99.00&-99.00&-99.00&-99.00&-99.00&     2.32& -3.00&    3\\
   345&  161.390&   58.690& 23.48& 22.85& 22.07& 21.51& 20.82& 20.62&-99.00& 19.98&-99.00&    -1.00&  0.65&   -1\\
   346&  161.396&   58.775&-99.00& 22.85& 22.10& 21.48& 20.69& 20.55& 19.88& 19.60&-99.00&     0.99& -3.00&    3\\
   347&  161.413&   59.213& 24.42& 23.68& 23.46& 23.32&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&  0.35&  -99\\
   348&  161.415&   59.207& 21.91& 21.82& 21.45& 21.39& 21.16& 21.11& 21.10& 20.65&-99.00&     1.76& -3.00&    4\\
   349&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   350&  161.417&   59.025& 20.97& 20.97& 20.70& 20.74& 20.40& 20.67& 20.26& 19.75& 17.66&     1.74& -3.00&    4\\
   351&  161.417&   58.715& 19.45& 19.03& 18.89& 18.41& 18.36& 18.03& 17.53& 17.72& 15.33&     0.32& -3.00&    4\\
   352&  161.418&   59.345& 23.62& 23.28& 22.54& 22.51&-99.00& 21.61& 21.10& 20.34&-99.00&    -1.00&  0.55&   -1\\
   353&  161.419&   58.696& 23.25& 22.65& 21.78& 21.47& 21.02& 20.99&-99.00& 19.81&-99.00&    -1.00&  0.45&   -1\\
   354&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.05&-99.00&     0.00&-99.00&  -99\\
   355&  161.421&   58.952& 25.18& 24.64& 24.76& 24.37&-99.00&-99.00&-99.00& 21.92&-99.00&     2.10& -3.00&    4\\
   356&  161.424&   59.345& 19.94& 18.66& 17.03& 16.07& 15.48& 15.68& 15.45& 16.13&-99.00&    -1.00&-99.00&   -1\\
   357&  161.425&   59.259& 24.06& 22.89& 21.67& 21.03& 20.22& 19.96& 19.52& 19.28&-99.00&     0.87& -3.00&    3\\
   358&  161.427&   59.016& 23.72& 23.21& 22.76& 22.28& 21.58&-99.00& 21.13& 21.06&-99.00&     1.18& -3.00&    1\\
   359&  161.428&   58.870& 15.08& 14.08& 13.98& 13.24& 13.36& 13.01& 12.40& 13.31& 17.51&    -2.00&-99.00&   -2\\
   360&  161.430&   59.116& 23.16& 22.83& 22.13& 22.26&-99.00& 20.94& 20.53& 19.03& 17.40&     1.57& -3.00&    4\\
   361&  161.431&   59.223& 20.29& 19.01& 17.58& 16.92& 16.46& 16.34& 16.50& 17.14&-99.00&    -2.00&-99.00&   -2\\
   362&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 17.44&     0.00&-99.00&  -99\\
   363&  161.434&   58.839& 24.79& 24.21& 23.50& 23.06&-99.00&-99.00&-99.00& 21.05&-99.00&    -1.00&  0.65&   -1\\
   364&  161.434&   59.266&-99.00&-99.00& 23.77& 23.21&-99.00&-99.00&-99.00& 21.14&-99.00&     0.00&  0.75&  -99\\
   365&  161.436&   59.197& 21.76& 20.19& 19.69& 19.35& 19.15& 18.85& 18.56& 18.93& 17.41&     0.45& -3.00&    1\\
   366&  161.439&   58.731&-99.00& 24.47& 23.35& 22.52& 21.61& 21.13& 20.42& 19.71&-99.00&     1.15& -3.00&    1\\
   367&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   368&  161.443&   58.764&-99.00& 23.94& 23.60& 23.08& 21.77&-99.00& 21.09& 20.70&-99.00&     0.00&  1.85&  -99\\
   369&  161.446&   59.316& 22.75& 21.98& 22.04& 21.44& 20.92& 21.39& 20.57& 19.85&-99.00&     1.22& -3.00&    4\\
   370&  161.454&   59.142& 25.06& 24.52& 23.62& 23.02& 21.63& 21.15& 20.61& 19.66& 17.57&     0.00&  1.35&  -99\\
   371&  161.454&   59.059& 24.46& 23.28&-99.00& 19.61&-99.00& 20.78& 20.00& 20.07&-99.00&    -1.00&-99.00&   -1\\
   372&  161.461&   59.324& 24.36& 23.68& 23.06& 22.49& 22.18& 22.72&-99.00& 20.84&-99.00&     0.00&-99.00&  -99\\
   373&  161.462&   58.859& 24.52& 23.60& 22.65& 21.72& 20.84& 20.51& 19.91& 19.46&-99.00&    -1.00&  1.25&   -1\\
   374&  161.466&   59.063& 25.01& 24.65&-99.00& 22.91&-99.00&-99.00& 20.94& 19.41& 17.24&     0.00&  1.15&  -99\\
   375&  161.466&   59.053& 21.94& 19.96& 19.31& 18.92& 18.26& 17.95& 17.51&-99.00& 17.07&     0.32& -3.00&    3\\
   376&  161.466&   58.767&-99.00& 22.73& 22.35& 22.11& 21.42& 20.95& 20.62& 20.20& 16.77&     1.93& -3.00&    3\\
   377&  161.469&   59.011&-99.00&-99.00&-99.00&-99.00& 19.75& 19.68& 20.35& 20.57&-99.00&    -1.00&-99.00&   -1\\
   378&  161.475&   58.795& 22.19& 21.56& 21.33& 21.32& 21.26& 21.66& 21.19& 21.69&-99.00&    -1.00&  1.15&   -1\\
   379&  161.484&   59.252& 21.71& 19.98& 19.47& 19.11& 18.65& 18.54& 18.25& 18.91&-99.00&     0.36& -3.00&    0\\
   380&  161.486&   58.991&-99.00& 24.59&-99.00&-99.00&-99.00&-99.00&-99.00& 21.16&-99.00&     0.00&-99.00&  -99\\
   381&  161.488&   59.000& 24.59& 23.67& 23.48& 22.97& 22.35&-99.00&-99.00& 21.62&-99.00&     0.00&  0.25&  -99\\
   382&  161.489&   59.120& 22.61& 22.27& 21.96& 21.78&-99.00&-99.00&-99.00& 20.76&-99.00&    -1.00&  0.55&   -1\\
   383&  161.489&   59.259& 24.38& 23.46& 22.39& 21.83& 21.00& 20.75& 20.61& 19.75& 17.62&     0.91& -3.00&    1\\
   384&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.88&-99.00&     0.00&-99.00&  -99\\
   385&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   386&  161.495&   58.650& 22.94& 22.87& 22.97& 22.45&-99.00&-99.00&-99.00& 20.80&-99.00&    -1.00&  0.45&   -1\\
   387&  161.499&   59.109& 19.32& 19.31&-99.00& 19.07& 19.41& 19.35& 18.84&-99.00& 16.50&     2.51& -3.00&    4\\
   388&  161.499&   59.288& 25.12& 25.13& 24.82&-99.00&-99.00&-99.00&-99.00& 20.86&-99.00&     0.00&  1.15&  -99\\
   389&  161.501&   59.233& 24.12& 24.22& 23.72& 23.91&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  1.85&   -1\\
   390&  161.504&   59.123& 22.06& 21.46& 21.26& 21.08& 20.49& 20.39& 19.91& 18.74&-99.00&    -1.00&-99.00&   -1\\
   391&  161.505&   59.121& 22.01& 22.09& 22.03& 21.88&-99.00&-99.00& 21.03& 20.56&-99.00&     2.42& -3.00&    4\\
   392&  161.505&   58.935&-99.00& 24.73& 23.67& 23.16& 22.00& 21.71& 20.68& 20.09&-99.00&     0.00&  1.35&  -99\\
   393&  161.505&   58.828& 23.14& 22.21& 21.26& 20.82& 20.29& 20.00& 19.55& 19.50&-99.00&     0.68& -3.00&    3\\
   394&  161.509&   58.977& 24.17& 24.04& 23.89& 23.74&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&  0.85&  -99\\
   395&  161.514&   58.895&-99.00& 25.02& 23.89& 23.16& 21.64& 21.24& 20.77& 20.07&-99.00&     0.00&  1.15&  -99\\
   396&  161.515&   59.112& 23.78& 22.81&-99.00& 22.25&-99.00&-99.00&-99.00& 20.79&-99.00&    -1.00&  0.25&   -1\\
   397&  161.517&   58.740& 20.92& 21.05& 20.71& 20.87& 20.45& 20.31& 20.12& 19.63&-99.00&     1.81& -3.00&    4\\
   398&  161.518&   58.777&-99.00& 21.60& 20.96& 20.44& 19.91& 19.60& 19.23& 18.71& 16.51&     0.79& -3.00&    4\\
   399&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   400&  161.527&   58.652&-99.00&-99.00&-99.00&-99.00& 16.23& 16.12&-99.00& 17.07&-99.00&    -1.00&-99.00&   -1\\
   401&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   402&  161.532&   58.934&-99.00&-99.00& 24.10&-99.00&-99.00&-99.00&-99.00& 21.10&-99.00&     0.00&-99.00&  -99\\
   403&  161.533&   58.812& 22.60& 22.29& 22.55& 22.43& 21.95&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.85&   -1\\
   404&  161.541&   58.926& 19.56& 18.81& 18.34& 18.09& 17.75& 17.55& 17.51&-99.00& 15.74&     0.29& -3.00&    3\\
   405&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   406&  161.545&   58.799& 24.84& 24.21& 23.27& 22.55& 21.21& 20.59& 20.50& 19.87&-99.00&     0.00&  1.45&  -99\\
   407&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   408&  161.546&   58.921& 23.84& 23.82& 23.49& 23.22& 22.23& 22.03&-99.00& 21.23&-99.00&     1.99& -3.00&    3\\
   409&  161.549&   59.018&-99.00& 24.49& 24.56& 22.88&-99.00&-99.00& 18.67& 20.01&-99.00&     1.34& -3.00&    1\\
   410&  161.554&   58.761&-99.00& 22.53& 21.88& 21.22& 20.72& 20.30& 19.91& 19.60& 17.97&     1.12& -3.00&    1\\
   411&  161.554&   58.789& 19.82& 19.49& 19.47& 19.36& 19.16& 18.98& 19.22& 18.93& 16.93&     3.04& -3.00&    4\\
   412&  161.555&   59.161& 22.10& 21.80& 21.55& 21.32& 20.86& 20.60& 20.13& 19.69& 18.24&     1.16& -3.00&    4\\
   413&  161.554&   58.707& 24.35& 23.84& 23.53& 23.30&-99.00&-99.00&-99.00& 20.48&-99.00&    -1.00&  0.45&   -1\\
   414&  161.556&   58.995& 23.03& 22.92& 22.50& 22.23& 21.80& 21.81& 20.93& 20.10& 16.10&     3.62& -3.00&    3\\
   415&  161.557&   58.744& 23.46& 23.13& 22.47& 22.10& 21.46& 21.68& 21.10& 20.82&-99.00&     0.86& -3.00&    1\\
   416&  161.562&   59.023& 23.57& 22.08& 21.35& 20.95& 20.56& 20.19& 19.95& 19.01&-99.00&     0.50& -3.00&    3\\
   417&  161.562&   59.127& 21.54& 21.38& 21.15& 20.96& 21.04& 21.01& 20.44& 19.63& 17.56&     2.02& -3.00&    4\\
   418&  161.563&   59.064&-99.00& 24.18&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   419&  161.564&   59.043& 24.53& 22.94& 22.23& 21.68& 20.42& 19.97&-99.00&-99.00&-99.00&     0.68& -3.00&    3\\
   420&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 18.30&    -2.00&-99.00&   -2\\
   421&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.37&-99.00&    -1.00&-99.00&   -1\\
   422&  161.568&   59.042&-99.00&-99.00&-99.00& 19.71&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   423&  161.568&   58.838& 20.07& 20.07& 20.11& 19.95& 20.21& 20.33& 19.99& 19.54& 17.61&    -1.00&  2.25&   -1\\
   424&  161.569&   58.989& 23.61& 22.17& 21.57& 21.28& 21.03& 20.75& 20.53& 21.01&-99.00&     0.47& -3.00&    0\\
   425&  161.569&   59.274&-99.00& 20.95& 20.45& 20.25& 19.79& 19.51& 19.25& 18.88& 17.32&     0.67& -3.00&    3\\
   426&  161.570&   58.651& 23.34& 22.59& 21.76& 21.34& 21.04& 20.50&-99.00& 19.83& 18.20&    -1.00&  0.55&   -1\\
   427&  161.571&   58.916&-99.00&-99.00& 23.36& 23.37& 22.61&-99.00& 21.43& 20.30&-99.00&     0.00&-99.00&  -99\\
   428&  161.573&   58.669& 26.10&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.01&-99.00&    -1.00&-99.00&   -1\\
   429&  161.573&   58.751& 18.38& 17.65& 17.22& 16.93& 16.51& 16.13& 16.28& 16.96& 16.04&     0.12& -3.00&    1\\
   430&  161.574&   59.098& 22.91& 22.62&-99.00& 22.15& 21.29&-99.00& 20.96& 20.36&-99.00&     2.63& -3.00&    4\\
   431&  161.575&   58.636& 22.03& 20.57& 20.02& 19.65& 19.24& 19.05&-99.00& 19.05& 17.33&    -1.00&  0.35&   -1\\
   432&  161.584&   59.238& 24.55& 23.59& 22.87& 22.04& 20.99& 20.74& 20.10& 19.43&-99.00&     0.00&  1.55&  -99\\
   433&  161.588&   58.837& 25.05& 24.47& 23.38& 22.61& 21.01& 20.46& 20.30& 19.64&-99.00&     1.57& -3.00&    3\\
   434&  161.591&   59.290& 24.39& 24.21& 23.71& 23.54& 23.21&-99.00&-99.00& 21.54&-99.00&     0.00&  0.15&  -99\\
   435&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   436&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.51&-99.00&     0.00&-99.00&  -99\\
   437&  161.592&   58.942& 19.64& 18.65& 18.21& 17.97& 17.63& 17.44& 17.22& 17.84& 16.90&     0.25& -3.00&    3\\
   438&  161.592&   59.283&-99.00& 21.68& 20.32& 20.00& 19.45& 19.16& 18.84& 18.74&-99.00&     0.67& -3.00&    3\\
   439&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.46&-99.00&    -1.00&-99.00&   -1\\
   440&  161.593&   58.656& 23.77& 23.29& 22.28& 21.78& 20.96& 20.85&-99.00& 20.04& 16.95&    -1.00&  0.95&   -1\\
   441&  161.593&   58.701&-99.00& 24.23& 22.88& 22.23& 21.51& 20.85& 20.73& 20.18&-99.00&    -1.00&  0.95&   -1\\
   442&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   443&  161.594&   59.288& 23.77& 23.48& 22.62& 22.14& 21.33& 21.24& 20.54& 19.46& 17.06&     1.83& -3.00&    4\\
   444&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.73&-99.00&     0.00&-99.00&  -99\\
   445&  161.600&   59.090& 24.27& 23.98&-99.00&-99.00&-99.00&-99.00&-99.00& 20.37&-99.00&     3.63& -3.00&    3\\
   446&  161.600&   58.725& 25.34& 24.36& 24.64& 24.26& 23.22&-99.00&-99.00&-99.00&-99.00&     3.38& -3.00&    4\\
   447&  161.604&   58.811& 19.18& 19.18& 19.01& 18.98& 18.84& 18.47& 17.97& 16.95& 15.09&     0.58& -3.00&    4\\
   448&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   449&  161.610&   58.871& 23.01& 22.78& 22.22& 22.21& 21.68& 21.20& 21.30& 20.83&-99.00&     1.55& -3.00&    4\\
   450&  161.612&   59.346& 23.59& 23.32& 23.15& 22.68& 22.23&-99.00&-99.00& 21.06&-99.00&    -1.00&-99.00&   -1\\
   451&  161.616&   59.380& 24.10& 22.78& 22.43& 22.57& 22.30&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   452&  161.622&   58.995& 24.44& 24.25& 23.59& 23.54&-99.00&-99.00&-99.00& 21.40&-99.00&    -1.00&  0.55&   -1\\
   453&  161.623&   58.731& 21.92& 21.96& 21.58& 21.33& 21.35& 20.59& 20.81& 20.07&-99.00&     2.07& -3.00&    4\\
   454&  161.626&   59.312& 22.55& 21.89& 22.05& 21.73& 21.70& 21.29&-99.00& 20.75&-99.00&     1.34& -3.00&    4\\
   455&  161.626&   59.142& 21.62& 21.54& 20.66& 20.46& 20.06& 19.88& 19.30& 19.06& 17.20&     0.82& -3.00&    1\\
   456&  161.627&   58.743& 21.46& 21.10& 20.94& 20.90& 20.44& 19.92& 19.95& 18.99& 16.90&     1.30& -3.00&    4\\
   457&  161.630&   59.103& 19.68& 19.76& 19.57& 19.42& 19.74& 19.75& 19.55& 19.18& 17.13&     1.99& -3.00&    4\\
   458&  161.633&   59.107& 25.21& 24.12& 23.03& 22.21& 21.36& 20.89& 20.36& 19.62& 17.62&     1.16& -3.00&    1\\
   459&  161.633&   59.208& 21.23& 21.59& 21.25& 21.25& 19.89& 21.26& 20.89& 20.87&-99.00&     2.45& -3.00&    4\\
   460&  161.634&   59.124& 23.67& 23.65& 22.99& 22.85& 21.96&-99.00&-99.00& 21.63&-99.00&     0.00&-99.00&  -99\\
   461&  161.638&   58.971&-99.00&-99.00&-99.00&-99.00&-99.00& 18.59& 18.91& 18.05& 16.51&     0.85& -3.00&    1\\
   462&  161.643&   59.225& 20.99& 20.84& 20.97& 20.85& 20.64& 20.79& 20.52& 20.56& 18.38&     2.64& -3.00&    4\\
   463&  161.650&   58.687& 25.18& 23.86& 22.50& 21.77& 21.21& 20.52&-99.00& 20.04&-99.00&     0.92& -3.00&    1\\
   464&  161.651&   58.670& 23.41& 23.70& 23.59& 23.61&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.15&   -1\\
   465&  161.656&   58.743& 22.03& 20.24& 19.63& 19.26& 18.97& 18.41& 18.23& 18.37&-99.00&     0.35& -3.00&    1\\
   466&  161.657&   58.987& 24.08& 23.44& 22.78& 22.36& 21.08& 20.55& 20.48& 20.17&-99.00&     0.00&  1.55&  -99\\
   467&  161.660&   58.945& 24.96& 24.28& 23.77& 23.24& 21.88& 21.54& 21.05& 20.07&-99.00&     0.00&  1.55&  -99\\
   468&  161.662&   59.288& 23.56&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.08&-99.00&    -1.00&-99.00&   -1\\
   469&  161.664&   58.680& 19.18& 18.86& 18.74& 18.66& 18.62& 18.55& 18.63& 18.61& 15.91&    -1.00&  1.05&   -1\\
   470&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   471&  161.668&   59.312& 21.31& 21.02& 20.15& 20.02& 19.60& 19.37& 19.10& 18.98&-99.00&     0.58& -3.00&    3\\
   472&  161.668&   58.629& 22.20& 22.01& 21.73& 21.47& 21.34& 21.39&-99.00& 21.09&-99.00&    -1.00&-99.00&   -1\\
   473&  161.668&   59.436&-99.00&-99.00&-99.00& 23.54& 22.37&-99.00& 21.22& 20.85&-99.00&    -1.00&  2.95&   -1\\
   474&  161.669&   59.090& 20.17& 19.71& 19.22& 18.99& 18.66& 18.44& 18.07& 18.18& 16.74&     0.45& -3.00&    4\\
   475&  161.671&   58.746&-99.00&-99.00&-99.00&-99.00& 22.45&-99.00&-99.00& 21.00&-99.00&     0.00&-99.00&  -99\\
   476&  161.672&   59.147& 24.04& 23.70& 23.20& 22.68& 21.60& 21.14& 20.88& 20.37&-99.00&     1.58& -3.00&    1\\
   477&  161.672&   58.870& 23.32& 22.95& 22.61& 22.43& 21.61& 21.01& 21.16& 19.87& 15.37&    -1.00&-99.00&   -1\\
   478&  161.675&   59.142& 21.70& 20.36& 19.29& 18.96& 18.64& 18.35& 17.84& 17.93& 17.46&     0.66& -3.00&    0\\
   479&  161.677&   59.301& 23.33& 23.32& 22.91& 22.98& 22.44&-99.00&-99.00& 21.52&-99.00&     2.86& -3.00&    4\\
   480&  161.678&   58.832& 24.80& 24.33& 23.78& 23.32& 22.10& 21.15& 20.69& 19.83& 17.59&     0.00&  1.15&  -99\\
   481&  161.679&   59.438& 24.95& 23.99& 23.50& 23.56&-99.00&-99.00&-99.00&-99.00&-99.00&     0.94& -3.00&    1\\
   482&  161.680&   59.429& 21.08& 20.98& 20.90& 20.56& 20.96& 20.51& 20.38& 19.48& 17.43&     1.70& -3.00&    4\\
   483&  161.680&   58.788& 17.86& 17.10& 16.66& 16.39& 15.95& 15.56& 15.71& 16.28& 14.69&     0.14& -3.00&    3\\
   484&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.87&-99.00&     0.00&-99.00&  -99\\
   485&  161.684&   59.363& 23.51& 22.90& 22.02& 21.41& 20.80& 20.56& 20.67& 19.85& 18.31&     0.85& -3.00&    3\\
   486&  161.684&   59.008& 23.03& 22.67& 22.28& 21.83& 21.28& 21.25& 20.66& 20.08&-99.00&     2.54& -3.00&    4\\
   487&  161.686&   59.188& 24.28& 23.88& 23.28& 22.92& 21.39& 21.39& 20.62& 19.92& 18.17&     1.62& -3.00&    3\\
   488&  161.690&   59.327& 23.33& 22.95& 22.37& 21.83& 21.37& 20.97& 20.63& 19.96& 17.11&     1.10& -3.00&    1\\
   489&  161.692&   58.748& 24.65&-99.00& 23.94& 24.04& 22.96&-99.00&-99.00&-99.00&-99.00&     0.00&  0.35&  -99\\
   490&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   491&  161.693&   59.263& 20.73& 20.48& 20.33& 20.26& 19.99& 20.04& 20.17& 19.58& 17.25&     1.67& -3.00&    4\\
   492&  161.694&   59.443& 23.91& 23.37& 22.57& 22.45& 21.40& 21.05& 20.63& 20.09& 18.31&    -1.00&  0.85&   -1\\
   493&  161.694&   59.212& 25.26&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     4.74& -3.00&    3\\
   494&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.89&-99.00&     4.08& -3.00&    3\\
   495&  161.697&   59.368& 25.19& 25.10& 25.18&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   496&  161.698&   59.023& 24.10& 23.96& 23.71& 23.31& 21.46& 21.31& 21.01& 20.35& 17.51&     3.29& -3.00&    3\\
   497&  161.698&   58.913&-99.00&-99.00&-99.00&-99.00& 21.91& 21.61& 21.46& 19.92&-99.00&     0.00&-99.00&  -99\\
   498&  161.700&   58.758& 24.28& 24.27& 24.09& 23.79&-99.00& 22.18&-99.00& 21.53&-99.00&     0.00&  0.75&  -99\\
   499&  161.700&   59.018& 25.22&-99.00& 24.70&-99.00&-99.00&-99.00&-99.00& 21.58&-99.00&     2.20& -3.00&    3\\
   500&  161.701&   58.776&-99.00& 20.34& 19.64& 19.28& 18.89& 18.40& 18.30& 18.70&-99.00&     0.49& -3.00&    3\\
   501&  161.705&   59.368&-99.00&-99.00& 23.90& 23.00& 22.25& 21.80& 20.90& 20.55&-99.00&    -1.00&  1.55&   -1\\
   502&  161.706&   58.925& 22.66& 22.35& 21.95& 21.81& 21.32& 21.09& 20.88& 20.46&-99.00&     1.55& -3.00&    4\\
   503&  161.710&   59.290& 19.58& 18.39& 17.87& 17.54& 17.18& 16.92& 16.66& 17.22& 15.76&     0.37& -3.00&    3\\
   504&  161.710&   59.177& 24.37& 23.30& 22.08& 21.50& 20.96& 20.57& 19.84& 19.35& 17.58&     0.89& -3.00&    3\\
   505&  161.713&   58.675& 21.21& 21.25& 21.06& 21.00& 20.62& 20.98&-99.00& 20.09& 17.49&    -1.00&  0.95&   -1\\
   506&  161.716&   58.814& 24.58& 23.86& 23.15& 22.53& 21.52& 20.96& 20.51& 19.81&-99.00&     0.00&  1.15&  -99\\
   507&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   508&  161.721&   59.431& 24.22& 23.20& 22.71& 22.19& 21.53& 21.43& 20.19& 19.50& 17.73&     1.43& -3.00&    1\\
   509&  161.721&   59.397&-99.00& 24.55& 23.37& 22.36& 21.33& 21.07& 20.45& 19.40&-99.00&     0.00&  1.15&  -99\\
   510&  161.722&   59.273&-99.00& 20.86& 20.08& 19.95& 19.56& 19.24& 18.95& 19.22&-99.00&     0.59& -3.00&    1\\
   511&  161.723&   58.960& 24.31& 23.37& 22.87& 22.33& 21.74& 21.44&-99.00& 20.16&-99.00&     0.00&  1.45&  -99\\
   512&  161.728&   58.968& 23.57& 23.03& 22.85& 22.34& 22.21& 21.44&-99.00& 21.03&-99.00&     1.20& -3.00&    4\\
   513&  161.728&   59.276&-99.00& 22.55& 21.68& 21.21& 20.78& 20.46& 20.14& 19.79&-99.00&     0.85& -3.00&    3\\
   514&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   515&  161.728&   59.193& 24.17& 23.90& 23.87& 23.09&-99.00&-99.00&-99.00&-99.00&-99.00&     1.31& -3.00&    1\\
   516&  161.729&   58.647&-99.00&-99.00&-99.00&-99.00& 20.80& 20.99&-99.00& 20.34& 18.15&    -1.00&-99.00&   -1\\
   517&  161.732&   59.050& 22.33&-99.00&-99.00& 20.21& 19.38& 19.88& 19.40& 18.36& 16.42&     0.83& -3.00&    3\\
   518&  161.736&   59.351& 21.91& 21.76& 21.63& 21.48& 21.29& 20.98& 20.79& 20.28&-99.00&    -1.00&  0.75&   -1\\
   519&  161.738&   59.389& 23.97& 23.41& 22.66& 21.86& 21.28& 21.01& 20.39& 19.71&-99.00&     1.22& -3.00&    1\\
   520&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.51&-99.00&     0.00&-99.00&  -99\\
   521&  161.749&   59.346& 22.72& 22.33& 21.90& 21.74& 21.26& 21.25& 21.17& 20.14&-99.00&    -1.00&  0.35&   -1\\
   522&  161.751&   59.317& 24.71&-99.00& 23.64& 23.16& 21.29& 21.38& 21.06& 20.45& 18.08&     0.00&  1.95&  -99\\
   523&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.96&-99.00&     0.00&-99.00&  -99\\
   524&  161.753&   58.736& 24.61& 24.63& 24.08&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&  0.15&  -99\\
   525&  161.753&   58.840& 23.90& 22.63& 21.73& 21.16& 20.51& 19.97& 19.56& 19.26&-99.00&    -1.00&  0.65&   -1\\
   526&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.37&-99.00&     0.00&-99.00&  -99\\
   527&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   528&  161.757&   59.243& 24.09& 23.67& 23.09& 22.92& 21.80& 21.78& 21.14& 20.90&-99.00&     0.00&  1.45&  -99\\
   529&  161.757&   59.114& 24.59& 23.76& 23.35& 22.98& 22.24&-99.00&-99.00& 21.36&-99.00&     0.00&  1.15&  -99\\
   530&  161.757&   58.840& 24.42& 23.47& 22.40& 21.57& 20.80& 20.32& 19.78& 19.11& 17.21&     1.05& -3.00&    0\\
   531&  161.759&   59.285&-99.00&-99.00&-99.00&-99.00& 22.56&-99.00&-99.00& 21.16&-99.00&     0.00&-99.00&  -99\\
   532&  161.758&   59.111&-99.00&-99.00&-99.00&-99.00&-99.00& 21.55&-99.00& 20.64&-99.00&     2.57& -3.00&    3\\
   533&  161.758&   59.420& 24.19& 24.23& 23.63& 23.59& 23.52&-99.00&-99.00& 21.58&-99.00&     2.88& -3.00&    3\\
   534&  161.759&   59.173& 18.69& 18.36& 18.12& 18.06& 18.07& 17.98& 17.97& 18.46& 16.53&     0.14& -3.00&    1\\
   535&  161.767&   58.881& 24.74& 24.73&-99.00& 23.73&-99.00& 21.82&-99.00& 20.78&-99.00&     0.00&  1.65&  -99\\
   536&  161.767&   59.408& 23.81& 23.55& 23.07& 23.00& 21.69&-99.00& 21.16& 20.60& 16.61&     0.00&  1.85&  -99\\
   537&  161.767&   59.387& 21.77& 21.55& 21.27& 21.21& 20.73& 20.68& 20.16& 19.56& 17.26&     1.68& -3.00&    4\\
   538&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   539&  161.770&   59.358& 23.47& 22.32& 21.67& 21.43& 20.85& 20.49& 20.26& 19.26& 17.33&     1.27& -3.00&    4\\
   540&  161.771&   59.058& 19.82& 18.88& 18.43& 18.15& 17.89& 17.63& 17.36& 17.98& 16.04&     0.29& -3.00&    1\\
   541&  161.771&   58.980& 24.81& 24.20& 24.08&-99.00&-99.00&-99.00&-99.00& 20.01& 17.30&     0.00&  1.15&  -99\\
   542&  161.771&   59.124& 18.58& 18.24& 18.30& 17.70& 17.87& 17.57& 17.07& 16.50& 14.34&     0.39& -3.00&    4\\
   543&  161.770&   59.186&-99.00&-99.00&-99.00&-99.00& 21.46& 21.14&-99.00& 20.45&-99.00&     0.00&-99.00&  -99\\
   544&  161.774&   58.751& 21.08& 21.17& 20.87& 20.98& 20.54& 20.16& 19.96& 19.09& 16.78&     1.38& -3.00&    4\\
   545&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.23&-99.00&     0.76& -3.00&    1\\
   546&  161.779&   58.864& 24.26& 24.14& 24.11& 23.70&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   547&  161.779&   59.337& 23.15& 22.46& 21.58& 20.60& 19.89& 19.53& 18.99& 18.44& 16.37&     1.00& -3.00&    1\\
   548&  161.779&   59.244& 24.50& 24.23& 23.52& 22.87& 22.24& 22.04&-99.00& 20.88&-99.00&    -1.00&  1.15&   -1\\
   549&  161.779&   59.169& 21.26& 21.00& 20.65& 20.48& 20.29& 20.07& 19.80& 19.71& 16.26&     0.50& -3.00&    3\\
   550&  161.780&   59.004& 22.72& 21.66& 21.23& 20.79& 20.43& 20.45& 20.13& 20.19&-99.00&     0.38& -3.00&    4\\
   551&  161.780&   59.214& 23.50& 23.18& 22.74& 22.52&-99.00&-99.00&-99.00& 21.11&-99.00&     0.00&  0.25&  -99\\
   552&  161.781&   59.385& 23.59& 22.13& 21.32& 20.99& 20.46& 20.24& 19.83& 20.34&-99.00&     0.46& -3.00&    0\\
   553&  161.781&   59.179& 23.00& 22.87& 22.54& 22.42& 21.80& 21.33& 20.73& 20.39&-99.00&     0.00&  0.25&  -99\\
   554&  161.781&   59.309& 23.92& 23.53& 23.06& 22.65& 21.65& 21.25& 20.84& 20.17&-99.00&     0.00&  1.45&  -99\\
   555&  161.781&   58.912&-99.00&-99.00& 24.29& 23.31& 22.10& 21.44& 20.86& 20.13&-99.00&     0.00&  1.75&  -99\\
   556&  161.783&   59.418&-99.00&-99.00&-99.00&-99.00& 22.42&-99.00&-99.00& 20.49&-99.00&     0.00&-99.00&  -99\\
   557&  161.782&   58.894& 18.97& 18.38& 17.98& 17.74& 17.48& 17.26& 17.16& 17.73& 16.72&     0.12& -3.00&    1\\
   558&  161.783&   58.643&-99.00&-99.00&-99.00&-99.00& 21.34& 21.85&-99.00& 20.91&-99.00&    -1.00&-99.00&   -1\\
   559&  161.784&   58.699& 23.86& 23.74& 23.71& 24.10&-99.00&-99.00&-99.00& 21.00&-99.00&     1.23& -3.00&    4\\
   560&  161.787&   59.081& 18.03& 17.11& 16.65& 16.36& 16.09& 15.90& 15.91& 16.50&-99.00&     0.12& -3.00&    0\\
   561&  161.789&   58.645& 23.40& 22.94& 22.77& 22.56& 21.90& 21.24&-99.00& 20.61& 18.23&    -1.00&  0.75&   -1\\
   562&  161.789&   58.800&-99.00& 24.09& 23.29& 22.82& 21.73& 20.90& 20.07& 18.53& 16.89&     1.00& -3.00&    0\\
   563&  161.794&   58.857& 23.91& 23.26& 22.79& 22.24& 21.32& 20.97& 20.65& 20.06&-99.00&    -1.00&  1.35&   -1\\
   564&  161.799&   58.821& 24.76& 24.02& 23.82& 23.85&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&  0.15&  -99\\
   565&  161.799&   59.035& 22.78& 22.06& 21.48& 20.93& 20.49& 20.28& 19.84& 19.32& 17.90&     0.79& -3.00&    4\\
   566&  161.799&   59.156& 21.43& 20.37& 19.76& 19.42& 18.67& 18.62& 17.85& 18.15& 16.89&     0.50& -3.00&    4\\
   567&  161.801&   59.322& 23.06& 22.91& 22.52& 22.03& 21.82& 21.28& 21.45& 21.13&-99.00&     1.21& -3.00&    3\\
   568&  161.802&   59.307& 23.60& 23.98& 23.63& 23.31&-99.00&-99.00&-99.00&-99.00&-99.00&     2.34& -3.00&    3\\
   569&  161.803&   59.397& 24.24& 23.53& 22.92& 22.58& 21.65& 21.01& 20.52& 19.86& 17.42&     0.81& -3.00&    0\\
   570&  161.806&   59.289& 23.89& 23.01& 22.04& 21.63& 20.95& 20.56& 20.07& 19.86&-99.00&     0.75& -3.00&    1\\
   571&  161.807&   59.250& 20.93& 20.33& 19.96& 19.57& 19.30& 18.94& 18.71& 18.84& 15.99&     0.36& -3.00&    4\\
   572&  161.807&   59.145& 21.50& 19.77& 19.11& 18.78& 18.37& 17.97& 17.78& 18.35&-99.00&    -1.00&  0.55&   -1\\
   573&  161.807&   58.711& 24.76& 22.98& 21.82& 20.82& 20.25& 19.98& 19.37& 18.87& 17.96&     0.97& -3.00&    1\\
   574&  161.809&   58.866&-99.00& 24.06& 22.67& 21.98& 21.31& 20.52& 20.12& 19.09&-99.00&    -1.00&  1.45&   -1\\
   575&  161.811&   58.763&-99.00& 22.23& 21.24& 20.61& 20.10& 19.62& 19.28& 19.00&-99.00&     0.79& -3.00&    3\\
   576&  161.812&   59.057& 23.75& 23.43& 22.98& 22.90& 22.01&-99.00& 20.76& 20.57&-99.00&     0.00&-99.00&  -99\\
   577&  161.813&   58.800& 25.42& 24.95& 24.42& 24.37& 22.16& 21.92& 21.34& 20.97&-99.00&    -1.00&  2.05&   -1\\
   578&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.83& 16.91&     0.00&-99.00&  -99\\
   579&  161.814&   59.163& 25.32& 24.20& 23.59& 23.07& 22.98&-99.00&-99.00&-99.00&-99.00&     0.00&  0.55&  -99\\
   580&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.74&-99.00&    -1.00&-99.00&   -1\\
   581&  161.826&   59.052& 24.41& 24.21& 23.84& 23.51&-99.00&-99.00& 21.23& 20.87&-99.00&     1.51& -3.00&    1\\
   582&  161.828&   58.855& 23.79& 22.44& 21.37& 20.67& 20.41& 19.95& 19.86& 19.83&-99.00&     0.00&  0.95&  -99\\
   583&  161.828&   59.021& 20.54& 19.35& 18.74& 18.33& 17.73& 17.30& 16.97& 17.36& 15.85&     0.29& -3.00&    3\\
   584&  161.828&   58.816& 22.30& 22.01& 21.37& 20.90& 20.68& 20.30& 20.30& 19.50&-99.00&     0.75& -3.00&    3\\
   585&  161.829&   59.000& 21.47& 21.24& 21.02& 20.94& 20.97& 20.84& 20.88&-99.00& 18.25&     1.19& -3.00&    4\\
   586&  161.837&   59.289& 24.06& 23.56& 22.75& 22.31& 21.06& 20.60& 20.35& 20.09&-99.00&     1.53& -3.00&    4\\
   587&  161.842&   58.707& 24.53& 23.43& 22.69& 22.06& 21.35& 21.22& 20.33& 19.92&-99.00&    -1.00&  1.15&   -1\\
   588&  161.844&   58.843& 22.04& 21.36& 20.43& 20.08& 19.73& 19.24& 19.21& 18.97&-99.00&     0.68& -3.00&    0\\
   589&  161.845&   58.716& 20.24& 20.23& 20.22& 20.12& 20.16& 20.19& 19.88& 20.00& 17.50&     2.26& -3.00&    4\\
   590&  161.846&   58.892& 24.07& 23.04& 21.94& 21.51& 20.90& 20.66& 19.87& 19.72& 17.71&     0.75& -3.00&    1\\
   591&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.30& -3.00&    0\\
   592&  161.848&   59.407& 24.04& 23.54& 23.26& 22.96& 22.93&-99.00&-99.00& 21.45&-99.00&     3.22& -3.00&    3\\
   593&  161.847&   59.371&-99.00& 24.75& 23.64& 23.01& 21.80& 21.35& 21.16& 20.10&-99.00&     1.12& -3.00&    1\\
   594&  161.849&   59.144& 23.37& 22.95& 22.71& 22.56&-99.00&-99.00& 21.16& 20.53&-99.00&     0.81& -3.00&    3\\
   595&  161.852&   59.209& 23.00& 22.54& 21.96& 21.54& 21.55& 21.09& 21.22& 20.84&-99.00&     0.71& -3.00&    3\\
   596&  161.854&   59.019& 24.76& 24.59& 24.18&-99.00&-99.00& 21.96& 21.39& 20.82&-99.00&    -1.00&  0.95&   -1\\
   597&  161.856&   58.988& 22.42& 21.98& 21.51& 21.24& 21.04& 21.08& 20.56& 20.13& 18.14&    -5.00&  0.25&  -99\\
   598&  161.858&   59.174& 22.97& 21.54& 21.12& 20.68& 20.51& 19.90& 19.63& 18.87& 16.77&     1.14& -3.00&    4\\
   599&  161.862&   59.317&-99.00&-99.00&-99.00& 24.10& 21.98& 21.79& 20.89& 20.28&-99.00&     0.00&  2.65&  -99\\
   600&  161.863&   59.025& 24.54& 24.19& 23.53& 22.83& 22.10& 21.43& 21.34& 20.22&-99.00&     0.95& -3.00&    1\\
   601&  161.871&   59.092& 22.16& 21.50& 20.87& 20.36& 19.74& 19.58& 19.27& 18.73& 16.87&     0.89& -3.00&    4\\
   602&  161.873&   59.052& 24.17& 22.59& 19.69& 18.33& 17.13& 16.93& 16.94& 17.51&-99.00&    -1.00&  1.35&   -1\\
   603&  161.876&   58.717& 21.13& 21.01& 21.05& 20.82& 20.59& 20.79& 20.12& 20.51&-99.00&     2.55& -3.00&    4\\
   604&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   605&  161.879&   59.428& 24.72& 23.87& 23.23& 22.71& 21.49& 21.51& 20.69& 20.05&-99.00&    -1.00&  1.75&   -1\\
   606&  161.879&   58.928& 22.74& 21.47& 20.36& 19.99& 19.54& 19.24& 18.74& 18.98&-99.00&     0.00&  0.65&  -99\\
   607&  161.883&   59.409& 24.87& 24.40& 23.73& 23.38& 21.81&-99.00& 20.93& 20.31&-99.00&     0.00&  1.65&  -99\\
   608&  161.882&   58.827&-99.00&-99.00&-99.00&-99.00& 16.18& 15.94& 15.88& 16.22&-99.00&     0.30& -3.00&    0\\
   609&  161.883&   59.334& 19.82& 18.45& 16.92& 15.90& 15.44& 15.31& 15.26& 15.95&-99.00&    -2.00&-99.00&   -2\\
   610&  161.887&   58.792& 23.48& 22.93& 22.67& 22.49& 22.43& 21.14& 20.76&-99.00&-99.00&    -5.00&  0.25&  -99\\
   611&  161.887&   59.167& 21.66& 19.75& 19.14& 18.78& 18.38& 18.01& 17.81& 18.50&-99.00&     0.35& -3.00&    3\\
   612&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   613&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 19.56& 16.85&     0.50& -3.00&    1\\
   614&  161.891&   59.042&-99.00& 23.75& 23.31& 22.72&-99.00&-99.00&-99.00&-99.00&-99.00&     4.50& -3.00&    4\\
   615&  161.892&   58.714& 23.58& 23.32& 22.80& 22.54& 21.19& 20.97& 20.35& 20.07&-99.00&    -1.00&  1.95&   -1\\
   616&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.90&-99.00&     0.00&-99.00&  -99\\
   617&  161.900&   59.097& 25.41&-99.00& 23.91& 23.66&-99.00&-99.00&-99.00& 20.75& 18.06&     0.89& -3.00&    1\\
   618&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.98&-99.00&     0.00&-99.00&  -99\\
   619&  161.903&   59.068& 25.34& 24.66& 24.73&-99.00&-99.00&-99.00&-99.00& 21.12&-99.00&     2.57& -3.00&    3\\
   620&  161.904&   59.328&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.29& 20.10& 17.67&     0.00&-99.00&  -99\\
   621&  161.905&   59.304&-99.00&-99.00& 23.87& 23.22& 21.76&-99.00&-99.00& 20.28&-99.00&     0.00&  1.55&  -99\\
   622&  161.905&   59.377& 23.29& 22.18& 21.63& 21.27& 20.68& 20.71& 20.32& 19.61& 16.61&     1.52& -3.00&    4\\
   623&  161.909&   59.027& 21.86& 22.47& 21.80& 21.84& 21.33& 21.00& 20.75& 20.02&-99.00&     2.09& -3.00&    4\\
   624&  161.910&   58.879& 24.51& 23.60& 22.55& 21.45& 20.50& 20.07& 19.56& 18.81&-99.00&     0.00&  1.35&  -99\\
   625&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.61&-99.00&     0.00&-99.00&  -99\\
   626&  161.914&   59.195& 23.00& 22.64& 22.19& 21.89& 21.63& 21.35& 20.94& 19.96& 17.83&     1.75& -3.00&    4\\
   627&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.53&-99.00&     0.00&-99.00&  -99\\
   628&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   629&  161.924&   59.336& 25.35& 24.99& 24.85& 24.19&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.75&   -1\\
   630&  161.931&   59.411& 14.60& 13.89& 13.45& 13.09& 12.69& 12.58& 12.80& 13.22& 16.31&    -1.00&  0.25&   -1\\
   631&  161.931&   59.314& 20.13& 19.66& 19.72& 19.55& 19.16& 19.29& 18.89& 18.01& 16.05&     1.02& -3.00&    4\\
   632&  161.937&   59.430& 17.51& 16.77& 16.36& 15.90& 15.97& 15.89& 16.07& 16.98&-99.00&    -1.00&  0.15&   -1\\
   633&  161.937&   59.094& 21.98& 21.59& 20.89& 20.53& 20.15& 19.80& 19.45& 19.29&-99.00&     0.81& -3.00&    1\\
   634&  161.941&   59.473& 24.40& 23.61& 22.61& 22.01& 21.65&-99.00& 21.10& 20.82&-99.00&    -1.00&  0.55&   -1\\
   635&  161.942&   59.434& 22.99& 22.90& 22.34& 22.32& 21.84&-99.00& 21.15& 20.35& 17.20&    -1.00&-99.00&   -1\\
   636&  161.943&   59.398& 17.22& 16.26& 15.72& 15.11& 15.11& 14.89& 14.80& 15.67& 17.36&    -1.00&  0.55&   -1\\
   637&  161.948&   59.136& 16.57& 15.93& 15.80& 15.20& 15.33& 15.39& 15.68& 16.65&-99.00&    -2.00&-99.00&   -2\\
   638&  161.948&   59.091& 23.56& 22.29& 20.59& 19.90& 19.23& 18.86& 18.57& 17.94&-99.00&     0.89& -3.00&    1\\
   639&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   640&  161.949&   59.338& 25.61&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   641&  161.950&   59.226& 24.68& 23.77& 23.30& 22.96& 22.70&-99.00&-99.00& 21.50&-99.00&     0.00&  0.35&  -99\\
   642&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.82&-99.00&     0.00&-99.00&  -99\\
   643&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.54&-99.00&    -1.00&-99.00&   -1\\
   644&  161.951&   59.344& 23.95& 23.65& 23.19& 23.07& 22.11&-99.00& 21.35& 20.82&-99.00&     0.00&  0.65&  -99\\
   645&  161.953&   59.391& 19.46& 19.25& 19.05& 19.00& 19.17& 18.89& 19.02& 18.52& 16.11&    -1.00&  1.75&   -1\\
   646&  161.954&   59.036& 21.23& 20.71& 20.54& 20.44& 20.55& 20.59& 20.66& 20.37&-99.00&     0.15& -3.00&    1\\
   647&  161.957&   58.813& 23.75& 23.26& 22.86& 22.63& 21.86& 21.15& 21.14& 20.47&-99.00&     0.00&  1.15&  -99\\
   648&  161.962&   59.092& 24.57&-99.00& 23.93& 23.59&-99.00&-99.00&-99.00& 21.70&-99.00&    -1.00&  0.45&   -1\\
   649&  161.962&   58.932& 22.62& 21.64& 20.71& 20.26& 19.76& 19.33& 18.84& 18.57& 18.09&     0.74& -3.00&    0\\
   650&  161.963&   58.990& 21.22& 20.13& 19.61& 19.27& 18.88& 18.54& 18.27& 18.75& 17.68&     0.44& -3.00&    3\\
   651&  161.963&   58.861& 22.69& 21.40& 20.36& 19.97& 19.42& 18.83& 18.34& 17.89& 15.37&    -1.00&  0.55&   -1\\
   652&  161.964&   58.810& 24.13& 23.80& 23.25& 22.97& 22.16& 21.69&-99.00& 21.52&-99.00&    -1.00&  1.15&   -1\\
   653&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.65&-99.00&     0.00&-99.00&  -99\\
   654&  161.968&   59.264&-99.00& 21.06& 20.50& 20.49& 20.47& 20.54& 20.26& 19.44& 16.56&     1.96& -3.00&    4\\
   655&  161.970&   59.207&-99.00& 23.84& 22.86& 22.18& 21.48& 20.85& 20.43& 19.71& 17.11&     0.93& -3.00&    1\\
   656&  161.977&   59.002& 24.55& 24.25& 23.52& 23.13& 21.65& 21.20& 20.72& 20.13&-99.00&     0.00&  1.55&  -99\\
   657&  161.977&   59.453& 23.83& 23.71& 24.05& 23.48&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.55&   -1\\
   658&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.46&-99.00&    -1.00&-99.00&   -1\\
   659&  161.985&   59.127& 23.94& 23.23& 22.58& 21.87& 21.16& 20.66& 20.14& 19.58&-99.00&     0.00&  1.05&  -99\\
   660&  161.987&   58.893& 24.49& 23.93& 23.50& 22.92& 22.31& 21.25& 20.98& 20.28&-99.00&     0.00&  1.15&  -99\\
   661&  161.990&   58.837& 24.04& 24.10&-99.00& 23.44&-99.00&-99.00&-99.00& 21.75&-99.00&    -1.00&  0.55&   -1\\
   662&  161.990&   58.837&-99.00&-99.00& 23.79&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   663&  161.994&   59.347& 24.73& 23.78& 22.71& 21.89& 21.40& 20.91& 20.58& 19.80&-99.00&    -1.00&  0.95&   -1\\
   664&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   665&  161.994&   59.037& 23.41& 22.42& 21.76& 21.54& 21.14& 20.82& 20.50& 20.95&-99.00&    -1.00&  0.35&   -1\\
   666&  161.996&   59.180& 22.38& 21.89& 21.73& 21.23& 21.06& 20.93& 20.52& 20.24&-99.00&    -1.00&  0.55&   -1\\
   667&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.49&-99.00&     0.00&-99.00&  -99\\
   668&  161.998&   59.035& 25.55& 24.48& 24.22& 24.03&-99.00&-99.00&-99.00& 21.49&-99.00&    -1.00&  0.45&   -1\\
   669&  162.000&   58.939& 25.08& 24.82& 24.38& 23.65&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  1.15&   -1\\
   670&  162.003&   58.836& 24.19& 23.11& 21.86& 21.01& 20.28& 19.99& 19.63& 19.12&-99.00&     1.04& -3.00&    1\\
   671&  162.004&   59.159& 22.43& 21.85& 21.14& 21.00& 20.63& 20.08& 19.91& 20.00&-99.00&     0.68& -3.00&    1\\
   672&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   673&  162.007&   59.351& 24.77& 23.62& 22.51& 22.05& 21.39&-99.00& 21.03& 21.00&-99.00&     0.81& -3.00&    3\\
   674&  162.013&   59.410& 22.44& 22.47& 22.01& 22.01& 21.62&-99.00& 21.07& 20.31&-99.00&    -1.00&-99.00&   -1\\
   675&  162.013&   59.330& 24.27& 23.29& 22.22& 21.83& 21.14& 21.24& 20.34& 19.64& 17.83&     1.79& -3.00&    4\\
   676&  162.014&   58.930& 20.55& 20.35& 20.00& 19.91& 19.90& 19.95& 19.65&-99.00& 16.95&     1.72& -3.00&    4\\
   677&  162.018&   59.169& 25.98& 25.22& 24.48& 24.41& 22.18& 21.69& 21.46& 20.78&-99.00&     0.00&  1.65&  -99\\
   678&  162.019&   59.013& 24.17& 23.67& 23.31& 22.98& 21.60& 21.26& 20.53& 19.74&-99.00&     0.00&  2.35&  -99\\
   679&  162.024&   58.860& 23.78& 23.13& 22.70& 22.65& 21.88& 21.38&-99.00& 20.32&-99.00&     1.47& -3.00&    1\\
   680&  162.029&   58.880& 24.60& 23.82& 23.55& 23.21& 22.17& 21.68&-99.00& 21.04&-99.00&     0.00&  1.15&  -99\\
   681&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   682&  162.028&   59.428&-99.00&-99.00&-99.00&-99.00& 19.68& 19.28&-99.00& 19.59&-99.00&    -1.00&-99.00&   -1\\
   683&  162.030&   58.806& 25.09& 24.79& 23.84& 23.06& 22.07& 21.79& 20.87& 20.36&-99.00&     1.24& -3.00&    1\\
   684&  162.030&   58.707& 21.00& 20.62& 20.40& 20.24& 19.92& 19.92& 19.64& 19.55& 17.16&    -1.00&  0.15&   -1\\
   685&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.90&-99.00&     0.00&-99.00&  -99\\
   686&  162.032&   59.261& 20.49& 19.61& 19.13& 18.84& 18.43& 18.05& 18.04& 18.49& 16.11&     0.22& -3.00&    1\\
   687&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.70&-99.00&    -1.00&-99.00&   -1\\
   688&  162.034&   59.321& 23.04& 21.89& 21.06& 20.81& 20.23& 20.02& 19.70& 19.89&-99.00&     0.58& -3.00&    3\\
   689&  162.038&   59.339& 24.07& 23.57& 22.91& 22.37& 21.20& 20.69& 20.39& 19.82&-99.00&     0.00&  1.35&  -99\\
   690&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   691&  162.038&   59.256& 24.02& 23.20& 22.55& 21.77& 21.14& 20.52& 20.31& 19.85&-99.00&     0.00&  0.65&  -99\\
   692&  162.042&   59.227& 21.79& 21.84& 21.54& 21.43& 21.73& 21.39& 21.28& 20.99&-99.00&    -1.00&  2.35&   -1\\
   693&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   694&  162.044&   59.010& 21.31& 21.01& 20.57& 20.38& 20.08& 19.70& 19.47& 19.37&-99.00&     0.59& -3.00&    4\\
   695&  162.047&   59.238&-99.00&-99.00&-99.00&-99.00& 21.02& 20.61& 20.86& 19.23&-99.00&     0.44& -3.00&    1\\
   696&  162.049&   59.180& 21.00& 20.96& 20.85& 20.61& 20.46& 19.93& 19.63& 18.88& 16.65&     0.71& -3.00&    4\\
   697&  162.050&   58.992& 25.13& 24.77& 24.23& 23.65&-99.00&-99.00&-99.00& 21.97&-99.00&    -1.00&  0.25&   -1\\
   698&  162.051&   59.050& 23.03& 22.52& 22.25& 21.99& 21.54&-99.00& 21.17& 20.85&-99.00&    -1.00&  0.25&   -1\\
   699&  162.053&   58.909& 25.06& 24.02& 22.86& 21.95& 21.02& 20.50& 20.20& 19.40&-99.00&    -1.00&  1.25&   -1\\
   700&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.98&-99.00&    -1.00&-99.00&   -1\\
   701&  162.058&   58.782&-99.00& 25.14& 24.67& 23.88& 22.70& 21.87&-99.00& 21.68&-99.00&    -1.00&-99.00&   -1\\
   702&  162.058&   58.843& 23.74& 22.69& 22.76& 22.04& 21.58& 20.95& 20.85& 20.35&-99.00&    -1.00&  1.15&   -1\\
   703&  162.062&   59.061& 23.57& 22.16& 21.50& 21.18& 20.86& 20.42& 20.36& 20.89&-99.00&    -1.00&  0.45&   -1\\
   704&  162.063&   59.394&-99.00&-99.00&-99.00&-99.00& 21.83&-99.00&-99.00& 20.57&-99.00&    -1.00&-99.00&   -1\\
   705&  162.064&   58.771&-99.00& 24.45& 24.54& 24.56&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.15&   -1\\
   706&  162.067&   59.179&-99.00&-99.00&-99.00&-99.00&-99.00& 21.75&-99.00& 21.38&-99.00&    -1.00&-99.00&   -1\\
   707&  162.069&   58.733&-99.00&-99.00&-99.00&-99.00&-99.00& 22.21&-99.00& 20.40&-99.00&     0.00&-99.00&  -99\\
   708&  162.070&   59.300& 21.17& 20.18& 19.73& 19.43& 19.05& 18.84& 18.61& 19.11&-99.00&     0.33& -3.00&    4\\
   709&  162.075&   58.998& 18.26& 17.08& 16.47& 15.70& 15.39& 15.28& 15.45& 16.17&-99.00&    -1.00&  0.35&   -1\\
   710&  162.077&   58.759&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.36& 21.11&-99.00&    -1.00&-99.00&   -1\\
   711&  162.079&   58.878& 21.09& 20.96& 20.78& 20.64& 20.48& 20.35& 20.20& 19.95& 16.69&    -1.00&  0.55&   -1\\
   712&  162.080&   58.775&-99.00& 21.37& 20.53& 20.24& 19.71& 19.47& 18.70& 18.02& 16.28&    -1.00&  0.65&   -1\\
   713&  162.082&   59.160& 22.25& 21.77& 20.82& 20.42& 20.23& 19.79& 19.57& 19.16& 17.75&    -1.00&  0.55&   -1\\
   714&  162.083&   59.156& 23.98& 23.66& 23.14& 22.40& 21.77& 21.15& 20.85& 20.67&-99.00&    -1.00&  0.55&   -1\\
   715&  162.084&   59.300& 25.48& 24.54& 24.76&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   716&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.32&-99.00&    -1.00&-99.00&   -1\\
   717&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   718&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   719&  162.093&   59.303& 24.22& 23.80& 23.13& 22.60& 22.41&-99.00&-99.00& 20.82&-99.00&    -1.00&  0.55&   -1\\
   720&  162.095&   59.258& 24.40& 23.97& 23.62& 23.30& 22.61& 22.05&-99.00& 21.25&-99.00&    -1.00&  1.15&   -1\\
   721&  162.103&   58.822& 22.12& 21.86& 21.38& 20.78& 20.53& 20.23& 19.78& 19.44& 17.62&    -1.00&  0.25&   -1\\
   722&  162.106&   59.191& 24.20& 23.94& 23.32& 22.98& 21.85& 21.09& 20.87& 20.21&-99.00&     0.00&  1.15&  -99\\
   723&  162.107&   59.228&-99.00&-99.00&-99.00&-99.00&-99.00& 20.77&-99.00& 19.86& 16.41&    -1.00&-99.00&   -1\\
   724&  162.109&   59.015& 21.19& 21.33& 21.09& 21.06& 21.15& 21.17& 20.41& 19.99& 18.21&    -1.00&  0.95&   -1\\
   725&  162.113&   58.911& 23.40&-99.00&-99.00&-99.00& 21.27& 20.89& 20.91&-99.00&-99.00&    -1.00&  0.35&   -1\\
   726&  162.113&   58.816& 25.34& 24.02& 22.67& 22.02& 21.26& 21.08& 20.57& 20.52&-99.00&    -1.00&  0.95&   -1\\
   727&  162.112&   58.911&-99.00& 23.02& 22.63& 22.35&-99.00&-99.00&-99.00& 20.22& 17.55&    -1.00&  0.75&   -1\\
   728&  162.120&   58.867&-99.00&-99.00&-99.00& 11.13& 11.85& 11.63& 10.75& 11.47& 14.75&    -1.00&-99.00&   -1\\
   729&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00&-99.00&  -99\\
   730&  162.123&   59.214& 21.90& 20.89& 20.41& 20.18& 19.91& 19.68& 19.65& 18.82& 16.57&     1.51& -3.00&    4\\
   731&  162.127&   58.857& 25.04& 24.54& 24.18& 23.79&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.55&   -1\\
   732&  162.132&   58.873& 25.33& 24.68& 23.99& 23.69&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&  0.35&   -1\\
   733&  162.137&   59.288& 23.63& 23.13& 22.56& 22.11& 21.72&-99.00& 21.15& 19.99&-99.00&    -1.00&  0.25&   -1\\
   734&  162.146&   58.940&-99.00&-99.00&-99.00&-99.00& 22.82&-99.00& 20.96& 20.05&-99.00&    -1.00&-99.00&   -1\\
   735&  162.148&   58.768&-99.00& 23.68& 23.13& 22.64& 21.74& 21.56& 20.95& 20.63&-99.00&    -1.00&  2.15&   -1\\
   736&  162.150&   59.202& 20.70& 20.67& 20.40& 20.39& 20.29& 20.19& 20.16& 19.76& 17.08&     1.74& -3.00&    4\\
   737&  162.153&   58.904& 24.14& 23.04& 22.06& 21.64& 21.08& 20.52& 20.30& 19.31& 16.51&    -1.00&  0.55&   -1\\
   738&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.06&-99.00&     0.00&-99.00&  -99\\
   739&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   740&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00&-99.00&   -1\\
   741&  162.158&   58.868& 23.65& 22.82&-99.00& 20.78& 19.82& 19.65& 19.38& 18.68&-99.00&    -1.00&  1.55&   -1\\
   742&  162.163&   59.014& 21.65& 21.56& 21.30& 21.13& 21.43& 21.15& 20.78& 20.50&-99.00&     2.19& -3.00&    4\\
   743&  162.165&   58.992& 23.22& 23.21& 23.14& 23.09& 22.12&-99.00& 21.43& 21.09&-99.00&    -1.00&-99.00&   -1\\
   744&  162.169&   59.172& 22.38& 20.95& 20.17& 19.84& 19.60& 18.96& 18.81& 18.85&-99.00&     0.51& -3.00&    3\\
   745&  162.172&   59.049& 22.11& 21.15& 21.45& 20.97& 20.81& 20.29& 20.17& 19.52& 17.73&     1.44& -3.00&    4\\
   746&  162.175&   58.971& 22.49& 21.90& 21.66& 21.36& 20.97& 20.82& 20.37& 20.07&-99.00&     1.18& -3.00&    4\\
   747&  162.180&   59.056& 24.92& 23.80& 23.32& 23.29& 22.18&-99.00& 21.03& 21.39& 16.58&     3.57& -3.00&    3\\
   748&  162.180&   58.761&-99.00& 23.88& 23.16& 22.49& 21.22& 21.06& 20.18& 19.24& 16.79&    -1.00&  1.55&   -1\\
   749&  162.181&   59.053& 22.59& 22.29& 22.02& 21.82& 21.52& 21.55& 20.71& 19.96& 17.09&     1.76& -3.00&    4\\
   750&  162.184&   59.118& 22.49& 22.14& 21.94& 21.76& 21.35& 20.84& 20.45& 19.93&-99.00&     1.44& -3.00&    3\\
   751&  162.189&   58.962& 20.98& 20.89& 20.83& 20.57& 20.70& 20.50& 19.97& 19.62&-99.00&     1.79& -3.00&    4\\
   752&  162.192&   58.880& 23.33& 22.74& 22.06& 21.63& 21.08& 20.66& 20.59& 20.11&-99.00&    -1.00&  0.55&   -1\\
   753&  162.196&   59.082& 22.14& 21.81& 21.47& 21.64& 21.84& 21.86& 21.53& 20.76&-99.00&     0.14& -3.00&    4\\
   754&  162.198&   59.095&-99.00& 24.78&-99.00&-99.00&-99.00&-99.00& 21.33& 20.71&-99.00&     0.00&  0.95&  -99\\
   755&  162.210&   58.986& 24.48&-99.00& 23.39& 22.72& 21.07& 20.73& 20.42& 20.09&-99.00&     0.00&  1.75&  -99\\
   756&  162.214&   58.740&-99.00&-99.00&-99.00&-99.00&-99.00& 19.65& 19.15& 19.18&-99.00&    -1.00&-99.00&   -1\\
   757&  162.218&   58.755&-99.00&-99.00&-99.00& 11.28& 11.96& 12.22& 11.23& 12.23& 16.18&    -1.00&-99.00&   -1\\
   758&  162.219&   58.936&-99.00&-99.00&-99.00&-99.00& 22.84&-99.00&-99.00& 21.78&-99.00&    -1.00&-99.00&   -1\\
   759&  162.218&   58.795& 22.84&-99.00& 22.55& 22.21& 22.25& 21.97&-99.00& 20.76&-99.00&    -1.00&  0.35&   -1\\
   760&  162.220&   59.006& 24.39& 23.63& 22.64& 21.72& 21.11& 20.67& 20.38& 19.98&-99.00&     1.20& -3.00&    1\\
   761&  162.221&   58.901& 22.13& 21.76& 21.44& 21.19& 20.71& 20.46& 20.05& 19.20& 17.08&    -1.00&  0.65&   -1\\
    ..&       ..&       ..&    ..&    ..&    ..&    ..&    ..&    ..&    ..&    ..&    ..&       ..&    ..&    ..\\
\tableline
\end{tabular}
\end{scriptsize}
\footnotesize
\tablecomments{All magnitudes are in AB magnitudes.\\
Typical photometric uncertainties are given in \S \ref{photodet}.\\
Magnitude $=-99$, source not detected ($2\sigma$ significance). \\
$z_{spec} = 0$ and corresponding class $= -99$, source spectroscopically observed but neither the redshift nor the class could be identified. \\
$z_{spec} = -1$ and corresponding class $= -1$, source not yet spectroscopically observed. \\
$z_{spec} = -2$ and corresponding class $= -2$, source is a star. \\
$z_{phot} = -3$, source has a spectroscopic redshift.\\
$z_{phot} = -99$, source has neither a spectroscopic nor a photometric redshift. \\
class $=0$, absorbers; class $=1$, star formers; class $=3$, high-excitation sources; class $=4$, broad-line AGNs.}
\end{table}


==> tab12.tex <==
\begin{table}
\begin{scriptsize}
\caption{CLASXS Optical/IR Counterparts Catalog}
\label{CLASXSopt table}
\begin{tabular}{cccccccccccccccccc}
\tableline\tableline
    \#&       RA&      DEC&   $u$&   $B$&   $g'$&   $V$&   $R$&   $i'$&   $z'$&   $J$&   $H$&   $K$&$3.6~\mu$m& $24~\mu$m&z$_{spec}$&z$_{phot}$& class\\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)& (10)&(11) & (12) & (13) & (14) & (15) & (16) & (17) & (18)\\
\tableline
     1&  157.731&   57.556& 24.33&-99.00& 23.69&-99.00& 22.44& 21.91&-99.00& 20.17& 20.30&-99.00& -1.00&-99.00&    -1.00$^s $&  0.55&   -1\\
     2&  157.748&   57.646&-99.00&-99.00& 23.74&-99.00& 21.97& 21.44&-99.00& 20.44& 20.17&-99.00& -1.00& 17.84&    -1.00$^s $&  0.45&   -1\\
     3&  157.764&   57.614& 23.96&-99.00&-99.00&-99.00& 22.80& 22.65&-99.00& 22.06& 21.88&-99.00& -1.00&-99.00&     0.00$^s $&  0.25&  -99\\
     4&  157.774&   57.630& 23.80&-99.00& 23.78&-99.00& 23.04& 22.96& 23.05& 22.56&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
     5&  157.800&   57.590& 25.29& 24.51& 24.27&-99.00& 23.24& 22.71& 22.39& 21.94& 21.76&-99.00& -1.00&-99.00&     0.00$^s $&  0.35&  -99\\
     6&  157.841&   57.526&-99.00&-99.00&-99.00&-99.00& 25.32&-99.00&-99.00& 21.93& 21.56&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
     7&  157.848&   57.719& 20.86& 20.78& 20.38&-99.00& 19.81& 19.48& 19.19& 18.90& 18.87&-99.00& -1.00& 16.71&    -1.00$^s $&  0.15&   -1\\
     8&  157.860&   57.629& 24.61& 24.37& 23.94&-99.00& 23.40& 23.29& 22.57& 21.84& 21.45&-99.00& -1.00&-99.00&     0.00$^s $&  0.35&  -99\\
     9&  157.874&   57.620& 24.75& 24.55& 24.30&-99.00& 23.75& 23.70& 23.29& 21.93& 21.69&-99.00& -1.00&-99.00&     0.00$^s $&  1.15&  -99\\
    10&  157.874&   57.545& 24.64& 24.62& 24.70&-99.00& 24.39&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     1.47$^s $& -3.00&    1\\
    11&  157.880&   57.660& 22.29& 20.92& 20.03&-99.00& 18.18& 17.89& 17.35& 17.01& 16.82& 16.34& -1.00&-99.00&     0.36$^s $& -3.00&    0\\
    12&  157.881&   57.726&-99.00& 26.68&-99.00&-99.00& 25.06&-99.00& 23.65& 21.86& 21.50&-99.00& -1.00&-99.00&     0.00$^s $&  1.95&  -99\\
    13&  157.889&   57.703& 24.66& 24.30& 23.88&-99.00& 22.44& 21.84& 21.19& 20.64& 20.50& 20.11& -1.00&-99.00&     0.72$^s $& -3.00&    1\\
    14&  157.891&   57.653&-99.00&-99.00&-99.00&-99.00& 26.13&-99.00&-99.00&-99.00& 22.05&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    15&  157.893&   57.707&-99.00& 24.23& 24.19&-99.00& 23.38& 23.36& 22.24& 21.41& 21.59& 19.96& -1.00& 14.95&     2.86$^s $& -3.00&    4\\
    16&  157.894&   57.746& 20.22& 20.20& 20.16&-99.00& 19.71& 19.48& 19.37& 19.72& 19.39& 19.34& -1.00& 16.68&     1.83$^s $& -3.00&    4\\
    17&  157.897&   57.718&-99.00&-99.00&-99.00&-99.00& 25.88&-99.00& 24.56&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    18&  157.900&   57.553& 22.06& 22.08& 21.72& 21.42& 21.62& 21.39& 21.33& 20.69& 20.83&-99.00& -1.00&-99.00&     1.84$^s $& -3.00&    4\\
    19&  157.902&   57.721&-99.00&-99.00&-99.00&-99.00& 26.29&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    20&  157.905&   57.533& 20.41& 19.14& 18.17& 17.52& 16.67& 15.88& 15.08& 14.58& 14.52& 14.47& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
    21&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    22&  157.913&   57.675& 22.03& 21.98& 22.14& 21.76& 21.50& 21.67& 21.48& 21.87& 21.67&-99.00& -1.00&-99.00&     1.60$^s $& -3.00&    4\\
    23&  157.916&   57.644& 24.65& 24.54& 24.31& 24.09& 23.65& 23.31& 22.33& 22.03&-99.00&-99.00& -1.00&-99.00&     1.21$^s $& -3.00&    1\\
    24&  157.919&   57.710&-99.00&-99.00&-99.00&-99.00&-99.00& 22.57& 21.17& 20.76& 20.67& 19.85& -1.00&-99.00&     0.88$^s $& -3.00&    0\\
    25&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.24$^s $& -3.00&    0\\
    26&  157.921&   57.688&-99.00&-99.00&-99.00&-99.00& 23.09&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     1.80$^s $& -3.00&    3\\
    27&  157.921&   57.628&-99.00& 26.07& 25.21&-99.00& 24.84&-99.00& 24.49&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    28&  157.925&   57.504&-99.00& 23.57& 22.92& 22.37& 20.38& 19.81& 19.18& 18.55& 18.54& 18.02& -1.00&-99.00&     0.66$^s $& -3.00&    3\\
    29&  157.930&   57.548& 22.72& 22.12& 22.15& 21.39& 20.55& 20.30& 19.87& 19.22& 19.55& 19.32& -1.00& 16.94&     1.01$^s $& -3.00&    1\\
    30&  157.931&   57.533& 19.55& 19.45& 19.16& 19.23& 19.09& 19.14& 18.75& 19.00& 19.30& 19.08& -1.00& 16.40&     2.00$^s $& -3.00&    4\\
    31&  157.932&   57.818&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
    32&  157.941&   57.567& 20.87& 21.02& 20.28& 20.29& 19.77& 19.61& 19.46& 19.35& 19.25& 18.95& -1.00& 16.55&     1.25$^s $& -3.00&    4\\
    33&  157.941&   57.562&-99.00& 24.25&-99.00&-99.00& 24.53&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    34&  157.941&   57.513& 25.10& 24.94& 25.35& 24.59& 24.47& 23.45& 23.75&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    35&  157.942&   57.678& 23.91& 23.73& 23.27& 22.84& 22.16& 21.77& 21.10& 20.39& 20.47& 19.86& -1.00&-99.00&     0.95$^s $& -3.00&    0\\
    36&  157.949&   57.518&-99.00& 25.01& 24.55& 24.38& 23.92& 24.13& 23.54&-99.00&-99.00&-99.00& -1.00&-99.00&     2.77$^s $& -3.00&    3\\
    37&  157.951&   57.728& 17.66& 17.17& 17.00& 16.99& 16.52& 16.24& 15.85& 16.10& 16.21& 16.49& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
    38&  157.951&   57.709&-99.00&-99.00&-99.00&-99.00& 26.34&-99.00& 24.78&-99.00&-99.00& 21.11& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    39&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    40&  157.961&   57.713& 22.55& 22.24& 22.22& 22.28& 21.38& 21.19& 21.05& 20.25& 20.09& 19.72& -1.00& 17.36&     1.55$^s $& -3.00&    4\\
    41&  157.962&   57.730&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 19.44& -1.00& 17.27&     0.88$^s $& -3.00&    4\\
    42&  157.979&   57.756& 24.78& 24.61& 24.32& 23.98& 23.39& 23.31& 23.19&-99.00&-99.00&-99.00& -1.00&-99.00&     0.49$^s $& -3.00&    3\\
    43&  157.980&   57.731& 23.92&-99.00& 24.36&-99.00&-99.00& 23.09&-99.00& 19.94& 21.01&-99.00& -1.00&-99.00&     1.38$^s $& -3.00&    1\\
    44&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    45&  157.986&   57.646& 25.03& 24.83& 24.28& 24.10&-99.00& 23.42&-99.00& 20.90& 20.55& 19.74& -1.00& 15.38&     0.00$^s $&  0.95&  -99\\
    46&  157.989&   57.798& 19.50& 19.35& 18.95& 18.89& 18.71& 18.97& 18.60& 18.37& 18.94& 18.43& -1.00& 16.01&     0.84$^s $& -3.00&    4\\
    47&  157.995&   57.517& 23.07& 22.54& 22.53& 22.12& 21.38& 21.21& 20.62& 20.30& 20.15& 19.82& -1.00&-99.00&    -1.00$^s $&  0.15&   -1\\
    48&  158.000&   57.737& 23.71& 22.88& 22.22& 21.30& 20.17& 19.87& 19.31& 19.12& 19.13& 18.60& -1.00&-99.00&     0.52$^s $& -3.00&    3\\
    49&  158.006&   57.611&-99.00& 26.19& 25.32& 24.83& 24.12& 24.43& 23.82&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.15&  -99\\
    50&  158.007&   57.738& 21.12& 21.22& 21.20& 20.82& 20.90& 20.90& 20.50& 20.43& 20.61& 20.22& -1.00&-99.00&     2.32$^s $& -3.00&    4\\
    51&  158.008&   57.602&-99.00&-99.00&-99.00&-99.00& 23.76& 22.99& 21.46& 20.82& 20.52& 19.99& -1.00&-99.00&     1.16$^s $& -3.00&    1\\
    52&  158.012&   57.536& 22.20& 21.97& 21.81& 21.79& 21.40& 21.43& 21.02& 20.29& 20.47& 20.05& -1.00&-99.00&     0.89$^s $& -3.00&    4\\
    53&  158.016&   57.870& 22.64& 21.95& 21.12& 20.21& 19.48& 19.23& 18.74& 18.65& 18.35& 17.92& 18.56& 16.17&     0.32$^s $& -3.00&    3\\
    54&  158.016&   57.583&-99.00&-99.00&-99.00&-99.00& 25.62&-99.00& 24.23&-99.00&-99.00&-99.00& -1.00& 16.97&     0.00$^s $&-99.00&  -99\\
    55&  158.021&   57.599& 23.09& 22.85& 22.45& 22.13& 21.26& 20.81& 20.37& 19.99& 19.88& 19.39& -1.00& 17.33&     0.66$^s $& -3.00&    1\\
    56&  158.021&   57.600& 25.13& 24.67& 24.53& 24.41& 23.67& 23.18& 22.87& 21.93& 21.45&-99.00& -1.00&-99.00&     0.00$^s $&  0.95&  -99\\
    57&  158.021&   57.649&-99.00& 25.82& 25.76&-99.00& 24.87&-99.00& 24.26&-99.00&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&  0.15&   -1\\
    58&  158.025&   57.741& 22.49& 22.62& 22.50& 22.31& 21.81& 22.19& 21.66& 21.53& 21.36& 20.62& -1.00&-99.00&     1.22$^s $& -3.00&    4\\
    59&  158.027&   57.805& 22.02& 22.23& 21.97& 21.89& 21.99& 22.02& 21.68& 21.60& 21.34& 21.15& -1.00&-99.00&     2.29$^s $& -3.00&    4\\
    60&  158.028&   57.763& 21.99& 22.13& 21.52& 21.13& 21.47& 20.91& 21.10& 20.60& 20.62& 20.09& -1.00& 17.28&     1.82$^s $& -3.00&    4\\
    61&  158.035&   57.690& 24.62& 24.46& 24.14& 24.08& 23.43& 23.34& 22.32& 21.97& 21.83&-99.00& -1.00&-99.00&     1.21$^s $& -3.00&    1\\
    62&  158.041&   57.647&-99.00& 23.68& 22.57& 21.60& 21.79& 22.04& 21.96& 21.45& 21.66& 20.77& -1.00&-99.00&     3.48$^s $& -3.00&    4\\
    63&  158.042&   57.837& 22.75& 22.47& 22.11& 21.78& 21.00& 20.46& 19.86& 19.45& 19.36& 18.77&-99.00& 16.94&     0.84$^s $& -3.00&    1\\
    64&  158.045&   57.717&-99.00& 25.01& 24.62& 24.40& 24.01& 24.13& 23.25& 22.11&-99.00& 21.41& -1.00&-99.00&     0.00$^s $&  0.85&  -99\\
    65&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    66&  158.053&   57.760& 23.62& 23.31& 23.12& 22.58& 22.00& 21.45& 20.70& 20.10& 20.08& 19.49& -1.00&-99.00&     0.00$^s $&  0.85&  -99\\
    67&  158.055&   57.572& 25.00& 24.94& 24.17& 23.51& 22.53& 21.71& 20.96& 20.39& 20.25& 19.62& -1.00& 17.57&     0.82$^s $& -3.00&    1\\
    68&  158.056&   57.807&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00& 17.71&     0.00$^s $&-99.00&  -99\\
    69&  158.057&   57.880& 22.37& 22.22& 21.84& 21.83& 21.82& 21.73& 21.71& 21.52& 21.77&-99.00& 20.16& 16.77&     1.88$^s $& -3.00&    4\\
    70&  158.060&   57.541&-99.00& 24.79& 24.11& 23.64& 22.97& 22.29& 22.02& 21.18& 20.94& 20.53& -1.00& 17.93&     0.00$^s $&  0.75&  -99\\
    71&  158.061&   57.880&-99.00& 25.19& 24.71& 24.31& 24.27& 23.76& 23.42& 22.18& 21.57&-99.00& 20.53&-99.00&     2.26$^s $& -3.00&    3\\
    72&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     5.35& -3.00&    3\\
    73&  158.063&   57.797&-99.00&-99.00&-99.00&-99.00& 26.15& 25.02& 23.89& 22.69&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    74&  158.064&   57.546&-99.00&-99.00& 25.31& 24.88& 25.15&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     3.12$^s $& -3.00&    3\\
    75&  158.066&   57.824& 19.76& 19.45& 19.57& 19.43& 19.15& 19.04& 18.81& 19.00& 19.33& 18.89&-99.00& 16.06&     1.82$^s $& -3.00&    4\\
    76&  158.070&   57.771& 24.41& 24.16& 23.97&-99.00& 23.32& 22.94& 22.10& 21.16& 20.97& 20.57& -1.00&-99.00&     0.94$^s $& -3.00&    1\\
    77&  158.071&   57.862& 24.57& 25.09& 24.87& 24.67& 24.45& 24.36& 23.45& 22.13& 21.61& 20.89& 20.65&-99.00&     2.19& -3.00&    3\\
    78&  158.075&   57.642& 21.66& 21.43& 20.80& 20.24& 19.56& 19.31& 18.85& 18.67& 18.44& 18.10& -1.00&-99.00&     0.36$^s $& -3.00&    4\\
    79&  158.079&   57.662& 24.16& 23.98& 23.74& 23.67& 23.46& 23.36& 23.33& 22.47&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    80&  158.083&   57.572&-99.00&-99.00&-99.00&-99.00& 25.56&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
    81&  158.084&   57.536&-99.00&-99.00& 25.35& 24.74& 24.41& 24.55& 23.83& 22.58& 21.33& 20.39& -1.00& 17.08&     1.32$^s $& -3.00&    1\\
    82&  158.085&   57.950&-99.00&-99.00&-99.00&-99.00& 25.13&-99.00& 24.81&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
    83&  158.087&   57.823& 21.65& 20.46& 19.38& 18.66& 17.71& 16.65& 15.95& 15.50& 15.48& 15.50& 16.31&-99.00&    -2.00$^s $&-99.00&   -2\\
    84&  158.089&   57.632& 24.95&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     1.20& -3.00&    1\\
    85&  158.091&   57.566&-99.00&-99.00& 25.78& 25.34& 24.81& 24.20& 23.33& 22.03& 21.13& 20.69& -1.00&-99.00&     0.00$^s $&  1.25&  -99\\
    86&  158.092&   57.615& 21.70& 21.57& 21.04& 21.08& 21.03& 21.36& 20.87& 20.94& 20.86& 20.71& -1.00&-99.00&    -1.00$^s $&  0.65&   -1\\
    87&  158.093&   57.660& 23.67& 23.96& 23.98& 23.97& 23.19& 23.08& 22.90& 21.91& 21.95&-99.00& -1.00&-99.00&     1.51$^s $& -3.00&    4\\
    88&  158.095&   57.592&-99.00&-99.00&-99.00&-99.00& 25.65&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    89&  158.095&   57.931& 19.98& 20.96& 19.84& 20.23& 20.11& 20.13& 19.98& 19.91& 19.59& 19.16& 18.74& 17.34&     1.25$^s $& -3.00&    4\\
    90&  158.096&   57.614& 20.04& 18.70& 17.97& 17.68& 16.96& 16.67& 16.20& 16.16& 16.13& 16.30& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
    91&  158.098&   57.644&-99.00&-99.00&-99.00&-99.00& 25.18&-99.00& 24.91&-99.00&-99.00&-99.00& -1.00& 17.14&     0.00$^s $&-99.00&  -99\\
    92&  158.101&   57.550& 25.55& 25.11& 24.71& 24.13& 23.29& 22.82& 22.40& 21.81& 21.44&-99.00& -1.00&-99.00&     1.22& -3.00&    4\\
    93&  158.102&   57.997&-99.00& 16.09&-99.00&-99.00& 15.23&-99.00& 13.57& 12.71& 11.94& 10.97& 12.14& 16.04&    -2.00$^s $&-99.00&   -2\\
    94&  158.104&   57.532& 22.58& 21.34& 20.65& 19.87& 18.97& 18.68& 18.16& 17.90& 17.65& 17.18& -1.00& 16.48&     0.42$^s $& -3.00&    3\\
    95&  158.104&   57.471& 20.69& 20.25& 19.81& 19.57& 19.42& 18.82& 18.03& 17.79& 17.74& 17.63& -1.00& 16.68&     2.43$^s $& -3.00&    4\\
    96&  158.109&   57.815& 24.65& 24.67& 24.18& 23.69& 23.11& 22.43& 21.91& 21.30& 21.48& 20.88& 20.75&-99.00&     0.88$^s $& -3.00&    3\\
    97&  158.113&   57.642&-99.00&-99.00&-99.00&-99.00& 25.98&-99.00& 23.97& 23.15&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
    98&  158.113&   57.763&-99.00&-99.00& 25.61& 25.95& 24.53& 23.39& 22.87& 21.83& 21.60& 20.99& -1.00&-99.00&     0.00$^s $&  1.25&  -99\\
    99&  158.116&   57.640& 20.58& 20.91&-99.00& 20.53& 20.67& 20.50& 20.25& 20.55& 20.11& 19.86& -1.00& 17.49&     1.96$^s $& -3.00&    4\\
   100&  158.118&   57.853&-99.00&-99.00&-99.00&-99.00& 25.82&-99.00& 24.36&-99.00&-99.00&-99.00& 21.22&-99.00&     0.00$^s $&-99.00&  -99\\
   101&  158.119&   57.913&-99.00& 26.38&-99.00& 24.75& 23.62& 23.11& 22.41& 22.33& 21.87& 20.89& 20.89&-99.00&     0.74$^s $& -3.00&    1\\
   102&  158.121&   57.582& 22.08& 21.54& 21.82& 21.30& 21.24& 21.31& 21.00& 21.17& 21.28&-99.00& -1.00&-99.00&     2.10$^s $& -3.00&    4\\
   103&  158.121&   57.683&-99.00&-99.00&-99.00& 25.94& 25.28& 24.66& 23.71& 22.50& 22.75&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   104&  158.123&   57.691& 25.07& 24.67& 24.46& 24.03& 23.18& 23.14& 22.41& 21.69& 21.92& 20.80& -1.00&-99.00&     1.21$^s $& -3.00&    1\\
   105&  158.125&   57.494&-99.00& 25.71&-99.00& 24.66& 24.89& 23.97& 23.93& 22.29&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  1.55&  -99\\
   106&  158.129&   57.928& 22.18& 21.84&-99.00& 21.75& 21.54& 21.74& 21.25& 21.67& 21.41&-99.00& 20.35& 17.14&     2.09$^s $& -3.00&    4\\
   107&  158.137&   57.821& 24.79& 25.07& 25.30& 24.42& 23.96& 23.85& 22.77& 21.89& 21.47& 20.98& 20.54&-99.00&     0.00$^s $&  1.45&  -99\\
   108&  158.139&   57.803& 24.47& 24.20& 24.05& 23.93& 23.47& 23.34& 22.40& 21.81& 21.51& 21.00& 20.02& 17.41&    -1.00$^s $&  0.55&   -1\\
   109&  158.140&   57.622& 23.13& 23.00& 21.93& 21.98& 21.91& 21.97& 22.07& 21.56& 21.64& 21.38& -1.00&-99.00&     2.98$^s $& -3.00&    4\\
   110&  158.140&   57.732& 22.02& 21.90& 21.63& 21.73& 21.72& 21.08& 21.54& 20.81& 21.14& 20.63& -1.00&-99.00&     1.87$^s $& -3.00&    4\\
   111&  158.142&   57.940& 24.71& 24.87& 24.75& 24.81& 24.49& 24.39& 24.22&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.15&  -99\\
   112&  158.142&   57.940&-99.00& 25.05&-99.00& 24.83& 25.12& 24.23& 24.01&-99.00&-99.00&-99.00& 20.34&-99.00&    -1.00$^s $&  1.55&   -1\\
   113&  158.145&   57.703&-99.00&-99.00&-99.00&-99.00& 25.80&-99.00& 24.48& 22.63&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   114&  158.151&   58.010& 20.27& 20.24& 19.84& 19.73& 19.83& 19.90& 19.70& 19.71& 19.68& 19.09& 18.44& 16.75&     0.69$^s $& -3.00&    3\\
   115&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   116&  158.153&   57.589& 23.36& 23.63& 23.76& 23.22& 23.03& 23.46& 22.67& 22.31&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.35&  -99\\
   117&  158.155&   57.560&-99.00& 17.76&-99.00& 15.13& 16.59& 15.27& 16.06& 13.75& 13.42& 13.30& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   118&  158.157&   57.810&-99.00&-99.00&-99.00& 25.88& 25.38&-99.00& 24.35&-99.00&-99.00&-99.00& 21.65&-99.00&     0.00$^s $&  0.85&  -99\\
   119&  158.157&   57.869&-99.00& 25.00& 24.79& 24.79& 24.32&-99.00&-99.00&-99.00&-99.00&-99.00& 20.15&-99.00&     0.00$^s $&  1.15&  -99\\
   120&  158.164&   57.887& 19.94& 20.14& 19.86& 20.34& 19.52& 19.59& 19.41& 19.50& 18.91& 19.17& 18.69& 16.36&     1.53$^s $& -3.00&    4\\
   121&  158.164&   57.676&-99.00& 25.71& 25.24& 24.79& 24.00& 23.90& 23.54& 22.75& 21.79& 21.29& -1.00&-99.00&     0.00$^s $&  0.45&  -99\\
   122&  158.164&   57.627& 24.19& 24.18&-99.00&-99.00&-99.00& 22.67&-99.00& 22.36&-99.00&-99.00& -1.00&-99.00&     0.94$^s $& -3.00&    1\\
   123&  158.166&   57.589& 24.89& 24.91& 24.73&-99.00& 23.80& 23.62& 23.33&-99.00&-99.00&-99.00& -1.00&-99.00&     2.58$^s $& -3.00&    3\\
   124&  158.167&   57.754&-99.00& 25.00& 24.74& 24.10& 23.79& 23.79& 23.13& 22.48&-99.00&-99.00& -1.00&-99.00&     2.62$^s $& -3.00&    3\\
   125&  158.167&   57.868&-99.00&-99.00&-99.00& 25.62& 24.59& 24.07& 22.83& 22.62&-99.00&-99.00& 20.23&-99.00&     0.00$^s $&-99.00&  -99\\
   126&  158.173&   57.802& 23.29& 23.39& 23.77& 23.41& 23.00& 23.10& 22.73& 22.60&-99.00&-99.00& 21.58&-99.00&     2.32$^s $& -3.00&    4\\
   127&  158.174&   57.726& 24.80& 25.04& 24.88& 24.47&-99.00& 24.40& 23.72& 21.97& 21.65& 21.13& -1.00&-99.00&     0.00$^s $&  2.05&  -99\\
   128&  158.175&   57.669&-99.00& 24.90& 24.57& 24.33& 23.46& 23.16& 21.83& 20.93& 19.88& 19.82& -1.00& 16.03&     1.47$^s $& -3.00&    1\\
   129&  158.177&   57.741& 23.52& 23.54&-99.00& 22.15& 22.22& 21.43& 20.85& 20.10& 19.99& 19.48& -1.00&-99.00&     0.90$^s $& -3.00&    4\\
   130&  158.177&   57.502& 24.54& 24.51& 23.89& 23.32& 22.98& 22.50& 21.75& 21.01& 20.89& 20.50& -1.00&-99.00&     0.00$^s $&  0.85&  -99\\
   131&  158.177&   57.939& 23.10& 22.86& 23.24&-99.00& 22.68& 22.04& 22.34& 21.90&-99.00&-99.00& 19.69&-99.00&     0.39$^s $& -3.00&    1\\
   132&  158.179&   57.533& 23.00& 22.55& 21.95& 22.21& 21.83& 21.74& 21.50& 21.23& 21.13& 20.64& -1.00&-99.00&     2.40$^s $& -3.00&    4\\
   133&  158.179&   57.751& 22.99& 22.69& 22.84& 23.03& 22.43& 22.20& 22.04& 21.48& 21.46& 21.18& -1.00&-99.00&     1.81$^s $& -3.00&    4\\
   134&  158.182&   57.751& 24.50& 24.45& 24.13& 24.02& 23.54& 23.06& 22.20& 20.80& 20.43& 19.78& -1.00& 16.52&     0.00$^s $&  1.45&  -99\\
   135&  158.182&   57.810&-99.00& 24.83& 24.54& 24.82& 24.14& 24.47& 23.56&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  1.55&  -99\\
   136&  158.182&   57.599&-99.00& 25.00& 24.86& 24.50& 24.22& 23.98& 23.76& 22.11& 21.53&-99.00& -1.00&-99.00&     0.00$^s $&  2.05&  -99\\
   137&  158.185&   57.905&-99.00&-99.00&-99.00& 25.24& 24.75&-99.00& 23.83&-99.00&-99.00&-99.00& 20.63&-99.00&    -1.00$^s $&  0.85&   -1\\
   138&  158.187&   57.831& 22.07& 22.28& 22.37& 22.06& 21.84& 21.90& 21.91& 21.25& 21.45& 20.89& 20.56&-99.00&     1.52$^s $& -3.00&    4\\
   139&  158.188&   57.645&-99.00&-99.00&-99.00&-99.00& 27.50&-99.00& 25.12&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   140&  158.194&   57.981& 22.05& 22.56& 21.87& 22.15& 21.78& 21.54& 21.58& 21.27& 21.41& 20.83& 20.29&-99.00&     1.43$^s $& -3.00&    4\\
   141&  158.196&   57.920& 21.06& 21.41&-99.00& 20.77& 20.80& 20.74& 20.59& 20.84& 20.91& 20.27& 19.91& 16.82&     1.89$^s $& -3.00&    4\\
   142&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   143&  158.200&   57.940& 24.34& 23.55& 22.96& 22.50& 21.38& 20.74& 20.18& 20.00& 19.53& 18.97& 18.91&-99.00&     0.73$^s $& -3.00&    3\\
   144&  158.201&   57.608& 24.71& 22.35& 22.25& 21.69& 21.24& 21.19& 21.12& 21.03& 21.20& 20.76& -1.00&-99.00&     3.34$^s $& -3.00&    4\\
   145&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   146&  158.203&   57.691& 24.19& 24.29& 24.12& 24.09& 23.60& 23.42& 22.79& 21.46& 21.52& 20.98& -1.00&-99.00&     1.55$^s $& -3.00&    3\\
   147&  158.203&   57.639& 23.38& 23.08& 23.24& 22.80& 22.35& 22.18& 21.65& 21.79& 21.22& 20.79& -1.00&-99.00&     1.30$^s $& -3.00&    3\\
   148&  158.209&   58.038& 21.89& 21.86& 21.57&-99.00& 21.01& 20.94& 20.76& 20.32& 20.21& 20.04& 19.34& 16.14&     1.43$^s $& -3.00&    4\\
   149&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   150&  158.214&   57.976& 22.16& 22.10& 21.43& 22.29& 21.41& 21.37& 21.48& 20.97& 20.43& 20.23& 19.73&-99.00&     1.19$^s $& -3.00&    4\\
   151&  158.217&   57.763&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.91&-99.00&     1.92$^s $& -3.00&    4\\
   152&  158.219&   57.741& 23.17& 22.94& 22.75& 22.63& 22.23& 22.14& 21.41& 21.33& 21.03& 20.29& -1.00&-99.00&    -1.00$^s $&  0.35&   -1\\
   153&  158.222&   57.899&-99.00& 25.84&-99.00&-99.00& 25.45&-99.00& 24.77&-99.00&-99.00&-99.00& 21.46&-99.00&     0.00$^s $&  0.45&  -99\\
   154&  158.222&   57.688&-99.00&-99.00&-99.00&-99.00& 26.14&-99.00& 24.35& 22.70&-99.00& 21.50& -1.00&-99.00&     0.00$^s $&  1.45&  -99\\
   155&  158.225&   57.697& 24.95& 24.33& 24.68& 23.59& 23.77& 23.70& 23.17& 22.54&-99.00& 21.15& -1.00&-99.00&     2.09$^s $& -3.00&    3\\
   156&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   157&  158.235&   57.804&-99.00&-99.00&-99.00&-99.00& 22.01&-99.00&-99.00& 18.80& 18.88& 19.18& 19.80&-99.00&    -2.00$^s $&-99.00&   -2\\
   158&  158.240&   57.796& 24.72& 24.32& 24.17& 24.12& 23.56& 23.33& 22.74& 22.39& 21.98& 21.19& 20.79&-99.00&     1.45$^s $& -3.00&    1\\
   159&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   160&  158.242&   57.467&-99.00& 26.22& 25.70& 25.00& 24.37& 23.85& 23.21& 23.11&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.35&  -99\\
   161&  158.247&   57.857&-99.00&-99.00&-99.00&-99.00&-99.00& 22.85&-99.00& 20.90&-99.00& 20.02&-99.00&-99.00&     1.16$^s $& -3.00&    0\\
   162&  158.249&   57.889& 18.89& 18.11& 17.18& 16.60& 16.03& 15.91& 15.42& 15.18& 15.08& 15.07& 15.64& 16.57&     0.12$^s $& -3.00&    0\\
   163&  158.257&   57.781& 22.97& 21.95& 22.14& 20.98& 20.04& 19.80& 19.36& 19.35& 18.94& 18.50& 19.01&-99.00&     0.51$^s $& -3.00&    0\\
   164&  158.258&   57.766&-99.00& 25.65&-99.00& 25.75& 24.19& 23.63& 23.14& 21.99& 21.60& 21.24& 20.78&-99.00&    -1.00$^s $&  1.35&   -1\\
   165&  158.260&   57.476& 24.49& 24.46& 24.26& 24.04& 23.26& 22.57& 21.80& 20.82& 20.66& 20.12& -1.00&-99.00&     1.17$^s $& -3.00&    3\\
   166&  158.262&   58.045&-99.00&-99.00&-99.00&-99.00& 25.04&-99.00&-99.00& 21.56& 21.48& 20.81& 19.84&-99.00&     0.00$^s $&  2.15&  -99\\
   167&  158.266&   57.994& 25.27& 25.32& 25.33&-99.00& 25.48&-99.00& 24.96&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.25&  -99\\
   168&  158.266&   57.664& 24.19& 23.58& 23.74& 22.78& 23.20& 23.06& 22.75& 22.20& 21.96& 21.18& -1.00&-99.00&     1.97$^s $& -3.00&    3\\
   169&  158.267&   57.648&-99.00&-99.00&-99.00& 25.35& 24.91&-99.00& 23.97& 22.42& 22.28& 21.12& -1.00&-99.00&     0.00$^s $&  2.35&  -99\\
   170&  158.273&   57.819& 24.46& 24.73& 24.44& 24.24& 23.92& 23.68& 23.32& 21.75& 21.21& 20.65& 20.26& 17.62&     2.10$^s $& -3.00&    3\\
   171&  158.279&   57.709&-99.00& 25.67& 25.26& 25.19& 24.83& 24.59& 23.70&-99.00& 22.31& 21.13& -1.00& 18.12&     0.00$^s $&  2.05&  -99\\
   172&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   173&  158.285&   57.687&-99.00& 25.47& 25.27& 25.03& 24.81&-99.00& 25.08&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   174&  158.285&   57.584& 23.00& 23.00& 22.92& 22.57& 22.53& 22.57& 22.21& 22.06& 22.04&-99.00& -1.00&-99.00&     2.08$^s $& -3.00&    4\\
   175&  158.287&   57.955& 22.43& 22.14& 21.94& 22.11& 21.54& 21.63& 21.41& 21.07& 21.04& 20.63& 19.28&-99.00&     1.55$^s $& -3.00&    4\\
   176&  158.287&   57.642& 21.21& 20.70& 20.57& 20.46& 20.02& 20.17& 19.90& 20.24& 20.27& 19.99& -1.00& 17.27&     1.81$^s $& -3.00&    4\\
   177&  158.287&   57.907&-99.00&-99.00&-99.00&-99.00& 24.96&-99.00& 24.34& 22.43&-99.00& 20.91& 20.73&-99.00&    -1.00$^s $&  2.45&   -1\\
   178&  158.289&   57.968&-99.00& 24.57& 24.17& 23.97& 23.14& 22.76& 21.64& 21.11& 21.27& 20.32& 19.77&-99.00&     0.00$^s $&  1.05&  -99\\
   179&  158.294&   57.814&-99.00& 25.03& 24.95& 24.89& 24.59&-99.00& 24.01&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.25&  -99\\
   180&  158.293&   57.975&-99.00&-99.00&-99.00&-99.00& 26.11&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   181&  158.294&   57.487& 20.60& 19.89& 19.09& 18.48& 17.67& 16.84& 16.17& 15.82& 15.85& 15.85& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   182&  158.294&   57.693& 23.29& 22.83& 22.64& 22.33& 21.37& 21.04& 20.92& 20.73& 20.58& 20.04& -1.00&-99.00&     1.55$^s $& -3.00&    4\\
   183&  158.294&   57.814&-99.00&-99.00&-99.00& 25.09& 24.44& 24.01& 23.18& 21.81& 20.97& 20.62& 20.02&-99.00&    -1.00$^s $&  1.35&   -1\\
   184&  158.301&   57.671&-99.00& 25.91&-99.00& 25.82& 25.05&-99.00& 23.69&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.95&  -99\\
   185&  158.301&   57.798&-99.00&-99.00&-99.00&-99.00& 25.60& 24.90& 23.95&-99.00&-99.00& 21.47& 21.08&-99.00&    -1.00$^s $&  1.25&   -1\\
   186&  158.303&   57.574&-99.00&-99.00&-99.00&-99.00& 25.32&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   187&  158.303&   57.701&-99.00& 21.32&-99.00& 18.26& 17.96& 18.51& 18.12& 17.79& 17.40& 16.91& -1.00& 17.29&     0.33$^s $& -3.00&    0\\
   188&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.33$^s $& -3.00&    1\\
   189&  158.304&   57.568&-99.00& 26.12&-99.00& 25.72& 25.27&-99.00& 25.00&-99.00& 21.95&-99.00& -1.00& 17.42&     0.00$^s $&  1.55&  -99\\
   190&  158.305&   57.674& 24.94& 24.62& 24.32& 24.06& 23.47& 23.00& 22.38& 21.40& 21.08& 20.54& -1.00&-99.00&    -1.00$^s $&  1.45&   -1\\
   191&  158.305&   57.861&-99.00&-99.00& 25.52& 25.34& 24.98&-99.00& 24.40& 22.74&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  1.55&  -99\\
   192&  158.307&   58.081& 21.48&-99.00& 21.44&-99.00&-99.00& 21.15&-99.00& 20.82& 21.06& 20.67& 20.29& 18.00&    -1.00$^s $&  0.25&   -1\\
   193&  158.307&   57.598&-99.00& 24.76&-99.00& 24.59& 24.19& 23.87& 24.49&-99.00& 22.26&-99.00& -1.00&-99.00&     0.00$^s $&  0.25&  -99\\
   194&  158.309&   58.010& 25.31& 24.58& 24.70& 24.93& 23.73& 23.67& 23.42& 22.59&-99.00&-99.00&-99.00&-99.00&     0.89$^s $& -3.00&    1\\
   195&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   196&  158.310&   57.950& 23.79& 24.11& 23.28& 23.65& 23.54& 23.20& 22.99& 22.10&-99.00&-99.00& 21.14&-99.00&    -1.00$^s $&-99.00&   -1\\
   197&  158.311&   57.580&-99.00&-99.00& 25.46& 24.69& 23.68& 23.37& 23.17&-99.00& 22.16&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   198&  158.313&   57.667&-99.00& 25.27&-99.00& 25.34& 24.95&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   199&  158.316&   57.841& 24.04& 23.64& 23.19& 22.72& 21.79& 21.25& 20.78& 20.10& 20.03& 19.56& 19.47&-99.00&     0.72$^s $& -3.00&    1\\
   200&  158.316&   57.382&-99.00& 22.66& 22.87& 20.94& 19.93& 19.56& 18.99& 18.43& 18.32&-99.00& -1.00& 16.87&     0.44$^s $& -3.00&    0\\
   201&  158.317&   57.712& 24.06& 23.60& 23.10& 22.64& 21.56& 20.96& 20.51& 20.19& 19.93& 19.27& -1.00& 17.97&     0.70$^s $& -3.00&    3\\
   202&  158.319&   57.440& 21.20& 21.00& 21.00& 20.35& 20.35& 20.81& 20.32& 20.19& 20.00& 19.65& -1.00& 17.63&     1.26$^s $& -3.00&    4\\
   203&  158.323&   57.877& 20.73& 20.29& 19.77& 19.51& 19.19& 19.12& 18.92& 18.86& 18.90& 18.72& 19.39&-99.00&     0.09$^s $& -3.00&    1\\
   204&  158.323&   57.589& 23.77& 23.42& 22.92& 22.36& 22.10& 21.92& 21.29& 20.79& 20.58& 20.12& -1.00&-99.00&     0.00$^s $&  0.25&  -99\\
   205&  158.326&   57.434& 21.85& 21.39& 21.16& 21.37& 20.85& 20.92& 20.39& 20.04& 19.92& 19.49& -1.00&-99.00&     0.68$^s $& -3.00&    3\\
   206&  158.329&   57.858& 20.88& 21.08& 20.47& 20.42& 20.46& 20.24& 20.16& 20.08& 20.36& 19.88& 19.30& 16.49&     1.82$^s $& -3.00&    4\\
   207&  158.330&   57.408&-99.00& 25.31& 24.36& 24.94& 24.59&-99.00& 24.10&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   208&  158.331&   57.969& 21.86& 22.31& 21.38& 21.42& 21.52& 21.24& 20.98& 20.46& 20.34& 19.59& 19.41&-99.00&     1.05$^s $& -3.00&    4\\
   209&  158.331&   57.590&-99.00& 25.41& 24.59& 23.94& 22.65& 21.89& 21.18& 20.62& 20.17& 19.52& -1.00& 17.35&     0.70$^s $& -3.00&    0\\
   210&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   211&  158.333&   57.478& 25.36& 24.65& 24.61& 24.83& 24.42& 24.44& 23.94&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   212&  158.333&   57.806& 22.86& 22.57& 22.41& 22.33& 21.87& 21.35& 21.14& 20.76& 20.61& 20.37& 19.43& 16.50&     1.93$^s $& -3.00&    4\\
   213&  158.334&   57.622&-99.00& 25.55& 24.75& 24.03& 22.80& 21.89& 21.03& 20.67& 20.22& 19.64& -1.00&-99.00&     0.88$^s $& -3.00&    0\\
   214&  158.339&   57.649&-99.00&-99.00& 21.85&-99.00&-99.00& 20.38&-99.00& 20.87& 20.65& 20.53& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   215&  158.338&   57.537& 18.53& 18.59& 18.18& 18.47& 18.02& 18.09& 18.13& 18.25& 18.31& 18.12& -1.00& 15.46&     1.26$^s $& -3.00&    4\\
   216&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   217&  158.342&   57.550& 22.35& 22.17& 22.20& 22.01& 21.67& 21.68& 21.25& 21.20& 21.14& 20.56& -1.00&-99.00&     2.10$^s $& -3.00&    4\\
   218&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.63&-99.00&     0.00$^s $&-99.00&  -99\\
   219&  158.352&   57.413&-99.00& 24.84&-99.00& 24.48& 24.09& 23.90& 23.49& 22.18&-99.00& 21.03& -1.00&-99.00&     1.53$^s $& -3.00&    1\\
   220&  158.352&   57.632&-99.00& 25.34& 25.03& 24.85& 23.94& 23.42& 23.33& 22.29&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.65&  -99\\
   221&  158.356&   57.943&-99.00& 25.20& 24.83& 24.25& 24.51&-99.00& 24.35&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  2.35&  -99\\
   222&  158.356&   58.011& 20.41& 19.63& 18.98& 18.62& 18.16& 18.06& 17.77& 17.99& 17.85& 17.66& 18.16&-99.00&    -2.00$^s $&-99.00&   -2\\
   223&  158.359&   58.023& 20.60& 20.98& 20.39& 20.57& 20.08& 19.74& 19.52& 19.46& 19.15& 18.38& 18.16& 16.42&     0.74$^s $& -3.00&    4\\
   224&  158.362&   57.551& 23.26& 22.84& 22.39& 22.03& 21.10& 20.75& 20.32& 19.96& 19.72& 19.24& -1.00&-99.00&     0.62$^s $& -3.00&    1\\
   225&  158.364&   57.365& 21.79& 21.49& 21.05&-99.00& 19.99& 19.80& 19.42& 19.06& 19.06&-99.00& -1.00& 16.80&     0.52$^s $& -3.00&    1\\
   226&  158.364&   57.631&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 22.23&-99.00& 20.73& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   227&  158.364&   57.659&-99.00& 26.11&-99.00& 25.47& 24.81&-99.00& 24.37&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.15&  -99\\
   228&  158.365&   57.818& 23.00& 22.11& 22.32& 22.17& 21.30& 21.54& 21.05& 21.03& 21.12& 20.51& 20.67&-99.00&     2.05$^s $& -3.00&    4\\
   229&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   230&  158.370&   57.639& 24.23& 24.32& 24.18& 23.76& 23.64& 23.34& 22.61& 21.89& 21.23& 20.96& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   231&  158.372&   57.785& 22.77& 24.50& 23.18& 22.93& 23.35& 23.51& 23.41& 22.69&-99.00&-99.00& 21.40&-99.00&     1.38$^s $& -3.00&    3\\
   232&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   233&  158.377&   57.707& 23.69& 22.88& 22.14& 20.96& 19.81& 19.50& 18.94& 18.70& 18.38& 17.99& 18.30&-99.00&     0.50$^s $& -3.00&    0\\
   234&  158.382&   57.916&-99.00&-99.00&-99.00&-99.00& 25.71&-99.00&-99.00&-99.00&-99.00&-99.00& 21.30&-99.00&     0.00$^s $&-99.00&  -99\\
   235&  158.386&   57.506&-99.00& 24.95& 24.59& 24.38& 23.95& 23.62& 22.95& 21.49& 21.44& 20.66& -1.00&-99.00&     0.00$^s $&  2.35&  -99\\
   236&  158.386&   57.687&-99.00& 23.77& 24.07& 23.11& 22.47& 22.54& 21.15& 20.62& 20.28& 19.87& 19.59&-99.00&     0.00$^s $&  1.15&  -99\\
   237&  158.387&   57.872&-99.00&-99.00&-99.00&-99.00& 26.34&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   238&  158.386&   57.745& 24.24& 23.78& 23.10& 22.57& 21.32& 20.60& 20.03& 19.88& 19.38& 18.80& 18.59& 17.47&     0.76$^s $& -3.00&    3\\
   239&  158.386&   57.846& 23.24& 21.91& 20.60& 19.86& 18.65& 17.24& 16.26& 15.85& 15.82& 15.89& 16.55&-99.00&    -2.00$^s $&-99.00&   -2\\
   240&  158.392&   57.681&-99.00& 24.99& 24.88& 24.81& 24.69&-99.00& 24.65&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.95&  -99\\
   241&  158.391&   57.674&-99.00&-99.00&-99.00&-99.00& 24.99&-99.00& 22.77& 22.23& 21.56& 21.30& -1.00&-99.00&     0.00$^s $&  1.95&  -99\\
   242&  158.392&   57.560&-99.00& 25.90&-99.00& 25.08& 24.30& 24.02& 23.81&-99.00&-99.00&-99.00& -1.00&-99.00&     4.21& -3.00&    4\\
   243&  158.392&   57.934& 22.12& 21.32& 20.48& 19.85& 19.28& 19.05& 18.63& 18.60& 18.33& 17.99& 18.64&-99.00&     0.32$^s $& -3.00&    1\\
   244&  158.394&   57.890&-99.00&-99.00&-99.00& 25.78& 25.39&-99.00& 23.94& 22.15&-99.00&-99.00& 21.07&-99.00&     0.00$^s $&  1.65&  -99\\
   245&  158.398&   57.726& 22.49& 21.45& 20.52& 19.76& 19.08& 18.80& 18.36& 18.21& 17.89& 17.63& 18.36&-99.00&     0.26$^s $& -3.00&    1\\
   246&  158.401&   57.540&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 23.23& 21.89&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   247&  158.401&   57.519& 20.96& 20.48& 19.64& 18.98& 18.40& 18.24& 17.82& 17.58& 17.49& 17.02& -1.00& 16.44&     0.30$^s $& -3.00&    1\\
   248&  158.408&   57.874& 23.92& 23.79& 23.60& 23.53& 23.15& 23.20& 22.55& 21.87& 21.57& 21.19& 20.37&-99.00&     0.00$^s $&-99.00&  -99\\
   249&  158.408&   57.711& 19.97& 19.69& 19.90& 19.43& 19.20& 19.59& 19.30& 19.76& 19.51& 19.10& 18.17& 16.51&     1.26$^s $& -3.00&    4\\
   250&  158.409&   57.967& 21.61& 20.17& 19.07& 18.21& 17.48& 17.24& 16.79& 16.49& 16.31& 16.00& 16.71& 17.21&     0.23$^s $& -3.00&    0\\
   251&  158.409&   57.762& 21.55& 21.15& 20.88& 20.65& 20.54& 21.02& 20.47& 20.27& 20.37& 19.91& 19.16& 17.15&     0.95$^s $& -3.00&    4\\
   252&  158.410&   57.983&-99.00& 24.58& 24.78&-99.00&-99.00&-99.00& 23.25& 22.04&-99.00&-99.00& 19.97&-99.00&     0.00$^s $&  1.45&  -99\\
   253&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   254&  158.414&   57.805&-99.00&-99.00&-99.00&-99.00& 25.73&-99.00& 24.71&-99.00&-99.00&-99.00& 21.31&-99.00&     0.00$^s $&-99.00&  -99\\
   255&  158.415&   57.638&-99.00&-99.00&-99.00&-99.00& 25.75&-99.00& 24.86&-99.00&-99.00&-99.00& -1.00& 18.04&     0.00$^s $&-99.00&  -99\\
   256&  158.418&   57.710&-99.00& 25.00& 24.98& 24.66& 24.29&-99.00& 23.98&-99.00&-99.00&-99.00& 21.32&-99.00&     0.00$^s $&  0.75&  -99\\
   257&  158.423&   57.818&-99.00& 25.47& 25.17& 24.89& 24.45& 24.34& 23.50& 21.84& 21.46& 20.69& 20.34&-99.00&     0.00$^s $&  1.45&  -99\\
   258&  158.423&   57.480&-99.00&-99.00&-99.00& 25.71& 24.85& 23.97& 23.42& 22.07& 22.00& 21.07& -1.00&-99.00&    -1.00$^s $&  1.35&   -1\\
   259&  158.423&   57.612& 15.70& 15.80& 15.67& 15.71& 16.44& 14.83& 15.38& 14.56& 14.52& 14.51& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   260&  158.423&   57.678&-99.00& 25.10& 24.65& 24.24& 23.38& 22.80& 21.78& 20.91& 20.33& 19.71& 19.17&-99.00&     0.00$^s $&  1.25&  -99\\
   261&  158.432&   57.679& 22.99& 23.84& 23.80& 22.61& 23.13& 22.86& 23.17& 22.37& 21.77&-99.00& 20.69&-99.00&     0.00$^s $&-99.00&  -99\\
   262&  158.432&   57.413&-99.00&-99.00&-99.00&-99.00& 25.01&-99.00& 23.78&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   263&  158.436&   57.855& 23.93& 23.50& 23.78& 23.47& 22.86& 22.65& 22.71& 21.89& 21.13& 20.74& 20.11&-99.00&     0.75$^s $& -3.00&    1\\
   264&  158.438&   57.820& 21.27& 21.75& 21.15& 20.87& 21.10& 20.89& 20.90& 20.50& 20.57& 20.26& 19.86& 18.24&     0.71$^s $& -3.00&    4\\
   265&  158.440&   57.459&-99.00& 24.71& 24.59& 23.76& 23.40& 23.51& 22.95& 22.05&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  1.25&  -99\\
   266&  158.448&   57.629&-99.00& 24.89& 24.49& 24.19& 23.77& 23.31& 22.92& 22.11& 21.79&-99.00& -1.00&-99.00&     0.00$^s $&  0.55&  -99\\
   267&  158.450&   57.844&-99.00& 25.33&-99.00& 24.72& 23.82& 23.32& 22.75& 22.08&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.95&  -99\\
   268&  158.451&   57.789& 23.49& 23.36& 22.71& 22.79& 22.15& 21.79& 21.38& 20.87& 20.87& 20.41& 19.95&-99.00&     1.03$^s $& -3.00&    4\\
   269&  158.451&   57.969&-99.00& 25.89& 25.59& 25.35& 24.78&-99.00& 24.31&-99.00& 21.93&-99.00& 21.06&-99.00&     0.00$^s $&  2.35&  -99\\
   270&  158.451&   57.889&-99.00&-99.00&-99.00&-99.00& 25.45&-99.00&-99.00& 21.69& 21.27& 20.61& 20.12&-99.00&     2.15$^s $& -3.00&    3\\
   271&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   272&  158.453&   57.847& 24.44& 24.13& 24.05& 24.03& 23.52& 23.42& 22.63& 22.24&-99.00& 21.09& 20.93&-99.00&     1.47$^s $& -3.00&    1\\
   273&  158.453&   57.707&-99.00&-99.00&-99.00&-99.00& 26.18&-99.00& 24.76&-99.00&-99.00&-99.00& 20.57&-99.00&     0.00$^s $&-99.00&  -99\\
   274&  158.453&   57.697&-99.00& 25.32& 24.38& 23.66& 23.08& 22.47& 22.33& 21.48& 21.19& 20.96& 20.76&-99.00&     0.00$^s $&  0.55&  -99\\
   275&  158.454&   57.499& 21.20& 21.42& 20.91& 21.07& 20.61& 20.41& 20.14& 20.12& 20.11& 19.72& -1.00& 17.30&    -1.00$^s $&-99.00&   -1\\
   276&  158.454&   57.742&-99.00& 24.58& 24.06& 23.57& 23.43& 23.32& 22.96&-99.00& 21.46& 20.16& 19.44& 17.30&    -1.00$^s $&-99.00&   -1\\
   277&  158.455&   57.537&-99.00& 25.06& 24.55& 24.28& 23.50& 23.04& 22.41& 21.37& 21.06& 20.44& -1.00&-99.00&     1.26$^s $& -3.00&    3\\
   278&  158.455&   57.913& 23.61& 23.26& 22.80& 22.52& 21.81& 21.21& 20.57& 20.12& 19.92& 19.52& 19.22& 18.20&     0.84$^s $& -3.00&    1\\
   279&  158.461&   57.498&-99.00& 24.68& 24.22& 24.52& 23.35& 24.03& 23.26&-99.00&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   280&  158.461&   58.021&-99.00& 25.15& 25.39&-99.00& 24.00& 23.42& 22.50& 22.09&-99.00& 21.08& 20.77&-99.00&     1.07$^s $& -3.00&    1\\
   281&  158.462&   57.857&-99.00& 25.25& 24.77& 24.83& 24.34& 24.13& 23.54&-99.00&-99.00&-99.00& 20.88&-99.00&     0.00$^s $&  1.85&  -99\\
   282&  158.465&   57.417& 23.89& 23.37&-99.00& 23.31& 22.96& 22.86& 22.64& 22.11&-99.00& 20.87& -1.00&-99.00&     1.71$^s $& -3.00&    3\\
   283&  158.468&   57.776&-99.00& 25.06& 25.07& 24.66& 23.88& 23.43& 22.55& 21.74& 21.32& 20.80& 20.36&-99.00&     0.00$^s $&  1.25&  -99\\
   284&  158.468&   58.006&-99.00& 21.77&-99.00& 19.96& 19.86& 19.61& 19.25& 18.99& 18.93& 18.66& 19.31&-99.00&     0.26$^s $& -3.00&    1\\
   285&  158.470&   57.835&-99.00& 25.63& 25.21& 25.27& 24.51& 24.05& 23.03&-99.00&-99.00& 21.02& 19.77& 16.89&     0.00$^s $&  1.15&  -99\\
   286&  158.472&   57.545& 20.99& 20.68& 20.33& 20.02& 19.37& 19.22& 18.83& 18.61& 18.51& 18.08& -1.00& 16.15&     0.29$^s $& -3.00&    3\\
   287&  158.472&   57.840& 21.36& 21.98& 21.02& 21.03& 20.80& 20.34& 19.93& 19.74& 19.92& 19.29& 18.95& 16.37&     0.94$^s $& -3.00&    4\\
   288&  158.473&   57.866&-99.00&-99.00&-99.00&-99.00& 25.65&-99.00& 24.89&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   289&  158.480&   57.993& 24.02& 24.02& 23.77& 23.49& 23.20& 23.57& 23.18&-99.00&-99.00&-99.00&-99.00&-99.00&     0.41$^s $& -3.00&    1\\
   290&  158.480&   57.621&-99.00& 25.63& 24.99& 24.51& 24.05& 23.37& 22.45& 21.21& 20.74& 20.42& -1.00&-99.00&     0.00$^s $&  1.55&  -99\\
   291&  158.484&   57.914& 24.11& 23.83& 23.55& 23.49& 22.88& 22.50& 21.88& 20.94& 20.77& 20.15& 19.56&-99.00&     0.76$^s $& -3.00&    1\\
   292&  158.485&   57.657&-99.00& 25.35& 24.84& 24.13& 23.40& 22.62& 21.90& 21.22& 20.83& 20.18& 19.66& 17.56&     0.99$^s $& -3.00&    1\\
   293&  158.490&   57.615& 20.29& 19.47& 19.41& 19.26& 18.96& 19.23& 18.64& 18.91& 18.94& 18.66& -1.00& 16.34&     2.71$^s $& -3.00&    4\\
   294&  158.491&   57.828& 22.81& 21.96& 21.96& 21.63& 21.35& 21.46& 21.11& 21.22&-99.00& 20.83& 20.56& 17.55&     2.58$^s $& -3.00&    4\\
   295&  158.492&   57.712&-99.00&-99.00&-99.00&-99.00& 25.58&-99.00& 24.04& 22.45& 21.69& 20.87& 19.88&-99.00&     0.00$^s $&  1.25&  -99\\
   296&  158.493&   57.535&-99.00& 26.29&-99.00& 25.20& 25.13&-99.00& 24.51&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.15&  -99\\
   297&  158.495&   57.721& 19.96& 19.40& 18.58& 17.87& 17.26& 17.07& 16.52& 16.29& 16.00& 15.66& 16.31& 14.99&    -1.00$^s $&  0.25&   -1\\
   298&  158.495&   57.660& 24.18& 23.48& 23.14& 22.66& 22.10& 22.12& 21.48& 20.99& 20.55& 19.99& 19.23& 16.50&     1.22$^s $& -3.00&    4\\
   299&  158.496&   57.745&-99.00&-99.00&-99.00&-99.00& 26.30&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   300&  158.499&   57.739&-99.00&-99.00&-99.00&-99.00& 25.64&-99.00& 24.10&-99.00&-99.00&-99.00& 20.69&-99.00&    -1.00$^s $&-99.00&   -1\\
   301&  158.499&   57.983&-99.00&-99.00&-99.00&-99.00& 25.50&-99.00& 24.28& 22.69&-99.00&-99.00& 21.21&-99.00&     0.00$^s $&-99.00&  -99\\
   302&  158.503&   57.746&-99.00& 24.70&-99.00& 24.40& 24.89& 24.04& 24.14& 22.53& 21.79&-99.00& 21.36&-99.00&     0.00$^s $&-99.00&  -99\\
   303&  158.503&   57.796&-99.00&-99.00&-99.00& 25.58& 24.87& 24.66& 24.54&-99.00&-99.00&-99.00&-99.00&-99.00&     3.76$^s $& -3.00&    3\\
   304&  158.503&   57.481&-99.00& 25.39& 24.94& 24.95& 24.46&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   305&  158.504&   57.557& 23.07& 23.57& 24.04& 23.78& 23.80& 23.95& 23.50&-99.00&-99.00&-99.00& -1.00&-99.00&     2.33$^s $& -3.00&    3\\
   306&  158.505&   57.708&-99.00& 25.55&-99.00& 25.00& 24.57&-99.00& 23.80& 22.28& 21.81&-99.00& 19.82&-99.00&    -1.00$^s $&  1.95&   -1\\
   307&  158.508&   57.558& 24.51& 24.09& 23.76& 23.33& 22.67& 22.38& 21.52& 20.73& 20.56& 20.14& -1.00&-99.00&     1.23$^s $& -3.00&    1\\
   308&  158.508&   57.732&-99.00& 25.55& 25.40& 25.37& 24.86& 24.40& 24.14&-99.00& 21.84&-99.00& 20.11&-99.00&     1.50$^s $& -3.00&    1\\
   309&  158.511&   57.834& 22.95& 22.44& 21.82& 21.18& 20.43& 20.23& 19.75& 19.60& 19.39& 18.99& 19.49& 17.39&     0.34$^s $& -3.00&    0\\
   310&  158.511&   57.855&-99.00& 25.90& 25.31& 25.40& 25.28&-99.00& 24.73&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   311&  158.513&   57.653&-99.00& 25.85&-99.00& 25.57& 24.36& 23.90& 23.03& 21.75& 21.23& 20.84& 20.25&-99.00&     0.00$^s $&  1.45&  -99\\
   312&  158.515&   57.569& 24.79& 24.53& 24.14& 23.93& 23.55& 23.28& 23.03& 22.56&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.25&  -99\\
   313&  158.518&   57.949&-99.00& 24.66& 24.39& 24.13& 23.35& 22.95& 21.85& 21.09& 20.72& 20.13& 19.69&-99.00&     1.27$^s $& -3.00&    1\\
   314&  158.519&   57.867&-99.00& 25.17& 25.48&-99.00& 25.19&-99.00& 24.79&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&  0.15&   -1\\
   315&  158.520&   57.878&-99.00& 26.02&-99.00& 25.79& 25.95&-99.00& 24.50&-99.00&-99.00&-99.00&-99.00&-99.00&     1.38$^s $& -3.00&    1\\
   316&  158.521&   57.699&-99.00&-99.00&-99.00& 26.18& 25.80&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     1.22$^s $& -3.00&    1\\
   317&  158.523&   57.604& 23.25& 23.24& 23.56& 22.86& 22.58& 22.56& 22.36& 22.13& 21.96& 21.11& -1.00&-99.00&     1.53$^s $& -3.00&    4\\
   318&  158.525&   57.334&-99.00&-99.00& 24.53&-99.00&-99.00& 23.78&-99.00& 21.94&-99.00&-99.00& -1.00& 17.90&     0.00$^s $&-99.00&  -99\\
   319&  158.526&   57.342& 21.10& 21.71& 21.07&-99.00& 21.06& 20.91& 20.98& 20.53&-99.00&-99.00& -1.00& 18.12&     1.53$^s $& -3.00&    4\\
   320&  158.526&   57.891& 23.51& 23.63& 23.64& 22.97& 22.55& 22.59& 22.43& 22.04& 21.32& 21.46& 20.51&-99.00&     1.46$^s $& -3.00&    4\\
   321&  158.526&   57.835&-99.00&-99.00&-99.00& 25.79& 25.27&-99.00& 24.66&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   322&  158.528&   57.935& 21.96& 21.31& 20.72& 20.20& 19.68& 19.50& 19.11& 19.07& 19.04& 18.68& 19.25& 18.10&     0.20$^s $& -3.00&    1\\
   323&  158.529&   58.043& 21.30& 20.68& 20.12&-99.00& 19.28& 18.50& 18.06& 17.79& 17.70& 17.25& 17.81& 17.17&     0.26$^s $& -3.00&    4\\
   324&  158.532&   57.352&-99.00& 25.92& 25.85&-99.00& 24.40& 23.94& 22.64& 21.08&-99.00&-99.00& -1.00& 17.97&     0.00$^s $&-99.00&  -99\\
   325&  158.533&   57.906& 22.74& 21.43& 20.30& 19.57& 18.49& 17.29& 16.54& 16.14& 16.03& 16.12& 16.89&-99.00&    -2.00$^s $&-99.00&   -2\\
   326&  158.535&   57.753&-99.00& 25.72& 25.36& 25.34& 24.67& 23.99& 23.01& 22.80& 21.92&-99.00& 20.81&-99.00&     1.34$^s $& -3.00&    3\\
   327&  158.538&   57.425& 21.94& 22.11&-99.00& 21.95& 21.95& 21.81& 21.51& 21.42& 21.39& 21.08& -1.00&-99.00&     2.10$^s $& -3.00&    4\\
   328&  158.538&   57.306& 21.39&-99.00& 20.75&-99.00&-99.00& 20.59&-99.00& 19.90& 19.97&-99.00& -1.00&-99.00&     1.53& -3.00&    4\\
   329&  158.539&   57.498& 22.69& 22.32& 21.68& 21.13& 20.49& 20.37& 19.96& 19.63& 19.79& 19.40& -1.00& 17.71&     0.37$^s $& -3.00&    3\\
   330&  158.540&   57.791&-99.00&-99.00&-99.00& 25.75& 25.07&-99.00& 23.65& 22.30& 21.57& 21.30& 20.51&-99.00&     0.00$^s $&  1.35&  -99\\
   331&  158.543&   58.064& 16.94&-99.00& 16.47&-99.00& 16.54& 16.88&-99.00& 16.88& 17.17& 17.42& 17.61& 14.21&     0.01$^s $& -3.00&    1\\
   332&  158.544&   57.571& 22.79& 22.26& 22.14&-99.00& 21.89& 21.37& 20.96& 20.59& 20.14& 19.55& -1.00&-99.00&     0.67$^s $& -3.00&    4\\
   333&  158.544&   57.934&-99.00& 25.41&-99.00& 24.35& 22.96& 21.96& 21.09& 20.59& 20.51&-99.00& 19.64&-99.00&     0.96$^s $& -3.00&    1\\
   334&  158.544&   57.365&-99.00& 25.63& 25.16&-99.00& 24.81&-99.00& 23.96& 21.67&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  1.55&  -99\\
   335&  158.544&   57.558&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.89&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   336&  158.545&   57.989& 23.08& 23.40& 23.24& 22.91& 22.99& 22.67& 22.50& 22.26&-99.00&-99.00&-99.00&-99.00&     2.27$^s $& -3.00&    4\\
   337&  158.547&   57.925& 21.58& 20.60&-99.00& 19.26& 18.79& 18.58& 18.21& 18.07& 17.98& 17.64& 17.73& 14.85&     0.20$^s $& -3.00&    3\\
   338&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.37&-99.00&     0.00$^s $&-99.00&  -99\\
   339&  158.551&   57.506& 23.69&-99.00& 23.53& 23.24&-99.00& 23.24& 23.32& 22.19& 21.77& 21.16& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   340&  158.552&   57.733& 24.26& 23.90& 23.69& 23.67& 23.13& 23.12& 22.45& 21.82& 21.64& 20.91& 20.79&-99.00&     1.49$^s $& -3.00&    1\\
   341&  158.554&   57.809&-99.00&-99.00& 25.05& 24.22& 23.03& 22.28& 21.26& 20.79& 20.40& 19.94& 19.64&-99.00&     0.96$^s $& -3.00&    0\\
   342&  158.554&   57.472&-99.00& 24.68& 24.43&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   343&  158.557&   57.568&-99.00& 14.33&-99.00& 14.43& 14.53&-99.00& 13.87& 12.98& 12.57& 12.08& -1.00& 17.62&    -2.00$^s $&-99.00&   -2\\
   344&  158.559&   57.778& 23.60& 23.47& 23.03&-99.00&-99.00& 22.58& 22.22& 21.98&-99.00& 20.85& 20.04& 17.40&     0.00$^s $&-99.00&  -99\\
   345&  158.559&   57.763&-99.00& 27.02&-99.00& 25.90& 25.45&-99.00& 25.01&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.15&  -99\\
   346&  158.560&   57.374&-99.00&-99.00&-99.00&-99.00& 25.72& 23.88& 23.58&-99.00&-99.00&-99.00& -1.00&-99.00&     5.40$^s $& -3.00&    4\\
   347&  158.561&   57.581& 23.13& 22.66& 22.51& 22.28& 21.72& 21.63& 21.03& 20.78& 20.52& 19.82& -1.00&-99.00&     0.92$^s $& -3.00&    3\\
   348&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.84&-99.00&    -1.00$^s $&-99.00&   -1\\
   349&  158.562&   57.900&-99.00&-99.00&-99.00& 25.32& 24.85& 24.18& 23.32& 21.93&-99.00& 20.71& 20.52&-99.00&     1.34$^s $& -3.00&    1\\
   350&  158.562&   57.510&-99.00&-99.00&-99.00& 25.44& 24.41&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   351&  158.564&   57.357& 23.44& 22.71& 22.70&-99.00& 21.74& 21.89& 21.35& 20.62& 20.31&-99.00& -1.00& 17.39&    -1.00$^s $&  0.15&   -1\\
   352&  158.565&   57.993& 22.31& 21.87& 21.75& 21.32& 21.23& 20.93& 20.52& 19.91& 19.99& 19.64& 19.29& 17.89&     0.82$^s $& -3.00&    4\\
   353&  158.568&   58.059& 22.81&-99.00& 22.50&-99.00& 22.48& 22.02&-99.00& 21.23& 20.92& 20.57& 20.06&-99.00&     1.09$^s $& -3.00&    4\\
   354&  158.571&   57.723&-99.00& 26.15&-99.00& 25.79& 25.47&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   355&  158.573&   57.840& 21.55& 21.40& 21.29& 21.06& 20.45& 20.58& 20.17& 20.07& 19.88& 19.29& 18.29& 16.64&     1.10$^s $& -3.00&    3\\
   356&  158.578&   57.642&-99.00& 24.86& 24.90& 24.27& 23.24& 22.80& 21.84& 21.01& 20.49& 19.78& 19.16&-99.00&    -1.00$^s $&  1.15&   -1\\
   357&  158.582&   57.747& 21.83& 22.56& 20.95& 21.65& 21.51& 21.20& 21.20& 20.64& 20.36& 19.89& 19.50& 17.52&     1.10$^s $& -3.00&    4\\
   358&  158.583&   57.698&-99.00&-99.00&-99.00&-99.00& 25.24& 24.74& 23.75&-99.00&-99.00& 21.18& 21.17&-99.00&    -1.00$^s $&  1.25&   -1\\
   359&  158.584&   57.309& 23.96&-99.00& 22.82&-99.00&-99.00& 20.78&-99.00& 19.70& 19.61&-99.00& -1.00& 16.91&     0.00$^s $&  0.15&  -99\\
   360&  158.585&   57.885&-99.00& 24.30& 24.22& 23.95& 23.33& 23.02& 22.07& 21.30& 20.86& 20.48& 19.70&-99.00&     1.46$^s $& -3.00&    1\\
   361&  158.586&   57.817&-99.00& 25.14& 24.76& 24.42& 23.58& 23.34& 22.37& 21.77& 21.38& 20.53& 20.10&-99.00&     0.00$^s $&  0.85&  -99\\
   362&  158.589&   57.838&-99.00& 24.95&-99.00&-99.00& 24.49&-99.00& 23.97&-99.00&-99.00&-99.00& 20.34&-99.00&     0.00$^s $&  0.55&  -99\\
   363&  158.589&   57.775& 24.84& 24.68& 24.47& 24.22& 23.84& 23.69& 23.35& 22.38& 21.77& 21.17& 20.72&-99.00&     1.92$^s $& -3.00&    3\\
   364&  158.590&   57.842& 22.04& 21.91& 21.03& 20.90& 21.33& 21.47& 21.07& 21.20& 21.09& 20.58& 20.27&-99.00&     2.28$^s $& -3.00&    4\\
   365&  158.592&   57.875& 23.43& 23.20& 22.85& 22.55& 21.88& 21.27& 20.66& 20.26& 20.10& 19.49& 19.40&-99.00&     0.81$^s $& -3.00&    1\\
   366&  158.602&   57.970& 23.65& 23.45& 23.24& 22.90& 22.19& 21.95& 20.92& 20.47& 20.23& 19.61& 19.18&-99.00&     1.22$^s $& -3.00&    1\\
   367&  158.605&   57.823&-99.00&-99.00&-99.00& 25.16& 24.02& 23.35& 22.57& 21.56& 21.32& 20.33& 19.73&-99.00&     0.00$^s $&  1.35&  -99\\
   368&  158.607&   57.921&-99.00& 25.21&-99.00& 24.84& 24.25& 23.79& 23.42& 22.14&-99.00&-99.00& 20.26&-99.00&     0.00$^s $&  1.55&  -99\\
   369&  158.618&   57.485&-99.00& 26.37& 25.99& 25.79& 25.28&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   370&  158.620&   57.683& 23.30& 23.08& 22.71& 22.30& 21.74& 21.18& 20.52& 20.42& 20.24& 19.58& 19.20& 17.46&     0.99$^s $& -3.00&    1\\
   371&  158.623&   57.724&-99.00& 26.16&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   372&  158.623&   57.871& 22.54& 22.24& 22.16& 21.84& 21.45& 21.40& 20.93& 20.89& 20.73& 20.13& 19.48&-99.00&     1.05$^s $& -3.00&    4\\
   373&  158.624&   57.849& 23.04& 22.34& 21.91& 21.06& 20.27& 20.24& 19.54& 19.43& 19.41& 18.96& 19.48&-99.00&     0.33$^s $& -3.00&    4\\
   374&  158.625&   57.630&-99.00& 25.25& 24.77& 24.27& 23.26& 22.41& 21.70& 21.36& 20.75& 20.56& 20.31&-99.00&     0.96$^s $& -3.00&    1\\
   375&  158.625&   57.741&-99.00& 26.49& 26.18& 25.72& 24.88& 24.98& 23.97& 22.46& 21.88&-99.00& 21.50&-99.00&     0.00$^s $&  1.35&  -99\\
   376&  158.628&   57.480& 25.10& 24.57& 24.38& 24.05& 23.46& 23.16& 22.87& 21.65& 21.52& 20.82& -1.00&-99.00&     0.00$^s $&  0.85&  -99\\
   377&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   378&  158.637&   57.904& 24.04& 23.89& 23.65& 23.42& 22.46& 22.33& 22.01& 21.96&-99.00&-99.00&-99.00&-99.00&     0.61$^s $& -3.00&    1\\
   379&  158.637&   57.717&-99.00& 25.68& 25.52& 25.39& 24.19& 23.47& 22.50& 21.57& 21.48& 20.95& 20.48&-99.00&     1.27$^s $& -3.00&    1\\
   380&  158.640&   57.963&-99.00& 25.33& 24.52& 23.79& 22.51& 21.71& 20.80& 20.49& 20.21& 19.61& 19.46& 17.25&     0.82$^s $& -3.00&    0\\
   381&  158.640&   57.542& 20.16& 18.90& 17.91& 17.55& 16.80& 15.70& 15.19& 14.51& 14.15& 14.02& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   382&  158.645&   57.704&-99.00& 25.71& 25.29& 24.48& 23.89& 24.71& 24.40&-99.00&-99.00&-99.00&-99.00&-99.00&     3.58$^s $& -3.00&    4\\
   383&  158.647&   57.467& 22.91& 22.55& 22.79& 22.44& 22.23& 22.35& 21.84& 21.62& 21.44& 20.84& -1.00&-99.00&     2.04$^s $& -3.00&    4\\
   384&  158.649&   57.774& 21.96& 22.14& 21.47& 21.06& 20.86& 20.45& 19.61& 19.40& 19.16& 18.64& 18.21& 17.18&     0.90$^s $& -3.00&    4\\
   385&  158.650&   58.022& 23.32& 21.61& 20.76& 20.58& 18.82& 18.53& 17.93& 17.64& 17.47& 16.97& 17.54&-99.00&     0.44$^s $& -3.00&    0\\
   386&  158.653&   57.690& 24.91& 24.35& 24.07& 24.84& 23.40& 22.89& 22.74& 22.26& 21.92& 21.21& 21.07&-99.00&     0.00$^s $&  0.15&  -99\\
   387&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   388&  158.658&   57.912&-99.00& 25.67& 24.79& 24.32& 23.18& 22.67& 21.91& 21.25& 20.65& 19.92& 19.49& 17.78&     1.19$^s $& -3.00&    1\\
   389&  158.658&   57.588&-99.00&-99.00&-99.00&-99.00& 26.88&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   390&  158.662&   57.837& 23.90& 23.99& 24.09& 23.27& 23.43& 23.22& 22.60& 22.66& 21.36& 21.15& 20.72&-99.00&     2.27$^s $& -3.00&    4\\
   391&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.37&-99.00&     0.00$^s $&-99.00&  -99\\
   392&  158.666&   57.635& 22.31& 22.01& 21.72& 21.37& 20.82& 20.60& 20.10& 20.12& 19.81& 19.18& 19.30& 17.84&     0.50$^s $& -3.00&    4\\
   393&  158.666&   57.732& 21.65& 21.12& 20.68& 20.02& 19.35& 19.20& 18.68& 18.67& 18.34& 17.98& 17.88& 15.76&     0.45$^s $& -3.00&    1\\
   394&  158.667&   57.766&-99.00& 24.67& 23.91& 23.19& 22.00& 21.28& 20.64& 20.31& 19.83& 19.47& 19.54&-99.00&     0.62$^s $& -3.00&    1\\
   395&  158.669&   57.646&-99.00&-99.00&-99.00&-99.00& 25.57&-99.00& 23.84&-99.00&-99.00& 21.14& 20.70&-99.00&     0.00$^s $&  1.45&  -99\\
   396&  158.670&   57.838&-99.00& 25.32& 25.13& 24.50& 23.91& 23.91& 23.25& 22.14& 21.25& 20.73& 20.51&-99.00&     0.00$^s $&  0.85&  -99\\
   397&  158.671&   57.788& 19.81& 19.98& 19.49& 19.37& 19.20& 19.38& 19.11& 19.41& 19.29& 18.87& 18.19& 15.74&     1.08$^s $& -3.00&    3\\
   398&  158.673&   57.893& 24.08& 23.77& 23.62& 23.37& 23.03& 23.06& 22.50& 22.02&-99.00& 20.85& 20.21&-99.00&     0.00$^s $&  0.65&  -99\\
   399&  158.673&   57.544& 23.11& 23.24& 22.90& 22.77& 22.43& 22.20& 22.12& 21.47& 21.34& 20.77& -1.00&-99.00&     1.21$^s $& -3.00&    4\\
   400&  158.675&   57.983& 23.86& 23.76& 23.55& 23.34& 22.69& 22.45& 21.52& 21.03& 20.81& 20.25& 19.90&-99.00&     0.00$^s $&  0.55&  -99\\
   401&  158.676&   57.436&-99.00& 24.33& 24.11&-99.00&-99.00& 23.56& 22.54& 22.22&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.15&  -99\\
   402&  158.677&   57.895&-99.00& 24.56&-99.00& 23.76& 22.61& 22.38& 21.17& 20.57& 19.79& 19.32& 18.78&-99.00&     1.00$^s $& -3.00&    0\\
   403&  158.677&   57.653& 24.88& 24.97& 24.75& 24.63& 24.28& 24.52& 23.97&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   404&  158.686&   57.473&-99.00& 25.73&-99.00& 25.02& 24.92& 24.43& 23.79& 22.43&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  1.55&  -99\\
   405&  158.689&   57.929& 24.17& 23.97&-99.00& 23.72& 23.37& 23.40& 22.75& 22.59&-99.00&-99.00& 21.51&-99.00&    -1.00$^s $&-99.00&   -1\\
   406&  158.688&   57.405& 22.47& 23.63& 22.11& 22.94& 23.05& 22.40& 22.41& 20.42&-99.00& 20.55& -1.00&-99.00&     1.88$^s $& -3.00&    4\\
   407&  158.689&   57.676&-99.00& 25.32& 24.92& 24.45& 24.32& 23.21& 23.59& 21.71& 21.39& 20.76& 20.17& 17.34&     0.00$^s $&  1.75&  -99\\
   408&  158.689&   57.760&-99.00& 24.96& 24.78& 24.44& 23.69& 23.41& 22.88& 21.95& 21.26& 21.04& 20.04&-99.00&    -1.00$^s $&  1.25&   -1\\
   409&  158.694&   57.678&-99.00& 25.27& 25.30& 24.78& 24.07& 23.71& 22.80& 21.73& 21.36& 20.68& 20.14&-99.00&    -1.00$^s $&  1.35&   -1\\
   410&  158.695&   57.627& 23.67& 23.59& 23.05& 22.76& 22.07& 21.43& 20.42& 20.66& 19.71& 19.31& 18.86& 17.75&     0.90$^s $& -3.00&    1\\
   411&  158.696&   57.858& 21.96& 22.15& 21.69& 21.68& 21.53& 20.76& 20.47& 19.66& 19.71& 18.96& 18.95&-99.00&     0.77$^s $& -3.00&    4\\
   412&  158.696&   58.039&-99.00& 24.87& 24.79&-99.00& 23.22& 22.54& 21.79& 21.29& 21.17& 20.59& 20.52&-99.00&    -1.00$^s $&  0.85&   -1\\
   413&  158.699&   57.833& 24.07& 23.78& 23.54& 23.11& 22.07& 21.33& 20.03& 19.69& 19.43& 18.93& 18.57& 16.79&     1.01$^s $& -3.00&    3\\
   414&  158.699&   57.469&-99.00& 24.92& 24.43& 24.41& 24.03& 23.40& 23.08& 22.06&-99.00&-99.00& -1.00&-99.00&     0.00$^s $&  0.65&  -99\\
   415&  158.702&   57.693&-99.00& 25.21& 24.91& 24.80& 24.33& 24.19& 24.01&-99.00&-99.00&-99.00&-99.00&-99.00&     0.93& -3.00&    1\\
   416&  158.702&   57.737&-99.00&-99.00&-99.00& 25.44& 25.35&-99.00&-99.00&-99.00&-99.00&-99.00& 21.72&-99.00&     0.00$^s $&-99.00&  -99\\
   417&  158.703&   57.834& 21.91& 21.84& 21.66& 21.54& 21.38& 21.12& 20.95& 20.98& 20.92& 20.70& 20.06&-99.00&    -1.00$^s $&-99.00&   -1\\
   418&  158.706&   57.797&-99.00& 26.03& 25.15& 23.74& 24.55& 22.78& 22.31& 22.16& 21.28& 20.52& 19.01&-99.00&     0.00$^s $&  0.25&  -99\\
   419&  158.706&   57.922&-99.00&-99.00&-99.00&-99.00& 25.17&-99.00& 24.12&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   420&  158.707&   57.781&-99.00& 25.59& 25.29& 24.86& 23.46& 22.68& 21.50& 21.08& 20.79& 20.13& 19.71&-99.00&     1.14& -3.00&    3\\
   421&  158.707&   57.969&-99.00&-99.00&-99.00&-99.00& 24.42& 23.68& 22.61& 21.81& 21.40& 20.55& 19.81&-99.00&     1.23$^s $& -3.00&    0\\
   422&  158.707&   57.429& 22.84& 22.51& 22.53& 22.00& 21.66& 21.41& 20.95&-99.00& 20.51& 20.05& -1.00&-99.00&     0.77& -3.00&    4\\
   423&  158.709&   57.537& 24.85& 24.96& 25.13& 24.64& 24.83& 24.51& 24.24&-99.00& 22.17& 21.14& -1.00&-99.00&     0.00$^s $&-99.00&  -99\\
   424&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.40&-99.00&     0.00$^s $&-99.00&  -99\\
   425&  158.710&   57.688&-99.00&-99.00&-99.00& 25.55& 25.15&-99.00& 24.11& 22.68&-99.00&-99.00& 20.32& 17.25&     0.00$^s $&  1.55&  -99\\
   426&  158.713&   57.631& 25.03& 24.54& 24.34& 24.20& 23.69& 23.28& 22.76&-99.00& 21.12& 20.63& 19.94&-99.00&     0.00$^s $&  1.45&  -99\\
   427&  158.712&   57.562&-99.00& 25.61&-99.00& 25.13& 24.72& 23.92& 23.13&-99.00&-99.00&-99.00& 20.69&-99.00&     1.30$^s $& -3.00&    3\\
   428&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   429&  158.714&   57.473& 23.42& 23.63& 23.37& 23.04& 23.29& 23.04& 22.96& 22.12&-99.00&-99.00& -1.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   430&  158.716&   57.659& 20.97& 20.85& 20.41& 20.16& 19.84& 19.98& 19.66& 20.44& 19.73& 19.79& 20.01& 17.25&     0.29$^s $& -3.00&    1\\
   431&  158.717&   57.901&-99.00& 25.55& 24.85& 24.73& 23.80& 24.28& 24.02&-99.00&-99.00&-99.00&-99.00&-99.00&     3.25$^s $& -3.00&    3\\
   432&  158.717&   57.572&-99.00&-99.00&-99.00&-99.00& 25.08&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   433&  158.720&   57.779&-99.00& 25.85& 25.32& 25.02& 24.01& 23.65& 22.51& 21.58& 21.09& 20.39& 20.03&-99.00&     1.33$^s $& -3.00&    1\\
   434&  158.721&   57.676& 24.70& 24.05& 23.70& 23.53& 23.22& 22.95& 22.46& 22.08& 21.45& 20.97& 20.54&-99.00&     0.00$^s $&  0.75&  -99\\
   435&  158.722&   57.580& 23.99& 23.39& 23.21& 23.02& 22.20& 21.91& 21.58& 21.53& 21.10& 20.51& 19.77& 17.23&     1.97$^s $& -3.00&    4\\
   436&  158.722&   57.565&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.48& 20.71& 20.13& 17.66&    -1.00$^s $&-99.00&   -1\\
   437&  158.725&   57.723& 15.07& 15.19& 13.71& 15.44& 14.50& 15.17& 15.05& 13.90& 13.28& 13.10& 14.08&-99.00&    -2.00$^s $&-99.00&   -2\\
   438&  158.728&   57.702& 23.40& 22.98& 22.25& 22.79& 21.99& 21.60& 21.25& 21.45& 21.23& 20.54& 20.14&-99.00&     2.08$^s $& -3.00&    4\\
   439&  158.729&   57.782& 24.48& 23.51& 22.62& 21.98& 20.46& 20.05& 19.45& 19.50& 18.99& 18.48& 18.92&-99.00&     0.51$^s $& -3.00&    0\\
   440&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&    -1.00$^s $&-99.00&   -1\\
   441&  158.734&   57.790& 24.16& 23.60& 22.98& 22.34& 21.05& 20.77& 20.24& 20.41& 19.71& 19.64& 19.51&-99.00&     0.39$^s $& -3.00&    1\\
   442&  158.736&   57.633& 23.32& 23.25& 22.68& 22.45& 22.30& 22.29& 21.58& 21.74& 21.07& 20.25& 20.12&-99.00&     0.90& -3.00&    4\\
   443&  158.736&   57.794&-99.00&-99.00&-99.00&-99.00& 25.39& 24.25& 23.74&-99.00& 22.48&-99.00& 20.96&-99.00&     0.00$^s $&  0.45&  -99\\
   444&  158.737&   57.553& 23.93& 22.96& 22.84& 22.26& 21.56& 21.40& 20.74& 20.35& 20.16& 19.61& 19.21&-99.00&     0.94$^s $& -3.00&    3\\
   445&  158.737&   57.806& 24.02& 22.54& 21.45& 20.77& 19.54& 17.91& 16.89& 16.55& 16.30& 16.33& 17.01&-99.00&    -2.00$^s $&-99.00&   -2\\
   446&  158.740&   57.951&-99.00&-99.00&-99.00&-99.00& 25.80&-99.00& 24.47&-99.00&-99.00&-99.00& 20.98&-99.00&     0.00$^s $&-99.00&  -99\\
   447&  158.740&   57.632&-99.00& 25.98& 25.34& 24.73& 23.65& 22.77& 22.03& 21.72& 21.16& 20.23& 19.62&-99.00&     0.61& -3.00&    3\\
   448&  158.742&   57.632& 25.41& 25.10& 24.46& 23.99& 23.13& 22.40& 22.36&-99.00& 21.49&-99.00&-99.00&-99.00&     0.62$^s $& -3.00&    3\\
   449&  158.742&   57.846& 24.10& 24.26& 23.18& 22.61& 22.94& 22.84& 22.94& 22.05& 21.88&-99.00&-99.00&-99.00&     3.43$^s $& -3.00&    4\\
   450&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.17&-99.00&     0.00$^s $&-99.00&  -99\\
   451&  158.744&   57.694& 25.37& 24.89& 24.40& 24.57& 23.84& 23.84& 23.34&-99.00&-99.00&-99.00&-99.00&-99.00&     1.31$^s $& -3.00&    4\\
   452&  158.746&   57.509& 20.84& 20.35& 20.73& 19.60& 19.80& 19.87& 19.42&-99.00&-99.00& 18.42& -1.00& 17.03&     3.80$^s $& -3.00&    4\\
   453&  158.752&   57.724&-99.00& 25.78& 25.24& 24.51& 23.51& 22.82& 21.84& 21.60& 21.10& 20.48& 20.34&-99.00&     0.00$^s $&  0.85&  -99\\
   454&  158.751&   57.509& 19.31& 18.08& 17.34& 17.09& 15.88& 15.15& 14.57& 13.86& 13.51& 13.24& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   455&  158.755&   57.950&-99.00& 24.91& 24.14& 23.77& 22.89& 22.06& 21.17& 20.91& 20.52& 20.04& 19.61&-99.00&     0.88$^s $& -3.00&    0\\
   456&  158.759&   57.835& 23.59& 23.35& 23.15& 22.94& 22.43& 22.18& 21.13& 20.57& 20.21& 19.69& 19.05& 17.74&     1.34$^s $& -3.00&    1\\
   457&  158.764&   57.685&-99.00& 25.23& 24.88&-99.00& 23.48& 23.38& 22.91& 21.82& 21.49& 20.91& 19.73&-99.00&     1.54$^s $& -3.00&    1\\
   458&  158.767&   57.731&-99.00& 25.79& 25.69& 24.98& 24.44& 23.87& 23.25&-99.00&-99.00& 21.51& 21.12&-99.00&     0.00$^s $&  1.05&  -99\\
   459&  158.772&   57.700& 17.56& 16.75& 16.38& 16.57& 15.87& 15.24& 15.33& 15.23& 14.70& 14.77& 15.70&-99.00&    -2.00$^s $&-99.00&   -2\\
   460&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 21.40&-99.00&     0.00$^s $&-99.00&  -99\\
   461&  158.779&   57.611& 21.91& 21.17& 20.35& 19.70& 19.11& 18.87& 18.39& 18.48& 18.00& 17.57& 18.43& 17.58&     0.29$^s $& -3.00&    1\\
   462&  158.781&   57.720&-99.00& 26.57&-99.00&-99.00& 25.88&-99.00&-99.00&-99.00&-99.00&-99.00& 20.23&-99.00&     0.94$^s $& -3.00&    1\\
   463&  158.784&   57.647& 23.54& 23.28& 22.76& 22.48& 21.75& 21.36& 20.58& 20.79& 20.10& 19.69& 19.39& 17.84&     2.12$^s $& -3.00&    4\\
   464&  158.784&   57.983&-99.00&-99.00&-99.00&-99.00& 25.58&-99.00& 24.48& 22.36&-99.00&-99.00& 21.24&-99.00&     0.00$^s $&-99.00&  -99\\
   465&  158.784&   57.805& 25.01& 24.73& 24.62& 24.38& 23.75& 23.50& 22.57& 21.82& 21.07& 20.76& 20.17&-99.00&     1.42$^s $& -3.00&    1\\
   466&  158.785&   57.962& 23.85& 23.63& 23.36& 22.98& 21.78& 21.16& 20.32& 19.70& 19.31& 18.56& 17.33& 15.03&     1.26$^s $& -3.00&    3\\
   467&  158.786&   57.978&-99.00& 25.69& 25.60&-99.00& 25.03&-99.00& 24.24&-99.00&-99.00&-99.00& 21.34&-99.00&     0.00$^s $&  1.85&  -99\\
   468&  158.789&   58.033&-99.00& 21.68&-99.00&-99.00& 21.15&-99.00& 20.99&-99.00&-99.00&-99.00&-99.00&-99.00&     1.60$^s $& -3.00&    4\\
   469&  158.792&   57.737&-99.00&-99.00&-99.00&-99.00& 24.69& 23.79& 22.75& 22.35& 22.04& 20.95& 20.59&-99.00&     0.00$^s $&  0.85&  -99\\
   470&  158.793&   57.514& 15.85& 15.37& 15.34& 15.32& 14.63& 14.47& 14.19& 13.90& 13.62& 13.65& -1.00&-99.00&    -2.00$^s $&-99.00&   -2\\
   471&  158.801&   57.930& 23.98& 23.64&-99.00& 23.03& 22.29& 21.94& 20.89& 20.75& 20.18& 19.82& 19.07& 16.52&     0.72$^s $& -3.00&    3\\
   472&  158.806&   57.661& 24.67& 24.22& 23.53& 22.91& 21.73& 21.19& 20.61& 20.55& 20.01& 19.53& 19.58&-99.00&     0.00$^s $&  0.45&  -99\\
   473&  158.810&   57.951& 24.08& 23.24& 22.78& 22.83& 22.74& 22.95& 22.46& 22.31& 21.44&-99.00&-99.00&-99.00&     0.00$^s $&  0.35&  -99\\
   474&  158.814&   57.516& 24.17& 23.91& 23.27& 22.65& 21.62& 20.85& 20.13& 19.71& 19.65& 18.96& 18.84& 17.20&    -1.00$^s $&  0.75&   -1\\
   475&  158.817&   57.765& 23.32& 23.65& 23.75& 23.01& 22.83& 22.65& 22.46& 21.75& 21.09& 20.51& 19.39&-99.00&     1.59$^s $& -3.00&    4\\
   476&  158.828&   57.565& 24.09& 23.44& 23.31& 23.12& 22.93& 23.16& 22.11& 22.09& 21.26& 20.52& 20.06& 16.36&     0.00$^s $&  0.25&  -99\\
   477&  158.832&   57.911& 22.81& 22.04& 21.31& 20.51& 19.85& 19.66& 19.11& 19.02& 18.88& 18.59& 19.15&-99.00&     0.26$^s $& -3.00&    1\\
   478&  158.832&   57.789&-99.00& 26.31&-99.00& 25.79& 25.60&-99.00& 24.82&-99.00&-99.00&-99.00& 21.42&-99.00&    -1.00$^s $&  1.45&   -1\\
   479&  158.833&   57.849&-99.00&-99.00&-99.00&-99.00& 25.80&-99.00& 24.34&-99.00& 21.98&-99.00& 19.87& 16.33&     0.00$^s $&  1.65&  -99\\
   480&  158.837&   57.564&-99.00&-99.00&-99.00& 25.38& 24.92&-99.00&-99.00&-99.00& 21.86& 21.04& 20.48&-99.00&    -1.00$^s $&  0.75&   -1\\
   481&  158.842&   57.623& 22.54& 22.59& 22.37& 21.79& 21.88& 21.85& 21.42& 21.64& 21.25& 20.89& 19.72&-99.00&     0.00$^s $&  2.35&  -99\\
   482&  158.846&   57.688& 21.00& 21.72& 20.60& 21.25& 20.76& 20.89& 20.36& 20.27& 19.76& 19.22& 18.85&-99.00&     1.16$^s $& -3.00&    4\\
   483&  158.846&   57.768& 23.62& 23.07& 22.53& 22.03& 20.50& 20.03& 19.33& 19.34& 18.74& 18.27& 18.17& 17.67&     0.62$^s $& -3.00&    1\\
   484&  158.849&   57.758&-99.00&-99.00&-99.00&-99.00& 25.65&-99.00& 23.95& 24.31& 21.88& 21.23& 20.74&-99.00&     0.00$^s $&-99.00&  -99\\
   485&  158.851&   57.743& 21.33& 20.79& 20.04& 19.46& 19.05& 18.82& 18.41& 18.63& 18.10& 17.78& 18.02& 14.87&     0.23$^s $& -3.00&    1\\
   486&  158.859&   57.927&-99.00& 24.34&-99.00& 22.91& 21.76& 21.08& 20.34& 19.91& 19.58& 19.10& 18.98&-99.00&     0.72$^s $& -3.00&    1\\
   487&  158.858&   57.872& 23.03& 22.02& 22.11& 21.91& 21.68& 21.97& 21.56& 21.56& 21.25& 21.01& 20.72&-99.00&     2.66$^s $& -3.00&    4\\
   488&  158.861&   58.008& 24.74& 23.94&-99.00&-99.00& 23.22&-99.00& 22.43&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&  0.25&  -99\\
   489&  158.863&   57.786&-99.00& 25.45& 25.11& 25.05& 24.34&-99.00&-99.00&-99.00&-99.00&-99.00& 18.99&-99.00&     0.00$^s $&  1.15&  -99\\
   490&  158.864&   57.700& 22.56& 22.00& 20.98& 21.01& 19.97& 19.66& 19.08& 19.19& 18.65& 18.21& 18.48&-99.00&     0.51$^s $& -3.00&    0\\
   491&  158.866&   57.770&-99.00& 25.60&-99.00& 24.53& 24.25& 23.24& 23.36&-99.00& 20.29&-99.00& 19.29&-99.00&    -1.00$^s $&  1.25&   -1\\
   492&  158.871&   57.709& 23.25& 23.44& 23.33& 23.27& 23.14& 23.31& 22.75&-99.00&-99.00&-99.00&-99.00&-99.00&     2.22$^s $& -3.00&    4\\
   493&  158.871&   57.600&-99.00&-99.00& 24.65&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 20.30&-99.00&     0.00$^s $&-99.00&  -99\\
   494&  158.876&   57.819& 24.07& 22.77& 21.66& 20.99& 19.84& 18.39& 17.33& 17.01& 16.93& 16.89& 17.59&-99.00&    -2.00$^s $&-99.00&   -2\\
   495&  158.879&   57.644& 25.31& 25.08& 24.51& 24.08& 23.19& 22.30& 21.53& 21.39& 20.72& 20.21& 19.88&-99.00&    -1.00$^s $&  0.75&   -1\\
   496&  158.879&   57.763& 24.07& 23.20& 22.46& 21.45& 20.25& 19.88& 19.26& 19.35& 18.75& 18.32& 18.64&-99.00&     0.51$^s $& -3.00&    0\\
   497&  158.883&   57.872& 24.83& 24.76& 24.30& 24.19& 24.72&-99.00& 23.39& 21.68& 20.94& 20.61& 19.96&-99.00&     0.00$^s $&  2.05&  -99\\
   498&  158.883&   57.882& 22.24& 21.99& 21.50& 20.83& 19.85& 19.68& 19.22& 19.23& 18.92& 18.47& 18.51&-99.00&     0.52$^s $& -3.00&    3\\
   499&  158.883&   57.596& 22.84& 22.57& 22.11& 21.73& 21.28& 20.95& 20.32& 20.69& 20.29& 19.91& 19.51& 17.36&     0.00$^s $&  0.35&  -99\\
   500&  158.884&   57.943& 23.55& 23.55& 23.32& 23.26& 22.83& 22.44& 22.28& 21.32& 20.78& 20.16& 19.65&-99.00&     0.95$^s $& -3.00&    1\\
   501&  158.885&   57.779&-99.00& 25.16& 24.46& 23.93& 23.21& 23.09& 22.73& 22.18& 20.87& 20.45& 20.03&-99.00&     0.00$^s $&-99.00&  -99\\
   502&  158.888&   57.804& 24.16& 23.21& 22.37& 21.33& 20.48& 20.13& 19.51& 19.28& 18.85& 18.33& 18.89&-99.00&     0.32$^s $& -3.00&    3\\
   503&  158.891&   57.647&-99.00& 24.80& 23.95& 23.26& 22.04& 21.50& 21.04& 21.06& 20.45& 20.06& 20.39&-99.00&    -1.00$^s $&  0.65&   -1\\
   504&  158.892&   57.709& 25.04& 23.78& 23.70& 23.47& 23.23& 23.22& 23.13&-99.00&-99.00&-99.00&-99.00&-99.00&     2.77$^s $& -3.00&    4\\
   505&  158.893&   57.732&-99.00& 25.20& 25.45& 25.04& 25.17& 24.72& 24.24&-99.00& 21.84& 21.43& 21.00&-99.00&     2.38$^s $& -3.00&    3\\
   506&  158.896&   57.843& 23.64& 23.65& 23.31&-99.00&-99.00& 22.32& 21.66& 21.08& 20.90& 20.51& 19.74&-99.00&     1.06$^s $& -3.00&    4\\
   507&  158.901&   57.895& 23.77& 23.64& 23.36& 23.18& 22.68& 22.26& 21.93& 21.65& 21.02& 20.60& 20.12& 17.38&     1.21$^s $& -3.00&    3\\
   508&  158.902&   57.820& 23.81& 22.90& 22.23& 21.24& 20.40& 20.04& 19.47& 19.24& 18.93& 18.48& 19.10&-99.00&     0.38$^s $& -3.00&    1\\
   509&  158.916&   57.715& 24.68&-99.00&-99.00&-99.00&-99.00& 22.57&-99.00& 21.85& 21.77&-99.00&-99.00&-99.00&     1.02$^s $& -3.00&    3\\
   510&  158.917&   57.830&-99.00& 25.32& 25.01& 24.88& 23.61& 23.25& 21.97& 21.15& 20.66& 20.09& 19.43&-99.00&     1.19$^s $& -3.00&    1\\
   511&  158.920&   57.844& 20.27& 20.02& 19.99& 19.76& 19.36& 19.53& 19.33& 19.61& 19.47& 19.46& 18.63& 15.61&     1.37$^s $& -3.00&    4\\
   512&  158.933&   57.744& 23.15&-99.00&-99.00&-99.00&-99.00& 20.42&-99.00& 20.88& 20.64& 20.28& 19.29&-99.00&     0.47$^s $& -3.00&    3\\
   513&  -99.000&  -99.000&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   514&  158.949&   57.718& 21.51& 21.87& 21.36& 21.27& 21.01& 20.78& 20.28& 20.43& 20.19& 19.52& 19.85&-99.00&     2.23$^s $& -3.00&    4\\
   515&  158.953&   57.726&-99.00& 25.80& 26.03& 25.15& 24.48&-99.00& 24.66&-99.00&-99.00&-99.00&-99.00&-99.00&     0.00$^s $&-99.00&  -99\\
   516&  158.962&   57.867& 23.87& 23.29& 23.13& 23.73& 23.22& 22.91& 22.78& 22.21&-99.00&-99.00& 21.53&-99.00&     2.04$^s $& -3.00&    4\\
   517&  158.963&   57.726& 21.05& 21.20& 20.70& 20.30& 20.21& 19.58& 19.38& 19.16& 18.79& 18.21& 17.78& 16.56&     0.62$^s $& -3.00&    3\\
   518&  159.003&   57.801& 23.51& 23.10& 22.56& 22.12& 20.95& 20.40& 19.75& 19.63& 18.95& 18.50& 18.15& 17.15&     0.68$^s $& -3.00&    1\\
   519&  159.007&   57.727& 24.18& 23.79& 23.39& 22.98& 22.26& 21.67& 20.55& 20.57& 19.93& 19.30& 18.90& 18.19&    -1.00$^s $&  0.65&   -1\\
   520&  159.008&   57.860&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00&-99.00& 19.67& 20.03&-99.00& 18.60& 16.29&     0.85$^s $& -3.00&    3\\
   521&  159.015&   57.804&-99.00& 24.36& 23.92&-99.00& 23.20& 22.86& 22.61&-99.00&-99.00&-99.00&-99.00&-99.00&     0.62$^s $& -3.00&    1\\
   522&  159.018&   57.797& 23.96& 23.40& 22.88& 22.46& 21.77& 21.45& 20.96& 21.13& 20.57& 20.27& 20.48&-99.00&     0.51$^s $& -3.00&    3\\
   523&  159.032&   57.836& 21.13& 20.57& 20.79& 20.14& 19.74& 19.53& 19.02& 19.12& 18.78& 18.19& 17.60& 16.55&     0.68$^s $& -3.00&    4\\
   524&  159.050&   57.849&-99.00& 26.18& 25.27& 24.82& 24.48&-99.00& 24.49& 21.51& 21.36&-99.00& 20.70&-99.00&     1.28$^s $& -3.00&    4\\
   525&  159.052&   57.774&-99.00& 26.44& 25.37& 24.55& 23.12& 22.25& 21.24& 21.01& 20.29& 19.80& 19.58&-99.00&     0.87$^s $& -3.00&    1\\
\tableline
\end{tabular}
\end{scriptsize}
\footnotesize
\tablecomments{All magnitudes are in AB magnitudes.\\
Typical photometric uncertainties are given in \S \ref{photodet}.\\
Magnitude $=-99$, source not detected ($2\sigma$ significance). \\
z$_{spec} = 0$ and corresponding class $= -99$, source spectroscopically observed but neither the redshift nor the class could be identified. \\
z$_{spec} = -1$ and corresponding class $= -1$, source not yet spectroscopically observed. \\
z$_{spec} = -2$ and corresponding class $= -2$, source is a star. \\
$z_{phot} = -3$, source has a spectroscopic redshift.\\
$z_{phot} = -99$, source has neither a spectroscopic nor a photometric redshift. \\
class $=0$, absorbers; class $=1$, star formers; class $=3$, high-excitation sources; class $=4$, broad-line AGNs.\\
Reference for z$_{spec}$: s=Steffen et al.~(2004). All other spectroscopic redshifts presented here for the first time.}
\end{table}


==> tab13.tex <==
\begin{table}
\begin{scriptsize}
\caption{CDF-N Optical/IR Counterparts Catalog}
\label{cdfnspect table}
\begin{tabular}{ccccccccccccccccc}
\tableline\tableline
    \#& RA&DEC&       $U$&       $B$&       $V$&       $R$&       $I$&$z^{\prime}$&       $J$&       $H$&     $K_s$&3.6$~\mu$m& 24$~\mu$m&z$_{spec}$&z$_{phot}$& class\\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)& (10)&(11) & (12) & (13) & (14) & (15) & (16) & (17)\\
\tableline
     1&   188.813&    62.235&      26.4&      25.7&      25.3&      25.1&      25.2&      24.8&     -99.0&     -99.0&     23.12&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
     2&   188.820&    62.261&      25.4&      24.9&      24.9&      24.5&      24.7&      24.5&     -99.0&      22.1&     21.41&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
     3&   188.828&    62.264&      21.3&      20.2&      19.1&      18.6&      18.2&      18.0&      17.0&      16.7&     16.62&    -99.00&    -99.00&      0.14$^a $&     -3.00&    0\\
     4&   188.831&    62.228&      27.2&      26.7&      25.6&      24.4&      23.6&      23.2&     -99.0&      22.3&     21.70&    -99.00&    -99.00&     -1.00  &      0.65&   -1\\
     5&   188.839&    62.274&      23.2&      22.8&      22.4&      21.8&      21.4&      21.2&      20.6&      20.2&     20.06&    -99.00&    -99.00&      0.56$^a $&     -3.00&    1\\
     6&   188.840&    62.302&      21.1&      20.2&      19.3&      18.8&      18.2&      18.1&      17.0&      16.6&     16.39&    -99.00&    -99.00&      0.14$^a $&     -3.00&    1\\
     7&   188.840&    62.250&      27.8&      27.7&      26.9&      27.4&      25.9&      26.7&     -99.0&     -99.0&     24.17&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
     8&   188.843&    62.231&      27.7&      25.7&      24.9&      24.3&      24.1&      24.1&     -99.0&     -99.0&     22.37&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
     9&   188.854&    62.257&      26.4&      26.1&      26.0&      25.7&      25.0&      24.7&     -99.0&      22.3&     22.21&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    10&   188.870&    62.241&     -30.3&      28.2&      29.0&      26.4&      26.0&      24.9&     -99.0&      22.1&     21.55&    -99.00&    -99.00&      0.00$^a $&      0.95&  -99\\
    11&   188.872&    62.216&      25.2&      23.7&      23.6&      23.0&      22.5&      22.1&      21.4&      21.0&     20.58&     20.47&    -99.00&      2.41$^a $&     -3.00&    4\\
    12&   188.873&    62.306&      27.2&      27.1&      27.2&      26.0&      26.0&      25.9&     -99.0&     -99.0&     24.17&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    13&   188.897&    62.241&      25.0&      24.4&      24.5&      24.3&      24.3&      24.1&     -99.0&      22.4&     22.17&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    14&   188.901&    62.317&      25.8&      25.5&      25.6&      24.8&      24.0&      23.3&      21.6&      21.1&     20.75&    -99.00&    -99.00&      0.00$^a $&      0.95&  -99\\
    15&   188.900&    62.280&      17.4&      18.0&      16.6&      18.4&      16.8&      15.3&      14.1&      13.8&     14.00&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
    16&   188.905&    62.290&      21.7&      22.3&      22.3&      22.3&      21.9&      22.0&      21.5&      21.0&     20.87&    -99.00&    -99.00&      2.05$^a $&     -3.00&    4\\
    17&   188.909&    62.328&      28.0&      26.2&      26.1&      25.2&      24.9&      24.6&     -99.0&     -99.0&     22.41&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
    18&   188.909&    62.326&      25.9&      25.6&      25.1&      24.0&      22.9&      22.1&      20.8&      19.9&     19.70&    -99.00&    -99.00&      1.22$^a $&     -3.00&    1\\
    19&   188.910&    62.279&      20.6&      20.3&      20.2&      20.0&      19.6&      19.7&      19.1&      19.0&     18.73&    -99.00&    -99.00&      0.71$^a $&     -3.00&    4\\
    20&   188.913&    62.267&      23.7&      23.3&      23.2&      23.3&      23.3&      23.3&      22.4&      22.9&     22.45&    -99.00&    -99.00&      2.57$^a $&     -3.00&    4\\
    21&   188.914&    62.220&     -30.2&      27.3&      28.3&      29.5&      28.0&     -29.2&     -99.0&     -99.0&     24.13&     22.81&    -99.00&      0.00$^a $&    -99.00&  -99\\
    22&   188.919&    62.249&      24.3&      23.1&      22.0&      21.2&      20.8&      20.6&      19.8&      19.5&     19.22&    -99.00&    -99.00&      0.32$^a $&     -3.00&    0\\
    23&   188.926&    62.329&      27.6&      26.9&      27.4&      27.5&      25.9&      25.3&      23.2&      22.3&     21.74&    -99.00&    -99.00&      0.00$^a $&      1.05&  -99\\
    24&   188.929&    62.195&      26.6&      26.2&      26.1&      25.8&      25.8&      25.7&     -99.0&     -99.0&     23.73&     23.47&    -99.00&      0.00$^a $&    -99.00&  -99\\
    25&   188.937&    62.293&      26.3&      25.3&      25.4&      25.0&      24.6&      24.6&     -99.0&      22.6&     21.91&    -99.00&    -99.00&      0.00$^a $&      1.95&  -99\\
    26&   188.939&    62.300&      29.2&      27.3&      28.4&      27.1&      25.7&      25.1&     -99.0&     -99.0&     24.03&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    27&   188.941&    62.231&      26.1&      25.5&      25.2&      24.9&      24.8&      24.1&     -99.0&      22.6&     23.01&     22.82&    -99.00&      0.00$^a $&    -99.00&  -99\\
    28&   188.942&    62.267&      27.7&      27.2&      27.0&      27.4&      25.4&      24.7&      22.9&      22.2&     21.78&    -99.00&    -99.00&     -1.00  &      0.85&   -1\\
    29&   188.943&    62.292&      27.1&      27.6&      28.1&      27.3&      26.5&      26.1&     -99.0&     -99.0&     23.81&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    30&   188.948&    62.232&      25.5&      24.9&      24.9&      24.1&      23.6&      23.2&      22.0&      21.4&     20.92&     20.77&     18.29&      0.00$^a $&      1.25&  -99\\
    31&   188.948&    62.254&      26.1&      26.4&      25.7&      25.6&      25.1&      24.7&      22.5&      21.7&     20.86&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
    32&   188.951&    62.284&      23.8&      23.8&      23.9&      23.3&      23.0&      22.7&      21.5&      20.9&     20.46&    -99.00&    -99.00&      1.48  &     -3.00&    4\\
    33&   188.953&    62.255&      24.2&      24.1&      23.6&      23.0&      22.3&      22.1&      21.2&      20.9&     20.51&     21.06&     18.48&      0.89$^a $&     -3.00&    1\\
    34&   188.952&    62.325&      28.2&      26.2&      25.6&      25.0&      24.8&      24.7&     -99.0&      23.6&     22.69&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    35&   188.956&    62.260&      24.6&      23.9&      23.6&      23.3&      23.1&      22.9&      21.8&      21.3&     20.45&    -99.00&    -99.00&      2.20  &     -3.00&    1\\
    36&   188.960&    62.302&      26.3&      26.1&      26.0&      25.5&      25.1&      24.6&      22.8&      22.0&     21.56&    -99.00&    -99.00&      0.00  &      0.85&  -99\\
    37&   188.961&    62.248&      27.5&      27.1&      26.2&      25.9&      25.5&      24.8&      22.2&     -99.0&     21.65&     24.21&    -99.00&      0.00$^a $&      0.85&  -99\\
    38&   188.966&    62.299&      26.5&      26.6&      27.1&      26.7&      26.7&      25.6&      23.6&      22.4&     22.23&    -99.00&    -99.00&      0.00  &      0.85&  -99\\
    39&   188.966&    62.348&      27.8&      26.8&      25.8&      25.2&      24.9&      25.0&     -99.0&     -99.0&     23.14&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    40&   188.971&    62.177&      21.6&      21.9&      21.9&      21.4&      21.4&      21.3&      20.6&      19.9&     19.73&     19.23&     17.49&      1.38$^a $&     -3.00&    4\\
    41&   188.974&    62.365&       0.0&      -0.1&       0.0&       0.2&       0.5&       0.0&     -99.0&     -99.0&    -99.00&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
    42&   188.975&    62.337&     -28.7&     -28.0&      27.2&      26.7&      26.1&      25.1&     -99.0&     -99.0&     22.46&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
    43&   188.979&    62.270&      26.9&      25.7&      25.4&      24.3&      23.4&      22.9&      22.0&      21.4&    -99.00&    -99.00&    -99.00&      1.02$^a $&     -3.00&    1\\
    44&   188.980&    62.150&      24.4&      24.2&      24.1&      23.8&      23.5&      23.2&      21.9&      21.2&     20.84&     19.98&     17.47&      1.88$^c $&     -3.00&   10\\
    45&   188.980&    62.300&      24.2&      22.3&      21.1&      20.0&      18.5&      17.8&      17.1&      17.0&     17.28&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
    46&   188.980&    62.251&      21.2&      20.7&      20.2&      19.8&      19.6&      19.6&      18.5&      18.3&     18.13&     19.52&     17.42&      0.21$^a $&     -3.00&    1\\
    47&   188.984&    62.265&      25.0&      23.8&      22.7&      21.6&      21.1&      20.8&      20.0&      19.8&     19.46&     19.82&     18.92&      0.44$^a $&     -3.00&    1\\
    48&   188.984&    62.205&      25.8&      25.7&      24.9&      23.9&      22.7&      22.1&      21.1&      20.5&     19.85&     19.46&     17.32&      0.96  &     -3.00&    0\\
    49&   188.984&    62.272&      22.5&      21.1&      19.8&      18.9&      18.5&      18.3&      17.0&      16.7&     16.30&    -99.00&    -99.00&      0.30$^a $&     -3.00&    0\\
    50&   188.984&    62.134&      26.0&      25.4&      25.3&      24.3&      23.5&      22.8&      21.7&      21.3&     20.92&    -99.00&    -99.00&      1.15$^a $&     -3.00&    1\\
    51&   188.989&    62.254&      25.2&      24.3&      24.2&      24.1&      24.0&      23.7&      23.0&      22.3&     21.96&     21.56&    -99.00&      2.42$^a $&     -3.00&    3\\
    52&   188.990&    62.173&      24.1&      23.1&      22.7&      22.5&      22.4&      22.5&      22.2&      22.0&     21.86&     21.35&     18.81&      3.07$^a $&     -3.00&    4\\
    53&   188.991&    62.220&      25.8&      25.6&      25.7&      25.4&      25.2&      24.8&     -99.0&     -99.0&     23.64&     23.21&    -99.00&      0.00$^a $&    -99.00&  -99\\
    54&   188.991&    62.353&      24.4&      24.3&      23.9&      23.1&      22.7&      22.1&      21.4&      20.9&     20.62&    -99.00&    -99.00&     -1.00  &      0.85&   -1\\
    55&   188.994&    62.184&      23.2&      22.8&      22.4&      21.4&      20.8&      20.6&      19.8&      19.5&     19.09&     19.31&     18.68&      0.64$^a $&     -3.00&    0\\
    56&   188.995&    62.262&      21.7&      21.1&      20.8&      20.5&      20.3&      20.3&      19.9&      19.7&     19.62&     20.80&     19.09&      0.11$^a $&     -3.00&    1\\
    57&   188.999&    62.264&      21.3&      21.0&      20.3&      19.7&      19.5&      19.2&      18.3&      18.0&     17.60&     18.56&     15.98&      0.38$^a $&     -3.00&    1\\
    58&   189.000&    62.304&      24.6&      24.5&      24.5&      23.9&      23.1&      22.5&      21.6&      21.1&     20.82&    -99.00&    -99.00&      1.14$^a $&     -3.00&    1\\
    59&   189.002&    62.324&      24.5&      24.2&      23.7&      23.6&      23.5&      23.7&      23.7&      22.6&     22.52&    -99.00&    -99.00&      3.19$^a $&     -3.00&    4\\
    60&   189.006&    62.243&      25.7&      24.8&      24.0&      23.0&      22.5&      22.3&      21.7&      21.5&     21.26&     21.51&    -99.00&      0.53$^a $&     -3.00&    0\\
    61&   189.006&    62.235&      24.3&      23.9&      23.9&      23.6&      23.4&      23.3&      22.2&      21.9&     21.67&     21.19&    -99.00&      0.00$^a $&    -99.00&  -99\\
    62&   189.009&    62.264&      20.9&      19.7&      18.9&       0.2&      18.0&      17.7&      16.8&      16.6&     16.49&     17.66&     18.29&      0.09$^a $&     -3.00&    0\\
    63&   189.010&    62.346&      25.0&      24.7&      24.0&      23.2&      22.2&      21.8&      21.0&      20.5&     20.19&    -99.00&    -99.00&      0.80$^a $&     -3.00&    1\\
    64&   189.010&    62.401&      24.3&      23.9&      23.6&      23.5&      23.1&      23.2&      23.1&      22.1&     21.96&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
    65&   189.011&    62.191&      26.8&      25.5&      25.2&      24.7&      26.3&      23.5&      22.5&      22.1&     21.59&     21.23&    -99.00&     -1.00  &      1.05&   -1\\
    66&   189.013&    62.392&      22.8&      21.9&      20.9&      20.1&      19.6&      19.4&      18.5&      18.1&     17.87&    -99.00&    -99.00&      0.33$^a $&     -3.00&    1\\
    67&   189.014&    62.186&      22.8&      22.3&      21.8&      20.8&      20.3&      20.1&      19.5&      19.0&     18.66&     18.61&     16.19&      0.64$^a $&     -3.00&    1\\
    68&   189.020&    62.337&      22.4&      20.7&      19.6&       0.2&      17.9&      16.9&      16.3&      16.1&     16.32&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
    69&   189.022&    62.326&      24.0&      23.3&      22.6&      21.5&      21.0&      20.7&      20.1&      19.6&     19.29&    -99.00&    -99.00&      0.52$^a $&     -3.00&    1\\
    70&   189.023&    62.336&      24.3&      24.2&      24.1&      23.8&      23.5&      23.0&     -99.0&     -99.0&     20.01&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
    71&   189.023&    62.115&      28.2&      27.3&      26.8&      26.0&      25.6&      24.5&     -99.0&      23.0&     22.41&    -99.00&    -99.00&      0.00$^a $&      1.05&  -99\\
    72&   189.024&    62.168&      24.6&      24.3&      23.8&      23.1&      22.3&      21.9&      20.8&      20.5&     20.03&     19.77&     17.08&      0.94$^a $&     -3.00&    1\\
    73&   189.024&    62.144&     -27.8&     -28.4&      26.8&      26.6&      26.1&      25.5&     -99.0&     -99.0&     22.81&     22.17&    -99.00&      0.00$^a $&      1.75&  -99\\
    74&   189.024&    62.197&      24.8&      23.7&      23.7&      23.2&      23.2&      22.5&      21.7&      21.0&     20.65&     19.88&     18.34&      1.48  &     -3.00&    3\\
    75&   189.026&    62.209&      27.8&      27.4&      26.9&      26.0&      25.5&      25.1&      23.4&      22.5&     21.84&     21.08&     18.67&      0.00$^a $&      0.95&  -99\\
    76&   189.028&    62.164&      25.5&      24.8&      23.8&      22.5&      21.8&      21.4&      20.5&      19.6&     18.99&     18.93&     17.15&      0.64$^a $&     -3.00&    1\\
    77&   189.028&    62.264&      23.8&      23.3&      23.3&      23.2&      23.1&      23.1&      23.4&      23.0&     21.93&     21.52&     18.71&      2.42$^a $&     -3.00&    3\\
    78&   189.028&    62.206&      26.8&      25.8&      25.0&      24.0&      23.1&      22.8&      21.9&      21.5&     21.10&     21.15&    -99.00&      0.75$^a $&     -3.00&    1\\
    79&   189.029&    62.173&      26.2&      25.2&      25.1&      24.4&      24.3&      23.9&      22.1&      21.2&     20.90&     20.47&    -99.00&      2.50$^b $&     -3.00&   10\\
    80&   189.032&    62.251&      25.0&      24.6&      24.5&      24.2&      23.7&      23.5&      21.9&      21.4&     21.18&     20.83&    -99.00&      1.68$^a $&     -3.00&    3\\
    81&   189.033&    62.147&      24.6&      22.9&      21.8&      20.6&      20.2&      19.9&      19.1&      18.7&     18.40&     19.89&    -99.00&      0.41$^a $&     -3.00&    0\\
    82&   189.034&    62.177&      24.2&      23.7&      22.9&      21.8&      20.9&      20.8&      20.1&      19.7&     19.40&     19.29&     15.50&      0.68$^a $&     -3.00&    3\\
    83&   189.033&    62.265&      23.5&      23.2&      22.6&      21.9&      21.6&      21.5&      20.9&      20.6&     20.20&     21.33&     18.66&      0.46$^a $&     -3.00&    1\\
    84&   189.036&    62.243&      27.7&      26.7&      26.9&      26.1&      26.8&      25.2&     -99.0&     -99.0&     23.08&     22.17&    -99.00&      0.00$^a $&    -99.00&  -99\\
    85&   189.037&    62.306&      27.1&      26.6&      27.3&      26.8&      26.3&      25.4&     -99.0&      23.3&     22.36&    -99.00&    -99.00&      0.00$^a $&      0.55&  -99\\
    86&   189.040&    62.278&      23.7&      23.6&      23.6&      23.4&      23.2&      22.8&      22.4&      22.0&     21.97&     22.04&    -99.00&      1.34$^a $&     -3.00&    1\\
    87&   189.041&    62.196&      21.8&      20.8&      20.0&      19.5&      19.2&      19.0&      17.9&      17.7&     17.70&     19.11&    -99.00&      0.14$^a $&     -3.00&    0\\
    88&   189.044&    62.336&      27.9&      26.2&      26.0&      25.6&      25.7&      25.4&     -99.0&     -99.0&    -99.00&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
    89&   189.046&    62.375&      22.3&      22.3&      22.1&      21.8&      21.1&      20.8&      19.8&      19.6&     19.41&    -99.00&    -99.00&      0.98$^a $&     -3.00&    3\\
    90&   189.047&    62.151&      24.5&      24.6&      24.5&      23.7&      23.1&      22.5&      21.4&      20.8&     20.45&     20.00&     16.97&      1.14$^a $&     -3.00&    3\\
    91&   189.047&    62.364&      28.1&      26.3&      25.9&      25.3&      24.8&      24.3&      22.6&      22.0&     21.72&    -99.00&    -99.00&      0.00$^a $&      1.05&  -99\\
    92&   189.049&    62.171&      26.8&      26.4&      26.6&      26.0&      25.1&      25.0&      23.0&      22.1&     21.69&     20.68&     18.43&      0.00$^a $&      0.95&  -99\\
    93&   189.050&    62.194&      21.8&      21.2&      20.4&      19.7&      19.4&      19.2&      18.4&      18.1&     17.76&     18.66&     18.10&      0.28$^a $&     -3.00&    4\\
    94&   189.050&    62.150&      25.9&      25.6&      25.6&      24.9&      24.4&      23.8&      23.2&      22.0&     21.51&     21.23&    -99.00&      1.14  &     -3.00&    3\\
    95&   189.050&    62.328&      21.1&      20.9&      21.1&      21.1&      20.9&      20.7&      21.0&      20.5&     20.10&    -99.00&    -99.00&      2.22$^a $&     -3.00&    4\\
    96&   189.051&    62.349&      24.8&      24.8&      24.6&      23.9&      23.1&      22.3&      21.5&      21.1&     20.94&    -99.00&    -99.00&      1.19$^a $&     -3.00&    0\\
    97&   189.054&    62.325&      26.3&      24.6&      23.7&      23.0&      22.9&      23.0&      23.5&      23.4&     22.64&    -99.00&    -99.00&      3.94$^a $&     -3.00&    4\\
    98&   189.054&    62.206&      25.5&      25.5&      25.8&      25.8&      25.7&      25.6&      23.7&      23.0&     23.24&     22.38&    -99.00&      0.00$^a $&      2.05&  -99\\
    99&   189.057&    62.133&      27.1&      26.1&      26.7&      26.0&      25.9&      25.2&      22.9&      22.4&     22.09&     21.74&    -99.00&     -1.00  &      0.75&   -1\\
   100&   189.059&    62.172&     -28.8&      29.2&      28.5&      29.1&     -27.0&     -27.1&     -99.0&     -99.0&     24.06&     23.54&    -99.00&      0.00$^a $&    -99.00&  -99\\
   101&   189.060&    62.222&      23.2&      22.5&      21.8&      20.9&      20.4&      20.2&      19.4&      19.0&     18.71&     19.32&     18.39&      0.45$^a $&     -3.00&    1\\
   102&   189.060&    62.179&      25.6&      25.4&      25.6&      25.1&      25.0&      24.7&      23.3&      22.5&     22.17&     21.65&    -99.00&      0.00$^a $&      1.85&  -99\\
   103&   189.060&    62.122&      23.9&      23.7&      23.2&      22.5&      21.9&      21.5&      20.7&      20.4&     19.88&     19.73&     17.40&      0.97$^a $&     -3.00&    1\\
   104&   189.063&    62.174&      24.8&      23.1&      22.2&      21.2&      19.7&      19.2&      18.6&      18.6&     18.82&     20.64&    -99.00&     -2.00  &    -99.00&   -2\\
   105&   189.064&    62.206&      24.8&      23.3&      22.2&      21.3&      20.9&      20.7&      20.1&      19.8&     19.52&     20.57&    -99.00&      0.32$^a $&     -3.00&    0\\
   106&   189.064&    62.193&      25.2&      24.9&      24.5&      23.6&      22.7&      22.1&      21.2&      20.8&     20.40&     20.01&     18.56&      1.02$^a $&     -3.00&    3\\
   107&   189.066&    62.254&      28.5&      28.8&      26.6&      27.2&      26.3&      25.7&     -99.0&      22.6&     22.00&     21.15&    -99.00&     -1.00  &      1.15&   -1\\
   108&   189.067&    62.186&      27.8&      26.2&      26.4&      25.7&      24.9&      24.3&      22.7&      22.3&     21.62&     20.90&     18.31&      0.00$^a $&      0.85&  -99\\
   109&   189.067&    62.254&      27.8&      26.6&      26.1&      25.3&      25.1&      25.0&     -99.0&      22.7&     22.55&     21.31&     17.66&      2.58$^c $&     -3.00&   10\\
   110&   189.070&    62.104&      25.7&      25.0&      24.6&      23.4&      22.4&      21.5&      20.5&      20.1&     19.77&     19.65&     19.12&      1.14$^a $&     -3.00&    0\\
   111&   189.070&    62.244&      23.4&      23.1&      22.5&      21.6&      21.0&      20.7&      19.9&      19.4&     18.90&     19.75&    -99.00&      0.52$^a $&     -3.00&    1\\
   112&   189.071&    62.357&      26.6&      26.5&      25.6&      24.5&      24.5&      24.0&     -99.0&     -99.0&    -99.00&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
   113&   189.071&    62.170&      24.4&      24.1&      23.9&      22.9&      22.1&      21.6&      20.7&      20.3&     19.72&     19.81&     19.04&      0.84$^a $&     -3.00&    1\\
   114&   189.074&    62.229&      25.7&      24.1&      23.0&      21.7&      21.0&      20.7&      20.0&      19.6&     19.23&     19.58&    -99.00&      0.53$^a $&     -3.00&    0\\
   115&   189.075&    62.276&      22.6&      22.2&      21.8&      21.2&      20.6&      20.5&      19.6&      19.2&     18.96&     19.14&     16.84&      0.68$^a $&     -3.00&    3\\
   116&   189.078&    62.188&      21.8&      21.8&      21.8&      21.5&      21.3&      21.0&      20.2&      19.7&     19.16&     19.11&     17.41&      1.02$^a $&     -3.00&    4\\
   117&   189.080&    62.245&      26.9&      27.5&      25.9&      25.5&      25.0&      25.1&     -99.0&      22.4&     21.77&     21.84&    -99.00&      0.00$^a $&      1.25&  -99\\
   118&   189.080&    62.406&      26.3&      25.8&      25.6&      24.9&      24.5&      24.1&      22.9&      22.2&     21.60&    -99.00&    -99.00&     -1.00  &      1.25&   -1\\
   119&   189.081&    62.215&      23.5&      22.7&      21.9&      20.9&      20.4&      20.2&      19.3&     -99.0&     18.56&     18.95&     16.43&      0.47$^a $&     -3.00&    3\\
   120&   189.083&    62.214&      21.9&      21.7&      21.6&      20.9&      20.7&      20.7&      20.4&     -99.0&     20.01&     19.77&    -99.00&      0.69$^a $&     -3.00&    3\\
   121&   189.082&    62.319&      23.9&      23.2&      22.3&      21.3&      20.8&      20.4&      19.3&      18.7&     18.27&    -99.00&    -99.00&      0.00  &      0.65&  -99\\
   122&   189.086&    62.211&      27.3&      26.7&      26.5&      25.7&      25.2&      24.1&      23.5&      22.4&     21.51&     20.77&    -99.00&      1.34$^a $&     -3.00&    1\\
   123&   189.087&    62.238&      25.4&      25.2&      25.0&      24.6&      24.3&      23.9&      22.7&      21.9&     21.44&     21.48&     18.61&      0.00$^a $&    -99.00&  -99\\
   124&   189.087&    62.237&      26.0&      25.3&      25.0&      24.5&      24.1&      23.8&      22.1&      21.8&     21.66&     22.55&    -99.00&      0.00$^a $&    -99.00&  -99\\
   125&   189.088&    62.218&      26.2&      26.3&      26.0&      25.5&      25.2&      24.3&     -99.0&     -99.0&     22.74&     23.02&     18.27&      0.00$^a $&    -99.00&  -99\\
   126&   189.088&    62.202&      24.6&      24.0&      23.5&      22.7&      22.0&      21.6&      20.8&      20.4&     19.90&     19.89&     17.93&      0.78$^a $&     -3.00&    1\\
   127&   189.089&    62.186&      25.8&      25.6&      25.2&      23.9&      22.8&      22.2&      21.0&      20.3&     19.78&     19.17&     18.01&      1.01$^a $&     -3.00&    1\\
   128&   189.090&    62.131&      27.2&      25.9&      25.7&      25.6&      25.6&      25.5&     -99.0&     -99.0&     23.69&     24.56&    -99.00&      0.00$^a $&    -99.00&  -99\\
   129&   189.091&    62.268&      27.4&      27.1&      26.8&      27.0&      26.8&      25.9&     -99.0&      23.6&     22.38&     21.48&     18.75&     -1.00  &    -99.00&   -1\\
   130&   189.092&    62.238&      24.1&      23.8&      23.8&      23.3&      23.0&      22.4&      21.6&      21.2&     20.78&     21.21&     18.92&      1.38$^a $&     -3.00&    1\\
   131&   189.094&    62.211&      26.2&      25.2&      24.2&      23.1&      22.5&      22.2&     -99.0&     -99.0&     20.74&     20.52&     19.06&      0.63$^a $&     -3.00&    0\\
   132&   189.094&    62.262&      22.7&      22.3&      21.9&      21.1&      20.7&      20.5&      19.8&      19.5&     19.09&     19.71&     16.76&      0.64$^a $&     -3.00&    1\\
   133&   189.094&    62.218&      27.1&      25.5&      25.2&      25.0&      24.7&      24.9&     -99.0&      22.8&     22.70&     22.66&    -99.00&      2.98  &     -3.00&    1\\
   134&   189.095&    62.175&      29.6&      26.1&      25.7&      25.3&      25.3&      25.0&      23.4&      22.7&     22.33&     21.86&     18.85&      0.00$^a $&      0.55&  -99\\
   135&   189.094&    62.275&      25.6&      25.2&      25.1&      24.8&      24.5&      24.2&      22.8&      22.4&     21.91&     20.80&     17.36&      2.47$^b $&     -3.00&   10\\
   136&   189.095&    62.217&      24.2&      23.0&      22.1&      21.0&      20.6&      20.4&      19.8&      19.4&     19.13&     19.52&    -99.00&      0.47$^a $&     -3.00&    0\\
   137&   189.096&    62.257&      20.9&      20.4&      20.4&      20.5&      20.5&      20.3&      20.2&      20.1&     20.12&     19.89&     17.09&      2.59$^a $&     -3.00&    4\\
   138&   189.096&    62.230&      23.1&      22.6&      22.1&      21.3&      21.0&      20.8&      20.2&      19.9&     19.51&     19.96&     17.79&      0.48$^a $&     -3.00&    1\\
   139&   189.098&    62.310&      25.3&      25.0&      24.3&      23.3&      22.3&      21.7&      20.8&      20.0&     19.51&     19.46&     19.03&      1.01$^a $&     -3.00&    0\\
   140&   189.099&    62.169&      29.8&     -28.2&      27.7&      27.5&      26.5&      25.8&     -99.0&     -99.0&     22.78&     22.14&     18.65&      0.00$^a $&      1.15&  -99\\
   141&   189.100&    62.383&      26.1&      25.2&      23.9&      22.8&      21.8&      21.4&      20.6&      20.1&     19.71&    -99.00&    -99.00&      0.75$^a $&     -3.00&    0\\
   142&   189.102&    62.187&      25.6&      24.9&      23.9&      22.9&      21.9&      21.5&      20.7&      20.3&     19.93&     19.95&    -99.00&      0.75$^a $&     -3.00&    0\\
   143&   189.103&    62.295&      25.6&      25.1&      25.1&      24.5&      24.0&      23.7&      23.0&      22.1&     21.51&     20.70&     18.07&     -1.00  &      0.55&   -1\\
   144&   189.103&    62.318&      27.2&      27.6&      28.7&      26.7&      27.1&      25.3&     -99.0&      22.8&     22.96&     21.93&    -99.00&     -1.00  &      1.65&   -1\\
   145&   189.104&    62.354&      15.5&      22.0&      18.7&      20.6&      16.5&      15.0&      13.5&      13.1&     13.23&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
   146&   189.106&    62.294&      31.0&      27.0&      26.2&      25.8&      24.9&      24.4&      22.6&      21.8&     21.17&     20.68&    -99.00&      0.00$^a $&      0.95&  -99\\
   147&   189.106&    62.235&      22.2&      20.2&      19.1&       0.2&      17.7&      16.8&      16.1&      15.9&     16.09&     16.71&    -99.00&     -2.00  &    -99.00&   -2\\
   148&   189.109&    62.100&      27.1&      26.4&      26.5&      25.8&      24.8&      24.0&     -99.0&     -99.0&    -99.00&     21.14&    -99.00&      0.00$^a $&    -99.00&  -99\\
   149&   189.114&    62.216&      23.8&      23.6&      23.4&      22.9&      22.5&      22.1&      21.5&      21.1&     20.75&     20.45&     18.55&      1.22$^a $&     -3.00&    1\\
   150&   189.115&    62.174&      26.3&      25.7&      24.9&      23.9&      23.1&      22.8&      22.0&      21.6&     21.22&     21.06&    -99.00&      0.76$^a $&     -3.00&    1\\
   151&   189.115&    62.205&      27.7&      28.7&      27.1&     -27.7&     -29.5&      28.0&     -99.0&     -99.0&    -99.00&     23.76&    -99.00&      0.00$^a $&    -99.00&  -99\\
   152&   189.115&    62.200&      26.6&      25.7&      24.9&      24.2&      24.0&      23.7&      23.1&      22.7&     22.23&     22.21&     18.84&      0.00$^a $&      0.55&  -99\\
   153&   189.116&    62.071&      26.6&      25.9&      24.8&      23.7&      23.1&      22.8&     -99.0&      18.7&     18.35&    -99.00&    -99.00&      0.57  &     -3.00&    0\\
   154&   189.119&    62.361&      27.1&      25.9&      26.0&      25.2&      24.5&      24.1&      22.0&      21.2&     20.39&    -99.00&    -99.00&      1.19  &     -3.00&    1\\
   155&   189.120&    62.135&      27.4&      26.7&      26.5&      25.6&      25.5&      25.1&      22.9&      21.8&     21.42&     20.88&    -99.00&      0.00$^a $&      1.15&  -99\\
   156&   189.120&    62.194&      29.0&     -29.3&      28.5&     -30.6&      29.4&     -27.7&     -99.0&     -99.0&     23.53&     22.88&    -99.00&     -1.00  &    -99.00&   -1\\
   157&   189.121&    62.104&      23.3&      23.1&      23.0&      22.4&      22.0&      21.4&      20.5&      20.1&     19.63&     19.24&     17.59&      1.26$^a $&     -3.00&    1\\
   158&   189.122&    62.180&      26.1&      25.7&      25.0&      24.0&      22.9&      22.4&      21.1&      20.5&     19.61&     19.10&     16.75&      1.01$^a $&     -3.00&    1\\
   159&   189.122&    62.399&      24.9&      24.7&      24.4&      24.0&      23.8&      23.6&     -99.0&     -99.0&     22.30&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
   160&   189.122&    62.270&      23.9&      23.7&      23.1&      22.2&      21.2&      20.8&      20.0&      19.6&     18.68&     19.52&     18.10&      0.85$^a $&     -3.00&    1\\
   161&   189.123&    62.254&      32.8&      25.3&      24.5&      23.9&      23.6&      23.3&      23.1&      22.3&     22.12&     22.04&    -99.00&      3.65$^a $&     -3.00&    4\\
   162&   189.123&    62.371&      23.6&      23.1&      22.7&      22.3&      21.7&      21.3&      20.6&      20.2&     19.65&    -99.00&    -99.00&      0.85$^a $&     -3.00&    4\\
   163&   189.125&    62.095&      23.1&      22.5&      21.8&      21.0&      20.5&      20.3&      19.7&      19.2&     18.95&     19.21&     15.42&      0.48$^a $&     -3.00&    3\\
   164&   189.125&    62.157&      26.1&      25.4&      24.9&      24.1&      22.9&      22.4&      21.6&      21.4&     21.06&     20.44&     18.03&      0.95$^a $&     -3.00&    1\\
   165&   189.126&    62.439&      24.5&      24.2&      24.2&      23.9&      23.3&      22.9&      21.4&      20.6&     20.27&    -99.00&    -99.00&     -1.00  &      0.95&   -1\\
   166&   189.130&    62.210&      23.2&      23.0&      22.5&      22.0&      21.9&      21.6&      21.3&      21.1&     20.90&     21.75&    -99.00&      0.46$^a $&     -3.00&    1\\
   167&   189.130&    62.166&      27.1&      27.1&      26.3&      26.2&      25.5&      25.3&      23.5&      22.7&     21.95&     21.62&     18.15&      0.00$^a $&      1.05&  -99\\
   168&   189.131&    62.348&      27.4&      26.9&      26.8&      25.6&      24.3&      23.6&      21.9&      21.2&     20.86&    -99.00&    -99.00&      0.00$^a $&      0.85&  -99\\
   169&   189.132&    62.152&      22.1&      21.7&      21.0&      20.5&      20.3&      20.0&      18.3&      17.9&     17.48&     18.31&     17.79&      0.84$^a $&     -3.00&    0\\
   170&   189.133&    62.296&      25.5&      24.6&      23.8&      22.7&      22.0&      21.7&      21.0&      20.4&     19.86&     19.82&     17.73&      0.68$^a $&     -3.00&    0\\
   171&   189.136&    62.133&      23.3&      23.8&      23.9&      23.7&      23.2&      23.0&      22.4&     -99.0&    -99.00&     21.28&     16.62&      2.00$^a $&     -3.00&    3\\
   172&   189.136&    62.341&      21.5&      19.5&      18.3&       0.2&      17.8&      16.9&      15.8&      15.5&     15.75&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
   173&   189.138&    62.193&      22.5&      21.9&      21.7&      21.5&      21.5&      21.4&      21.1&      20.9&     20.52&     21.09&     18.73&      0.08$^a $&     -3.00&    3\\
   174&   189.138&    62.143&      22.4&      22.5&      22.3&      22.0&      21.5&      21.1&      20.3&      20.0&     19.36&     19.02&     16.68&      0.93$^a $&     -3.00&    3\\
   175&   189.140&    62.341&      22.9&      22.8&      22.4&      21.8&      21.4&      21.0&     -99.0&     -99.0&     19.49&    -99.00&    -99.00&      1.01$^a $&     -3.00&    1\\
   176&   189.140&    62.238&      27.8&      25.8&      25.4&      25.2&      25.4&      25.7&     -99.0&     -99.0&     23.15&     22.73&    -99.00&      3.40$^a $&     -3.00&    3\\
   177&   189.140&    62.168&      23.9&      23.9&      23.4&      22.8&      22.1&      21.7&      20.7&      20.4&     19.68&     19.30&     16.99&      1.02$^a $&     -3.00&    1\\
   178&   189.141&    62.220&      28.6&      26.6&      26.1&      25.7&      25.4&      25.6&     -99.0&      22.8&     22.61&    -24.65&    -99.00&      0.00$^a $&    -99.00&  -99\\
   179&   189.141&    62.135&      19.8&      18.4&      18.3&      17.7&      16.8&      15.4&      14.4&      14.2&     14.30&     15.02&     17.88&     -2.00  &    -99.00&   -2\\
   180&   189.144&    62.204&      22.6&      21.9&      20.9&      20.0&      19.6&      19.3&      18.2&      17.8&     17.39&     17.92&     16.12&      0.46$^a $&     -3.00&    3\\
   181&   189.144&    62.162&      26.9&      27.4&      26.7&      26.9&      25.6&      25.3&     -99.0&     -99.0&     23.48&     22.72&    -99.00&      0.00$^a $&    -99.00&  -99\\
   182&   189.144&    62.211&      24.3&      24.1&      24.0&      23.4&      22.8&      22.2&      21.5&      21.0&     20.25&     19.48&     17.28&      1.22$^a $&     -3.00&    1\\
   183&   189.144&    62.104&      28.7&      31.1&     -31.0&      28.9&      26.7&      26.3&     -99.0&     -99.0&    -99.00&     24.74&    -99.00&      0.00$^a $&    -99.00&  -99\\
   184&   189.144&    62.324&      24.7&      24.5&      23.8&      22.8&      21.9&      21.3&      20.5&      19.7&     19.26&     19.40&     17.81&      0.87$^a $&     -3.00&    1\\
   185&   189.145&    62.239&      25.9&      25.5&      25.4&      25.2&      24.8&      24.7&     -99.0&      23.6&     22.43&     22.28&     18.96&      0.00$^a $&    -99.00&  -99\\
   186&   189.145&    62.077&     -29.4&      26.4&      26.2&      25.9&      25.4&      24.8&     -99.0&      23.1&     22.00&     21.55&    -99.00&      0.00$^a $&      1.25&  -99\\
   187&   189.145&    62.275&      25.2&      24.9&      24.3&      23.4&      22.5&      22.2&      21.1&      20.6&     20.04&     19.63&     17.19&      0.85$^a $&     -3.00&    0\\
   188&   189.147&    62.198&      26.9&      27.0&      26.1&      25.5&      24.6&      24.0&      23.1&      22.4&     21.90&     21.48&    -99.00&      1.22  &     -3.00&    1\\
   189&   189.147&    62.186&      25.4&      23.6&      22.5&      21.4&      20.9&      20.7&      20.0&      19.7&     19.38&     20.09&    -99.00&      0.41$^a $&     -3.00&    0\\
   190&   189.148&    62.240&      24.0&      24.0&      24.0&      23.8&      23.4&      23.1&      21.6&      21.0&     20.40&     19.56&     15.97&      2.00$^a $&     -3.00&    3\\
   191&   189.149&    62.118&      25.4&      25.5&      25.2&      24.4&      23.9&      23.6&      20.8&      20.2&     19.41&     19.06&     17.33&      0.00  &      0.85&  -99\\
   192&   189.151&    62.222&      23.7&      23.6&      23.5&      22.8&      22.6&      22.5&      22.1&      22.0&     21.90&     22.05&    -99.00&      0.68$^a $&     -3.00&    1\\
   193&   189.153&    62.230&      22.4&      22.3&      22.0&      21.6&      21.3&      21.1&      20.2&      20.2&     19.68&     19.75&     17.21&      0.96$^a $&     -3.00&    3\\
   194&   189.153&    62.199&      24.3&      23.4&      23.1&      22.4&      21.9&      21.6&      21.0&      20.6&     20.43&     20.82&    -99.00&      0.56$^a $&     -3.00&    1\\
   195&   189.154&    62.374&      27.9&      28.6&      27.5&      26.6&      26.8&      29.6&      23.5&      22.8&     22.16&    -99.00&    -99.00&      0.00$^a $&      0.55&  -99\\
   196&   189.154&    62.222&      30.0&      27.9&      28.6&      28.3&     -27.7&      27.7&     -99.0&     -99.0&     23.88&     23.30&    -99.00&      0.00$^a $&    -99.00&  -99\\
   197&   189.154&    62.193&      20.4&      19.9&      19.4&      19.2&      19.2&      19.0&      17.8&      17.7&     17.68&     19.85&     16.74&      0.08$^a $&     -3.00&    1\\
   198&   189.155&    62.110&      27.4&      26.4&      26.2&      25.8&      25.4&      25.3&     -99.0&      22.8&     22.68&     21.90&    -99.00&      0.00$^a $&      0.95&  -99\\
   199&   189.156&    62.171&      27.4&      28.2&      27.3&      26.3&      25.4&      24.8&      23.4&      22.4&     21.87&     21.27&    -99.00&      0.00$^a $&      1.05&  -99\\
   200&   189.155&    62.142&      24.2&      24.1&      23.9&      23.3&      22.5&      22.0&      21.1&      20.8&     20.26&     20.31&    -99.00&      0.97$^a $&     -3.00&    1\\
   201&   189.161&    62.228&      24.4&      24.2&      23.6&      23.0&      22.5&      22.1&      21.0&      20.7&     20.07&     19.85&    -99.00&      1.02$^a $&     -3.00&    1\\
   202&   189.161&    62.365&      24.9&      24.6&      24.1&      23.2&      22.5&      22.1&      21.2&      20.7&     20.22&    -99.00&    -99.00&      0.64  &     -3.00&    0\\
   203&   189.162&    62.216&      23.9&      23.8&      23.4&      22.8&      22.3&      21.7&      20.9&      20.5&     19.93&     19.55&     17.93&      1.14$^a $&     -3.00&    1\\
   204&   189.162&    62.178&     -28.7&     -27.3&      29.2&     -27.7&     -27.8&     -27.4&     -99.0&     -99.0&     23.99&     22.68&    -99.00&      0.00$^a $&    -99.00&  -99\\
   205&   189.163&    62.162&      25.3&      25.1&      24.8&      24.0&      23.6&      22.9&      21.8&      21.4&     20.93&     20.38&     18.68&      0.00$^a $&      0.95&  -99\\
   206&   189.165&    62.345&     -28.5&      27.5&      26.3&      24.6&      23.5&      22.8&      21.9&      21.4&     20.69&    -99.00&    -99.00&      0.00$^a $&      1.05&  -99\\
   207&   189.166&    62.208&      24.9&      24.2&      23.9&      23.7&      23.4&      23.3&      23.0&      22.4&     22.47&     22.34&    -99.00&      1.50  &     -3.00&    1\\
   208&   189.165&    62.160&     -29.4&     -29.4&      28.6&      28.0&      27.5&      25.8&     -99.0&      22.5&     22.28&     21.78&    -99.00&     -1.00  &      1.85&   -1\\
   209&   189.166&    62.169&      24.5&      23.8&      23.1&      22.2&      21.7&      21.4&      20.8&      20.4&     20.05&     20.54&     18.84&      0.51$^a $&     -3.00&    0\\
   210&   189.166&    62.263&      27.3&      25.6&      24.1&      22.8&      21.6&      21.1&      19.9&      19.4&     19.03&     19.38&    -99.00&      0.85$^a $&     -3.00&    0\\
   211&   189.166&    62.214&      24.0&      23.6&      22.9&      22.3&      21.5&      21.2&      20.4&      20.2&     19.73&     19.57&     17.17&      0.85$^a $&     -3.00&    1\\
   212&   189.167&    62.282&      25.7&      25.3&      24.3&      23.3&      22.0&      21.6&      21.0&      20.5&     20.31&     20.10&    -99.00&      0.94$^a $&     -3.00&    0\\
   213&   189.167&    62.328&      19.7&      18.2&      16.9&      17.9&      16.5&      14.9&      14.1&      13.7&     13.80&     14.70&     18.22&     -2.00  &    -99.00&   -2\\
   214&   189.169&    62.309&      25.5&      24.9&      24.4&      23.5&      22.4&      21.6&      20.8&      20.4&     19.72&     19.64&     18.42&      1.14$^a $&     -3.00&    0\\
   215&   189.170&    62.180&      26.4&      26.4&      25.6&      24.8&      24.0&      23.6&      22.3&      22.2&     21.54&     21.27&     18.64&      1.01$^a $&     -3.00&    1\\
   216&   189.170&    62.178&      24.3&      24.3&      24.4&      24.2&      24.0&      23.7&      23.1&      23.2&     24.39&     23.07&    -99.00&      1.24  &     -3.00&    3\\
   217&   189.173&    62.163&      24.5&      23.5&      22.5&      21.3&      20.7&      20.3&      19.3&      18.8&     18.35&     18.87&     17.31&      0.52$^a $&     -3.00&    1\\
   218&   189.174&    62.192&      21.4&      20.8&      20.5&      20.3&      20.2&      20.2&      19.7&      19.5&     19.54&     21.15&    -99.00&      0.09$^a $&     -3.00&    1\\
   219&   189.174&    62.162&      26.2&      25.3&      24.3&      23.2&      22.1&      21.7&      20.8&      20.3&     19.63&     19.97&     18.73&      0.84$^a $&     -3.00&    0\\
   220&   189.175&    62.225&      26.8&      27.5&      26.2&      25.8&      25.2&      25.0&     -99.0&      23.2&     22.42&     21.82&     18.06&      0.00$^a $&      1.35&  -99\\
   221&   189.176&    62.411&      24.9&      24.7&      24.7&      24.6&      24.3&      24.1&     -99.0&      22.1&     21.56&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
   222&   189.176&    62.263&      24.7&      24.2&      23.3&      22.5&      21.6&      21.2&      20.3&      19.7&     19.13&     18.88&     16.58&      0.86$^a $&     -3.00&    1\\
   223&   189.176&    62.286&      27.1&      25.7&      25.0&      24.4&      24.3&      24.0&      23.0&      22.0&     21.64&     21.37&     18.84&      0.00$^a $&      0.55&  -99\\
   224&   189.176&    62.104&     -27.7&      27.4&      27.1&      25.8&      25.2&      25.3&     -99.0&     -99.0&     24.46&     23.95&    -99.00&      0.00$^a $&    -99.00&  -99\\
   225&   189.180&    62.186&      25.0&      24.1&      23.5&      23.0&      22.9&      22.8&      22.2&      21.8&     21.51&     21.36&    -99.00&      3.23  &     -3.00&    1\\
   226&   189.183&    62.272&      27.4&      25.7&      25.6&      24.9&      24.8&      24.2&      22.7&      21.4&     20.45&     20.76&    -99.00&      1.01  &     -3.00&    1\\
   227&   189.183&    62.214&      23.5&      22.9&      22.4&      21.5&      21.2&      20.9&      20.4&      19.9&     19.46&     19.87&     17.33&      0.56$^a $&     -3.00&    1\\
   228&   189.184&    62.212&      26.2&      25.9&      25.3&      24.9&      24.3&      23.7&      22.0&      21.4&     20.82&     20.69&    -99.00&     -1.00  &      1.15&   -1\\
   229&   189.185&    62.248&      24.7&      24.5&      24.5&      24.0&      23.7&      23.3&      22.3&      21.8&     21.54&     21.53&     19.12&      1.49$^a $&     -3.00&    1\\
   230&   189.185&    62.193&      26.7&      25.7&      24.3&      22.8&      21.7&      20.9&      19.6&      19.0&     18.54&     18.56&    -99.00&      1.01$^a $&     -3.00&    0\\
   231&   189.186&    62.196&      25.1&      25.3&      25.1&      24.6&      24.4&      24.5&     -99.0&     -99.0&     24.18&    -23.70&    -99.00&      0.56  &     -3.00&    3\\
   232&   189.187&    62.447&      25.6&      25.2&      25.3&      24.9&      24.4&      24.2&     -99.0&     -99.0&     21.76&    -99.00&    -99.00&      0.00  &      1.95&  -99\\
   233&   189.188&    62.052&      22.7&      22.4&      22.3&      22.4&      22.3&      22.1&      21.6&      21.4&     21.19&    -99.00&    -99.00&      2.46$^a $&     -3.00&    4\\
   234&   189.189&    62.317&      23.0&      22.5&      21.8&      21.1&      20.8&      20.5&      20.0&      19.7&     19.40&     19.88&     16.93&      0.46$^a $&     -3.00&    3\\
   235&   189.190&    62.314&      26.2&      25.6&      25.6&      25.4&      25.3&      24.8&     -99.0&      22.3&     21.85&     21.25&     18.51&      0.00$^a $&      0.95&  -99\\
   236&   189.191&    62.246&      25.8&      25.5&      25.6&      25.3&      25.4&      24.8&     -99.0&      22.7&     22.37&     22.33&    -99.00&     -1.00  &      2.05&   -1\\
   237&   189.191&    62.132&      23.6&      23.4&      23.4&      22.9&      22.6&      22.2&      21.3&      20.7&     20.65&     20.08&     17.48&      1.43$^a $&     -3.00&    1\\
   238&   189.192&    62.363&      25.5&      25.1&      24.6&      24.2&      24.0&      23.7&      22.7&      22.1&     21.60&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
   239&   189.192&    62.247&     -29.5&     -29.0&      26.6&      26.2&      26.8&      25.3&     -99.0&      23.1&     22.55&     22.38&     18.36&     -1.00  &    -99.00&   -1\\
   240&   189.193&    62.235&      24.1&      23.6&      22.9&      22.3&      21.5&      21.0&      20.2&      19.8&     19.36&     19.23&     18.09&      0.96$^a $&     -3.00&    1\\
   241&   189.193&    62.258&      26.4&      26.1&      24.7&      23.6&      22.4&      22.0&      21.2&      20.8&     20.38&     20.01&     17.06&      0.85$^a $&     -3.00&    0\\
   242&   189.194&    62.149&      26.5&      26.2&      25.7&      24.6&      23.6&      22.9&     -99.0&      21.4&     20.84&     20.30&    -99.00&      0.00$^a $&      1.05&  -99\\
   243&   189.195&    62.246&      25.4&      25.5&      25.4&      25.1&      25.0&      24.8&      20.2&      19.8&     19.44&     20.89&     17.79&     -1.00  &    -99.00&   -1\\
   244&   189.194&    62.143&      23.3&      23.0&      22.6&      22.1&      21.3&      20.9&      20.0&      19.7&     19.15&     19.09&     16.42&      0.97$^a $&     -3.00&    1\\
   245&   189.196&    62.210&      22.7&      22.4&      21.8&      21.4&      21.1&      21.0&      20.7&      20.5&     20.28&     21.52&    -99.00&      0.32$^a $&     -3.00&    1\\
   246&   189.200&    62.172&      28.2&      26.8&      26.8&      27.2&      28.0&      26.6&     -99.0&      23.4&     22.75&     21.98&    -99.00&      0.00$^a $&      0.95&  -99\\
   247&   189.200&    62.162&      25.6&      25.4&      25.0&      24.4&      23.4&      23.6&      23.3&      23.4&     23.74&    -23.89&    -99.00&      5.19$^a $&     -3.00&    3\\
   248&   189.200&    62.132&      26.1&      25.4&      25.2&      25.2&      25.7&      24.8&     -99.0&     -99.0&    -99.00&    -24.80&    -99.00&      0.00$^a $&    -99.00&  -99\\
   249&   189.200&    62.219&      24.9&      23.5&      22.4&      21.2&      20.7&      20.4&      19.7&      19.4&     19.03&     19.60&    -99.00&      0.47$^a $&     -3.00&    1\\
   250&   189.201&    62.249&      27.8&      27.6&      27.6&      27.7&      26.3&      26.3&     -99.0&     -99.0&     25.40&     26.34&    -99.00&      0.00$^a $&    -99.00&  -99\\
   251&   189.201&    62.241&      20.6&      20.0&      19.7&      19.4&      19.2&      19.2&      18.8&      18.6&     18.44&     19.21&     17.24&      0.14$^a $&     -3.00&    1\\
   252&   189.201&    62.164&      25.8&      25.0&      24.8&      24.6&      24.6&      24.8&     -99.0&     -99.0&     25.59&     29.88&    -99.00&      2.72$^d $&     -3.00&   10\\
   253&   189.204&    62.365&      26.3&      26.1&      26.0&      25.7&      25.8&      24.6&      23.1&      22.2&     21.66&    -99.00&     18.87&      0.00$^a $&      1.15&  -99\\
   254&   189.204&    62.057&      24.5&      24.3&      23.7&      22.9&      21.9&      21.2&      20.3&      19.8&     19.43&    -99.00&    -99.00&      0.97$^a $&     -3.00&    1\\
   255&   189.204&    62.077&      19.8&      18.7&      17.6&      17.7&      17.1&      16.4&      14.9&      14.6&     14.50&    -99.00&     15.93&      0.11$^a $&     -3.00&    0\\
   256&   189.205&    62.313&      23.1&      22.9&      22.6&      21.7&      21.3&      21.2&      20.6&      20.3&     19.98&     20.43&    -99.00&      0.59$^a $&     -3.00&    1\\
   257&   189.206&    62.230&      21.3&      20.2&      19.3&      18.8&      18.4&      18.2&      17.6&      17.4&     17.35&     18.46&    -99.00&      0.09$^a $&     -3.00&    0\\
   258&   189.206&    62.235&      24.0&      23.6&      23.3&      22.6&      21.9&      21.7&      21.0&      20.6&     20.22&     20.18&     18.23&      0.75$^a $&     -3.00&    1\\
   259&   189.207&    62.127&      24.0&      23.8&      23.8&      23.4&      23.2&      22.8&      21.2&      21.2&     21.18&     20.28&     16.00&      1.61$^a $&     -3.00&    3\\
   260&   189.207&    62.220&      24.4&      23.7&      23.0&      22.1&      21.7&      21.5&      20.8&      20.3&     19.85&     20.26&     17.48&      0.47$^a $&     -3.00&    1\\
   261&   189.209&    62.205&      25.7&      25.3&      24.6&      23.6&      22.6&      22.1&      21.2&      20.8&     20.43&     20.09&    -99.00&      0.90$^a $&     -3.00&    0\\
   262&   189.210&    62.335&      27.6&      26.5&      25.3&      24.3&      23.2&      22.6&      21.7&      21.2&     20.87&     20.65&    -99.00&      1.01$^a $&     -3.00&    1\\
   263&   189.210&    62.362&      23.0&      22.9&      22.4&      21.6&      21.2&      20.9&      20.3&      19.9&     19.64&    -99.00&     18.96&      0.48$^a $&     -3.00&    1\\
   264&   189.213&    62.292&      23.7&      23.4&      22.8&      22.4&      22.2&      22.0&      21.7&      21.6&     21.35&     21.92&    -99.00&      0.32$^a $&     -3.00&    1\\
   265&   189.213&    62.175&      23.6&      22.8&      21.8&      21.0&      20.6&      20.2&      19.4&      19.0&     18.57&     19.01&     16.42&      0.41$^a $&     -3.00&    1\\
   266&   189.214&    62.181&     -29.2&      26.2&      26.1&      24.9&      23.9&      23.0&      22.0&      21.4&     20.98&     20.33&    -99.00&      0.00$^a $&      0.95&  -99\\
   267&   189.216&    62.206&      24.2&      23.5&      22.6&      22.0&      21.7&      21.4&      20.8&      20.5&     20.13&     21.36&     18.65&      0.30  &     -3.00&    1\\
   268&   189.216&    62.251&      26.6&      25.8&      25.5&      25.4&      25.0&      24.8&     -99.0&      23.0&     22.25&     21.92&     18.84&      0.00$^a $&      2.05&  -99\\
   269&   189.217&    62.249&      23.4&      23.3&      22.7&      22.2&      22.2&      22.0&      21.8&      21.5&     21.25&     21.78&    -99.00&      0.36$^a $&     -3.00&    1\\
   270&   189.218&    62.469&      20.4&      -0.1&      19.7&      19.2&      18.7&      18.4&      17.4&      17.0&     16.89&    -99.00&    -99.00&      0.33$^a $&     -3.00&    4\\
   271&   189.220&    62.056&      26.1&      25.6&      25.2&      24.8&      24.5&      23.8&      22.1&      21.4&     20.75&    -99.00&    -99.00&      0.00$^a $&      0.85&  -99\\
   272&   189.220&    62.232&      22.6&      22.5&      22.5&      22.3&      22.3&      21.9&      21.6&      21.2&     21.27&     21.28&     18.90&      1.36$^a $&     -3.00&    3\\
   273&   189.220&    62.277&      24.8&      24.6&      24.5&      24.3&      24.3&      24.0&     -99.0&     -99.0&     23.02&     22.83&    -99.00&     -1.00  &    -99.00&   -1\\
   274&   189.220&    62.246&      23.4&      22.0&      20.8&      19.9&      19.4&      19.2&      18.3&      18.0&     17.58&     18.71&    -99.00&      0.32$^a $&     -3.00&    0\\
   275&   189.221&    62.124&      18.0&      17.7&      17.0&      18.3&      16.8&      14.8&      13.4&      13.0&     12.94&     14.34&     16.69&     -2.00  &    -99.00&   -2\\
   276&   189.221&    62.330&      27.6&      26.3&      25.9&      25.5&      24.8&      24.7&      23.0&      22.3&     21.97&     21.48&    -99.00&     -1.00  &      1.15&   -1\\
   277&   189.223&    62.194&      23.4&      23.3&      23.2&      22.9&      22.6&      22.2&      21.6&      21.0&     20.52&     20.19&     17.63&      1.27$^a $&     -3.00&    1\\
   278&   189.223&    62.339&      26.1&      25.7&      25.3&      24.5&      23.7&      23.1&      22.1&      21.7&     21.41&     21.77&     18.87&      1.02$^a $&     -3.00&    3\\
   279&   189.224&    62.188&      23.8&      23.8&      23.8&      23.5&      23.0&      22.7&      22.2&      22.0&     21.63&     21.19&    -99.00&      0.89$^a $&     -3.00&    1\\
   280&   189.224&    62.152&      27.2&      26.9&      26.0&      25.1&      24.0&      23.4&      22.4&      21.8&     21.72&     21.63&    -99.00&      0.00$^a $&      0.95&  -99\\
   281&   189.226&    62.143&      26.9&      25.5&      24.4&      23.2&      22.6&      22.1&      21.4&      20.8&     20.33&     20.05&     17.87&      0.53  &     -3.00&    1\\
   282&   189.226&    62.129&      22.0&      21.4&      20.7&      20.2&      19.9&      19.7&      19.1&      18.7&     18.40&     19.15&     16.67&      0.20$^a $&     -3.00&    1\\
   283&   189.226&    62.262&      26.7&      26.8&      26.8&      26.0&      25.9&      25.6&     -99.0&     -99.0&     25.03&     27.62&    -99.00&      0.00$^a $&    -99.00&  -99\\
   284&   189.228&    62.187&      26.8&      26.6&      26.2&      25.9&      25.8&      25.9&     -99.0&     -99.0&     23.30&     22.82&    -99.00&     -1.00  &    -99.00&   -1\\
   285&   189.228&    62.074&      21.7&      21.3&      20.2&      19.7&      19.4&      19.1&      18.0&      17.5&     17.31&    -99.00&     16.36&      0.29$^a $&     -3.00&    1\\
   286&   189.231&    62.220&      27.2&      25.8&      24.6&      23.5&      22.4&      21.7&      20.7&      20.3&     19.66&     19.62&    -99.00&      0.95$^a $&     -3.00&    1\\
   287&   189.233&    62.200&      25.6&      25.0&      24.8&      24.7&      24.5&      24.0&      22.8&      22.2&     21.74&     21.04&     18.15&      0.00$^a $&      1.85&  -99\\
   288&   189.233&    62.136&      25.6&      24.8&      23.8&      22.6&      21.6&      21.1&      20.2&      19.7&     19.18&     19.04&     16.60&      0.79$^a $&     -3.00&    1\\
   289&   189.235&    62.399&      26.8&      24.7&      24.3&      24.1&      24.1&      24.0&     -99.0&     -99.0&     22.89&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
   290&   189.236&    62.254&     -28.3&      26.7&      28.1&      27.0&      26.5&      25.9&     -99.0&     -99.0&     23.16&     22.37&    -99.00&     -1.00  &    -99.00&   -1\\
   291&   189.236&    62.213&      24.9&      23.7&      22.5&      21.3&      20.7&      20.4&      19.3&      18.9&     18.54&     19.42&    -99.00&      0.52$^a $&     -3.00&    0\\
   292&   189.237&    62.187&      24.6&      24.3&      24.3&      24.0&      23.7&      23.6&      22.9&      22.3&     22.22&     22.05&    -99.00&      0.00$^a $&    -99.00&  -99\\
   293&   189.237&    62.083&      24.6&      24.1&      23.2&      22.2&      21.1&      20.6&      19.6&      19.1&     18.74&    -99.00&     18.65&      0.84$^a $&     -3.00&    1\\
   294&   189.237&    62.217&      24.8&      24.6&      24.4&      23.8&      23.2&      22.5&      21.3&      20.9&     20.35&     20.22&    -99.00&      1.24  &     -3.00&    1\\
   295&   189.239&    62.174&      25.3&      25.0&      24.5&      23.8&      22.8&      22.5&      21.8&      21.4&     21.00&     21.20&    -99.00&      0.85$^a $&     -3.00&    1\\
   296&   189.240&    62.203&      24.1&      23.8&      23.0&      22.0&      21.2&      20.9&      19.9&      19.6&     19.19&     19.43&    -99.00&      0.66$^a $&     -3.00&    0\\
   297&   189.240&    62.054&      26.4&      25.1&      24.6&      24.4&      24.4&      24.0&     -99.0&      22.5&     22.42&    -99.00&    -99.00&     -1.00  &      0.15&   -1\\
   298&   189.241&    62.392&      25.5&      25.3&      24.9&      24.1&      23.1&      22.4&      21.2&      20.5&     19.78&    -99.00&     17.32&      1.20  &     -3.00&    1\\
   299&   189.241&    62.358&      26.7&      25.9&      25.4&      24.8&      24.3&      23.8&     -99.0&      22.4&     21.75&     20.84&     18.09&      0.00$^a $&      0.85&  -99\\
   300&   189.243&    62.166&      20.8&      20.0&      19.3&      18.8&      18.5&      18.3&      17.2&      17.0&     16.85&     18.31&     17.11&      0.14$^a $&     -3.00&    1\\
   301&   189.244&    62.067&      22.2&      21.5&      21.6&      21.6&      21.7&      21.4&      21.7&      21.4&     21.22&    -99.00&    -99.00&      2.75  &     -3.00&    3\\
   302&   189.245&    62.250&      28.8&      26.2&      26.5&      26.0&      25.2&      25.2&     -99.0&      23.1&     23.43&     22.01&     18.63&      0.00$^a $&      0.85&  -99\\
   303&   189.245&    62.173&      26.3&      25.9&      25.8&      25.5&      24.8&      24.5&      22.7&      22.1&     21.71&     21.04&    -99.00&      0.00$^a $&      0.95&  -99\\
   304&   189.245&    62.243&      23.3&      22.9&      22.4&      21.6&      20.9&      20.6&      19.9&      19.5&     19.03&     19.19&     18.19&      0.68$^a $&     -3.00&    0\\
   305&   189.245&    62.277&      22.4&      21.8&      20.9&      20.4&      20.1&      19.9&      19.1&      18.7&     18.42&     19.58&     17.80&      0.30$^a $&     -3.00&    1\\
   306&   189.246&    62.423&      21.9&      21.0&      20.8&      20.7&      20.9&      20.8&      20.3&      20.2&     20.35&    -99.00&    -99.00&      3.05$^a $&     -3.00&    4\\
   307&   189.247&    62.309&      28.1&      26.9&      26.6&      26.2&      26.0&      25.5&     -99.0&      22.8&     22.42&     21.67&     17.74&      0.00$^a $&      0.95&  -99\\
   308&   189.250&    62.235&      23.5&      23.2&      23.0&      22.6&      22.5&      22.5&      19.7&      19.6&     19.67&     23.23&    -99.00&      0.52$^a $&     -3.00&    3\\
   309&   189.249&    62.326&      25.6&      25.0&      24.6&      24.0&      23.3&      22.6&      21.5&      21.1&     20.58&     20.34&    -99.00&      1.14$^a $&     -3.00&    1\\
   310&   189.250&    62.247&      24.1&      23.6&      23.0&      22.3&      21.7&      21.4&      20.7&      20.2&     19.72&     19.67&     17.23&      0.76$^a $&     -3.00&    1\\
   311&   189.252&    62.271&      23.9&      23.9&      23.4&      23.0&      22.3&      22.0&      21.2&      21.0&     20.56&     20.17&     17.15&      0.91$^a $&     -3.00&    1\\
   312&   189.252&    62.252&      27.8&      26.5&      25.8&      25.5&      25.3&      24.9&      23.0&      22.3&     21.68&     21.12&    -99.00&      0.00$^a $&      0.95&  -99\\
   313&   189.255&    62.353&      25.9&      24.6&      23.2&      22.2&      21.0&      20.5&      19.3&      18.9&     18.45&     19.74&     17.80&      0.80$^a $&     -3.00&    0\\
   314&   189.254&    62.171&      25.9&      25.6&      25.4&      25.3&      24.9&      24.4&      23.3&      22.7&     22.64&     22.35&     18.04&      0.00$^a $&    -99.00&  -99\\
   315&   189.256&    62.108&      23.3&      22.6&      21.6&      20.4&      19.7&      19.3&      18.3&      17.8&     17.43&    -99.00&     18.02&      0.56$^a $&     -3.00&    0\\
   316&   189.257&    62.312&      21.8&      21.3&      20.2&      19.7&      19.4&      19.1&      17.7&      17.4&    -99.00&     20.13&    -99.00&      0.23$^a $&     -3.00&    0\\
   317&   189.257&    62.196&      26.7&      25.8&      25.7&      25.3&      24.5&      24.3&      22.2&      21.4&     20.82&     19.68&     16.77&      0.00$^a $&      0.85&  -99\\
   318&   189.257&    62.122&      30.0&     -28.1&      27.8&      27.9&      30.2&     -25.4&     -99.0&     -99.0&     23.57&     22.61&     17.52&      0.00$^a $&    -99.00&  -99\\
   319&   189.258&    62.340&      29.0&      28.5&      27.7&      26.9&      26.7&      25.8&     -99.0&     -99.0&     23.54&    -23.07&    -99.00&     -1.00  &    -99.00&   -1\\
   320&   189.259&    62.190&      21.4&      20.8&      20.3&      19.9&      19.8&      19.6&      18.6&      18.5&     18.35&     19.78&     18.20&      0.14  &     -3.00&    1\\
   321&   189.260&    62.324&      26.4&      25.3&      25.5&      25.5&      25.8&      25.0&     -99.0&      22.7&     22.58&     21.83&    -99.00&      0.00$^a $&      2.05&  -99\\
   322&   189.261&    62.212&      25.9&      25.8&      25.4&      25.0&      24.8&      24.6&      22.6&      22.7&     22.22&     21.41&    -99.00&      0.00$^a $&      1.95&  -99\\
   323&   189.261&    62.262&      21.6&      20.9&      20.7&      20.2&      19.9&      19.7&      19.1&      18.7&     18.37&     18.66&     17.21&      0.51$^a $&     -3.00&    4\\
   324&   189.262&    62.267&      26.5&      26.1&      26.2&      25.5&      25.1&      24.8&      23.1&      22.7&     22.81&     22.32&    -99.00&      1.58  &     -3.00&    1\\
   325&   189.265&    62.086&      27.9&      26.6&      25.4&      24.2&      23.0&      22.4&      21.4&      21.0&     20.68&    -99.00&    -99.00&      0.86$^a $&     -3.00&    1\\
   326&   189.264&    62.275&      23.2&      22.9&      22.1&      21.6&      21.4&      21.2&      21.0&      20.8&     19.62&     20.44&    -99.00&      0.36$^a $&     -3.00&    1\\
   327&   189.266&    62.190&      23.9&      23.7&      23.7&      23.6&      23.2&      22.9&      22.5&      22.3&     21.83&     21.63&     18.38&      0.91$^a $&     -3.00&    1\\
   328&   189.266&    62.168&     -29.8&     -31.1&      28.2&      25.9&      26.4&      26.6&     -99.0&     -99.0&     23.56&     23.71&    -99.00&     -1.00  &    -99.00&   -1\\
   329&   189.266&    62.259&      27.5&      27.2&      27.1&      27.0&      26.3&      25.8&     -99.0&     -99.0&     24.75&     24.79&    -99.00&      0.00$^a $&    -99.00&  -99\\
   330&   189.267&    62.199&     -27.3&      26.6&      25.2&      25.1&      25.1&      24.9&     -99.0&      23.4&     22.51&     22.96&     18.74&      3.41$^a $&     -3.00&    4\\
   331&   189.267&    62.132&      22.5&      22.6&      22.4&      22.0&      21.8&      21.4&      20.7&      20.1&     19.63&     19.26&     17.16&      1.25$^a $&     -3.00&    3\\
   332&   189.269&    62.241&      24.0&      23.4&      22.7&      21.7&      21.2&      20.9&      20.1&      19.7&     19.24&     19.52&     18.30&      0.56$^a $&     -3.00&    0\\
   333&   189.269&    62.281&      22.6&      22.2&      21.5&      20.9&      20.7&      20.5&      19.9&      19.6&     19.26&     19.97&     18.23&      0.38$^a $&     -3.00&    1\\
   334&   189.270&    62.267&      27.6&      26.9&      26.7&      26.1&      25.4&      25.2&      23.0&      22.4&     22.19&     21.55&    -99.00&      0.00$^a $&      0.85&  -99\\
   335&   189.271&    62.276&      28.2&     -28.6&      27.3&      27.3&      26.4&      25.6&     -99.0&     -99.0&     24.00&     23.09&    -99.00&      0.00$^a $&    -99.00&  -99\\
   336&   189.272&    62.415&      27.8&      26.4&     -30.3&      26.8&     -27.1&      28.3&     -99.0&     -99.0&     22.57&    -99.00&    -99.00&      0.00$^a $&      2.35&  -99\\
   337&   189.275&    62.198&      23.4&      23.1&      22.6&      22.0&      21.2&      20.9&      20.1&      19.8&     19.30&     19.22&     16.86&      0.90$^a $&     -3.00&    1\\
   338&   189.275&    62.025&      25.6&      24.4&      23.3&      22.1&      21.5&      21.0&      20.4&      19.9&     19.78&    -99.00&    -99.00&      0.52$^a $&     -3.00&    1\\
   339&   189.276&    62.287&      21.7&      21.1&      20.1&      19.6&      19.2&      19.0&      17.9&      17.7&     17.35&     18.85&     16.96&      0.25$^a $&     -3.00&    1\\
   340&   189.276&    62.360&      22.8&      22.4&      22.1&      21.8&      21.4&      21.1&      20.3&      20.2&     19.56&     19.10&     17.59&      0.90$^a $&     -3.00&    4\\
   341&   189.279&    62.374&      25.6&      25.3&      25.2&      25.2&      25.2&      24.9&     -99.0&     -99.0&     23.78&    -27.76&    -99.00&     -1.00  &    -99.00&   -1\\
   342&   189.279&    62.123&      25.5&      25.0&      24.6&      23.8&      23.0&      22.3&      21.4&      20.8&     20.13&     19.53&     17.27&      0.00$^a $&      1.15&  -99\\
   343&   189.278&    62.430&      21.2&      20.8&      20.8&      20.3&      19.9&      19.6&      19.0&      18.4&     18.09&    -99.00&    -99.00&      0.47$^a $&     -3.00&    3\\
   344&   189.279&    62.284&      19.8&      20.0&      19.7&      19.7&      19.8&      19.8&      19.5&      19.5&     19.10&     18.45&     16.51&      1.02$^a $&     -3.00&    4\\
   345&   189.279&    62.142&      27.5&      26.0&      25.9&      24.8&      24.2&      23.4&      22.4&      21.7&     21.19&     21.08&    -99.00&      0.00$^a $&      0.95&  -99\\
   346&   189.281&    62.279&      24.9&      24.8&      24.8&      24.2&      23.4&      22.9&      21.7&      21.3&     20.86&     20.96&    -99.00&      1.02$^a $&     -3.00&    1\\
   347&   189.280&    62.236&      27.5&      26.8&      26.3&      25.6&      25.6&      24.7&     -99.0&      22.2&     21.62&     20.94&     17.97&      2.49$^b $&     -3.00&   10\\
   348&   189.281&    62.363&      22.7&      23.0&      23.2&      22.5&      22.4&      22.0&      20.8&      20.4&     20.24&     19.87&     17.93&      1.45$^a $&     -3.00&    4\\
   349&   189.282&    62.332&      28.7&      28.5&      26.6&      25.5&      24.4&      23.6&      22.8&      22.1&     21.26&     20.72&    -99.00&     -1.00  &      1.35&   -1\\
   350&   189.282&    62.093&      28.1&      28.0&      26.4&      26.2&      25.6&      25.3&     -99.0&      22.5&     22.09&    -99.00&    -99.00&      0.00$^a $&      0.95&  -99\\
   351&   189.282&    62.271&      24.7&      24.4&      23.7&      22.9&      22.0&      21.4&      20.5&      20.0&     19.43&     19.27&     18.13&      0.94$^a $&     -3.00&    0\\
   352&   189.283&    62.268&      24.2&      23.9&      23.3&      22.6&      21.7&      21.3&      20.4&      20.0&     19.40&     19.32&     17.28&      0.94$^a $&     -3.00&    0\\
   353&   189.285&    62.182&      22.1&      21.8&      21.2&      20.6&      20.5&      20.3&      19.7&      19.5&     19.11&     19.60&     16.87&      0.42$^a $&     -3.00&    1\\
   354&   189.286&    62.250&      26.0&      24.8&      23.7&      22.5&      21.8&      21.5&      20.9&      20.5&     20.08&     20.71&    -99.00&      0.57$^a $&     -3.00&    0\\
   355&   189.287&    62.123&      26.8&      25.9&      25.0&      23.7&      22.7&      21.9&      21.0&      20.4&     20.03&    -99.00&    -99.00&      1.03$^a $&     -3.00&    0\\
   356&   189.287&    62.089&      25.8&      25.2&      24.2&      23.1&      22.0&      21.2&      20.3&      19.8&     19.36&    -99.00&    -99.00&      0.96$^a $&     -3.00&    0\\
   357&   189.289&    62.371&      26.4&      25.8&      25.3&      24.8&      23.9&      23.5&      21.5&      20.9&     20.43&     19.91&     18.47&      0.00$^a $&      0.95&  -99\\
   358&   189.289&    62.144&      24.7&      24.3&      23.3&      22.2&      21.1&      20.5&      19.4&      19.0&     18.58&     18.77&    -99.00&      0.91$^a $&     -3.00&    0\\
   359&   189.291&    62.145&      24.2&      24.1&      23.6&      22.9&      22.0&      21.6&      20.5&      20.1&     19.42&     19.23&     16.28&      0.90$^a $&     -3.00&    1\\
   360&   189.291&    62.134&      22.6&      23.0&      23.1&      23.1&      22.6&      22.2&      22.0&      21.6&     21.24&     20.83&     18.40&      2.18$^a $&     -3.00&    4\\
   361&   189.291&    62.143&      27.7&      28.0&      25.6&      24.4&      23.3&      22.7&      21.7&      21.1&     20.65&     22.62&    -99.00&      1.22  &     -3.00&    1\\
   362&   189.291&    62.383&      26.2&      25.7&      25.6&      24.7&      23.8&      23.1&      21.6&      21.0&     20.24&     19.69&     17.49&      0.00$^a $&      0.85&  -99\\
   363&   189.292&    62.097&      26.5&      26.9&      26.1&      25.3&      24.8&      24.1&     -99.0&     -99.0&     22.23&    -99.00&    -99.00&      0.00$^a $&      0.95&  -99\\
   364&   189.296&    62.391&      24.6&      24.4&      24.3&      23.7&      23.7&      23.1&      22.1&      21.3&     21.03&     20.92&    -99.00&      1.39$^a $&     -3.00&    4\\
   365&   189.297&    62.120&      27.9&      27.9&      27.4&      26.0&      25.2&      24.4&     -99.0&      22.6&     22.30&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
   366&   189.297&    62.225&      25.3&      24.5&      24.1&      23.7&      23.4&      23.1&      21.5&      21.1&     20.50&     20.14&     17.08&      1.97$^b $&     -3.00&   10\\
   367&   189.299&    62.263&      27.7&      26.8&      25.7&      24.6&      23.4&      22.9&      22.2&      21.7&     21.30&     21.33&    -99.00&      0.94$^a $&     -3.00&    0\\
   368&   189.300&    62.224&      26.1&      25.7&      25.7&      25.6&      25.0&      25.1&     -99.0&      22.9&     22.46&     21.71&     18.02&      2.00$^c $&     -3.00&   10\\
   369&   189.300&    62.203&      27.8&      28.0&      26.4&      26.1&      25.6&      24.8&     -99.0&      23.2&     22.34&     21.61&    -99.00&      2.91$^c $&     -3.00&   10\\
   370&   189.301&    62.298&      25.3&      25.2&      24.7&      24.0&      23.4&      22.8&      21.8&      21.2&     20.65&     20.20&     18.49&      1.25  &     -3.00&    1\\
   371&   189.306&    62.290&      31.2&      27.1&      28.4&     -28.7&     -28.6&      28.8&     -99.0&     -99.0&    -99.00&    -25.61&    -99.00&      0.00$^a $&    -99.00&  -99\\
   372&   189.307&    62.263&      31.6&      27.0&      26.6&      26.4&      26.1&      27.6&     -99.0&      23.6&     22.69&     22.11&     18.46&      0.00$^a $&      1.15&  -99\\
   373&   189.308&    62.240&      25.0&      24.0&      23.2&      22.2&      21.7&      21.4&      20.7&      20.2&     19.88&     20.19&     18.90&      0.47$^a $&     -3.00&    3\\
   374&   189.308&    62.307&     -27.4&     -29.5&      27.4&      27.3&      26.5&     -32.8&     -99.0&     -99.0&     24.64&     22.68&    -99.00&      0.00$^a $&    -99.00&  -99\\
   375&   189.308&    62.250&      27.0&      26.0&      25.8&      25.7&      25.3&      25.5&     -99.0&      23.6&     23.26&     22.91&    -99.00&     -1.00  &    -99.00&   -1\\
   376&   189.308&    62.155&      26.9&      26.0&      25.5&      24.9&      24.6&      24.1&      22.3&      21.7&     21.35&     21.09&    -99.00&      0.00$^a $&      1.55&  -99\\
   377&   189.310&    62.202&      25.2&      24.4&      24.1&      24.0&      23.8&      23.4&      22.5&      21.9&     21.29&     21.11&     18.06&      0.00  &      1.25&  -99\\
   378&   189.310&    62.206&      25.7&      25.2&      24.9&      24.3&      23.5&      22.9&      22.2&      21.8&     21.40&     21.46&    -99.00&      1.08$^a $&     -3.00&    1\\
   379&   189.310&    62.085&      23.2&      22.7&      21.8&      21.1&      20.8&      20.4&      19.8&      19.4&     19.02&    -99.00&    -99.00&      0.44$^a $&     -3.00&    1\\
   380&   189.311&    62.311&     -29.4&      27.1&      26.1&      25.9&      25.3&      25.3&      23.9&      22.8&     22.56&     21.99&     18.75&      0.00$^a $&      0.85&  -99\\
   381&   189.312&    62.271&      24.4&      24.1&      24.2&      23.9&      23.6&      23.4&      22.5&      22.1&     21.51&     20.85&     18.68&      1.52  &     -3.00&    1\\
   382&   189.313&    62.042&      26.4&      26.1&      26.1&      26.0&      25.7&      25.2&     -99.0&      22.1&     21.68&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
   383&   189.316&    62.200&      21.5&      20.3&      19.4&      18.9&      18.5&      18.2&      17.3&      17.1&     17.05&     18.03&     18.04&      0.10$^a $&     -3.00&    0\\
   384&   189.316&    62.204&      25.5&      25.2&      24.7&      23.9&      22.9&      22.3&      21.3&      20.8&     20.10&     19.80&     18.39&      1.02$^a $&     -3.00&    1\\
   385&   189.317&    62.056&      19.9&      20.1&      20.0&      19.9&      19.5&      19.4&      19.3&      19.0&     18.66&    -99.00&    -99.00&      2.07$^a $&     -3.00&    4\\
   386&   189.317&    62.119&      22.4&      21.6&      21.5&      21.2&      20.9&      20.7&      20.1&      19.7&     19.30&    -99.00&     17.82&      0.68$^a $&     -3.00&    4\\
   387&   189.317&    62.192&      28.1&      27.1&      26.2&      24.6&      23.6&      22.8&      21.7&      21.2&     20.71&     20.52&    -99.00&      1.08$^a $&     -3.00&    1\\
   388&   189.318&    62.253&      23.7&      23.0&      22.2&      21.2&      20.5&      20.2&      18.9&      18.5&     18.18&     18.95&     18.05&      0.56$^a $&     -3.00&    0\\
   389&   189.319&    62.279&      23.7&      23.5&      23.2&      22.6&      22.3&      22.2&      21.3&      20.8&     20.05&     19.56&     17.13&      0.56$^a $&     -3.00&    3\\
   390&   189.320&    62.293&      25.1&      24.8&      24.2&      23.4&      22.6&      22.2&      21.2&      20.6&     20.28&     19.47&     16.18&      1.15$^a $&     -3.00&    1\\
   391&   189.320&    62.106&      25.3&      24.8&      24.4&      23.8&      23.1&      22.5&      22.0&      21.4&     21.13&    -99.00&    -99.00&      0.97$^a $&     -3.00&    3\\
   392&   189.320&    62.169&      23.6&      22.8&      21.8&      21.0&      20.6&      20.3&      19.5&      19.1&     18.75&     19.42&     16.99&      0.41$^a $&     -3.00&    1\\
   393&   189.321&    62.098&      21.9&      22.0&      21.9&      21.9&      21.7&      21.6&      21.3&      21.0&     20.64&    -99.00&    -99.00&      1.94$^a $&     -3.00&    4\\
   394&   189.325&    62.315&      22.9&      22.2&      22.1&      22.2&      22.2&      21.9&      22.3&      21.8&     21.16&     21.24&     18.23&      2.22$^a $&     -3.00&    4\\
   395&   189.327&    62.136&      22.3&      22.2&      21.4&      21.0&      20.9&      20.6&      19.8&      19.6&     19.40&    -99.00&    -99.00&      0.41$^a $&     -3.00&    1\\
   396&   189.329&    62.114&      24.0&      23.9&      23.8&      23.6&      23.5&      23.3&      22.8&      22.5&     22.40&    -99.00&    -99.00&      2.73$^a $&     -3.00&    4\\
   397&   189.329&    62.174&     -29.0&      27.9&      26.9&      25.6&      25.4&      26.2&     -99.0&     -99.0&     24.13&     23.36&    -99.00&      4.14$^a $&     -3.00&    3\\
   398&   189.333&    62.165&      25.8&      25.1&      24.8&      24.5&      24.4&      24.0&      23.4&      22.5&     22.49&     21.77&     18.52&      2.64$^a $&     -3.00&    1\\
   399&   189.333&    62.076&      25.4&      25.1&      24.6&      24.0&      23.3&      22.9&      21.9&      21.5&     20.91&    -99.00&    -99.00&      0.91  &     -3.00&    1\\
   400&   189.334&    62.124&      28.5&      27.5&      27.9&      26.7&      25.1&      24.6&      22.5&      21.8&     21.57&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
   401&   189.335&    62.257&      27.0&      26.2&      24.9&      23.5&      22.4&      21.6&      20.7&      20.3&     19.66&     19.67&    -99.00&      0.94$^a $&     -3.00&    0\\
   402&   189.335&    62.231&      26.4&      25.7&      25.0&      24.1&      23.2&      22.7&      21.6&      21.1&     20.49&     20.16&     18.52&      0.85  &     -3.00&    0\\
   403&   189.339&    62.192&      24.8&      24.3&      24.3&      23.8&      23.5&      23.0&      21.8&      21.1&     20.57&     20.58&     18.08&      1.60  &     -3.00&    1\\
   404&   189.339&    62.213&      21.1&      20.4&      19.6&      19.2&      18.9&      18.7&      16.7&      16.6&     16.52&     19.40&    -99.00&      0.10$^a $&     -3.00&    1\\
   405&   189.341&    62.177&      24.2&      24.0&      23.5&      22.8&      21.9&      21.4&      20.4&      20.1&     19.64&     19.43&     17.89&      0.98$^a $&     -3.00&    1\\
   406&   189.344&    62.093&     -28.5&      28.1&      27.7&      28.0&     -31.2&      26.0&     -99.0&     -99.0&     24.38&    -99.00&    -99.00&     -1.00  &    -99.00&   -1\\
   407&   189.344&    62.348&      27.2&      26.0&      25.3&      24.6&      24.7&      23.4&      21.9&      21.2&     20.84&     20.55&    -99.00&      0.00$^a $&      1.15&  -99\\
   408&   189.344&    62.160&      25.4&      25.1&      25.0&      24.7&      24.7&      24.8&      24.1&      23.1&     22.62&     22.50&    -99.00&      0.00$^a $&      1.25&  -99\\
   409&   189.347&    62.261&      24.8&      24.6&      24.4&      24.1&      23.9&      23.6&      22.6&      22.2&     21.96&     22.05&    -99.00&      2.24$^a $&     -3.00&    3\\
   410&   189.349&    62.179&      21.8&      21.1&      20.4&      20.1&      19.9&      19.6&      18.6&      18.4&    -99.00&     21.37&    -99.00&      0.11$^a $&     -3.00&    1\\
   411&   189.349&    62.354&      26.7&      24.9&      24.1&      23.8&      23.9&      23.6&      23.1&      22.5&     22.25&     22.13&    -99.00&      3.52$^a $&     -3.00&    4\\
   412&   189.350&    62.218&      25.2&      25.0&      25.0&      24.7&      24.3&      23.8&      22.1&      22.0&     21.74&     21.23&    -99.00&      0.00$^a $&    -99.00&  -99\\
   413&   189.351&    62.233&      25.9&      25.5&      25.7&      25.0&      24.7&      24.2&      22.8&      22.2&     21.98&     21.36&    -99.00&      0.47$^a $&     -3.00&    0\\
   414&   189.351&    62.212&      26.0&      25.5&      24.3&      23.3&      22.2&      21.8&      20.8&      20.5&     19.92&     20.11&    -99.00&      0.80$^a $&     -3.00&    0\\
   415&   189.355&    62.141&      22.0&      21.2&      20.6&      20.3&      20.1&      19.9&      18.8&      18.6&     18.56&    -99.00&    -99.00&      0.12$^a $&     -3.00&    1\\
   416&   189.354&    62.149&      25.9&      25.4&      24.8&      23.9&      22.8&      22.1&      21.0&      20.5&     19.89&    -99.00&     17.37&      0.94$^a $&     -3.00&    0\\
   417&   189.356&    62.285&     -28.0&     -28.8&      26.3&      25.7&      26.9&      25.2&     -99.0&      22.9&     22.18&     21.59&     18.42&     -1.00  &      2.05&   -1\\
   418&   189.356&    62.328&      21.0&      20.6&      19.9&      19.5&      19.2&      19.0&      17.9&      17.7&     17.37&     19.05&     16.40&      0.28$^a $&     -3.00&    1\\
   419&   189.357&    62.280&      23.8&      22.0&      20.9&      19.9&      18.6&      18.0&      17.6&      17.5&     17.67&     18.33&    -99.00&     -2.00  &    -99.00&   -2\\
   420&   189.357&    62.379&      23.4&      23.3&      23.2&      23.3&      23.2&      22.9&      23.1&     -99.0&     21.71&     25.17&    -99.00&      2.21$^a $&     -3.00&    3\\
   421&   189.358&    62.042&      22.2&      21.9&      21.6&      21.2&      20.8&      20.6&      20.2&      19.7&     19.49&    -99.00&    -99.00&      0.60$^a $&     -3.00&    3\\
   422&   189.360&    62.076&      24.2&      24.1&      23.9&      23.6&      23.3&      22.9&      22.5&      21.7&     20.87&    -99.00&    -99.00&      2.23  &     -3.00&    4\\
   423&   189.360&    62.341&      26.7&      25.8&      25.5&      25.1&      24.7&      24.1&      22.4&      21.9&     21.26&     20.26&     16.48&      0.00$^a $&      0.95&  -99\\
   424&   189.361&    62.297&      26.4&      25.5&      25.4&      25.2&      25.1&      24.7&     -99.0&      23.4&     22.49&     21.54&     18.13&      0.00$^a $&    -99.00&  -99\\
   425&   189.365&    62.177&      21.4&      20.6&      19.7&      19.2&      18.8&      18.6&      17.2&      17.0&     16.75&     18.68&     16.55&      0.21$^a $&     -3.00&    0\\
   426&   189.374&    62.210&      23.6&      23.2&      22.8&      22.7&      22.7&      22.6&      22.3&      22.3&     22.22&     23.62&    -99.00&      0.16$^a $&     -3.00&    1\\
   427&   189.377&    62.325&     -27.9&      28.8&      30.0&      26.9&      28.3&      25.7&     -99.0&     -99.0&    -99.00&    -23.80&    -99.00&      0.00$^a $&    -99.00&  -99\\
   428&   189.378&    62.162&      21.6&      21.2&      20.4&      20.0&      19.8&      19.6&      18.4&      18.2&     18.00&     20.30&     16.95&      0.30$^a $&     -3.00&    1\\
   429&   189.379&    62.147&      25.2&      24.6&      23.7&      22.6&      21.6&      21.1&      20.3&      19.8&     19.41&    -99.00&    -99.00&      0.78$^a $&     -3.00&    1\\
   430&   189.380&    62.175&      27.3&      26.4&      25.9&      25.5&      25.2&      24.8&      23.4&      22.8&     22.37&     22.15&    -99.00&      0.00$^a $&      0.95&  -99\\
   431&   189.382&    62.218&     -29.0&      27.2&      26.4&      25.7&      25.9&      25.3&     -99.0&     -99.0&    -99.00&     23.38&    -99.00&      0.00$^a $&    -99.00&  -99\\
   432&   189.381&    62.284&      24.8&      24.8&      24.6&      24.1&      23.7&      23.4&      22.8&      22.7&     23.19&    -23.14&    -99.00&      0.00$^a $&      0.25&  -99\\
   433&   189.384&    62.213&      25.0&      24.6&      24.0&      23.1&      22.1&      21.5&      20.4&      20.0&     19.37&     19.18&     18.58&      1.02$^a $&     -3.00&    0\\
   434&   189.392&    62.273&      28.4&      27.4&      26.7&      25.3&      25.5&      23.0&      22.8&      22.4&     21.79&     21.60&    -99.00&     -1.00  &      1.25&   -1\\
   435&   189.393&    62.194&      21.5&      20.9&      20.3&      19.9&      19.8&      19.6&      18.9&      18.7&     18.61&     19.59&     17.05&      0.20$^a $&     -3.00&    1\\
   436&   189.393&    62.159&      21.7&      20.9&      20.1&      19.5&      19.1&      18.9&      18.0&      17.7&     17.42&    -99.00&     16.29&      0.19$^a $&     -3.00&    1\\
   437&   189.394&    62.232&      23.7&      23.4&      22.8&      22.1&      21.3&      21.0&      19.9&      19.6&     19.05&     19.14&     17.71&      0.84$^a $&     -3.00&    0\\
   438&   189.395&    62.321&      26.4&      25.4&      24.9&      24.6&      24.3&      24.1&     -99.0&      22.6&     22.66&     21.12&     17.18&     -1.00  &      0.85&   -1\\
   439&   189.396&    62.219&      26.9&      25.9&      24.8&      23.5&      22.7&      22.3&      21.4&      20.9&     20.57&     20.54&    -99.00&      0.64$^a $&     -3.00&    1\\
   440&   189.397&    62.232&      25.8&      25.5&      25.3&      24.6&      24.2&      23.7&      22.3&      21.5&     21.12&     20.66&    -99.00&      0.00$^a $&      1.05&  -99\\
   441&   189.400&    62.302&      25.2&      25.0&      24.5&      23.9&      23.5&      23.2&     -99.0&     -99.0&    -99.00&    -25.25&    -99.00&      0.00  &    -99.00&  -99\\
   442&   189.402&    62.226&      25.1&      24.7&      24.0&      23.2&      22.2&      21.7&      20.9&      20.6&     20.20&     20.26&    -99.00&      0.85$^a $&     -3.00&    1\\
   443&   189.402&    62.181&      25.4&      25.0&      24.6&      24.4&      24.5&      24.3&      22.1&      21.9&     21.95&     22.33&    -99.00&      0.00  &    -99.00&  -99\\
   444&   189.404&    62.241&      29.2&      26.6&      26.6&      26.1&      25.9&      25.3&     -99.0&      23.0&     22.24&     21.92&     18.68&      0.00$^a $&      1.05&  -99\\
   445&   189.404&    62.310&      27.7&      27.5&      27.0&      26.9&      25.7&      25.4&     -99.0&      24.4&     22.16&     21.41&    -99.00&     -1.00  &    -99.00&   -1\\
   446&   189.404&    62.201&      21.8&      21.3&      20.6&      19.9&      19.6&      19.3&      18.5&      18.2&     17.81&     18.81&     16.69&      0.41$^a $&     -3.00&    0\\
   447&   189.408&    62.287&      25.8&      25.9&      25.5&      24.8&      24.3&      23.7&     -99.0&     -99.0&     23.20&    -22.26&    -99.00&      0.00$^a $&    -99.00&  -99\\
   448&   189.408&    62.219&      26.7&      26.2&      26.1&      24.7&      23.6&      22.9&      21.5&      21.0&     20.70&     20.28&    -99.00&      1.24$^a $&     -3.00&    1\\
   449&   189.408&    62.275&      15.9&      20.8&      27.1&      23.2&      15.9&      14.7&      13.3&      13.0&     12.81&     14.34&     16.85&     -2.00  &    -99.00&   -2\\
   450&   189.409&    62.141&      23.2&      23.1&      22.8&      22.4&      21.8&      21.4&      20.6&      20.6&     20.18&    -99.00&    -99.00&      0.94$^a $&     -3.00&    1\\
   451&   189.414&    62.350&      22.3&      21.4&      21.1&      21.0&      20.7&      20.3&      19.7&      19.4&     18.85&     18.78&     16.70&      0.84$^a $&     -3.00&    4\\
   452&   189.414&    62.378&      28.3&     -28.4&      28.3&     -28.5&      26.3&      25.8&     -99.0&     -99.0&     22.39&     23.28&     18.06&     -1.00  &    -99.00&   -1\\
   453&   189.416&    62.227&      25.3&      24.8&      23.6&      22.6&      21.5&      21.0&      20.1&      19.7&     19.16&     19.03&     18.78&      0.84$^a $&     -3.00&    0\\
   454&   189.416&    62.284&      24.0&      23.2&      22.3&      21.3&      20.9&      20.6&      19.8&      19.5&     19.24&     19.92&    -99.00&      0.46$^a $&     -3.00&    0\\
   455&   189.421&    62.200&      23.1&      23.0&      23.0&      22.6&      22.2&      21.8&      20.9&      20.3&     19.48&     18.94&     16.97&      1.17$^a $&     -3.00&    1\\
   456&   189.421&    62.180&      27.3&      26.9&      26.4&      26.8&      25.6&      25.1&      23.5&      22.8&     22.19&    -99.00&    -99.00&     -1.00  &      0.65&   -1\\
   457&   189.422&    62.214&      25.2&      24.5&      24.3&      23.7&      23.1&      22.6&      21.0&      20.5&     20.02&     19.43&     17.45&      1.60  &     -3.00&    1\\
   458&   189.426&    62.255&      20.8&      20.0&      19.5&       0.2&      19.0&      18.9&      18.2&      18.0&     17.99&     18.94&     16.41&      0.07$^a $&     -3.00&    1\\
   459&   189.427&    62.303&      22.2&      21.8&      21.6&      21.7&      21.6&      21.4&      21.0&      20.8&     20.51&     20.43&     18.17&      2.30$^a $&     -3.00&    4\\
   460&   189.428&    62.131&      23.4&      23.3&      23.0&      22.5&      22.0&      21.5&      21.0&      20.6&     20.19&    -99.00&    -99.00&      1.08$^a $&     -3.00&    1\\
   461&   189.432&    62.094&      26.5&      27.4&      26.8&      26.1&      25.6&      24.9&     -99.0&      22.0&     21.70&    -99.00&    -99.00&      0.00$^a $&      1.15&  -99\\
   462&   189.434&    62.233&      24.8&      23.8&      22.8&      21.7&      21.2&      20.9&      20.3&      19.7&     19.48&     20.20&    -99.00&      0.51$^a $&     -3.00&    0\\
   463&   189.438&    62.122&      28.3&      26.7&      26.8&      26.9&      28.0&      26.3&     -99.0&     -99.0&     23.10&    -99.00&    -99.00&      0.00$^a $&      0.65&  -99\\
   464&   189.442&    62.177&      26.9&      26.3&      26.2&      25.9&      26.1&      25.9&     -99.0&     -99.0&     23.63&    -99.00&    -99.00&      0.00$^a $&    -99.00&  -99\\
   465&   189.445&    62.120&      26.5&      26.5&      26.1&      26.3&      25.5&      25.2&     -99.0&      23.2&     22.65&    -99.00&    -99.00&     -1.00  &      0.85&   -1\\
   466&   189.446&    62.276&      24.4&      23.0&      21.9&      20.8&      20.3&      19.9&      19.0&      18.5&     18.03&     18.66&     17.46&      0.44$^a $&     -3.00&    3\\
   467&   189.451&    62.358&      22.4&      20.5&      19.5&      18.8&      18.1&       0.0&      16.9&      16.7&     16.85&     18.79&    -99.00&     -2.00  &    -99.00&   -2\\
   468&   189.453&    62.220&      26.0&      25.8&      24.6&      23.6&      22.4&      21.9&      21.1&      20.9&     20.63&     20.32&     17.40&      0.91$^a $&     -3.00&    0\\
   469&   189.460&    62.195&      21.9&      21.1&      20.0&      19.5&      19.1&      18.7&      17.4&      17.1&     16.80&    -99.00&     16.53&      0.19$^a $&     -3.00&    1\\
   470&   189.459&    62.233&     -30.8&      26.8&      27.0&      26.2&      25.2&      24.5&      23.4&      22.4&     21.62&     21.03&    -99.00&      0.00  &      1.45&  -99\\
   471&   189.462&    62.267&      24.7&      24.3&      23.9&      23.0&      22.2&      21.3&      20.2&      19.8&     19.21&     18.80&     18.24&      1.17$^a $&     -3.00&    1\\
   472&   189.469&    62.122&      24.1&      24.0&      23.5&      22.7&      21.8&      21.2&      20.4&      19.9&     19.41&    -99.00&    -99.00&      0.97$^a $&     -3.00&    1\\
   473&   189.470&    62.275&      19.7&      20.4&      20.0&      19.5&      19.1&      18.9&      18.3&      18.0&     17.66&     18.11&     15.81&      0.31$^a $&     -3.00&    4\\
   474&   189.477&    62.183&      26.5&      25.8&      25.6&      24.7&      23.9&      22.9&      21.5&      20.8&     20.19&    -99.00&    -99.00&      0.00$^a $&      0.85&  -99\\
   475&   189.477&    62.169&      28.8&      26.7&      26.4&      26.1&      25.4&      25.5&     -99.0&      22.5&     22.08&    -99.00&    -99.00&      0.00$^a $&      1.25&  -99\\
   476&   189.476&    62.311&      25.0&      24.7&      24.3&      23.7&      23.6&      23.4&      22.7&      22.4&     22.44&     22.86&    -99.00&      0.47$^a $&     -3.00&    3\\
   477&   189.481&    62.282&      27.7&      25.8&      25.1&      24.5&      24.2&      23.9&     -99.0&     -99.0&    -99.00&     24.21&    -99.00&     -1.00  &    -99.00&   -1\\
   478&   189.489&    62.274&      24.3&      23.1&      22.6&      22.0&      21.9&      21.8&      21.3&      21.1&     20.98&     20.82&     18.33&      2.92$^a $&     -3.00&    4\\
   479&   189.494&    62.205&      21.0&      20.1&      19.3&      18.8&      18.6&      18.3&     -99.0&     -99.0&    -99.00&    -99.00&    -99.00&      0.09$^a $&     -3.00&    0\\
   480&   189.495&    62.249&      24.8&      24.0&      23.2&      22.2&      21.7&      21.3&      20.3&      19.9&     19.39&     19.12&     18.35&      0.46$^a $&     -3.00&    0\\
   481&   189.498&    62.184&      20.3&      19.3&      19.0&       0.2&      19.6&      19.0&      18.3&      18.6&     18.21&    -99.00&    -99.00&      0.91$^a $&     -3.00&    4\\
   482&   189.504&    62.145&      26.3&      25.6&      24.8&      24.0&      22.9&      22.4&      21.5&      21.0&     20.52&    -99.00&    -99.00&      0.91$^a $&     -3.00&    0\\
   483&   189.504&    62.227&      19.1&      19.2&      19.2&      18.9&      18.8&      18.5&      18.1&      17.8&     17.33&     16.90&     14.82&      0.44$^a $&     -3.00&    4\\
   484&   189.510&    62.321&      25.8&      25.8&      25.6&      25.1&      24.4&      23.8&      23.1&      22.3&     21.93&     21.71&    -99.00&      1.23  &     -3.00&    1\\
   485&   189.513&    62.184&      24.6&      24.5&      24.3&      24.0&      23.7&      23.3&      22.1&      21.6&     21.54&    -99.00&    -99.00&      1.18$^a $&     -3.00&    1\\
   486&   189.518&    62.257&      24.8&      24.4&      24.3&      24.1&      23.9&      23.6&      22.0&      21.6&     21.26&     21.09&     18.30&      0.00$^a $&    -99.00&  -99\\
   487&   189.522&    62.128&      23.9&      23.6&      23.1&      22.5&      21.8&      21.3&      20.6&      20.2&     19.69&    -99.00&    -99.00&      0.96  &     -3.00&    0\\
   488&   189.524&    62.180&      22.4&      22.1&      21.6&      20.7&      20.2&      19.9&      19.1&      18.7&     18.27&    -99.00&    -99.00&      0.57$^a $&     -3.00&    0\\
   489&   189.528&    62.212&      25.4&      25.1&      24.3&      22.9&      21.9&      21.0&      19.5&      19.0&     18.38&    -99.00&    -99.00&      1.02$^a $&     -3.00&    1\\
   490&   189.544&    62.292&      28.1&      25.9&      25.4&      24.4&      23.7&      22.9&      21.9&      21.4&     20.88&     20.43&    -99.00&      1.25  &     -3.00&    0\\
   491&   189.556&    62.149&      26.3&      26.0&      26.1&      25.6&      25.2&      24.8&      21.6&      21.0&     23.42&    -99.00&    -99.00&      0.00$^a $&      0.55&  -99\\
   492&   189.570&    62.181&      23.8&      23.7&      23.4&      22.9&      22.2&      21.6&      20.7&      20.3&     19.81&    -99.00&    -99.00&      1.01  &     -3.00&    1\\
   493&   189.572&    62.269&      23.9&      23.8&      23.9&      23.4&      23.2&      22.8&      21.9&      21.6&     21.12&     21.21&    -99.00&      1.25  &     -3.00&    1\\
   494&   189.578&    62.248&      24.7&      24.2&      23.9&      23.3&      22.6&      21.8&      21.0&      20.5&     19.99&     19.73&    -99.00&      1.21  &     -3.00&    1\\
   495&   189.593&    62.238&      23.9&      23.8&      23.5&      22.9&      22.1&      21.6&      20.7&      20.3&     19.73&    -99.00&    -99.00&      0.99$^a $&     -3.00&    3\\
   496&   189.595&    62.178&      26.6&      26.1&      25.2&      24.2&      23.1&      22.4&      21.4&      21.0&     20.81&    -99.00&    -99.00&      0.96$^a $&     -3.00&    0\\
   497&   189.597&    62.255&     -27.6&     -27.2&      26.8&      27.0&      25.5&      24.7&      22.0&      21.5&     21.00&    -99.00&    -99.00&      0.00$^a $&      0.95&  -99\\
   498&   189.599&    62.162&      26.2&      25.9&      25.8&      25.4&      26.0&      24.9&     -99.0&     -99.0&     22.98&    -99.00&    -99.00&      0.00$^a $&      1.95&  -99\\
   499&   189.617&    62.151&      22.6&      22.4&      22.1&      22.0&      22.1&      21.8&      21.2&      21.2&     20.95&    -99.00&    -99.00&      0.96$^a $&     -3.00&    3\\
   500&   189.630&    62.206&      23.2&      22.9&      22.7&      22.7&      22.5&      22.4&      22.1&      21.9&     21.50&    -99.00&    -99.00&      1.99  &     -3.00&    4\\
   501&   189.643&    62.245&      28.3&      26.4&      27.4&      26.1&      25.3&      24.9&     -99.0&      22.7&     22.03&    -99.00&    -99.00&      0.00  &      1.65&  -99\\
   502&   189.671&    62.200&      23.8&      23.8&      23.5&      23.0&      22.2&      21.6&      20.8&      20.5&     19.84&    -99.00&    -99.00&      0.96  &     -3.00&    1\\
   503&   189.690&    62.167&      18.2&      21.5&      17.4&      18.3&      17.1&      15.9&      14.2&      14.0&     14.16&    -99.00&    -99.00&     -2.00  &    -99.00&   -2\\
\tableline
\end{tabular}
\end{scriptsize}
\footnotesize
\tablecomments{All magnitudes are in AB magnitudes.\\
Typical photometric uncertainties are given in \S \ref{photodet}.\\
Magnitude $=-99$, source not detected ($2\sigma$ significance). \\
z$_{spec} = 0$ and corresponding class $= -99$, source spectroscopically observed but neither the redshift nor the class could be identified. \\
z$_{spec} = -1$ and corresponding class $= -1$, source not yet spectroscopically observed. \\
z$_{spec}>0$ and class $= 10$, spectroscopic redshift from the literature without a corresponding spectrum.\\
z$_{spec} = -2$ and corresponding class $= -2$, source is a star. \\
$z_{phot} = -3$, source has a spectroscopic redshift.\\
$z_{phot} = -99$, source has neither a spectroscopic nor a photometric redshift. \\
class $=0$, absorbers; class $=1$, star formers; class $=3$, high-excitation sources; class $=4$, broad-line AGNs.\\
Reference for z$_{spec}$: a=Barger et al.~(2003), b=Swinbank et al.~(2004), c=Chapman et al.~(2005), d=Reddy et al.~(2006). All other spectroscopic redshifts presented here for the first time.}
\end{table}


==> tab4.tex <==
\begin{table}
\begin{small}
\caption{CLANS X-ray Catalog: Basic Source Properties}
\label{xcat table1}
\begin{tabular}{cccccccccccccccccccc}
\tableline\tableline
& & & $\Delta\alpha$ &  $\Delta\delta$  & & & & & & & & & & & & & & &  \\
Number & $\alpha_{2000}$ & $\delta_{2000}$ &(arcsec)  & (arcsec) & $f_{0.5-2~{\rm keV}}$\tablenotemark{a} &  $1\sigma_{low}$ & $1\sigma_{hi}$ & $f_{2-8~{\rm keV}}$\tablenotemark{a} &  $1\sigma_{low}$ & $1\sigma_{hi}$ & $f_{0.5-8~{\rm keV}}$ & $1\sigma_{low}$ & $1\sigma_{hi}$ & HR\tablenotemark{b} & $1\sigma_{low}$ & $1\sigma_{hi}$ & $\Gamma$\tablenotemark{c} & $1\sigma_{low}$ & $1\sigma_{hi}$ \\
(1) & (2) & (3) & (4) & (5) & (6) & (6lo) & (6hi) & (7) & (7lo) & (7hi) & (8) & (8lo) & (8hi) & (9) & (9lo) & (9hi) & (10) & (10lo) & (10hi)\\
\tableline
    1 &   160.58846 &    59.25157 &       0.831 &       0.457 &        3.37 &        0.51 &        0.70 &       11.82 &        2.31 &        2.80 &       14.36 &        1.80 &        2.17 &        0.79 &   0.20 &   0.25 &   1.05 &   0.26 &   0.25\\
    2 &   160.64172 &    59.17641 &       0.301 &       0.239 &        7.79 &        0.83 &        0.97 &       10.01 &        1.75 &        2.28 &       17.98 &        1.62 &        1.94 &        0.37 &   0.08 &   0.10 &   1.71 &   0.19 &   0.20\\
    3 &   160.64175 &    59.16873 &       0.710 &       0.376 &        0.63 &        0.22 &        0.38 &        0.75 &        0.52 &        0.79 &        1.45 &        0.50 &        0.60 &        0.34 &   0.27 &   0.42 &   1.76 &   0.69 &   0.78\\
    4 &   160.65615 &    59.11504 &       1.231 &       0.581 &        1.52 &        0.57 &        1.01 &        0.51 &        0.42 &        1.74 &        2.20 &        0.67 &        1.30 &        0.13 &   0.12 &   0.46 &   2.37 &   1.08 &   0.36\\
    5 &   160.66704 &    59.07057 &       0.983 &       0.559 &        1.19 &        0.31 &        0.46 &        6.34 &        1.83 &        2.12 &        7.88 &        1.51 &        1.83 &        1.09 &   0.42 &   0.56 &   0.74 &   0.13 &   0.44\\
    6 &   160.66924 &    59.25401 &       1.004 &       0.460 &        0.93 &        0.28 &        0.37 &        4.63 &        1.38 &        1.86 &        5.86 &        1.21 &        1.49 &        1.03 &   0.44 &   0.59 &   0.80 &   0.18 &   0.49\\
    7 &   160.67195 &    59.20742 &       0.664 &       0.486 &        0.35 &        0.13 &        0.30 &        4.72 &        1.47 &        2.01 &        4.29 &        1.18 &        1.55 &        2.28 &   1.11 &   2.19 &   0.48 &   0.44 &   0.22\\
    8 &   160.67259 &    59.23265 &       0.595 &       0.254 &        1.92 &        0.43 &        0.53 &        3.24 &        1.00 &        1.61 &        5.68 &        1.02 &        1.21 &        0.45 &   0.17 &   0.26 &   1.54 &   0.41 &   0.41\\
    9 &   160.67681 &    59.22360 &       0.978 &       0.517 &        0.42 &        0.19 &        0.25 &        4.09 &        1.34 &        1.86 &        5.15 &        1.24 &        1.58 &        1.76 &   1.00 &   1.32 &   0.59 &   0.26 &   0.49\\
   10 &   160.68472 &    59.17066 &       0.706 &       0.523 &        1.02 &        0.29 &        0.44 &        0.93 &        0.52 &        0.90 &        2.02 &        0.53 &        0.69 &        0.29 &   0.18 &   0.30 &   1.93 &   0.62 &   0.52\\
   11 &   160.69992 &    59.25157 &       0.908 &       0.468 &        0.39 &        0.17 &        0.27 &        6.68 &        1.93 &        2.24 &        7.05 &        1.43 &        2.18 &        2.74 &   1.43 &   2.06 &   0.39 &   0.41 &   0.29\\
   12 &   160.71153 &    59.21258 &       0.319 &       0.153 &        2.71 &        0.49 &        0.59 &        4.44 &        1.22 &        1.60 &        7.20 &        1.03 &        1.39 &        0.44 &   0.15 &   0.19 &   1.55 &   0.31 &   0.34\\
   13 &   160.71415 &    59.19993 &       0.205 &       0.120 &        5.28 &        0.70 &        0.75 &        7.61 &        1.58 &        1.94 &       13.43 &        1.38 &        1.71 &        0.40 &   0.10 &   0.12 &   1.63 &   0.20 &   0.25\\
   14 &   160.71593 &    59.19225 &       0.448 &       0.208 &        0.77 &        0.23 &        0.36 &        3.80 &        1.12 &        1.76 &        5.19 &        1.10 &        1.36 &        1.03 &   0.43 &   0.67 &   0.80 &   0.20 &   0.49\\
   15 &   160.72220 &    59.17281 &       0.121 &       0.100 &        5.09 &        0.64 &        0.69 &       35.33 &        3.78 &        4.21 &       37.68 &        3.19 &        3.32 &        1.34 &   0.22 &   0.24 &   0.67 &   0.05 &   0.04\\
   16 &   160.72546 &    59.15141 &       0.506 &       0.245 &        0.48 &        0.19 &        0.28 &        1.87 &        0.81 &        1.26 &        2.20 &        0.72 &        0.86 &        0.86 &   0.51 &   0.77 &   0.97 &   0.36 &   0.77\\
   17 &   160.72712 &    59.17037 &       0.239 &       0.250 &        1.64 &        0.35 &        0.44 &       21.71 &        3.19 &        3.70 &       20.47 &        2.43 &        3.10 &        2.25 &   0.59 &   0.72 &   0.49 &   0.14 &   0.12\\
   18 &   160.73250 &    59.07445 &       0.179 &       0.151 &       12.58 &        1.05 &        1.09 &       36.60 &        3.66 &        4.04 &       50.30 &        3.13 &        3.44 &        0.68 &   0.09 &   0.10 &   1.15 &   0.10 &   0.14\\
   19 &   160.73713 &    58.95981 &       0.812 &       0.692 &        3.29 &        0.64 &        0.78 &       17.07 &        3.27 &        3.96 &       17.82 &        2.62 &        3.03 &        1.07 &   0.29 &   0.35 &   0.76 &   0.11 &   0.30\\
   20 &   160.73738 &    59.23934 &       0.237 &       0.105 &        2.76 &        0.43 &        0.59 &       35.75 &        3.99 &        4.72 &       35.48 &        3.39 &        3.73 &        2.21 &   0.42 &   0.55 &   0.50 &   0.11 &   0.08\\
   21 &   160.74383 &    59.16072 &       0.320 &       0.130 &        0.42 &        0.16 &        0.28 &        6.16 &        1.86 &        1.91 &        4.71 &        1.15 &        1.66 &        2.43 &   1.17 &   1.78 &   0.45 &   0.36 &   0.23\\
   22 &   160.76081 &    59.21955 &       0.369 &       0.233 &        0.38 &        0.14 &        0.33 &        5.82 &        1.73 &        2.33 &        5.44 &        1.25 &        2.04 &        2.51 &   1.20 &   2.38 &   0.44 &   0.48 &   0.24\\
   23 &   160.76450 &    58.95508 &       0.935 &       0.432 &        0.38 &        0.18 &        0.30 &        6.86 &        2.25 &        2.33 &        7.60 &        1.91 &        2.18 &        2.90 &   1.70 &   2.49 &   0.36 &   0.50 &   0.34\\
   24 &   160.76752 &    59.10955 &       0.269 &       0.196 &        0.13 &        0.09 &        0.18 &       15.86 &        2.85 &        4.14 &       15.72 &        3.13 &        3.46 &       12.89 &   8.83 &  17.27 &  -1.42 &   0.49 &   1.54\\
   25 &   160.77129 &    59.03118 &       0.876 &       0.555 &        2.12 &        0.42 &        0.57 &        2.95 &        1.14 &        1.19 &        4.58 &        0.83 &        1.09 &        0.39 &   0.17 &   0.19 &   1.65 &   0.33 &   0.46\\
   26 &   160.77262 &    58.94768 &       0.800 &       0.507 &        0.35 &        0.17 &        0.28 &       11.97 &        2.60 &        3.63 &       14.10 &        2.55 &        3.35 &        4.77 &   2.53 &   4.03 &  -0.02 &   0.81 &   0.51\\
   27 &   160.77615 &    59.19111 &       0.211 &       0.197 &        0.28 &        0.13 &        0.26  &$<$        2.01 &         -99 &         -99 &        0.84 &        0.49 &        0.68  &$<$        1.37 & -99.00\\
   28 &   160.77887 &    59.21408 &       0.425 &       0.150 &        1.60 &        0.44 &        0.58 &        0.18 &        0.15 &        0.61 &        1.59 &        0.38 &        0.49 &        0.06 &   0.05 &   0.20 &   2.59 &   0.59 &   0.15\\
   29 &   160.78195 &    59.20211 &       0.399 &       0.123 &        0.06 &        0.05 &        0.19 &        0.66 &        0.60 &        0.79 &        1.36 &        0.51 &        1.17 &        2.07 &   2.53 &   7.41 &   0.53 &   1.48 &   3.61\\
   30 &   160.78380 &    59.05556 &       0.231 &       0.157 &       16.76 &        1.30 &        1.40 &       24.71 &        2.99 &        3.37 &       40.98 &        2.74 &        2.84 &        0.41 &   0.06 &   0.07 &   1.61 &   0.11 &   0.14\\
   31 &   160.78691 &    59.20261 &       0.232 &       0.184 &        0.14 &        0.09 &        0.19 &        4.85 &        1.68 &        2.02 &        4.62 &        1.45 &        1.71 &        4.78 &   3.57 &   6.59 &  -0.02 &   1.32 &   0.71\\
   32 &   160.79133 &    59.28109 &       1.147 &       0.431 &        0.52 &        0.25 &        0.41 &        8.53 &        2.66 &        3.63 &        8.34 &        2.21 &        2.87 &        2.65 &   1.53 &   2.38 &   0.41 &   0.47 &   0.31\\
   33 &   160.79303 &    58.98792 &       0.417 &       0.326 &        5.30 &        0.73 &        0.78 &       28.63 &        3.56 &        4.29 &       34.18 &        3.22 &        3.38 &        1.10 &   0.20 &   0.23 &   0.73 &   0.06 &   0.21\\
   34 &   160.79680 &    59.19133 &       0.208 &       0.193  &$<$        0.08 &         -99 &         -99 &        5.68 &        1.67 &        2.63 &        6.19 &        1.86 &        2.18  &$>$        8.70 & -99.00\\
   35 &   160.79842 &    59.10399 &       0.260 &       0.255 &        1.11 &        0.28 &        0.41 &        6.59 &        1.71 &        1.96 &        7.20 &        1.35 &        1.63 &        1.19 &   0.43 &   0.56 &   0.70 &   0.11 &   0.38\\
   36 &   160.79905 &    59.00015 &       0.907 &       0.821 &        0.92 &        0.27 &        0.37  &$<$        6.26 &         -99 &         -99 &        2.54 &        0.83 &        1.16  &$<$        1.32 & -99.00\\
   37 &   160.80446 &    59.17308 &       0.255 &       0.155 &        0.20 &        0.10 &        0.22 &        3.72 &        1.29 &        1.83 &        3.53 &        0.94 &        1.65 &        3.01 &   1.86 &   3.76 &   0.34 &   0.75 &   0.37\\
   38 &   160.80960 &    59.22434 &       0.000 &       0.000 &        0.64 &        0.27 &        0.34 &        0.84 &        0.59 &        0.89 &        1.50 &        0.43 &        0.81 &        0.38 &   0.31 &   0.45 &   1.69 &   0.67 &   0.88\\
   39 &   160.81056 &    59.16506 &       0.138 &       0.070 &        1.75 &        0.36 &        0.48 &        3.70 &        1.16 &        1.37 &        6.25 &        1.06 &        1.16 &        0.53 &   0.20 &   0.25 &   1.40 &   0.34 &   0.39\\
   40 &   160.81481 &    58.93993 &       0.690 &       0.410 &        1.29 &        0.36 &        0.41 &        4.36 &        1.23 &        1.89 &        5.83 &        1.05 &        1.52 &        0.77 &   0.30 &   0.41 &   1.07 &   0.37 &   0.45\\
   41 &   160.81546 &    59.19214 &       0.282 &       0.121 &        0.21 &        0.11 &        0.24 &        1.04 &        0.53 &        1.20 &        1.99 &        0.62 &        0.99 &        1.04 &   0.75 &   1.68 &   0.79 &   0.40 &   1.13\\
   42 &   160.81883 &    59.18525 &       0.164 &       0.087 &        1.30 &        0.33 &        0.43 &        1.98 &        0.79 &        1.18 &        3.53 &        0.78 &        0.87 &        0.42 &   0.20 &   0.29 &   1.59 &   0.46 &   0.53\\
   43 &   160.82339 &    59.14450 &       0.172 &       0.088  &$<$        0.08 &         -99 &         -99 &        2.39 &        1.04 &        1.61 &        1.71 &        0.64 &        1.47  &$>$        4.28 & -99.00\\
   44 &   160.82539 &    59.17359 &       0.155 &       0.074 &        2.18 &        0.42 &        0.55 &        2.18 &        0.86 &        1.06 &        4.56 &        0.79 &        0.94 &        0.31 &   0.13 &   0.17 &   1.87 &   0.37 &   0.39\\
   45 &   160.82607 &    59.00072 &       0.485 &       0.232 &        3.25 &        0.50 &        0.69 &       12.75 &        2.32 &        2.78 &       14.84 &        1.91 &        2.17 &        0.86 &   0.20 &   0.26 &   0.97 &   0.26 &   0.22\\
   46 &   160.83263 &    59.14367 &       0.092 &       0.060 &        3.52 &        0.52 &        0.65 &       12.85 &        2.01 &        2.78 &       14.76 &        1.82 &        1.94 &        0.81 &   0.17 &   0.23 &   1.02 &   0.24 &   0.20\\
   47 &   160.83371 &    58.83733 &       0.881 &       0.499 &        2.05 &        0.41 &        0.62 &        9.41 &        1.90 &        2.92 &       10.15 &        1.71 &        2.02 &        0.97 &   0.27 &   0.42 &   0.86 &   0.20 &   0.28\\
   48 &   160.83529 &    59.07230 &       0.314 &       0.245 &        4.37 &        0.66 &        0.76 &        6.65 &        1.63 &        1.85 &       10.25 &        1.30 &        1.58 &        0.42 &   0.12 &   0.14 &   1.59 &   0.23 &   0.30\\
   49 &   160.83546 &    59.10271 &       0.261 &       0.232 &        0.16 &        0.11 &        0.17 &        3.12 &        1.09 &        1.86 &        3.42 &        1.07 &        1.46 &        3.03 &   2.37 &   3.68 &   0.33 &   0.73 &   0.84\\
   50 &   160.83557 &    58.93928 &       0.230 &       0.139 &        4.89 &        0.67 &        0.77 &       11.41 &        2.15 &        2.37 &       14.99 &        1.77 &        1.88 &        0.58 &   0.13 &   0.15 &   1.32 &   0.22 &   0.23\\
   51 &   160.83580 &    58.89789 &       0.690 &       0.448 &        0.44 &        0.15 &        0.33 &       13.78 &        2.80 &        3.42 &       12.67 &        2.47 &        2.74 &        4.48 &   1.79 &   3.50 &   0.04 &   0.70 &   0.36\\
   52 &   160.83713 &    58.89671 &       0.726 &       0.315 &        0.66 &        0.23 &        0.32 &        9.64 &        2.20 &        2.76 &        8.95 &        1.78 &        2.17 &        2.44 &   1.01 &   1.39 &   0.45 &   0.28 &   0.20\\
   53 &   160.83763 &    59.03198 &       0.274 &       0.167 &        7.94 &        0.81 &        0.94 &       19.36 &        2.65 &        3.04 &       26.55 &        2.30 &        2.41 &        0.60 &   0.10 &   0.12 &   1.29 &   0.17 &   0.17\\
   54 &   160.83889 &    59.16201 &       0.022 &       0.012 &       65.11 &        2.28 &        2.36 &      145.23 &        7.03 &        7.21 &      211.33 &        6.00 &        6.17 &        0.56 &   0.03 &   0.03 &   1.36 &   0.06 &   0.06\\
   55 &   160.84052 &    59.11883 &       0.173 &       0.101 &        2.10 &        0.43 &        0.48 &        3.42 &        1.02 &        1.37 &        5.13 &        0.92 &        1.01 &        0.44 &   0.16 &   0.20 &   1.56 &   0.34 &   0.39\\
   56 &   160.84118 &    59.21516 &       0.105 &       0.053 &       13.80 &        1.36 &        1.58 &       18.24 &        2.96 &        3.79 &       33.03 &        2.91 &        3.04 &        0.38 &   0.07 &   0.09 &   1.69 &   0.17 &   0.18\\
   57 &   160.84169 &    58.82230 &       0.549 &       0.448 &        7.33 &        0.91 &        0.97 &        8.21 &        1.63 &        2.21 &       14.96 &        1.61 &        1.79 &        0.33 &   0.08 &   0.10 &   1.80 &   0.23 &   0.22\\
   58 &   160.84202 &    59.11370 &       0.170 &       0.189  &$<$        0.06 &         -99 &         -99 &        8.78 &        2.53 &        2.94 &       10.47 &        2.52 &        3.20  &$>$       16.28 & -99.00\\
   59 &   160.84460 &    58.99873 &       0.467 &       0.231 &        6.78 &        0.87 &        1.06 &        3.78 &        1.13 &        1.52 &       10.60 &        1.27 &        1.44 &        0.20 &   0.06 &   0.08 &   2.19 &   0.25 &   0.19\\
   60 &   160.84587 &    59.27148 &       0.418 &       0.302 &        1.82 &        0.39 &        0.53 &        2.30 &        0.80 &        1.37 &        4.17 &        0.81 &        0.99 &        0.36 &   0.15 &   0.24 &   1.72 &   0.44 &   0.42\\
   61 &   160.84692 &    59.04816 &       0.538 &       0.371 &        2.15 &        0.42 &        0.56 &        6.93 &        1.67 &        2.12 &        8.04 &        1.24 &        1.71 &        0.74 &   0.23 &   0.30 &   1.10 &   0.30 &   0.34\\
   62 &   160.84777 &    58.88010 &       0.394 &       0.230 &        1.03 &        0.32 &        0.44 &        1.99 &        0.87 &        1.34 &        3.31 &        0.78 &        1.12 &        0.50 &   0.27 &   0.40 &   1.45 &   0.52 &   0.63\\
   63 &   160.85231 &    59.16584 &       0.201 &       0.121 &        0.54 &        0.22 &        0.32 &        0.44 &        0.40 &        0.52 &        1.09 &        0.40 &        0.49 &        0.26 &   0.26 &   0.35 &   2.00 &   0.73 &   0.76\\
   64 &   160.85428 &    59.28599 &       0.952 &       0.230 &        0.19 &        0.14 &        0.16 &        4.99 &        1.73 &        2.08 &        6.32 &        1.77 &        1.82 &        3.87 &   3.13 &   3.67 &   0.16 &   0.73 &   0.93\\
   65 &   160.86171 &    58.91735 &       0.397 &       0.305 &        1.34 &        0.37 &        0.43 &        2.22 &        0.94 &        1.18 &        3.93 &        0.87 &        0.97 &        0.45 &   0.23 &   0.28 &   1.54 &   0.43 &   0.57\\
   66 &   160.86418 &    59.09240 &       0.233 &       0.325 &        0.91 &        0.26 &        0.40 &        1.43 &        0.53 &        1.23 &        2.42 &        0.54 &        0.87 &        0.43 &   0.20 &   0.41 &   1.58 &   0.58 &   0.52\\
   67 &   160.87135 &    58.96578 &       0.403 &       0.339 &        0.74 &        0.22 &        0.40 &        9.06 &        2.02 &        2.84 &        8.60 &        1.57 &        2.30 &        2.10 &   0.77 &   1.31 &   0.52 &   0.26 &   0.15\\
   68 &   160.88223 &    58.87707 &       0.400 &       0.357 &        0.68 &        0.22 &        0.37 &        9.85 &        2.14 &        2.99 &        9.63 &        1.73 &        2.51 &        2.42 &   0.95 &   1.50 &   0.46 &   0.30 &   0.19\\
   69 &   160.88411 &    59.06132 &       0.339 &       0.276 &        4.53 &        0.63 &        0.77 &       12.24 &        2.31 &        2.54 &       16.55 &        1.75 &        2.18 &        0.64 &   0.15 &   0.17 &   1.21 &   0.19 &   0.25\\
   70 &   160.88443 &    58.90123 &       0.291 &       0.209 &        3.01 &        0.51 &        0.73 &        1.77 &        0.66 &        1.18 &        5.04 &        0.77 &        1.05 &        0.20 &   0.08 &   0.15 &   2.16 &   0.41 &   0.25\\
   71 &   160.88543 &    58.97429 &       0.330 &       0.181 &        5.09 &        0.78 &        0.91 &        6.02 &        1.75 &        1.80 &       10.70 &        1.35 &        1.76 &        0.35 &   0.11 &   0.12 &   1.76 &   0.25 &   0.32\\
   72 &   160.88577 &    59.12622 &       0.261 &       0.232 &        0.44 &        0.18 &        0.26  &$<$        2.98 &         -99 &         -99 &        1.83 &        0.56 &        1.08  &$<$        1.31 & -99.00\\
   73 &   160.88608 &    58.92036 &       0.513 &       0.291 &        0.45 &        0.17 &        0.39 &        0.40 &        0.36 &        0.66 &        0.68 &        0.25 &        0.58 &        0.28 &   0.27 &   0.52 &   1.94 &   0.91 &   0.80\\
   74 &   160.88756 &    58.84812 &       0.471 &       0.234 &        2.36 &        0.49 &        0.54 &       11.04 &        2.42 &        2.46 &       12.42 &        1.71 &        2.27 &        0.98 &   0.30 &   0.32 &   0.85 &   0.17 &   0.30\\
   75 &   160.88999 &    58.82788 &       1.061 &       0.535 &        0.02 &        0.02 &        0.12 &        1.89 &        0.97 &        2.18 &        2.85 &        1.06 &        2.45 &       11.15 &  12.53 &  71.43 &  -1.29 &   2.11 &   8.09\\
   76 &   160.89210 &    59.02476 &       0.412 &       0.202 &        1.98 &        0.43 &        0.53 &        5.11 &        1.33 &        1.98 &        7.05 &        1.22 &        1.45 &        0.62 &   0.21 &   0.29 &   1.25 &   0.33 &   0.36\\
   77 &   160.89263 &    58.93742 &       0.436 &       0.368 &        0.40 &        0.15 &        0.34  &$<$        2.68 &         -99 &         -99 &        1.72 &        0.64 &        1.15  &$<$        1.31 & -99.00\\
   78 &   160.89665 &    59.27504 &       0.596 &       0.245 &        2.65 &        0.49 &        0.64 &        2.14 &        0.74 &        1.27 &        4.97 &        0.78 &        1.08 &        0.26 &   0.10 &   0.17 &   2.00 &   0.42 &   0.30\\
   79 &   160.89784 &    58.97271 &       0.258 &       0.150 &        3.22 &        0.55 &        0.72 &        3.55 &        1.11 &        1.51 &        7.59 &        1.13 &        1.31 &        0.33 &   0.12 &   0.16 &   1.81 &   0.33 &   0.34\\
   80 &   160.89832 &    58.97812 &       0.602 &       0.445 &        0.00 &        0.00 &        0.03 &       88.37 &       32.50 &       39.51 &      145.61 &       47.86 &       66.40 &      -99.00 &******* &******* & -99.00 &   0.00 &   0.00\\
   81 &   160.89867 &    58.88039 &       0.523 &       0.321 &        0.54 &        0.23 &        0.28 &        8.32 &        2.06 &        2.64 &        7.29 &        1.74 &        1.96 &        2.56 &   1.25 &   1.58 &   0.43 &   0.32 &   0.25\\
   82 &   160.90034 &    59.28941 &       0.842 &       0.298 &        0.72 &        0.22 &        0.36 &        7.84 &        1.94 &        2.49 &        6.69 &        1.45 &        1.80 &        1.93 &   0.77 &   1.14 &   0.55 &   0.23 &   0.15\\
   83 &   160.90059 &    59.04360 &       0.472 &       0.284 &        5.93 &        0.70 &        0.84 &       10.06 &        1.93 &        2.13 &       16.69 &        1.72 &        1.81 &        0.45 &   0.10 &   0.12 &   1.53 &   0.19 &   0.21\\
   84 &   160.90695 &    59.15383 &       0.281 &       0.123 &        0.36 &        0.16 &        0.24 &        4.78 &        1.50 &        1.77 &        3.73 &        0.92 &        1.55 &        2.25 &   1.21 &   1.73 &   0.49 &   0.35 &   0.30\\
   85 &   160.90960 &    58.84660 &       0.489 &       0.509 &        0.37 &        0.14 &        0.31 &        5.41 &        1.61 &        2.17 &        4.58 &        1.26 &        1.65 &        2.46 &   1.17 &   2.33 &   0.45 &   0.47 &   0.23\\
   86 &   160.91396 &    59.03402 &       0.588 &       0.346 &        1.04 &        0.26 &        0.38 &       34.86 &        4.26 &        5.13 &       34.28 &        3.75 &        4.43 &        4.74 &   1.33 &   1.88 &  -0.01 &   0.38 &   0.26\\
   87 &   160.91398 &    58.88324 &       0.406 &       0.186 &        0.70 &        0.21 &        0.41  &$<$        2.23 &         -99 &         -99 &        1.94 &        0.56 &        1.05  &$<$        0.73 & -99.00\\
   88 &   160.91765 &    59.05128 &       0.847 &       0.503 &        1.24 &        0.46 &        0.67  &$<$        9.68 &         -99 &         -99 &        5.02 &        1.75 &        2.47  &$<$        1.48 & -99.00\\
   89 &   160.91836 &    58.92191 &       0.260 &       0.134 &        0.37 &        0.14 &        0.32 &        1.94 &        0.79 &        1.48 &        1.07 &        0.55 &        0.73 &        1.08 &   0.59 &   1.24 &   0.75 &   0.28 &   0.73\\
   90 &   160.92204 &    59.00601 &       0.521 &       0.250 &        1.69 &        0.40 &        0.50 &        3.49 &        1.21 &        1.45 &        4.69 &        0.99 &        1.10 &        0.53 &   0.22 &   0.27 &   1.41 &   0.37 &   0.46\\
   91 &   160.92223 &    59.28174 &       0.869 &       0.395 &        1.03 &        0.29 &        0.45 &        1.69 &        0.91 &        1.00 &        2.86 &        0.80 &        0.82 &        0.44 &   0.27 &   0.32 &   1.56 &   0.48 &   0.71\\
   92 &   160.92290 &    59.21508 &       0.208 &       0.107 &        0.42 &        0.18 &        0.28 &        0.73 &        0.51 &        0.77 &        1.77 &        0.53 &        0.71 &        0.46 &   0.38 &   0.58 &   1.52 &   0.73 &   1.01\\
   93 &   160.92299 &    59.29877 &       0.633 &       0.191 &        8.09 &        0.85 &        0.99 &       12.37 &        1.93 &        2.68 &       20.69 &        1.85 &        2.11 &        0.42 &   0.08 &   0.10 &   1.59 &   0.18 &   0.18\\
   94 &   160.92740 &    58.89198 &       0.263 &       0.189 &        1.92 &        0.46 &        0.52 &        2.78 &        0.91 &        1.50 &        5.01 &        0.85 &        1.22 &        0.40 &   0.16 &   0.24 &   1.62 &   0.42 &   0.44\\
   95 &   160.92858 &    58.89191 &       0.322 &       0.135 &        1.50 &        0.38 &        0.50 &        2.36 &        0.76 &        1.55 &        4.17 &        0.86 &        1.06 &        0.43 &   0.18 &   0.31 &   1.58 &   0.48 &   0.45\\
   96 &   160.92890 &    58.84012 &       0.497 &       0.426 &        1.84 &        0.49 &        0.86 &        0.06 &        0.06 &        0.39 &        1.23 &        0.32 &        0.44 &        0.02 &   0.02 &   0.15 &   2.69 &   0.44 &   0.07\\
   97 &   160.92968 &    59.13275 &       0.271 &       0.156 &        0.76 &        0.24 &        0.38 &        1.32 &        0.64 &        1.04 &        2.24 &        0.53 &        0.88 &        0.46 &   0.26 &   0.43 &   1.52 &   0.58 &   0.67\\
   98 &   160.92994 &    58.92665 &       0.050 &       0.031 &       25.50 &        1.53 &        1.58 &       48.62 &        4.14 &        4.50 &       75.20 &        3.57 &        3.93 &        0.49 &   0.05 &   0.06 &   1.46 &   0.09 &   0.09\\
   99 &   160.93163 &    58.85179 &       0.548 &       0.269 &        0.81 &        0.24 &        0.37 &        5.31 &        1.30 &        2.20 &        6.21 &        1.23 &        1.67 &        1.28 &   0.49 &   0.80 &   0.68 &   0.16 &   0.36\\
  100 &   160.93191 &    59.23844 &       0.478 &       0.105 &        0.47 &        0.17 &        0.31 &        5.01 &        1.33 &        2.34 &        4.13 &        1.07 &        1.60 &        1.90 &   0.87 &   1.55 &   0.56 &   0.31 &   0.24\\
  101 &   160.93205 &    58.83646 &       0.558 &       0.450 &        1.38 &        0.40 &        0.46 &        1.04 &        0.61 &        0.85 &        2.58 &        0.55 &        0.86 &        0.25 &   0.16 &   0.22 &   2.04 &   0.53 &   0.47\\
  102 &   160.93264 &    59.14115 &       0.177 &       0.114 &        2.67 &        0.52 &        0.58 &        1.65 &        0.66 &        0.98 &        4.80 &        0.71 &        0.97 &        0.21 &   0.09 &   0.13 &   2.14 &   0.39 &   0.28\\
  103 &   160.93843 &    58.91828 &       0.134 &       0.165 &        1.93 &        0.44 &        0.63 &        0.48 &        0.29 &        0.79 &        2.21 &        0.45 &        0.68 &        0.11 &   0.07 &   0.18 &   2.45 &   0.52 &   0.20\\
  104 &   160.94535 &    58.96527 &       0.253 &       0.195 &        0.06 &        0.05 &        0.19 &        3.34 &        1.63 &        1.74 &        3.62 &        1.35 &        1.95 &        7.45 &   7.12 &  25.52 &  -0.55 &   1.44 &   2.34\\
  105 &   160.94737 &    58.70897 &       0.930 &       0.433 &        0.21 &        0.10 &        0.28 &        8.39 &        2.42 &        2.81 &        5.38 &        1.42 &        2.52 &        5.46 &   2.98 &   7.66 &  -0.15 &   1.27 &   0.59\\
  106 &   160.94892 &    59.15553 &       0.289 &       0.138 &        0.28 &        0.14 &        0.22 &        7.25 &        1.94 &        2.24 &        6.04 &        1.32 &        2.09 &        3.80 &   2.10 &   3.22 &   0.18 &   0.64 &   0.42\\
  107 &   160.95495 &    58.92739 &       0.435 &       0.088 &        0.12 &        0.11 &        0.14 &        1.37 &        0.76 &        1.33 &        1.33 &        0.68 &        0.91 &        2.04 &   2.17 &   3.13 &   0.53 &   0.63 &   2.62\\
  108 &   160.95993 &    58.66965 &       1.085 &       0.428 &        0.74 &        0.21 &        0.40 &        8.47 &        1.84 &        2.93 &        8.94 &        1.60 &        2.34 &        2.00 &   0.73 &   1.29 &   0.54 &   0.26 &   0.14\\
  109 &   160.96217 &    58.67622 &       0.480 &       0.230 &        1.89 &        0.39 &        0.61 &        2.44 &        0.80 &        1.56 &        3.80 &        0.74 &        1.11 &        0.37 &   0.14 &   0.26 &   1.71 &   0.47 &   0.40\\
  110 &   160.96328 &    58.95561 &       0.148 &       0.064 &        3.57 &        0.58 &        0.68 &        4.27 &        1.17 &        1.54 &        7.90 &        1.07 &        1.31 &        0.35 &   0.11 &   0.14 &   1.75 &   0.28 &   0.32\\
  111 &   160.96342 &    58.92903 &       0.143 &       0.067 &        3.09 &        0.54 &        0.59 &        6.06 &        1.28 &        2.01 &        9.29 &        1.23 &        1.51 &        0.50 &   0.14 &   0.19 &   1.45 &   0.31 &   0.26\\
  112 &   160.96385 &    58.82693 &       0.582 &       0.400 &        1.45 &        0.38 &        0.56 &        0.98 &        0.52 &        1.05 &        2.89 &        0.64 &        0.86 &        0.23 &   0.13 &   0.26 &   2.10 &   0.62 &   0.39\\
  113 &   160.96633 &    58.83156 &       0.362 &       0.335 &        0.43 &        0.19 &        0.29 &       29.55 &        4.24 &        5.72 &       28.05 &        4.30 &        4.65 &        8.36 &   3.84 &   5.87 &  -0.73 &   0.72 &   0.77\\
  114 &   160.97134 &    59.28917 &       0.579 &       0.227 &        6.12 &        0.73 &        0.88 &        9.17 &        1.72 &        2.28 &       16.37 &        1.59 &        1.94 &        0.41 &   0.09 &   0.12 &   1.60 &   0.20 &   0.22\\
  115 &   160.97258 &    58.75717 &       0.531 &       0.253 &        6.05 &        0.72 &        0.93 &       13.82 &        2.36 &        2.80 &       20.21 &        2.07 &        2.29 &        0.57 &   0.12 &   0.14 &   1.34 &   0.22 &   0.20\\
  116 &   160.97259 &    58.88791 &       0.095 &       0.104 &        1.25 &        0.31 &        0.40 &       14.93 &        2.37 &        3.29 &       14.67 &        2.13 &        2.47 &        2.07 &   0.61 &   0.80 &   0.52 &   0.16 &   0.12\\
  117 &   160.97363 &    58.87009 &       0.346 &       0.302 &        0.38 &        0.14 &        0.32 &        2.70 &        1.14 &        1.44 &        2.83 &        0.88 &        1.20 &        1.38 &   0.78 &   1.40 &   0.66 &   0.28 &   0.62\\
  118 &   160.97476 &    58.67874 &       0.648 &       0.358 &        1.25 &        0.33 &        0.43  &$<$        6.56 &         -99 &         -99 &        4.69 &        1.13 &        1.44  &$<$        1.08 & -99.00\\
  119 &   160.97826 &    58.98409 &       0.358 &       0.197 &        0.06 &        0.05 &        0.19 &        4.16 &        1.85 &        1.97 &        6.43 &        1.64 &        2.83 &        8.90 &   8.32 &  30.40 &  -0.84 &   1.33 &   2.16\\
  120 &   160.97900 &    58.82487 &       0.972 &       0.523 &        0.46 &        0.20 &        0.31 &        2.37 &        1.10 &        1.41 &        3.82 &        0.96 &        1.41 &        1.06 &   0.68 &   0.96 &   0.77 &   0.23 &   0.90\\
  121 &   160.97952 &    59.05154 &       0.296 &       0.179 &       18.10 &        1.40 &        1.45 &       28.48 &        3.33 &        3.74 &       46.15 &        2.91 &        3.20 &        0.43 &   0.06 &   0.07 &   1.58 &   0.11 &   0.13\\
  122 &   160.98063 &    59.01704 &       0.516 &       0.267 &        2.59 &        0.69 &        0.80 &        4.20 &        1.78 &        2.24 &        6.03 &        1.25 &        1.93 &        0.44 &   0.22 &   0.27 &   1.56 &   0.43 &   0.57\\
  123 &   160.98350 &    58.74237 &       0.610 &       0.275 &        0.31 &        0.14 &        0.28  &$<$       11.39 &         -99 &         -99 &        2.47 &        1.08 &        1.66  &$<$        5.05 & -99.00\\
  124 &   160.98728 &    58.91819 &       0.224 &       0.096 &        0.82 &        0.27 &        0.38 &        4.38 &        1.21 &        2.19 &        5.39 &        1.17 &        1.63 &        1.09 &   0.47 &   0.74 &   0.74 &   0.17 &   0.51\\
  125 &   160.98892 &    58.82512 &       0.338 &       0.302 &        3.91 &        0.63 &        0.80 &        2.08 &        0.72 &        1.23 &        5.85 &        0.87 &        1.09 &        0.19 &   0.07 &   0.12 &   2.21 &   0.35 &   0.21\\
  126 &   160.99054 &    58.86350 &       0.234 &       0.167 &        1.27 &        0.31 &        0.40 &       14.74 &        2.37 &        3.31 &       14.65 &        2.00 &        2.65 &        2.03 &   0.60 &   0.79 &   0.53 &   0.16 &   0.12\\
  127 &   160.99898 &    58.79449 &       0.606 &       0.510 &        1.18 &        0.30 &        0.44  &$<$        9.77 &         -99 &         -99 &        4.46 &        1.03 &        1.68  &$<$        1.55 & -99.00\\
  128 &   161.00180 &    58.97927 &       0.116 &       0.056 &        4.71 &        0.64 &        0.73 &       12.87 &        2.12 &        2.72 &       17.59 &        1.88 &        2.09 &        0.65 &   0.14 &   0.17 &   1.20 &   0.19 &   0.23\\
  129 &   161.00246 &    58.86944 &       0.170 &       0.241 &        0.63 &        0.25 &        0.37 &        0.92 &        0.43 &        1.25 &        1.06 &        0.39 &        0.70 &        0.41 &   0.25 &   0.60 &   1.62 &   0.80 &   0.69\\
  130 &   161.00255 &    59.11346 &       0.312 &       0.168 &        2.07 &        0.39 &        0.52 &        8.05 &        1.63 &        2.22 &        9.85 &        1.40 &        1.74 &        0.85 &   0.24 &   0.32 &   0.98 &   0.28 &   0.28\\
  131 &   161.00533 &    58.96715 &       0.000 &       0.000 &        0.30 &        0.13 &        0.27  &$<$        3.06 &         -99 &         -99 &        0.69 &        0.48 &        0.73  &$<$        1.84 & -99.00\\
  132 &   161.00544 &    58.99524 &       0.338 &       0.174 &        0.89 &        0.39 &        0.60 &        0.37 &        0.30 &        1.25 &        1.20 &        0.45 &        0.80 &        0.16 &   0.15 &   0.54 &   2.30 &   1.17 &   0.43\\
  133 &   161.00734 &    58.87467 &       0.235 &       0.185 &        0.08 &        0.07 &        0.19 &        2.91 &        1.27 &        1.96 &        4.13 &        1.36 &        1.88 &        4.87 &   4.72 &  11.60 &  -0.03 &   1.48 &   2.36\\
  134 &   161.01524 &    58.98407 &       0.176 &       0.102 &        1.13 &        0.37 &        0.44 &        3.00 &        1.27 &        1.59 &        4.45 &        0.94 &        1.48 &        0.63 &   0.34 &   0.42 &   1.23 &   0.45 &   0.67\\
  135 &   161.01655 &    59.02623 &       0.593 &       0.177 &        0.60 &        0.18 &        0.36 &       11.86 &        2.62 &        2.94 &       12.35 &        2.09 &        2.71 &        3.08 &   1.16 &   1.97 &   0.32 &   0.39 &   0.23\\
  136 &   161.01667 &    59.04503 &       0.150 &       0.060 &       33.59 &        1.79 &        1.94 &       49.20 &        4.15 &        4.71 &       83.07 &        3.75 &        4.10 &        0.41 &   0.04 &   0.04 &   1.62 &   0.08 &   0.10\\
  137 &   161.01802 &    59.15030 &       0.535 &       0.320 &        0.60 &        0.22 &        0.32 &        7.23 &        1.72 &        2.85 &        5.95 &        1.30 &        2.06 &        2.08 &   0.38 &   0.51 &   0.52 &   0.10 &   0.08\\
  138 &   161.01886 &    59.29741 &       1.110 &       0.416 &        3.01 &        0.52 &        0.67 &        3.67 &        1.21 &        1.44 &        6.69 &        1.05 &        1.23 &        0.35 &   0.13 &   0.16 &   1.74 &   0.31 &   0.37\\
  139 &   161.02037 &    58.98455 &       0.203 &       0.095 &        0.85 &        0.26 &        0.36 &        8.33 &        2.01 &        2.55 &        7.94 &        1.45 &        2.13 &        1.78 &   0.70 &   0.93 &   0.58 &   0.19 &   0.17\\
  140 &   161.02091 &    58.75939 &       0.691 &       0.415 &        0.75 &        0.23 &        0.44 &        1.23 &        0.72 &        1.01 &        2.07 &        0.62 &        0.83 &        0.44 &   0.29 &   0.45 &   1.55 &   0.61 &   0.77\\
  141 &   161.02100 &    58.89289 &       0.188 &       0.123 &        1.08 &        0.31 &        0.41 &        1.51 &        0.61 &        1.15 &        2.38 &        0.64 &        0.73 &        0.39 &   0.19 &   0.33 &   1.65 &   0.54 &   0.54\\
  142 &   161.02355 &    59.09052 &       0.183 &       0.107 &       16.90 &        1.21 &        1.40 &       18.55 &        2.29 &        2.95 &       35.54 &        2.32 &        2.47 &        0.33 &   0.05 &   0.06 &   1.81 &   0.14 &   0.13\\
  143 &   161.02597 &    58.98735 &       0.244 &       0.087 &        2.96 &        0.60 &        0.82 &        0.34 &        0.30 &        0.55 &        2.85 &        0.57 &        0.63 &        0.06 &   0.05 &   0.10 &   2.59 &   0.29 &   0.16\\
  144 &   161.02635 &    58.66525 &       0.366 &       0.292 &        0.53 &        0.17 &        0.35 &       12.48 &        2.37 &        3.53 &       11.04 &        1.95 &        2.82 &        3.57 &   1.34 &   2.55 &   0.22 &   0.51 &   0.27\\
  145 &   161.02643 &    59.03490 &       0.256 &       0.097 &        9.23 &        0.97 &        1.03 &       18.18 &        2.48 &        3.28 &       27.79 &        2.35 &        2.55 &        0.51 &   0.09 &   0.11 &   1.44 &   0.18 &   0.15\\
  146 &   161.02785 &    58.85869 &       0.314 &       0.377 &        0.66 &        0.20 &        0.39  &$<$        4.78 &         -99 &         -99 &        3.33 &        1.04 &        1.23  &$<$        1.38 & -99.00\\
  147 &   161.02831 &    59.15977 &       0.490 &       0.215 &        0.98 &        0.26 &        0.40 &        2.72 &        0.89 &        1.47 &        3.07 &        0.76 &        0.97 &        0.66 &   0.28 &   0.45 &   1.18 &   0.47 &   0.49\\
  148 &   161.02966 &    58.93697 &       0.082 &       0.042 &        4.96 &        0.69 &        0.74 &        6.26 &        1.43 &        1.79 &       11.38 &        1.36 &        1.45 &        0.36 &   0.10 &   0.12 &   1.72 &   0.23 &   0.27\\
  149 &   161.03033 &    58.94361 &       0.163 &       0.084 &        0.39 &        0.18 &        0.35  &$<$        3.39 &         -99 &         -99 &        2.37 &        1.00 &        1.26  &$<$        1.61 & -99.00\\
  150 &   161.03242 &    58.67003 &       0.697 &       0.372 &        0.00 &        0.00 &        0.03 &      119.55 &       29.88 &       48.70 &      162.07 &       50.84 &       59.94 &      -99.00 &******* &******* & -99.00 &   0.00 &   0.00\\
  151 &   161.03335 &    58.74364 &       0.301 &       0.206 &        1.94 &        0.41 &        0.51 &       15.60 &        2.51 &        3.50 &       15.49 &        2.12 &        2.60 &        1.51 &   0.40 &   0.52 &   0.64 &   0.10 &   0.08\\
  152 &   161.03389 &    58.99061 &       0.161 &       0.073 &        5.10 &        0.68 &        0.89 &        4.88 &        1.36 &        1.57 &       10.15 &        1.23 &        1.48 &        0.29 &   0.09 &   0.11 &   1.90 &   0.28 &   0.27\\
  153 &   161.03908 &    59.00069 &       0.205 &       0.072 &        3.90 &        0.58 &        0.73 &        8.19 &        1.66 &        2.26 &       11.85 &        1.47 &        1.78 &        0.53 &   0.13 &   0.18 &   1.40 &   0.27 &   0.23\\
  154 &   161.04144 &    58.87354 &       0.206 &       0.174  &$<$        0.16 &         -99 &         -99 &        6.30 &        2.07 &        2.14 &        5.06 &        1.59 &        1.87  &$>$        5.49 & -99.00\\
  155 &   161.04176 &    58.98028 &       0.326 &       0.199 &        0.34 &        0.16 &        0.27 &        1.02 &        0.52 &        1.17 &        1.02 &        0.44 &        0.69 &        0.70 &   0.49 &   0.98 &   1.13 &   0.53 &   1.02\\
  156 &   161.04629 &    58.90686 &       0.090 &       0.049 &        6.21 &        0.74 &        0.88 &        9.06 &        1.80 &        2.00 &       15.27 &        1.62 &        1.71 &        0.40 &   0.09 &   0.11 &   1.62 &   0.18 &   0.23\\
  157 &   161.04686 &    58.87419 &       0.326 &       0.190 &        0.46 &        0.16 &        0.34 &        1.46 &        0.71 &        1.15 &        1.28 &        0.54 &        0.68 &        0.73 &   0.43 &   0.79 &   1.11 &   0.47 &   0.79\\
  158 &   161.04778 &    59.10781 &       0.937 &       0.327 &        0.92 &        0.23 &        0.40 &        5.56 &        1.68 &        1.73 &        5.81 &        1.10 &        1.64 &        1.20 &   0.47 &   0.65 &   0.70 &   0.13 &   0.41\\
  159 &   161.04900 &    58.88629 &       0.212 &       0.092 &        1.53 &        0.32 &        0.51 &        4.57 &        1.37 &        1.61 &        5.57 &        1.02 &        1.35 &        0.70 &   0.26 &   0.34 &   1.14 &   0.35 &   0.41\\
  160 &   161.05044 &    58.91619 &       0.164 &       0.108 &        0.39 &        0.23 &        0.32 &        7.01 &        2.52 &        2.73 &        5.80 &        1.54 &        2.71 &        2.89 &   1.99 &   2.62 &   0.36 &   0.52 &   0.57\\
  161 &   161.05047 &    58.94237 &       0.163 &       0.086 &        0.78 &        0.24 &        0.33 &        4.82 &        1.38 &        1.83 &        5.24 &        1.09 &        1.49 &        1.22 &   0.52 &   0.70 &   0.69 &   0.14 &   0.44\\
  162 &   161.05120 &    58.82482 &       0.562 &       0.480 &        2.60 &        0.68 &        0.77 &        0.22 &        0.18 &        0.75 &        2.24 &        0.45 &        0.69 &        0.05 &   0.04 &   0.16 &   2.62 &   0.48 &   0.12\\
  163 &   161.05189 &    58.53875 &       0.602 &       0.518 &        7.11 &        0.82 &        0.98 &       15.90 &        2.48 &        3.14 &       23.00 &        2.18 &        2.52 &        0.56 &   0.11 &   0.13 &   1.36 &   0.21 &   0.18\\
  164 &   161.05296 &    59.27520 &       0.734 &       0.414 &        1.49 &        0.36 &        0.53 &        3.56 &        1.31 &        1.59 &        5.71 &        1.18 &        1.31 &        0.59 &   0.26 &   0.33 &   1.31 &   0.40 &   0.50\\
  165 &   161.05334 &    59.22538 &       0.507 &       0.166 &        5.53 &        0.70 &        0.91 &        3.19 &        1.10 &        1.14 &        8.47 &        1.09 &        1.17 &        0.20 &   0.07 &   0.08 &   2.17 &   0.23 &   0.22\\
  166 &   161.05512 &    58.87644 &       0.381 &       0.216 &        0.22 &        0.15 &        0.29 &        0.07 &        0.07 &        0.43 &        0.49 &        0.25 &        0.34 &        0.13 &   0.15 &   0.81 &   2.40 &   1.50 &   0.44\\
  167 &   161.05753 &    58.92745 &       0.000 &       0.174 &        1.32 &        0.53 &        0.79 &        0.85 &        0.76 &        1.38 &        3.28 &        0.92 &        1.42 &        0.22 &   0.21 &   0.38 &   2.12 &   0.83 &   0.63\\
  168 &   161.05767 &    58.92720 &       0.225 &       0.171 &        0.91 &        0.44 &        0.72 &        4.77 &        1.94 &        3.64 &        5.55 &        1.72 &        2.76 &        1.07 &   0.68 &   1.17 &   0.76 &   0.27 &   0.89\\
  169 &   161.05855 &    59.13757 &       0.443 &       0.185 &        2.77 &        0.50 &        0.55 &        9.15 &        1.75 &        2.33 &       12.10 &        1.63 &        1.75 &        0.75 &   0.20 &   0.24 &   1.08 &   0.25 &   0.28\\
  170 &   161.06468 &    58.72153 &       0.195 &       0.114 &        1.45 &        0.31 &        0.48 &       15.84 &        2.75 &        3.26 &       16.92 &        2.27 &        2.78 &        1.93 &   0.53 &   0.75 &   0.55 &   0.15 &   0.11\\
  171 &   161.06532 &    58.99193 &       0.314 &       0.124 &        0.94 &        0.29 &        0.47 &        1.10 &        0.61 &        1.07 &        2.19 &        0.57 &        0.85 &        0.34 &   0.22 &   0.37 &   1.76 &   0.65 &   0.63\\
  172 &   161.06578 &    59.01703 &       0.112 &       0.042 &       30.26 &        1.65 &        1.84 &       45.30 &        3.90 &        4.45 &       75.92 &        3.52 &        3.87 &        0.41 &   0.04 &   0.05 &   1.60 &   0.08 &   0.10\\
  173 &   161.06940 &    58.91270 &       0.316 &       0.112 &        0.15 &        0.10 &        0.20 &        3.73 &        1.14 &        2.21 &        2.49 &        1.11 &        1.18 &        3.68 &   2.68 &   5.30 &   0.20 &   1.06 &   0.63\\
  174 &   161.07033 &    58.91063 &       0.200 &       0.159 &        0.02 &        0.02 &        0.10 &       10.94 &        2.60 &        4.32 &        7.80 &        2.30 &        3.61 &       53.01 &  54.49 & 334.80 &  -2.56 &   9.55 &   9.65\\
  175 &   161.07073 &    59.00471 &       0.393 &       0.107 &        2.85 &        0.52 &        0.68 &        2.94 &        0.85 &        1.59 &        6.52 &        1.03 &        1.20 &        0.31 &   0.11 &   0.18 &   1.85 &   0.39 &   0.31\\
  176 &   161.07128 &    58.93590 &       0.180 &       0.109 &        0.59 &        0.20 &        0.35  &$<$        2.17 &         -99 &         -99 &        1.87 &        0.69 &        0.84  &$<$        0.82 & -99.00\\
  177 &   161.07319 &    58.69225 &       0.230 &       0.108 &        1.68 &        0.34 &        0.52 &        6.70 &        1.46 &        2.32 &        9.18 &        1.46 &        1.72 &        0.87 &   0.26 &   0.40 &   0.96 &   0.28 &   0.30\\
  178 &   161.07573 &    59.11184 &       0.573 &       0.340 &        5.10 &        0.70 &        0.87 &        2.70 &        0.89 &        1.23 &        8.03 &        0.97 &        1.24 &        0.19 &   0.07 &   0.09 &   2.21 &   0.27 &   0.20\\
  179 &   161.07687 &    58.57561 &       0.693 &       0.382 &        4.26 &        0.67 &        0.72 &        7.57 &        1.61 &        2.22 &       12.31 &        1.54 &        1.74 &        0.47 &   0.12 &   0.16 &   1.51 &   0.27 &   0.25\\
  180 &   161.07744 &    58.67035 &       0.229 &       0.168 &        1.22 &        0.40 &        0.66 &        0.67 &        0.37 &        1.40 &        2.12 &        0.56 &        0.99 &        0.20 &   0.12 &   0.42 &   2.19 &   0.93 &   0.36\\
  181 &   161.08138 &    58.94064 &       0.000 &       0.000 &        0.57 &        0.20 &        0.34 &        1.29 &        0.58 &        1.17 &        1.30 &        0.51 &        0.63 &        0.56 &   0.32 &   0.61 &   1.35 &   0.64 &   0.70\\
  182 &   161.08433 &    58.66336 &       0.146 &       0.105 &        2.26 &        0.39 &        0.56 &       18.10 &        2.95 &        3.20 &       18.08 &        2.35 &        2.52 &        1.50 &   0.36 &   0.46 &   0.64 &   0.09 &   0.07\\
  183 &   161.08620 &    58.97542 &       0.300 &       0.112 &        0.55 &        0.19 &        0.32 &        3.55 &        1.03 &        1.92 &        3.13 &        0.85 &        1.28 &        1.28 &   0.58 &   1.03 &   0.68 &   0.20 &   0.45\\
  184 &   161.08865 &    59.12981 &       0.667 &       0.294 &        0.57 &        0.24 &        0.30 &        0.95 &        0.48 &        1.09 &        2.44 &        0.68 &        0.78 &        0.45 &   0.30 &   0.56 &   1.55 &   0.73 &   0.78\\
  185 &   161.08935 &    58.90607 &       0.262 &       0.136 &        0.07 &        0.06 &        0.16 &        7.17 &        1.83 &        3.15 &        7.70 &        2.22 &        2.58 &       11.32 &  10.21 &  26.36 &  -1.32 &   0.80 &   2.05\\
  186 &   161.09074 &    59.12917 &       1.063 &       0.296 &        0.56 &        0.24 &        0.30 &        1.14 &        0.67 &        0.93 &        1.31 &        0.51 &        0.63 &        0.52 & -99.00 & -99.00 &   1.42 &-289.79 &  -5.30\\
  187 &   161.09193 &    59.13446 &       0.637 &       0.533 &        1.64 &        0.39 &        0.56 &        1.76 &        0.71 &        1.34 &        4.01 &        0.87 &        0.97 &        0.32 &   0.15 &   0.27 &   1.83 &   0.52 &   0.44\\
  188 &   161.09421 &    59.21788 &       0.157 &       0.063 &       48.39 &        2.06 &        2.15 &      110.14 &        6.19 &        6.94 &      158.20 &        5.49 &        5.68 &        0.57 &   0.04 &   0.04 &   1.34 &   0.07 &   0.07\\
  189 &   161.09534 &    59.29719 &       0.805 &       0.614 &        1.34 &        0.39 &        0.45 &        2.11 &        0.73 &        1.56 &        4.20 &        0.93 &        1.04 &        0.43 &   0.19 &   0.35 &   1.58 &   0.52 &   0.50\\
  190 &   161.09851 &    58.89168 &       0.266 &       0.152 &        1.02 &        0.27 &        0.42  &$<$        2.68 &         -99 &         -99 &        2.96 &        0.79 &        0.91  &$<$        0.63 & -99.00\\
  191 &   161.10040 &    58.74766 &       0.379 &       0.330 &        1.02 &        0.30 &        0.47  &$<$        2.77 &         -99 &         -99 &        2.62 &        0.74 &        1.13  &$<$        0.65 & -99.00\\
  192 &   161.10114 &    58.77508 &       0.478 &       0.210 &        1.35 &        0.34 &        0.50 &        2.16 &        0.81 &        1.44 &        3.68 &        0.82 &        1.02 &        0.43 &   0.20 &   0.33 &   1.57 &   0.49 &   0.50\\
  193 &   161.10153 &    58.76086 &       0.336 &       0.174 &        0.51 &        0.21 &        0.31 &        3.81 &        1.40 &        1.71 &        4.09 &        1.03 &        1.51 &        1.42 &   0.77 &   1.06 &   0.66 &   0.21 &   0.55\\
  194 &   161.10264 &    58.76079 &       0.459 &       0.222 &        0.30 &        0.12 &        0.31 &        2.33 &        1.02 &        1.57 &        2.87 &        0.79 &        1.44 &        1.47 &   0.88 &   1.83 &   0.64 &   0.37 &   0.66\\
  195 &   161.10558 &    58.78256 &       0.397 &       0.235 &        1.99 &        0.39 &        0.58 &       10.97 &        2.27 &        2.79 &       12.58 &        1.91 &        2.22 &        1.11 &   0.32 &   0.43 &   0.72 &   0.09 &   0.32\\
  196 &   161.10586 &    58.77938 &       0.593 &       0.358 &        0.64 &        0.22 &        0.38 &        1.50 &        0.67 &        1.36 &        2.26 &        0.65 &        0.95 &        0.58 &   0.33 &   0.63 &   1.32 &   0.62 &   0.71\\
  197 &   161.10642 &    58.74219 &       0.404 &       0.209 &        0.20 &        0.09 &        0.28 &        4.14 &        1.35 &        2.24 &        3.74 &        1.03 &        1.88 &        3.19 &   1.81 &   4.68 &   0.30 &   0.94 &   0.36\\
  198 &   161.10661 &    58.61005 &       0.436 &       0.323 &        1.34 &        0.35 &        0.46 &        5.54 &        1.58 &        2.10 &        6.83 &        1.36 &        1.66 &        0.89 &   0.35 &   0.46 &   0.94 &   0.27 &   0.44\\
  199 &   161.10831 &    58.67323 &       0.258 &       0.134 &        0.80 &        0.36 &        0.73 &        2.55 &        1.86 &        2.17 &        3.68 &        1.19 &        2.41 &        0.73 &   0.63 &   0.91 &   1.10 &   0.49 &   1.35\\
  200 &   161.11428 &    58.98371 &       0.147 &       0.052 &        8.72 &        0.88 &        1.08 &        7.71 &        1.63 &        1.82 &       16.75 &        1.61 &        1.69 &        0.28 &   0.07 &   0.07 &   1.95 &   0.20 &   0.19\\
  201 &   161.11648 &    59.23492 &       0.745 &       0.379 &        1.68 &        0.37 &        0.58 &        2.75 &        1.02 &        1.48 &        4.63 &        0.94 &        1.15 &        0.44 &   0.19 &   0.28 &   1.56 &   0.44 &   0.47\\
  202 &   161.11838 &    59.26152 &       0.379 &       0.264 &        2.50 &        0.49 &        0.54 &       12.58 &        2.55 &        2.58 &       14.60 &        2.05 &        2.18 &        1.04 &   0.29 &   0.31 &   0.79 &   0.12 &   0.30\\
  203 &   161.11941 &    58.90862 &       0.136 &       0.074 &        3.70 &        0.55 &        0.69 &        7.82 &        1.55 &        2.10 &       11.49 &        1.35 &        1.73 &        0.54 &   0.13 &   0.18 &   1.39 &   0.27 &   0.23\\
  204 &   161.12007 &    58.85532 &       0.211 &       0.120 &        6.45 &        0.78 &        0.88 &        9.59 &        1.73 &        2.28 &       16.65 &        1.64 &        1.90 &        0.41 &   0.09 &   0.11 &   1.61 &   0.19 &   0.22\\
  205 &   161.12371 &    59.25950 &       0.311 &       0.177 &        3.77 &        0.58 &        0.70 &       10.68 &        1.88 &        2.72 &       14.47 &        1.83 &        1.94 &        0.67 &   0.16 &   0.21 &   1.17 &   0.22 &   0.26\\
  206 &   161.12578 &    58.70658 &       0.095 &       0.051 &        6.60 &        0.79 &        0.89 &        7.52 &        1.43 &        2.13 &       13.62 &        1.42 &        1.67 &        0.34 &   0.08 &   0.11 &   1.79 &   0.23 &   0.22\\
  207 &   161.12683 &    58.57530 &       0.782 &       0.648 &        0.47 &        0.24 &        0.32 &        1.31 &        0.67 &        1.51 &        3.08 &        0.83 &        1.26 &        0.66 &   0.48 &   0.88 &   1.18 &   0.55 &   1.05\\
  208 &   161.12749 &    58.85371 &       0.685 &       0.285 &        0.60 &        0.24 &        0.29 &        6.15 &        1.79 &        2.04 &        6.06 &        1.45 &        1.62 &        1.84 &   0.90 &   1.07 &   0.57 &   0.21 &   0.32\\
  209 &   161.12834 &    58.85313 &       0.754 &       0.482 &        0.63 &        0.19 &        0.37 &        3.55 &        1.35 &        1.48 &        4.15 &        0.98 &        1.40 &        1.13 &   0.55 &   0.82 &   0.71 &   0.16 &   0.61\\
  210 &   161.12864 &    58.60245 &       0.413 &       0.364 &        1.11 &        0.28 &        0.49  &$<$        4.96 &         -99 &         -99 &        3.84 &        1.02 &        1.32  &$<$        0.95 & -99.00\\
  211 &   161.13081 &    59.09386 &       0.567 &       0.281 &        6.08 &        0.75 &        0.85 &       33.26 &        4.00 &        4.50 &       38.41 &        3.35 &        3.66 &        1.11 &   0.19 &   0.22 &   0.72 &   0.04 &   0.20\\
  212 &   161.13096 &    58.89389 &       0.367 &       0.171 &        0.72 &        0.21 &        0.39 &        2.66 &        0.99 &        1.43 &        3.20 &        0.74 &        1.20 &        0.82 &   0.38 &   0.62 &   1.02 &   0.37 &   0.55\\
  213 &   161.13222 &    59.00720 &       0.206 &       0.268 &        0.10 &        0.09 &        0.17  &$<$        6.30 &         -99 &         -99 &        0.72 &        0.64 &        1.17  &$<$        7.69 & -99.00\\
  214 &   161.13321 &    59.08251 &       0.676 &       0.237 &        5.77 &        0.73 &        0.82 &       39.37 &        4.17 &        5.19 &       44.92 &        3.60 &        4.23 &        1.32 &   0.22 &   0.26 &   0.67 &   0.05 &   0.05\\
  215 &   161.13466 &    59.17415 &       0.592 &       0.460 &        0.92 &        0.24 &        0.43 &        5.44 &        1.55 &        2.07 &        6.19 &        1.26 &        1.71 &        1.18 &   0.46 &   0.71 &   0.70 &   0.14 &   0.41\\
  216 &   161.13746 &    58.98036 &       0.159 &       0.051 &       15.21 &        1.26 &        1.37 &       13.29 &        2.02 &        2.55 &       28.64 &        2.07 &        2.31 &        0.28 &   0.05 &   0.06 &   1.96 &   0.17 &   0.14\\
  217 &   161.14091 &    59.18638 &       0.681 &       0.309 &        1.82 &        0.46 &        0.52 &        2.76 &        1.02 &        1.48 &        4.30 &        0.95 &        1.06 &        0.42 &   0.19 &   0.25 &   1.60 &   0.43 &   0.50\\
  218 &   161.14292 &    58.72850 &       0.312 &       0.119 &        0.41 &        0.18 &        0.28 &        3.26 &        1.28 &        1.58 &        3.71 &        0.97 &        1.44 &        1.50 &   0.88 &   1.24 &   0.64 &   0.25 &   0.62\\
  219 &   161.14374 &    59.20588 &       0.865 &       0.435 &        0.13 &        0.08 &        0.22 &        3.78 &        1.49 &        1.83 &        2.34 &        0.87 &        1.56 &        4.17 &   0.92 &   1.39 &   0.10 &   0.28 &   0.18\\
  220 &   161.14463 &    58.82127 &       0.699 &       0.445 &        2.18 &        0.47 &        0.52 &        5.16 &        1.49 &        1.73 &        7.15 &        1.20 &        1.42 &        0.58 &   0.21 &   0.24 &   1.31 &   0.30 &   0.38\\
  221 &   161.14582 &    58.76728 &       0.263 &       0.116 &        5.83 &        0.72 &        0.93 &        6.16 &        1.31 &        2.05 &       11.92 &        1.39 &        1.56 &        0.32 &   0.08 &   0.12 &   1.84 &   0.27 &   0.23\\
  222 &   161.14934 &    59.00559 &       0.697 &       0.245 &        0.86 &        0.28 &        0.34 &        5.73 &        1.57 &        2.07 &        5.70 &        1.32 &        1.49 &        1.30 &   0.56 &   0.69 &   0.68 &   0.14 &   0.42\\
  223 &   161.15109 &    58.81445 &       0.569 &       0.267 &        8.40 &        1.01 &        1.08 &        3.56 &        1.12 &        1.32 &       11.44 &        1.28 &        1.36 &        0.16 &   0.05 &   0.06 &   2.30 &   0.18 &   0.16\\
  224 &   161.15205 &    58.78405 &       0.733 &       0.173 &        3.30 &        0.68 &        0.94 &        4.85 &        1.69 &        2.39 &        8.32 &        1.48 &        1.94 &        0.41 &   0.16 &   0.23 &   1.61 &   0.39 &   0.44\\
  225 &   161.15509 &    58.69981 &       0.177 &       0.168 &        0.13 &        0.08 &        0.22 &        3.80 &        1.41 &        2.04 &        3.01 &        1.18 &        1.46 &        4.14 &   2.97 &   7.17 &   0.11 &   1.43 &   0.59\\
  226 &   161.15607 &    58.88528 &       0.283 &       0.149 &        1.57 &        0.37 &        0.42 &       15.11 &        2.49 &        3.19 &       15.88 &        2.26 &        2.43 &        1.74 &   0.50 &   0.60 &   0.59 &   0.12 &   0.10\\
  227 &   161.15979 &    58.98442 &       0.465 &       0.407 &        0.42 &        0.16 &        0.36 &        1.08 &        0.55 &        1.24 &        1.99 &        0.55 &        1.00 &        0.62 &   0.39 &   0.89 &   1.25 &   0.61 &   0.85\\
  228 &   161.16009 &    59.26393 &       0.662 &       0.414 &        0.58 &        0.20 &        0.34  &$<$        3.70 &         -99 &         -99 &        1.34 &        0.55 &        1.02  &$<$        1.26 & -99.00\\
  229 &   161.16025 &    59.21786 &       0.298 &       0.257 &        3.88 &        0.58 &        0.72 &        8.29 &        1.68 &        2.29 &       12.95 &        1.59 &        1.80 &        0.54 &   0.14 &   0.18 &   1.39 &   0.27 &   0.23\\
  230 &   161.16102 &    58.67290 &       0.191 &       0.121 &        0.31 &        0.14 &        0.28 &        6.30 &        1.80 &        2.39 &        6.20 &        1.46 &        2.10 &        3.17 &   1.69 &   3.12 &   0.31 &   0.62 &   0.34\\
  231 &   161.16103 &    58.61003 &       0.550 &       0.232 &        0.32 &        0.15 &        0.25 &        6.98 &        2.01 &        2.34 &        7.58 &        1.73 &        2.17 &        3.36 &   1.89 &   2.88 &   0.27 &   0.57 &   0.38\\
  232 &   161.16104 &    58.74936 &       0.181 &       0.091 &        2.88 &        0.53 &        0.59 &        5.85 &        1.64 &        1.68 &        9.06 &        1.22 &        1.62 &        0.52 &   0.17 &   0.18 &   1.42 &   0.29 &   0.34\\
  233 &   161.16464 &    59.22810 &       0.118 &       0.117 &       16.99 &        1.27 &        1.42 &       20.60 &        2.60 &        3.15 &       38.03 &        2.51 &        2.68 &        0.35 &   0.05 &   0.06 &   1.75 &   0.14 &   0.14\\
  234 &   161.17004 &    58.77317 &       0.481 &       0.154 &        2.28 &        0.47 &        0.73 &        2.69 &        1.07 &        1.60 &        4.99 &        1.01 &        1.24 &        0.34 &   0.16 &   0.23 &   1.76 &   0.44 &   0.45\\
  235 &   161.17036 &    58.56773 &       0.662 &       0.446 &        1.23 &        0.32 &        0.48 &        2.42 &        1.02 &        1.29 &        3.87 &        0.82 &        1.13 &        0.51 &   0.25 &   0.33 &   1.44 &   0.45 &   0.57\\
  236 &   161.17056 &    58.78532 &       0.425 &       0.307 &        0.22 &        0.10 &        0.29 &        6.16 &        1.81 &        2.85 &        5.52 &        1.40 &        2.42 &        4.16 &   2.28 &   5.99 &   0.11 &   1.20 &   0.46\\
  237 &   161.17181 &    59.21432 &       0.632 &       0.288 &        0.91 &        0.28 &        0.54 &        0.22 &        0.18 &        0.73 &        0.95 &        0.33 &        0.47 &        0.10 &   0.09 &   0.36 &   2.46 &   0.94 &   0.27\\
  238 &   161.17307 &    58.92259 &       0.692 &       0.109 &        0.24 &        0.13 &        0.24 &        3.30 &        1.23 &        1.78 &        3.29 &        0.97 &        1.52 &        2.30 &   1.53 &   2.55 &   0.48 &   0.51 &   0.59\\
  239 &   161.17442 &    59.05012 &       1.349 &       0.345 &        3.25 &        0.72 &        1.03 &        0.23 &        0.19 &        0.79 &        2.73 &        0.62 &        0.65 &        0.04 &   0.04 &   0.14 &   2.64 &   0.42 &   0.11\\
  240 &   161.17644 &    59.04453 &       0.782 &       0.338 &        2.81 &        0.53 &        0.64 &        4.28 &        1.34 &        1.58 &        7.28 &        1.23 &        1.27 &        0.42 &   0.15 &   0.18 &   1.59 &   0.31 &   0.39\\
  241 &   161.17750 &    59.29392 &       0.696 &       0.463 &        0.80 &        0.34 &        0.43 &        0.14 &        0.10 &        0.78 &        0.23 &        0.15 &        0.30 &        0.08 &   0.07 &   0.46 &   2.52 &   1.14 &   0.20\\
  242 &   161.17803 &    59.32209 &       0.460 &       0.188 &        6.91 &        0.79 &        1.00 &       12.17 &        2.38 &        2.41 &       19.81 &        1.89 &        2.30 &        0.47 &   0.11 &   0.11 &   1.51 &   0.19 &   0.21\\
  243 &   161.18088 &    59.28470 &       0.671 &       0.347  &$<$        0.18 &         -99 &         -99 &        3.50 &        1.48 &        1.86 &        3.60 &        1.12 &        1.79  &$>$        3.07 & -99.00\\
  244 &   161.18630 &    58.66059 &       0.144 &       0.095 &        2.08 &        0.41 &        0.51 &        7.79 &        1.62 &        2.21 &        8.52 &        1.36 &        1.59 &        0.83 &   0.24 &   0.31 &   1.01 &   0.30 &   0.30\\
  245 &   161.18693 &    59.04804 &       0.806 &       0.297 &        1.60 &        0.36 &        0.51  &$<$       14.60 &         -99 &         -99 &        7.93 &        1.68 &        1.96  &$<$        1.67 & -99.00\\
  246 &   161.18866 &    58.90222 &       0.210 &       0.097 &       10.93 &        1.01 &        1.11 &       18.07 &        2.50 &        2.87 &       28.83 &        2.20 &        2.47 &        0.44 &   0.07 &   0.08 &   1.55 &   0.14 &   0.15\\
  247 &   161.19066 &    59.34619 &       0.784 &       0.338 &        0.03 &        0.02 &        0.19 &       29.62 &        5.38 &        6.45 &       25.02 &        5.07 &        5.63 &       62.44 &  47.10 & 348.33 &  -2.83 &   9.93 &   1.34\\
  248 &   161.19172 &    58.74388 &       0.319 &       0.106 &        1.41 &        0.37 &        0.55 &        0.52 &        0.32 &        0.85 &        2.05 &        0.53 &        0.61 &        0.14 &   0.10 &   0.24 &   2.34 &   0.68 &   0.28\\
  249 &   161.19217 &    58.82453 &       1.000 &       0.701 &        1.47 &        0.38 &        0.49  &$<$       11.52 &         -99 &         -99 &        5.67 &        1.54 &        1.57  &$<$        1.48 & -99.00\\
  250 &   161.19959 &    59.17319 &       0.745 &       0.259 &        0.12 &        0.11 &        0.14  &$<$        8.34 &         -99 &         -99 &        1.62 &        0.83 &        1.86  &$<$        8.42 & -99.00\\
  251 &   161.20138 &    59.10835 &       0.503 &       0.325 &       12.10 &        1.27 &        1.41 &        8.86 &        1.72 &        2.58 &       22.25 &        1.94 &        2.32 &        0.24 &   0.05 &   0.08 &   2.06 &   0.22 &   0.16\\
  252 &   161.20411 &    58.79018 &       0.206 &       0.439 &        0.93 &        0.29 &        0.40  &$<$        4.33 &         -99 &         -99 &        3.08 &        0.97 &        1.14  &$<$        0.98 & -99.00\\
  253 &   161.20429 &    59.16876 &       0.383 &       0.268 &        2.90 &        0.49 &        0.71 &        5.31 &        1.26 &        2.09 &        7.82 &        1.29 &        1.40 &        0.48 &   0.14 &   0.22 &   1.49 &   0.35 &   0.29\\
  254 &   161.20490 &    58.64824 &       0.222 &       0.192 &        0.03 &        0.03 &        0.09 &       11.79 &        2.72 &        4.43 &       10.41 &        3.00 &        3.49 &       29.54 &  30.32 &  79.12 &  -1.89 &   2.26 &   6.92\\
  255 &   161.21415 &    59.32962 &       0.237 &       0.116 &        5.40 &        0.66 &        0.84 &       36.35 &        4.08 &        4.84 &       40.36 &        3.37 &        3.99 &        1.31 &   0.22 &   0.27 &   0.68 &   0.05 &   0.06\\
  256 &   161.21583 &    58.91202 &       0.331 &       0.211 &        4.14 &        0.59 &        0.75 &        9.20 &        1.83 &        2.23 &       12.85 &        1.58 &        1.78 &        0.56 &   0.14 &   0.17 &   1.36 &   0.25 &   0.23\\
  257 &   161.21610 &    58.75401 &       0.194 &       0.097 &        2.16 &        0.46 &        0.51 &       10.64 &        2.16 &        2.64 &       11.59 &        1.82 &        1.97 &        1.02 &   0.30 &   0.35 &   0.80 &   0.14 &   0.31\\
  258 &   161.21697 &    59.22238 &       0.215 &       0.290 &        1.31 &        0.32 &        0.55 &        0.78 &        0.36 &        1.06 &        2.02 &        0.47 &        0.76 &        0.21 &   0.11 &   0.29 &   2.16 &   0.71 &   0.32\\
  259 &   161.21758 &    59.23770 &       0.130 &       0.098 &        0.91 &        0.24 &        0.42 &        3.04 &        0.99 &        1.64 &        3.83 &        0.81 &        1.27 &        0.76 &   0.32 &   0.54 &   1.07 &   0.40 &   0.48\\
  260 &   161.21766 &    59.05206 &       1.276 &       0.502 &        0.99 &        0.30 &        0.40 &        5.57 &        1.59 &        2.12 &        6.70 &        1.45 &        1.62 &        1.13 &   0.47 &   0.63 &   0.71 &   0.13 &   0.46\\
  261 &   161.21891 &    58.72461 &       0.169 &       0.076 &        1.28 &        0.30 &        0.48 &        2.43 &        0.90 &        1.31 &        4.19 &        0.82 &        1.10 &        0.49 &   0.21 &   0.32 &   1.47 &   0.45 &   0.48\\
  262 &   161.22054 &    59.10927 &       0.472 &       0.303 &        4.19 &        0.60 &        0.75 &       20.52 &        3.05 &        3.54 &       23.94 &        2.53 &        2.97 &        1.02 &   0.21 &   0.25 &   0.81 &   0.13 &   0.22\\
  263 &   161.22114 &    58.91476 &       0.290 &       0.163 &        5.86 &        0.69 &        0.85 &       20.53 &        2.84 &        3.26 &       27.01 &        2.47 &        2.71 &        0.79 &   0.14 &   0.17 &   1.05 &   0.17 &   0.16\\
  264 &   161.22687 &    59.13104 &       0.527 &       0.312 &        2.96 &        0.51 &        0.66 &       11.24 &        2.24 &        2.73 &       13.52 &        1.93 &        2.07 &        0.84 &   0.22 &   0.28 &   0.99 &   0.28 &   0.26\\
  265 &   161.22730 &    59.07674 &       0.664 &       0.317 &        3.34 &        0.54 &        0.63 &       44.41 &        4.63 &        5.73 &       45.15 &        3.93 &        4.69 &        2.26 &   0.44 &   0.53 &   0.49 &   0.10 &   0.09\\
  266 &   161.22891 &    59.35950 &       0.285 &       0.112 &       20.94 &        1.45 &        1.61 &       25.59 &        3.01 &        3.60 &       48.12 &        2.88 &        3.15 &        0.35 &   0.05 &   0.06 &   1.74 &   0.14 &   0.13\\
  267 &   161.23030 &    59.08579 &       0.940 &       0.490 &        3.92 &        0.67 &        0.73 &        3.90 &        1.05 &        1.79 &        8.54 &        1.17 &        1.44 &        0.30 &   0.10 &   0.15 &   1.87 &   0.34 &   0.28\\
  268 &   161.23105 &    58.93019 &       0.616 &       0.250 &        1.76 &        0.36 &        0.54 &        6.05 &        1.62 &        1.87 &        7.05 &        1.26 &        1.51 &        0.78 &   0.26 &   0.34 &   1.06 &   0.34 &   0.37\\
  269 &   161.23110 &    58.76373 &       0.238 &       0.078 &        1.53 &        0.33 &        0.46 &       19.34 &        2.84 &        3.85 &       19.06 &        2.62 &        2.80 &        2.17 &   0.57 &   0.79 &   0.50 &   0.16 &   0.11\\
  270 &   161.23592 &    58.92401 &       0.247 &       0.096 &       20.48 &        1.46 &        1.62 &       23.85 &        3.03 &        3.24 &       44.99 &        2.85 &        2.94 &        0.34 &   0.05 &   0.05 &   1.77 &   0.13 &   0.14\\
  271 &   161.23862 &    59.20687 &       0.273 &       0.329 &        0.13 &        0.07 &        0.27  &$<$        3.88 &         -99 &         -99 &        0.93 &        0.61 &        1.22  &$<$        4.26 & -99.00\\
  272 &   161.23934 &    58.68250 &       0.183 &       0.073 &        0.91 &        0.27 &        0.42 &        1.23 &        0.56 &        1.12 &        2.45 &        0.66 &        0.76 &        0.38 &   0.21 &   0.39 &   1.67 &   0.61 &   0.57\\
  273 &   161.23992 &    58.56027 &       0.616 &       0.419 &        2.64 &        0.46 &        0.60 &       15.85 &        2.80 &        3.07 &       18.06 &        2.14 &        2.74 &        1.20 &   0.30 &   0.36 &   0.70 &   0.07 &   0.23\\
  274 &   161.24188 &    59.20894 &       0.399 &       0.204 &        0.27 &        0.16 &        0.22 &        3.09 &        1.00 &        2.02 &        2.63 &        0.91 &        1.29 &        2.02 &   1.35 &   2.12 &   0.53 &   0.42 &   0.64\\
  275 &   161.24769 &    58.64641 &       0.368 &       0.232 &        0.43 &        0.21 &        0.34 &        5.00 &        1.74 &        2.46 &        3.45 &        1.20 &        1.70 &        2.03 &   1.21 &   1.89 &   0.53 &   0.38 &   0.48\\
  276 &   161.25278 &    59.23150 &       0.265 &       0.160 &        0.52 &        0.17 &        0.34 &        5.87 &        1.44 &        2.44 &        4.78 &        1.22 &        1.58 &        1.99 &   0.81 &   1.55 &   0.54 &   0.31 &   0.16\\
  277 &   161.25942 &    59.19808 &       0.373 &       0.113 &        1.26 &        0.29 &        0.47 &        3.39 &        1.18 &        1.41 &        4.34 &        0.88 &        1.20 &        0.64 &   0.27 &   0.36 &   1.21 &   0.39 &   0.48\\
  278 &   161.26247 &    58.78695 &       0.345 &       0.142 &        5.67 &        0.76 &        0.82 &        8.86 &        1.80 &        2.20 &       14.20 &        1.51 &        1.89 &        0.43 &   0.10 &   0.12 &   1.58 &   0.21 &   0.24\\
  279 &   161.26409 &    59.21182 &       0.044 &       0.034 &       28.01 &        1.66 &        1.71 &       57.97 &        4.61 &        5.20 &       87.03 &        4.09 &        4.39 &        0.53 &   0.05 &   0.06 &   1.41 &   0.10 &   0.09\\
  280 &   161.26410 &    59.18938 &       0.386 &       0.233 &        0.56 &        0.20 &        0.34 &        3.16 &        0.96 &        1.87 &        2.34 &        0.72 &        1.16 &        1.13 &   0.52 &   0.95 &   0.71 &   0.19 &   0.56\\
  281 &   161.26442 &    58.77844 &       0.237 &       0.246 &        0.47 &        0.19 &        0.36  &$<$        2.82 &         -99 &         -99 &        1.53 &        0.57 &        1.31  &$<$        1.19 & -99.00\\
  282 &   161.26492 &    58.85274 &       0.654 &       0.639 &        0.88 &        0.26 &        0.41 &       11.55 &        2.61 &        2.93 &       10.50 &        1.90 &        2.50 &        2.23 &   0.83 &   1.18 &   0.49 &   0.24 &   0.17\\
  283 &   161.26950 &    59.21598 &       0.151 &       0.094 &        2.60 &        0.53 &        0.58 &        3.74 &        1.29 &        1.34 &        6.84 &        1.05 &        1.33 &        0.40 &   0.16 &   0.17 &   1.63 &   0.29 &   0.43\\
  284 &   161.27081 &    58.99674 &       0.503 &       0.317 &        0.06 &        0.06 &        0.15 &       53.12 &        6.82 &        8.28 &       52.32 &        6.86 &        7.81 &       59.04 &   4.17 &   5.17 &  -2.73 &   0.15 &   0.12\\
  285 &   161.27225 &    58.97700 &       1.205 &       0.391 &        0.95 &        0.28 &        0.44 &        1.72 &        0.64 &        1.48 &        3.21 &        0.74 &        1.04 &        0.48 &   0.23 &   0.47 &   1.49 &   0.61 &   0.54\\
  286 &   161.27376 &    59.35690 &       1.431 &       0.274 &        1.23 &        0.40 &        0.80 &        3.70 &        1.90 &        2.53 &        5.28 &        1.66 &        1.95 &        0.70 &   0.43 &   0.66 &   1.14 &   0.47 &   0.82\\
  287 &   161.27541 &    58.77341 &       0.388 &       0.169 &        0.32 &        0.14 &        0.29 &        7.96 &        1.89 &        3.14 &        7.71 &        1.94 &        2.21 &        3.71 &   1.89 &   3.67 &   0.20 &   0.73 &   0.38\\
  288 &   161.27727 &    58.66535 &       0.190 &       0.112 &        0.80 &        0.23 &        0.37 &       10.99 &        2.18 &        2.95 &        9.30 &        1.78 &        2.15 &        2.32 &   0.83 &   1.24 &   0.47 &   0.25 &   0.16\\
  289 &   161.27923 &    58.60840 &       0.222 &       0.157 &       10.15 &        0.98 &        1.13 &       13.15 &        2.15 &        2.53 &       23.61 &        2.00 &        2.18 &        0.37 &   0.07 &   0.08 &   1.70 &   0.17 &   0.18\\
  290 &   161.27929 &    58.66391 &       0.178 &       0.134 &        0.88 &        0.27 &        0.37 &        5.12 &        1.38 &        2.09 &        5.52 &        1.23 &        1.53 &        1.17 &   0.48 &   0.69 &   0.70 &   0.14 &   0.45\\
  291 &   161.28033 &    58.80642 &       0.921 &       0.275 &        1.26 &        0.32 &        0.46 &        5.18 &        1.40 &        2.12 &        6.53 &        1.17 &        1.71 &        0.89 &   0.33 &   0.49 &   0.94 &   0.28 &   0.41\\
  292 &   161.28137 &    59.28636 &       0.255 &       0.140 &        0.14 &        0.08 &        0.22 &        3.53 &        1.14 &        2.31 &        2.37 &        0.88 &        1.57 &        3.85 &   2.67 &   6.81 &   0.17 &   1.36 &   0.53\\
  293 &   161.28163 &    58.90677 &       1.167 &       0.440 &        1.06 &        0.41 &        0.43 &        0.30 &        0.26 &        0.69 &        2.08 &        0.54 &        0.62 &        0.12 &   0.11 &   0.27 &   2.42 &   0.77 &   0.33\\
  294 &   161.28280 &    59.07363 &       1.074 &       0.509 &        0.26 &        0.15 &        0.21  &$<$       15.43 &         -99 &         -99 &        2.80 &        1.22 &        1.89  &$<$        7.46 & -99.00\\
  295 &   161.28478 &    59.37065 &       0.725 &       0.541 &        1.45 &        0.34 &        0.49 &        5.57 &        1.67 &        1.96 &        7.40 &        1.42 &        1.57 &        0.85 &   0.32 &   0.41 &   0.99 &   0.30 &   0.43\\
  296 &   161.28694 &    59.37136 &       0.680 &       0.625 &        1.65 &        0.35 &        0.55 &        4.41 &        1.52 &        1.58 &        5.56 &        1.11 &        1.35 &        0.64 &   0.26 &   0.31 &   1.22 &   0.34 &   0.46\\
  297 &   161.29289 &    59.05289 &       0.742 &       0.444 &        0.77 &        0.22 &        0.42 &        4.42 &        1.22 &        2.22 &        5.62 &        1.34 &        1.51 &        1.16 &   0.46 &   0.85 &   0.71 &   0.17 &   0.44\\
  298 &   161.29655 &    59.27380 &       0.033 &       0.018 &       46.92 &        2.13 &        2.23 &       62.98 &        4.83 &        5.02 &      114.16 &        4.44 &        4.61 &        0.38 &   0.03 &   0.04 &   1.68 &   0.08 &   0.08\\
  299 &   161.29836 &    59.17730 &       0.150 &       0.077 &        5.34 &        0.64 &        0.83 &       13.09 &        2.10 &        2.67 &       18.12 &        1.83 &        2.13 &        0.60 &   0.12 &   0.15 &   1.29 &   0.20 &   0.20\\
  300 &   161.30291 &    59.03631 &       0.236 &       0.126 &       16.28 &        1.23 &        1.43 &       17.12 &        2.42 &        2.78 &       34.25 &        2.35 &        2.51 &        0.32 &   0.05 &   0.06 &   1.84 &   0.15 &   0.15\\
  301 &   161.30316 &    59.05658 &       0.628 &       0.334 &        2.36 &        0.46 &        0.56 &        6.58 &        1.51 &        2.14 &        8.43 &        1.24 &        1.68 &        0.66 &   0.20 &   0.27 &   1.19 &   0.28 &   0.34\\
  302 &   161.30640 &    58.68231 &       0.186 &       0.083 &        1.13 &        0.28 &        0.42 &       11.36 &        2.26 &        2.76 &       12.13 &        1.94 &        2.27 &        1.81 &   0.58 &   0.80 &   0.58 &   0.16 &   0.12\\
  303 &   161.30933 &    59.20054 &       0.113 &       0.194 &        0.73 &        0.21 &        0.40 &        1.88 &        0.87 &        1.12 &        2.32 &        0.66 &        0.88 &        0.62 &   0.34 &   0.50 &   1.25 &   0.54 &   0.69\\
  304 &   161.30954 &    58.82383 &       0.877 &       0.342 &        2.69 &        0.52 &        0.62 &       12.20 &        2.33 &        3.11 &       15.13 &        2.03 &        2.49 &        0.96 &   0.26 &   0.33 &   0.87 &   0.19 &   0.27\\
  305 &   161.31594 &    59.31953 &       0.455 &       0.134 &        0.54 &        0.20 &        0.47 &        2.71 &        1.45 &        1.67 &        1.93 &        0.89 &        1.15 &        1.03 &   0.67 &   1.10 &   0.79 &   0.28 &   0.93\\
  306 &   161.31688 &    59.38465 &       0.723 &       0.471 &        0.99 &        0.29 &        0.46 &        5.44 &        1.79 &        2.13 &        4.95 &        1.33 &        1.53 &        1.11 &   0.49 &   0.67 &   0.72 &   0.13 &   0.53\\
  307 &   161.31759 &    59.31457 &       0.139 &       0.056 &       10.03 &        1.01 &        1.06 &       18.95 &        2.73 &        3.15 &       29.77 &        2.47 &        2.57 &        0.49 &   0.09 &   0.10 &   1.47 &   0.16 &   0.15\\
  308 &   161.31778 &    59.09274 &       0.351 &       0.194 &        4.65 &        0.67 &        0.72 &       16.87 &        2.75 &        2.99 &       20.94 &        2.12 &        2.61 &        0.81 &   0.18 &   0.19 &   1.03 &   0.20 &   0.21\\
  309 &   161.31790 &    59.19267 &       0.120 &       0.119 &        2.98 &        0.53 &        0.76 &        2.14 &        0.90 &        1.14 &        5.14 &        0.94 &        1.03 &        0.24 &   0.11 &   0.14 &   2.07 &   0.38 &   0.32\\
  310 &   161.32166 &    58.65023 &       0.367 &       0.271 &        0.44 &        0.16 &        0.38 &        0.61 &        0.37 &        1.00 &        1.61 &        0.44 &        0.81 &        0.39 &   0.28 &   0.72 &   1.65 &   0.94 &   0.79\\
  311 &   161.32171 &    59.04640 &       0.733 &       0.392 &        0.75 &        0.26 &        0.37 &        1.29 &        0.80 &        0.89 &        1.95 &        0.55 &        0.84 &        0.46 &   0.32 &   0.39 &   1.53 &   0.54 &   0.85\\
  312 &   161.32372 &    59.20107 &       0.127 &       0.070 &        1.82 &        0.42 &        0.47 &        4.90 &        1.35 &        1.77 &        7.34 &        1.18 &        1.50 &        0.64 &   0.23 &   0.29 &   1.21 &   0.31 &   0.39\\
  313 &   161.32394 &    59.11483 &       0.506 &       0.301 &        7.29 &        0.80 &        0.95 &       17.85 &        2.70 &        3.01 &       24.50 &        2.26 &        2.48 &        0.60 &   0.11 &   0.13 &   1.29 &   0.18 &   0.19\\
  314 &   161.32780 &    59.11858 &       0.340 &       0.204 &       14.94 &        1.24 &        1.32 &       17.11 &        2.54 &        2.74 &       32.15 &        2.39 &        2.42 &        0.34 &   0.06 &   0.06 &   1.78 &   0.15 &   0.16\\
  315 &   161.32883 &    58.74405 &       0.440 &       0.180 &        0.71 &        0.21 &        0.39 &        7.09 &        1.73 &        2.50 &        4.78 &        1.16 &        1.69 &        1.79 &   0.68 &   1.16 &   0.58 &   0.23 &   0.14\\
  316 &   161.32935 &    59.17382 &       0.345 &       0.204 &        0.68 &        0.22 &        0.37 &        1.89 &        0.83 &        1.28 &        1.89 &        0.66 &        0.79 &        0.66 &   0.36 &   0.57 &   1.19 &   0.49 &   0.70\\
  317 &   161.33016 &    59.17540 &       0.521 &       0.245 &        0.55 &        0.22 &        0.33 &        5.50 &        1.55 &        2.39 &        4.84 &        1.11 &        1.82 &        1.80 &   0.88 &   1.33 &   0.58 &   0.27 &   0.33\\
  318 &   161.33044 &    58.72046 &       0.207 &       0.095 &        3.18 &        0.54 &        0.70 &        2.88 &        0.89 &        1.43 &        6.49 &        0.92 &        1.24 &        0.28 &   0.10 &   0.15 &   1.94 &   0.37 &   0.29\\
  319 &   161.33553 &    59.21440 &       0.157 &       0.100 &        1.79 &        0.40 &        0.49 &        2.89 &        0.89 &        1.44 &        4.43 &        0.81 &        1.08 &        0.44 &   0.17 &   0.25 &   1.56 &   0.41 &   0.41\\
  320 &   161.33926 &    59.18544 &       0.449 &       0.087 &        0.38 &        0.16 &        0.29 &        3.03 &        1.13 &        1.63 &        2.85 &        0.89 &        1.21 &        1.49 &   0.82 &   1.39 &   0.64 &   0.28 &   0.53\\
  321 &   161.34197 &    58.94141 &       0.562 &       0.480 &        0.46 &        0.19 &        0.35 &        0.98 &        0.72 &        0.84 &        1.12 &        0.55 &        0.59 &        0.54 &   0.45 &   0.62 &   1.39 &   0.68 &   1.11\\
  322 &   161.34845 &    58.93385 &       0.536 &       0.248 &        0.81 &        0.25 &        0.40 &        2.86 &        0.99 &        1.70 &        3.85 &        0.96 &        1.22 &        0.79 &   0.37 &   0.61 &   1.05 &   0.39 &   0.54\\
  323 &   161.34906 &    59.29503 &       0.371 &       0.189 &        0.14 &        0.09 &        0.23 &        0.84 &        0.55 &        1.10 &        1.57 &        0.63 &        0.94 &        1.18 &   1.07 &   2.49 &   0.70 &   0.50 &   1.72\\
  324 &   161.34952 &    58.99129 &       0.717 &       0.106 &        0.29 &        0.18 &        0.20 &        1.82 &        0.94 &        1.24 &        1.49 &        0.72 &        0.78 &        1.25 &   1.00 &   1.21 &   0.69 &   0.24 &   1.35\\
  325 &   161.35191 &    58.78435 &       1.163 &       0.301 &        1.93 &        0.41 &        0.64 &        1.49 &        0.77 &        1.02 &        3.69 &        0.77 &        0.94 &        0.25 &   0.14 &   0.19 &   2.03 &   0.48 &   0.41\\
  326 &   161.35233 &    59.11800 &       0.400 &       0.275 &       22.39 &        2.11 &        2.32 &        0.14 &        0.12 &        0.49 &        6.43 &        0.63 &        0.66 &        0.01 &   0.01 &   0.02 &   2.74 &   0.07 &   0.02\\
  327 &   161.35503 &    58.99710 &       0.338 &       0.246 &        1.06 &        0.32 &        0.37 &        2.91 &        0.95 &        1.57 &        3.38 &        0.78 &        1.10 &        0.65 &   0.29 &   0.42 &   1.20 &   0.44 &   0.52\\
  328 &   161.35534 &    58.71697 &       0.541 &       0.224 &        1.11 &        0.38 &        0.46 &        4.02 &        1.58 &        1.95 &        4.81 &        1.29 &        1.48 &        0.81 &   0.42 &   0.52 &   1.03 &   0.35 &   0.64\\
  329 &   161.36196 &    59.22609 &       0.131 &       0.079 &        1.06 &        0.27 &        0.39 &       15.48 &        2.85 &        2.95 &       15.77 &        2.13 &        2.81 &        2.44 &   0.76 &   1.01 &   0.45 &   0.20 &   0.15\\
  330 &   161.36426 &    59.18370 &       0.313 &       0.173 &        0.32 &        0.16 &        0.26 &       11.87 &        2.64 &        3.29 &        9.56 &        2.12 &        2.65 &        5.06 &   2.70 &   4.23 &  -0.07 &   0.85 &   0.54\\
  331 &   161.36804 &    59.22415 &       0.165 &       0.131 &        0.54 &        0.22 &        0.41 &        9.46 &        2.82 &        3.00 &        8.60 &        2.23 &        2.56 &        2.81 &   1.41 &   2.32 &   0.38 &   0.46 &   0.28\\
  332 &   161.36820 &    59.16761 &       0.311 &       0.341 &        1.05 &        0.34 &        0.41 &        2.48 &        0.93 &        1.65 &        2.85 &        0.70 &        1.18 &        0.58 &   0.29 &   0.45 &   1.31 &   0.52 &   0.59\\
  333 &   161.36824 &    58.61435 &       1.112 &       0.443 &        1.01 &        0.27 &        0.47 &        2.15 &        0.74 &        1.59 &        2.07 &        0.68 &        0.81 &        0.54 &   0.23 &   0.47 &   1.39 &   0.57 &   0.48\\
  334 &   161.37131 &    59.19082 &       0.286 &       0.246  &$<$        0.06 &         -99 &         -99 &        6.63 &        2.07 &        2.83 &        6.60 &        1.86 &        2.86  &$>$       12.37 & -99.00\\
  335 &   161.37261 &    58.74204 &       0.526 &       0.160 &        2.90 &        0.59 &        0.65 &        3.02 &        1.05 &        1.49 &        6.59 &        1.12 &        1.22 &        0.31 &   0.13 &   0.17 &   1.84 &   0.36 &   0.37\\
  336 &   161.37535 &    58.87712 &       0.483 &       0.388 &        7.14 &        0.87 &        0.92 &        9.44 &        1.77 &        2.35 &       17.42 &        1.79 &        1.88 &        0.38 &   0.08 &   0.11 &   1.69 &   0.20 &   0.22\\
  337 &   161.37543 &    58.92059 &       0.670 &       0.538 &        0.04 &        0.03 &        0.21 &        6.29 &        1.82 &        3.41 &        7.77 &        2.44 &        2.87 &       16.98 &  13.36 &  95.08 &  -1.53 &   2.71 &   1.75\\
  338 &   161.37732 &    58.65999 &       0.515 &       0.233 &        0.48 &        0.18 &        0.32  &$<$        7.13 &         -99 &         -99 &        3.28 &        1.08 &        1.50  &$<$        2.45 & -99.00\\
  339 &   161.38080 &    59.17433 &       0.208 &       0.204 &        0.33 &        0.15 &        0.30 &        3.23 &        1.04 &        2.12 &        2.58 &        0.84 &        1.40 &        1.78 &   0.98 &   1.99 &   0.58 &   0.40 &   0.46\\
  340 &   161.38412 &    58.58958 &       0.828 &       0.590 &        1.84 &        0.43 &        0.54 &        2.83 &        1.11 &        1.37 &        4.58 &        0.97 &        1.08 &        0.42 &   0.19 &   0.24 &   1.59 &   0.40 &   0.51\\
  341 &   161.38524 &    59.23229 &       0.087 &       0.052 &        4.62 &        0.63 &        0.73 &       10.62 &        2.00 &        2.21 &       15.78 &        1.67 &        1.96 &        0.57 &   0.13 &   0.15 &   1.34 &   0.22 &   0.22\\
  342 &   161.38689 &    59.29948 &       0.272 &       0.139 &        0.69 &        0.24 &        0.34 &        1.86 &        0.81 &        1.26 &        2.50 &        0.61 &        1.04 &        0.64 &   0.36 &   0.54 &   1.21 &   0.51 &   0.72\\
  343 &   161.38745 &    58.77750 &       0.454 &       0.196 &        8.07 &        0.91 &        0.98 &       14.41 &        2.22 &        2.98 &       21.23 &        2.07 &        2.21 &        0.47 &   0.09 &   0.11 &   1.50 &   0.19 &   0.17\\
  344 &   161.38953 &    59.22021 &       0.199 &       0.102 &        1.49 &        0.34 &        0.56 &        0.89 &        0.49 &        0.87 &        2.56 &        0.58 &        0.73 &        0.21 &   0.12 &   0.22 &   2.16 &   0.57 &   0.36\\
  345 &   161.38999 &    58.69004 &       0.569 &       0.331 &        0.77 &        0.24 &        0.38  &$<$        4.95 &         -99 &         -99 &        1.51 &        0.70 &        0.90  &$<$        1.27 & -99.00\\
  346 &   161.39567 &    58.77468 &       0.521 &       0.224 &        3.87 &        0.61 &        0.63 &       49.37 &        4.98 &        5.84 &       47.88 &        4.34 &        4.41 &        2.18 &   0.41 &   0.44 &   0.50 &   0.09 &   0.08\\
  347 &   161.41332 &    59.21329 &       0.109 &       0.063 &        6.31 &        0.74 &        0.88 &       12.25 &        2.17 &        2.37 &       19.23 &        1.83 &        2.12 &        0.50 &   0.11 &   0.12 &   1.45 &   0.20 &   0.19\\
  348 &   161.41503 &    59.20741 &       0.128 &       0.077 &        6.20 &        0.71 &        0.90 &       10.36 &        1.88 &        2.26 &       16.72 &        1.66 &        1.92 &        0.45 &   0.10 &   0.12 &   1.54 &   0.20 &   0.20\\
  349 &   161.41524 &    59.26519 &       0.191 &       0.152 &        0.84 &        0.24 &        0.45 &        0.61 &        0.41 &        0.81 &        1.71 &        0.51 &        0.60 &        0.24 &   0.17 &   0.34 &   2.06 &   0.74 &   0.51\\
  350 &   161.41647 &    59.02488 &       0.142 &       0.062 &        4.39 &        0.61 &        0.75 &        6.78 &        1.44 &        1.99 &       11.29 &        1.37 &        1.54 &        0.42 &   0.11 &   0.14 &   1.59 &   0.24 &   0.26\\
  351 &   161.41717 &    58.71526 &       0.172 &       0.068 &       65.12 &        2.65 &        2.76 &       59.58 &        4.49 &        5.02 &      125.21 &        4.45 &        4.78 &        0.28 &   0.02 &   0.03 &   1.93 &   0.08 &   0.07\\
  352 &   161.41769 &    59.34526 &       0.360 &       0.108 &        8.38 &        0.91 &        1.08 &        7.64 &        1.62 &        2.00 &       16.54 &        1.59 &        1.85 &        0.28 &   0.07 &   0.08 &   1.93 &   0.22 &   0.20\\
  353 &   161.41966 &    58.69559 &       0.717 &       0.605 &        0.55 &        0.20 &        0.36 &        1.52 &        0.68 &        1.38 &        2.93 &        0.84 &        0.98 &        0.66 &   0.39 &   0.74 &   1.19 &   0.53 &   0.78\\
  354 &   161.42030 &    58.66349 &       0.513 &       0.589 &        1.49 &        0.39 &        0.58 &        0.73 &        0.51 &        0.77 &        2.78 &        0.66 &        0.75 &        0.18 &   0.13 &   0.20 &   2.24 &   0.56 &   0.39\\
  355 &   161.42113 &    58.95155 &       0.343 &       0.264 &        0.93 &        0.26 &        0.41 &        3.99 &        1.18 &        1.85 &        4.20 &        1.06 &        1.20 &        0.92 &   0.37 &   0.58 &   0.91 &   0.28 &   0.47\\
  356 &   161.42401 &    59.34463 &       0.806 &       0.146 &        2.55 &        0.52 &        0.78 &        1.84 &        1.00 &        1.09 &        4.36 &        0.84 &        1.15 &        0.24 &   0.14 &   0.16 &   2.07 &   0.43 &   0.40\\
  357 &   161.42525 &    59.25924 &       0.262 &       0.134 &        0.17 &        0.14 &        0.38 &        4.75 &        2.30 &        3.75 &        5.24 &        1.96 &        3.49 &        4.14 &   4.11 &  10.02 &   0.11 &   1.56 &   2.56\\
  358 &   161.42646 &    59.01644 &       0.396 &       0.106 &        0.30 &        0.14 &        0.27  &$<$        1.41 &         -99 &         -99 &        0.89 &        0.40 &        0.80  &$<$        0.98 & -99.00\\
  359 &   161.42856 &    58.86991 &       1.483 &       0.601 &        1.60 &        0.33 &        0.51  &$<$       10.57 &         -99 &         -99 &        4.88 &        1.12 &        1.59  &$<$        1.29 & -99.00\\
  360 &   161.43010 &    59.11565 &       0.630 &       0.358 &        3.38 &        0.57 &        0.62 &       19.63 &        2.79 &        3.74 &       22.81 &        2.48 &        2.93 &        1.16 &   0.26 &   0.31 &   0.71 &   0.06 &   0.22\\
  361 &   161.43089 &    59.22317 &       0.247 &       0.143 &        3.07 &        0.72 &        0.91 &        0.05 &        0.05 &        0.31 &        1.36 &        0.32 &        0.36 &        0.01 &   0.01 &   0.09 &   2.72 &   0.25 &   0.04\\
  362 &   161.43177 &    59.30307 &       0.167 &       0.147 &        0.64 &        0.22 &        0.32 &        8.35 &        2.10 &        2.40 &        8.54 &        1.77 &        1.97 &        2.22 &   0.95 &   1.26 &   0.50 &   0.25 &   0.19\\
  363 &   161.43456 &    58.83880 &       0.898 &       0.470 &        7.29 &        1.19 &        1.41 &        0.05 &        0.05 &        0.31 &        2.52 &        0.42 &        0.42 &        0.01 &   0.01 &   0.04 &   2.74 &   0.13 &   0.02\\
  364 &   161.43465 &    59.26605 &       0.208 &       0.123 &        0.06 &        0.05 &        0.20 &        5.61 &        1.95 &        2.76 &        4.14 &        1.34 &        2.72 &       10.96 &   9.78 &  37.48 &  -1.25 &   1.18 &   1.95\\
  365 &   161.43515 &    59.19753 &       0.593 &       0.153 &        0.13 &        0.08 &        0.22 &        5.63 &        1.66 &        2.60 &        4.86 &        1.60 &        1.90 &        5.63 &   3.83 &   9.62 &  -0.19 &   1.30 &   0.77\\
  366 &   161.43895 &    58.73163 &       0.817 &       0.334 &        4.54 &        0.68 &        0.85 &        8.13 &        1.94 &        2.19 &       13.63 &        1.68 &        2.02 &        0.47 &   0.13 &   0.15 &   1.50 &   0.25 &   0.26\\
  367 &   161.44201 &    58.71414 &       1.680 &       0.739 &        0.52 &        0.20 &        0.35 &        4.26 &        1.23 &        2.31 &        3.28 &        1.02 &        1.40 &        1.53 &   0.72 &   1.31 &   0.63 &   0.26 &   0.40\\
  368 &   161.44320 &    58.76387 &       0.643 &       0.445 &        0.58 &        0.23 &        0.28 &        8.55 &        2.06 &        2.62 &        6.89 &        1.39 &        2.14 &        2.45 &   1.13 &   1.40 &   0.45 &   0.28 &   0.23\\
  369 &   161.44564 &    59.31561 &       0.224 &       0.106 &        5.08 &        0.65 &        0.85 &        6.56 &        1.43 &        1.99 &       11.27 &        1.41 &        1.50 &        0.37 &   0.09 &   0.13 &   1.71 &   0.24 &   0.25\\
  370 &   161.45378 &    59.14198 &       0.412 &       0.318 &        3.74 &        0.58 &        0.73 &        9.04 &        1.72 &        2.56 &       13.24 &        1.71 &        1.83 &        0.59 &   0.15 &   0.20 &   1.30 &   0.26 &   0.24\\
  371 &   161.45385 &    59.05933 &       0.182 &       0.139 &        0.88 &        0.23 &        0.41 &        3.36 &        1.30 &        1.36 &        3.16 &        0.84 &        1.09 &        0.84 &   0.39 &   0.52 &   0.99 &   0.33 &   0.55\\
  372 &   161.46024 &    59.32419 &       0.699 &       0.338 &        0.71 &        0.26 &        0.32 &        3.69 &        1.07 &        2.00 &        4.13 &        0.92 &        1.49 &        1.07 &   0.50 &   0.75 &   0.76 &   0.18 &   0.58\\
  373 &   161.46177 &    58.85888 &       1.269 &       0.484 &        0.70 &        0.25 &        0.42 &        0.59 &        0.36 &        0.98 &        1.25 &        0.44 &        0.62 &        0.27 &   0.19 &   0.47 &   1.98 &   0.88 &   0.55\\
  374 &   161.46573 &    59.06266 &       0.252 &       0.100 &        0.32 &        0.16 &        0.25 &        2.57 &        0.96 &        1.71 &        2.81 &        0.83 &        1.30 &        1.50 &   0.92 &   1.55 &   0.64 &   0.31 &   0.67\\
  375 &   161.46606 &    59.05331 &       0.286 &       0.147  &$<$        0.06 &         -99 &         -99 &        4.59 &        1.80 &        2.22 &        4.99 &        1.64 &        2.27  &$>$        9.17 & -99.00\\
  376 &   161.46617 &    58.76708 &       0.221 &       0.155 &        6.19 &        0.71 &        0.79 &       44.63 &        4.44 &        4.90 &       49.84 &        3.61 &        4.19 &        1.38 &   0.21 &   0.23 &   0.66 &   0.05 &   0.04\\
  377 &   161.46840 &    59.01022 &       0.163 &       0.092 &        0.25 &        0.13 &        0.28 &        0.33 &        0.29 &        0.75 &        0.98 &        0.41 &        0.52 &        0.38 &   0.38 &   0.97 &   1.68 &   1.01 &   1.09\\
  378 &   161.47479 &    58.79527 &       0.544 &       0.364 &        1.32 &        0.37 &        0.42 &        1.99 &        0.74 &        1.32 &        3.93 &        0.85 &        0.95 &        0.41 &   0.19 &   0.31 &   1.60 &   0.48 &   0.52\\
  379 &   161.48403 &    59.25172 &       0.482 &       0.156 &        1.57 &        0.37 &        0.53 &        1.66 &        0.72 &        1.12 &        3.12 &        0.66 &        0.91 &        0.32 &   0.16 &   0.24 &   1.84 &   0.48 &   0.46\\
  380 &   161.48571 &    58.99072 &       0.202 &       0.104 &        0.34 &        0.17 &        0.27 &        2.57 &        0.96 &        1.71 &        1.82 &        0.77 &        0.97 &        1.43 &   0.87 &   1.48 &   0.65 &   0.29 &   0.71\\
  381 &   161.48747 &    59.00011 &       0.159 &       0.133 &        2.61 &        0.67 &        0.86 &        3.35 &        1.16 &        2.49 &        6.43 &        1.30 &        1.78 &        0.37 &   0.16 &   0.30 &   1.71 &   0.53 &   0.44\\
  382 &   161.48925 &    59.12053 &       0.750 &       0.307 &        1.64 &        0.38 &        0.53 &        3.60 &        1.11 &        1.79 &        5.54 &        1.12 &        1.25 &        0.55 &   0.21 &   0.33 &   1.37 &   0.41 &   0.41\\
  383 &   161.48926 &    59.25918 &       0.416 &       0.202 &        0.32 &        0.15 &        0.25 &       12.59 &        2.55 &        3.48 &       11.42 &        2.32 &        2.84 &        5.43 &   2.85 &   4.54 &  -0.15 &   0.91 &   0.57\\
  384 &   161.49144 &    58.91784 &       0.658 &       0.355 &        0.61 &        0.26 &        0.32 &        1.02 &        0.52 &        1.18 &        2.46 &        0.71 &        0.82 &        0.45 &   0.30 &   0.57 &   1.54 &   0.73 &   0.78\\
  385 &   161.49431 &    59.05546 &       0.210 &       0.176 &        0.65 &        0.29 &        0.59  &$<$        3.43 &         -99 &         -99 &        3.10 &        1.24 &        1.85  &$<$        1.08 & -99.00\\
  386 &   161.49579 &    58.65024 &       0.762 &       0.626 &        2.68 &        0.47 &        0.68 &        2.79 &        0.97 &        1.37 &        5.95 &        0.91 &        1.24 &        0.31 &   0.12 &   0.17 &   1.84 &   0.37 &   0.36\\
  387 &   161.49837 &    59.10872 &       0.184 &       0.068 &       16.34 &        1.21 &        1.40 &       22.73 &        2.94 &        3.14 &       38.73 &        2.61 &        2.70 &        0.39 &   0.06 &   0.06 &   1.65 &   0.12 &   0.14\\
  388 &   161.49949 &    59.28856 &       0.418 &       0.300 &        0.79 &        0.31 &        0.39 &        0.39 &        0.35 &        0.63 &        1.51 &        0.45 &        0.60 &        0.18 &   0.17 &   0.30 &   2.24 &   0.76 &   0.51\\
  389 &   161.50106 &    59.23239 &       0.292 &       0.150 &        1.11 &        0.30 &        0.45 &        3.25 &        1.13 &        1.60 &        4.16 &        0.86 &        1.33 &        0.68 &   0.30 &   0.44 &   1.15 &   0.44 &   0.52\\
  390 &   161.50376 &    59.12295 &       0.429 &       0.137 &        6.81 &        0.80 &        0.95 &       14.51 &        2.33 &        2.96 &       21.02 &        2.00 &        2.42 &        0.54 &   0.11 &   0.13 &   1.39 &   0.23 &   0.18\\
  391 &   161.50427 &    59.12065 &       0.515 &       0.144 &        3.96 &        0.59 &        0.74 &       10.39 &        2.15 &        2.39 &       13.54 &        1.67 &        2.01 &        0.63 &   0.16 &   0.19 &   1.23 &   0.22 &   0.27\\
  392 &   161.50473 &    58.93555 &       0.448 &       0.165 &        0.79 &        0.22 &        0.39  &$<$        3.10 &         -99 &         -99 &        2.76 &        0.83 &        0.97  &$<$        0.86 & -99.00\\
  393 &   161.50526 &    58.82820 &       0.318 &       0.262 &        0.15 &        0.10 &        0.20 &        9.03 &        2.20 &        3.19 &       10.12 &        2.41 &        2.72 &        7.55 &   5.32 &  10.27 &  -0.57 &   0.99 &   1.06\\
  394 &   161.50836 &    58.97690 &       0.146 &       0.115 &        0.55 &        0.19 &        0.33 &        1.78 &        0.78 &        1.20 &        2.17 &        0.61 &        0.94 &        0.74 &   0.41 &   0.67 &   1.09 &   0.44 &   0.71\\
  395 &   161.51416 &    58.89453 &       0.585 &       0.623 &        0.87 &        0.32 &        0.47 &        0.22 &        0.18 &        0.76 &        1.81 &        0.42 &        0.68 &        0.11 &   0.10 &   0.38 &   2.44 &   0.97 &   0.29\\
  396 &   161.51587 &    59.11209 &       0.595 &       0.190 &        2.41 &        0.42 &        0.60 &        7.79 &        1.58 &        2.42 &        9.36 &        1.49 &        1.61 &        0.74 &   0.20 &   0.29 &   1.10 &   0.30 &   0.29\\
  397 &   161.51698 &    58.74012 &       0.142 &       0.114 &       14.23 &        1.33 &        1.45 &       13.77 &        2.27 &        2.91 &       27.20 &        2.22 &        2.51 &        0.30 &   0.06 &   0.07 &   1.89 &   0.18 &   0.16\\
  398 &   161.51797 &    58.77676 &       0.218 &       0.233 &        0.28 &        0.13 &        0.26 &        7.31 &        1.94 &        2.52 &        5.77 &        1.33 &        2.17 &        3.85 &   2.01 &   3.74 &   0.17 &   0.75 &   0.40\\
  399 &   161.51877 &    59.26832 &       0.924 &       0.108 &        0.72 &        0.23 &        0.39 &        1.71 &        0.93 &        1.01 &        2.18 &        0.61 &        0.96 &        0.59 &   0.37 &   0.47 &   1.31 &   0.54 &   0.82\\
  400 &   161.52669 &    58.65171 &       0.538 &       0.368 &        4.04 &        0.72 &        0.79 &        0.93 &        0.55 &        0.76 &        4.50 &        0.73 &        0.85 &        0.10 &   0.06 &   0.09 &   2.47 &   0.25 &   0.18\\
  401 &   161.52840 &    58.87914 &       1.278 &       0.552 &        1.02 &        0.33 &        0.55 &        0.14 &        0.14 &        0.36 &        0.86 &        0.30 &        0.42 &        0.07 &   0.07 &   0.18 &   2.57 &   0.53 &   0.21\\
  402 &   161.53175 &    58.93406 &       0.315 &       0.252 &        0.44 &        0.19 &        0.30 &        5.36 &        1.76 &        2.10 &        5.96 &        1.30 &        2.06 &        2.09 &   1.14 &   1.63 &   0.52 &   0.33 &   0.36\\
  403 &   161.53288 &    58.81198 &       0.302 &       0.140 &        1.89 &        0.37 &        0.55 &        3.79 &        1.07 &        1.64 &        5.59 &        1.00 &        1.19 &        0.51 &   0.18 &   0.27 &   1.43 &   0.38 &   0.35\\
  404 &   161.54076 &    58.92618 &       0.606 &       0.196 &        0.00 &        0.00 &        0.02 &      601.79 &       94.45 &      102.34 &      866.19 &      131.94 &      166.14 &      -99.00 &******* &******* & -99.00 &   0.00 &   0.00\\
  405 &   161.54323 &    58.72140 &       0.396 &       0.233 &        2.11 &        0.44 &        0.49 &        6.14 &        1.48 &        1.88 &        8.65 &        1.22 &        1.63 &        0.68 &   0.22 &   0.26 &   1.16 &   0.27 &   0.36\\
  406 &   161.54460 &    58.79922 &       0.201 &       0.091 &        2.29 &        0.43 &        0.57 &        3.72 &        1.11 &        1.49 &        5.59 &        0.89 &        1.23 &        0.44 &   0.15 &   0.21 &   1.56 &   0.35 &   0.37\\
  407 &   161.54592 &    58.81556 &       0.601 &       0.208 &        1.07 &        0.35 &        0.49 &        0.20 &        0.16 &        0.67 &        1.18 &        0.35 &        0.47 &        0.09 &   0.08 &   0.29 &   2.51 &   0.83 &   0.22\\
  408 &   161.54598 &    58.92146 &       0.315 &       0.163 &        3.69 &        0.62 &        0.67 &        3.93 &        1.09 &        1.56 &        7.86 &        1.03 &        1.35 &        0.32 &   0.10 &   0.14 &   1.83 &   0.31 &   0.30\\
  409 &   161.54934 &    59.01745 &       0.335 &       0.151 &        0.47 &        0.20 &        0.31 &        0.68 &        0.45 &        0.90 &        1.86 &        0.55 &        0.75 &        0.41 &   0.32 &   0.60 &   1.61 &   0.79 &   0.90\\
  410 &   161.55393 &    58.76116 &       0.413 &       0.184 &        0.80 &        0.24 &        0.37  &$<$        2.44 &         -99 &         -99 &        2.25 &        0.71 &        0.83  &$<$        0.71 & -99.00\\
  411 &   161.55420 &    58.78873 &       0.081 &       0.044 &       15.94 &        1.22 &        1.31 &       22.44 &        2.85 &        3.04 &       38.36 &        2.56 &        2.65 &        0.39 &   0.06 &   0.06 &   1.65 &   0.12 &   0.14\\
  412 &   161.55467 &    59.16137 &       0.690 &       0.298 &        5.96 &        0.77 &        0.94 &        6.13 &        1.41 &        1.99 &       12.14 &        1.35 &        1.70 &        0.31 &   0.08 &   0.11 &   1.85 &   0.27 &   0.24\\
  413 &   161.55471 &    58.70638 &       0.621 &       0.323 &        0.64 &        0.25 &        0.31 &        2.72 &        0.88 &        1.78 &        3.41 &        0.86 &        1.26 &        0.91 &   0.46 &   0.75 &   0.92 &   0.31 &   0.62\\
  414 &   161.55611 &    58.99488 &       0.069 &       0.040 &        7.30 &        0.76 &        0.89 &       21.90 &        2.62 &        3.35 &       29.98 &        2.48 &        2.59 &        0.70 &   0.11 &   0.14 &   1.14 &   0.14 &   0.17\\
  415 &   161.55672 &    58.74434 &       0.204 &       0.151 &        1.15 &        0.29 &        0.43 &        2.88 &        1.06 &        1.29 &        4.51 &        0.88 &        1.18 &        0.61 &   0.27 &   0.35 &   1.27 &   0.40 &   0.51\\
  416 &   161.56119 &    59.02257 &       0.200 &       0.155  &$<$        0.13 &         -99 &         -99 &        8.17 &        2.16 &        2.81 &        5.91 &        1.60 &        2.42  &$>$        7.79 & -99.00\\
  417 &   161.56187 &    59.12654 &       0.564 &       0.241 &        4.57 &        0.69 &        0.80 &        5.76 &        1.55 &        1.78 &       10.63 &        1.42 &        1.52 &        0.36 &   0.11 &   0.13 &   1.72 &   0.25 &   0.31\\
  418 &   161.56309 &    59.06404 &       0.279 &       0.112 &        0.75 &        0.28 &        0.41 &        0.29 &        0.25 &        0.65 &        1.36 &        0.40 &        0.54 &        0.15 &   0.14 &   0.34 &   2.33 &   0.87 &   0.40\\
  419 &   161.56373 &    59.04336 &       0.235 &       0.116  &$<$        0.05 &         -99 &         -99 &       14.69 &        3.41 &        3.84 &       13.40 &        2.71 &        4.15  &$>$       25.12 & -99.00\\
  420 &   161.56743 &    59.07510 &       0.641 &       0.108 &        0.56 &        0.23 &        0.34 &        0.66 &        0.44 &        0.87 &        1.18 &        0.36 &        0.70 &        0.34 &   0.27 &   0.50 &   1.77 &   0.77 &   0.77\\
  421 &   161.56772 &    58.78681 &       0.238 &       0.106 &        0.34 &        0.15 &        0.31 &        0.41 &        0.36 &        0.67 &        0.80 &        0.37 &        0.48 &        0.35 &   0.35 &   0.65 &   1.75 &   0.92 &   1.01\\
  422 &   161.56803 &    59.04149 &       0.177 &       0.063 &        1.20 &        0.33 &        0.43 &        2.79 &        1.10 &        1.35 &        4.64 &        0.96 &        1.18 &        0.58 &   0.28 &   0.35 &   1.32 &   0.42 &   0.56\\
  423 &   161.56818 &    58.83803 &       0.221 &       0.106 &        4.07 &        0.65 &        0.70 &        3.97 &        1.19 &        1.40 &        8.22 &        1.04 &        1.35 &        0.30 &   0.10 &   0.12 &   1.89 &   0.29 &   0.30\\
  424 &   161.56842 &    58.98925 &       0.184 &       0.085 &       33.55 &        6.67 &        9.01 &        0.00 &        0.00 &        0.05 &        0.06 &        0.01 &        0.01 &      -99.00 &   0.00 &   0.08 & -99.00 &   0.00 &   0.00\\
  425 &   161.56891 &    59.27415 &       0.501 &       0.259 &        0.96 &        0.25 &        0.42 &       30.36 &        4.24 &        4.87 &       26.48 &        3.63 &        3.90 &        4.50 &   1.31 &   2.10 &   0.04 &   0.42 &   0.26\\
  426 &   161.56993 &    58.65072 &       0.550 &       0.485 &        4.22 &        0.67 &        0.78 &        8.32 &        2.06 &        2.10 &       13.01 &        1.72 &        1.84 &        0.51 &   0.15 &   0.16 &   1.44 &   0.27 &   0.29\\
  427 &   161.57056 &    58.91597 &       0.457 &       0.242 &        2.88 &        0.51 &        0.73 &       12.42 &        2.31 &        3.42 &       14.39 &        2.12 &        2.45 &        0.92 &   0.24 &   0.35 &   0.91 &   0.22 &   0.24\\
  428 &   161.57311 &    58.66895 &       0.528 &       0.396 &        0.15 &        0.09 &        0.25 &        4.28 &        1.59 &        2.30 &        3.68 &        1.20 &        1.99 &        4.10 &   2.94 &   7.09 &   0.12 &   1.42 &   0.59\\
  429 &   161.57333 &    58.75095 &       0.234 &       0.267 &        0.58 &        0.26 &        0.53 &        1.04 &        0.64 &        1.71 &        2.03 &        0.71 &        1.21 &        0.47 &   0.36 &   0.88 &   1.50 &   0.84 &   0.93\\
  430 &   161.57346 &    59.09819 &       0.422 &       0.123 &        6.66 &        0.93 &        1.24 &        2.74 &        0.95 &        1.63 &        9.81 &        1.37 &        1.47 &        0.16 &   0.06 &   0.10 &   2.31 &   0.29 &   0.17\\
  431 &   161.57485 &    58.63617 &       0.450 &       0.305 &        7.61 &        0.78 &        0.97 &       20.04 &        2.61 &        3.41 &       27.92 &        2.46 &        2.57 &        0.63 &   0.10 &   0.13 &   1.23 &   0.16 &   0.18\\
  432 &   161.58379 &    59.23811 &       0.687 &       0.269 &        4.13 &        0.64 &        0.75 &        6.36 &        1.53 &        1.95 &       10.44 &        1.30 &        1.68 &        0.42 &   0.12 &   0.15 &   1.59 &   0.25 &   0.30\\
  433 &   161.58790 &    58.83756 &       0.292 &       0.194 &        0.04 &        0.03 &        0.21 &        6.61 &        1.91 &        3.58 &        5.19 &        2.04 &        2.51 &       17.59 &  13.85 &  98.54 &  -1.55 &   2.81 &   1.74\\
  434 &   161.59037 &    59.29021 &       0.539 &       0.372 &        2.59 &        0.44 &        0.63 &        9.27 &        1.96 &        2.43 &       12.15 &        1.70 &        1.95 &        0.80 &   0.22 &   0.29 &   1.04 &   0.29 &   0.28\\
  435 &   161.59055 &    58.99929 &       0.337 &       0.204 &        0.04 &        0.04 &        0.11 &        0.19 &        0.14 &        1.08 &        0.83 &        0.34 &        0.86 &        0.99 &   1.23 &   6.14 &   0.84 &   1.32 &   2.63\\
  436 &   161.59080 &    58.82538 &       0.162 &       0.133 &        0.61 &        0.20 &        0.33 &        4.62 &        1.30 &        2.00 &        5.53 &        1.23 &        1.53 &        1.44 &   0.62 &   1.00 &   0.65 &   0.20 &   0.37\\
  437 &   161.59153 &    58.94166 &       0.243 &       0.135 &        5.75 &        0.78 &        0.89 &        8.77 &        1.66 &        2.48 &       14.44 &        1.71 &        1.81 &        0.42 &   0.10 &   0.13 &   1.59 &   0.23 &   0.23\\
  438 &   161.59155 &    59.28293 &       0.841 &       0.304 &        4.50 &        0.69 &        0.77 &        7.32 &        1.67 &        2.09 &       11.68 &        1.49 &        1.70 &        0.44 &   0.12 &   0.15 &   1.56 &   0.26 &   0.29\\
  439 &   161.59229 &    58.72084 &       0.277 &       0.246 &        0.38 &        0.17 &        0.35 &        0.22 &        0.18 &        0.73 &        1.12 &        0.32 &        0.61 &        0.20 &   0.19 &   0.70 &   2.18 &   1.25 &   0.55\\
  440 &   161.59233 &    58.65613 &       0.590 &       0.428 &        2.78 &        0.50 &        0.72 &        5.56 &        1.60 &        1.86 &        8.53 &        1.41 &        1.53 &        0.51 &   0.17 &   0.22 &   1.43 &   0.33 &   0.34\\
  441 &   161.59300 &    58.70066 &       0.253 &       0.279 &        0.84 &        0.25 &        0.34 &       10.81 &        2.10 &        2.83 &        8.77 &        1.52 &        2.18 &        2.19 &   0.78 &   1.05 &   0.50 &   0.21 &   0.16\\
  442 &   161.59333 &    59.01463 &       0.187 &       0.091 &        1.17 &        0.33 &        0.44 &        9.79 &        2.23 &        2.80 &        9.58 &        1.73 &        2.28 &        1.56 &   0.57 &   0.74 &   0.63 &   0.15 &   0.21\\
  443 &   161.59396 &    59.28845 &       0.523 &       0.460 &        2.54 &        0.46 &        0.58 &       13.77 &        2.36 &        3.10 &       14.64 &        2.01 &        2.30 &        1.10 &   0.27 &   0.35 &   0.72 &   0.08 &   0.28\\
  444 &   161.59795 &    59.02437 &       0.228 &       0.161 &        1.27 &        0.34 &        0.52 &        1.03 &        0.57 &        1.00 &        2.76 &        0.70 &        0.79 &        0.26 &   0.16 &   0.27 &   2.00 &   0.60 &   0.47\\
  445 &   161.59977 &    59.08958 &       0.404 &       0.145 &        0.98 &        0.29 &        0.34 &       15.50 &        2.67 &        3.46 &       13.88 &        2.06 &        2.81 &        2.60 &   0.90 &   1.08 &   0.42 &   0.22 &   0.18\\
  446 &   161.60043 &    58.72477 &       0.284 &       0.124 &        1.64 &        0.34 &        0.53 &        2.21 &        0.82 &        1.19 &        3.73 &        0.79 &        0.88 &        0.38 &   0.16 &   0.24 &   1.68 &   0.42 &   0.45\\
  447 &   161.60402 &    58.81083 &       0.290 &       0.244 &        0.52 &        0.19 &        0.34 &        0.65 &        0.43 &        0.85 &        1.38 &        0.45 &        0.63 &        0.36 &   0.27 &   0.53 &   1.73 &   0.78 &   0.78\\
  448 &   161.60761 &    58.81888 &       0.172 &       0.086 &        2.13 &        0.40 &        0.53 &        6.58 &        1.47 &        2.06 &        8.57 &        1.36 &        1.48 &        0.72 &   0.21 &   0.29 &   1.12 &   0.29 &   0.32\\
  449 &   161.61056 &    58.87107 &       0.431 &       0.176 &        3.07 &        0.56 &        0.62 &        6.08 &        1.36 &        2.19 &        9.66 &        1.42 &        1.53 &        0.51 &   0.15 &   0.21 &   1.44 &   0.32 &   0.28\\
  450 &   161.61120 &    59.34566 &       0.303 &       0.270 &        1.31 &        0.35 &        0.45 &        2.99 &        0.98 &        1.62 &        3.64 &        0.85 &        1.07 &        0.57 &   0.24 &   0.36 &   1.34 &   0.44 &   0.46\\
  451 &   161.61539 &    59.37964 &       0.712 &       0.467 &        1.37 &        0.38 &        0.44 &        2.79 &        1.10 &        1.35 &        3.37 &        0.81 &        1.03 &        0.52 &   0.25 &   0.30 &   1.42 &   0.41 &   0.55\\
  452 &   161.62190 &    58.99483 &       0.109 &       0.054 &       10.14 &        0.96 &        1.16 &        7.91 &        1.48 &        1.97 &       18.48 &        1.66 &        1.74 &        0.25 &   0.05 &   0.07 &   2.02 &   0.20 &   0.16\\
  453 &   161.62294 &    58.73067 &       0.084 &       0.068 &        5.98 &        0.70 &        0.84 &        7.68 &        1.47 &        1.96 &       14.17 &        1.49 &        1.58 &        0.37 &   0.08 &   0.11 &   1.71 &   0.21 &   0.22\\
  454 &   161.62531 &    59.31151 &       0.288 &       0.203 &        3.98 &        0.63 &        0.69 &        7.72 &        1.53 &        2.32 &       12.77 &        1.56 &        1.76 &        0.50 &   0.13 &   0.17 &   1.45 &   0.29 &   0.24\\
  455 &   161.62567 &    59.14142 &       0.912 &       0.224 &        8.60 &        1.04 &        1.24 &        3.18 &        1.05 &        1.45 &       11.75 &        1.37 &        1.45 &        0.14 &   0.05 &   0.07 &   2.34 &   0.20 &   0.15\\
  456 &   161.62716 &    58.74351 &       0.082 &       0.048 &        6.61 &        0.80 &        0.96 &        3.02 &        0.85 &        1.31 &        9.08 &        0.99 &        1.24 &        0.17 &   0.05 &   0.08 &   2.27 &   0.23 &   0.15\\
  457 &   161.62951 &    59.10270 &       0.380 &       0.119 &       10.05 &        1.05 &        1.11 &       16.23 &        2.56 &        2.99 &       27.49 &        2.25 &        2.66 &        0.44 &   0.08 &   0.09 &   1.56 &   0.16 &   0.18\\
  458 &   161.63210 &    59.10727 &       0.837 &       0.316 &        1.44 &        0.47 &        0.50 &        5.73 &        1.61 &        2.81 &        7.00 &        1.63 &        1.81 &        0.87 &   0.37 &   0.52 &   0.96 &   0.30 &   0.50\\
  459 &   161.63387 &    59.20809 &       0.770 &       0.419 &        7.51 &        0.97 &        1.04 &        4.05 &        1.10 &        1.66 &       11.94 &        1.35 &        1.51 &        0.19 &   0.06 &   0.08 &   2.20 &   0.24 &   0.17\\
  460 &   161.63426 &    59.12392 &       0.729 &       0.250 &        1.90 &        0.38 &        0.59 &        5.87 &        1.69 &        1.97 &        8.60 &        1.33 &        1.83 &        0.72 &   0.25 &   0.33 &   1.12 &   0.33 &   0.40\\
  461 &   161.63827 &    58.97108 &       0.223 &       0.112 &        5.66 &        0.69 &        0.83 &       11.56 &        1.86 &        2.60 &       16.80 &        1.76 &        1.95 &        0.52 &   0.11 &   0.14 &   1.42 &   0.24 &   0.18\\
  462 &   161.64309 &    59.22449 &       0.678 &       0.487 &        2.71 &        0.49 &        0.71 &        2.73 &        1.13 &        1.19 &        5.61 &        0.89 &        1.24 &        0.31 &   0.14 &   0.16 &   1.87 &   0.35 &   0.40\\
  463 &   161.65042 &    58.68760 &       0.522 &       0.516 &        0.83 &        0.27 &        0.45 &        0.70 &        0.46 &        0.92 &        1.44 &        0.47 &        0.66 &        0.27 &   0.20 &   0.38 &   1.98 &   0.77 &   0.58\\
  464 &   161.65069 &    58.67000 &       0.764 &       0.547 &        1.30 &        0.34 &        0.45 &        1.67 &        0.73 &        1.13 &        2.84 &        0.63 &        0.89 &        0.37 &   0.19 &   0.28 &   1.71 &   0.50 &   0.53\\
  465 &   161.65625 &    58.74353 &       0.229 &       0.084 &        0.07 &        0.06 &        0.16 &        5.14 &        1.69 &        2.34 &        4.08 &        1.42 &        2.01 &        9.00 &   8.34 &  21.00 &  -0.86 &   1.04 &   2.04\\
  466 &   161.65634 &    58.98738 &       0.497 &       0.227 &        0.71 &        0.21 &        0.38 &        3.81 &        1.32 &        1.59 &        4.57 &        1.02 &        1.43 &        1.09 &   0.49 &   0.75 &   0.73 &   0.16 &   0.55\\
  467 &   161.66036 &    58.94529 &       0.342 &       0.188 &        3.12 &        0.53 &        0.63 &        6.80 &        1.66 &        1.89 &       10.09 &        1.40 &        1.60 &        0.55 &   0.16 &   0.19 &   1.37 &   0.27 &   0.29\\
  468 &   161.66230 &    59.28791 &       0.387 &       0.221 &        1.57 &        0.35 &        0.49 &        4.81 &        1.18 &        2.00 &        6.73 &        1.20 &        1.44 &        0.71 &   0.24 &   0.37 &   1.13 &   0.38 &   0.37\\
  469 &   161.66456 &    58.68008 &       0.407 &       0.275 &        3.00 &        0.50 &        0.72 &        2.06 &        0.72 &        1.22 &        5.42 &        0.81 &        1.10 &        0.23 &   0.09 &   0.15 &   2.09 &   0.41 &   0.26\\
  470 &   161.66477 &    58.87770 &       0.578 &       0.394 &        0.45 &        0.17 &        0.39 &        0.65 &        0.40 &        1.07 &        1.18 &        0.38 &        0.78 &        0.40 &   0.29 &   0.74 &   1.63 &   0.92 &   0.80\\
  471 &   161.66719 &    59.31199 &       0.187 &       0.251 &        1.68 &        0.40 &        0.45 &        5.73 &        1.32 &        2.16 &        6.95 &        1.29 &        1.42 &        0.77 &   0.26 &   0.36 &   1.06 &   0.35 &   0.36\\
  472 &   161.66730 &    58.62923 &       1.007 &       0.830 &        1.79 &        0.35 &        0.54 &        6.76 &        1.83 &        1.88 &        8.46 &        1.41 &        1.66 &        0.84 &   0.28 &   0.34 &   1.00 &   0.29 &   0.36\\
  473 &   161.66842 &    59.43584 &       0.428 &       0.202 &        4.61 &        0.68 &        0.73 &       17.44 &        2.97 &        3.00 &       23.47 &        2.49 &        2.62 &        0.84 &   0.19 &   0.20 &   1.00 &   0.20 &   0.21\\
  474 &   161.66879 &    59.09016 &       0.332 &       0.097 &       16.16 &        1.29 &        1.34 &       18.32 &        2.53 &        2.91 &       35.18 &        2.33 &        2.67 &        0.33 &   0.05 &   0.06 &   1.79 &   0.15 &   0.15\\
  475 &   161.67117 &    58.74583 &       0.358 &       0.225 &        0.56 &        0.21 &        0.30  &$<$        1.71 &         -99 &         -99 &        1.78 &        0.62 &        0.74  &$<$        0.71 & -99.00\\
  476 &   161.67192 &    59.14685 &       0.811 &       0.375 &        3.53 &        0.63 &        0.70 &        4.23 &        1.26 &        1.70 &        8.55 &        1.15 &        1.52 &        0.35 &   0.12 &   0.15 &   1.75 &   0.30 &   0.33\\
  477 &   161.67245 &    58.87047 &       0.921 &       0.456 &        0.66 &        0.26 &        0.32 &        1.80 &        0.98 &        1.06 &        2.76 &        0.72 &        1.07 &        0.65 &   0.43 &   0.49 &   1.20 &   0.49 &   0.93\\
  478 &   161.67481 &    59.14260 &       1.758 &       0.540 &        1.55 &        0.38 &        0.49 &        5.44 &        1.34 &        2.26 &        6.96 &        1.28 &        1.62 &        0.79 &   0.28 &   0.41 &   1.05 &   0.35 &   0.39\\
  479 &   161.67665 &    59.30094 &       0.390 &       0.182 &        0.90 &        0.24 &        0.42 &        4.44 &        1.18 &        2.08 &        4.50 &        0.95 &        1.49 &        1.02 &   0.38 &   0.68 &   0.81 &   0.21 &   0.41\\
  480 &   161.67755 &    58.83199 &       0.149 &       0.060 &        2.80 &        0.46 &        0.65 &        5.86 &        1.64 &        1.68 &        9.35 &        1.33 &        1.53 &        0.53 &   0.17 &   0.20 &   1.40 &   0.29 &   0.33\\
  481 &   161.67959 &    59.43756 &       0.800 &       0.265 &        0.48 &        0.17 &        0.35 &        7.96 &        2.22 &        2.53 &        5.89 &        1.47 &        2.02 &        2.68 &   1.21 &   2.10 &   0.40 &   0.42 &   0.24\\
  482 &   161.67964 &    59.42857 &       0.347 &       0.168 &       10.27 &        0.99 &        1.14 &       17.02 &        2.56 &        2.97 &       27.88 &        2.21 &        2.60 &        0.44 &   0.08 &   0.09 &   1.55 &   0.16 &   0.17\\
  483 &   161.68019 &    58.78761 &       0.258 &       0.129 &        0.68 &        0.28 &        0.52 &        2.68 &        1.30 &        2.12 &        4.02 &        1.32 &        1.57 &        0.86 &   0.55 &   0.95 &   0.97 &   0.39 &   0.87\\
  484 &   161.68311 &    59.04186 &       0.875 &       0.197 &        0.58 &        0.20 &        0.34 &        2.82 &        0.98 &        1.68 &        3.35 &        0.92 &        1.21 &        1.02 &   0.50 &   0.86 &   0.81 &   0.25 &   0.61\\
  485 &   161.68331 &    59.36296 &       0.324 &       0.139 &        0.76 &        0.21 &        0.38 &       15.28 &        2.83 &        3.40 &       14.08 &        2.42 &        2.64 &        3.13 &   1.04 &   1.72 &   0.31 &   0.34 &   0.21\\
  486 &   161.68364 &    59.00796 &       0.496 &       0.202 &        1.39 &        0.30 &        0.48 &        9.19 &        2.08 &        2.34 &        9.07 &        1.46 &        2.04 &        1.29 &   0.41 &   0.55 &   0.68 &   0.11 &   0.26\\
  487 &   161.68590 &    59.18812 &       0.848 &       0.448 &        2.84 &        0.46 &        0.65 &       17.74 &        2.67 &        3.65 &       20.69 &        2.34 &        2.95 &        1.23 &   0.27 &   0.38 &   0.69 &   0.08 &   0.18\\
  488 &   161.69038 &    59.32674 &       0.144 &       0.106 &        1.03 &        0.27 &        0.40 &       12.03 &        2.49 &        2.77 &       11.41 &        1.92 &        2.27 &        2.04 &   0.68 &   0.92 &   0.53 &   0.18 &   0.14\\
  489 &   161.69072 &    58.74867 &       0.211 &       0.144 &        0.53 &        0.21 &        0.31 &        0.63 &        0.42 &        0.83 &        1.64 &        0.51 &        0.60 &        0.35 &   0.27 &   0.50 &   1.76 &   0.77 &   0.78\\
  490 &   161.69079 &    59.16690 &       1.485 &       0.673 &        1.07 &        0.26 &        0.44 &        7.95 &        1.69 &        2.64 &        8.53 &        1.52 &        1.99 &        1.42 &   0.46 &   0.75 &   0.66 &   0.15 &   0.22\\
  491 &   161.69312 &    59.26248 &       0.275 &       0.309 &        1.21 &        0.30 &        0.45 &        7.63 &        1.84 &        2.33 &        8.59 &        1.59 &        1.91 &        1.24 &   0.43 &   0.60 &   0.69 &   0.12 &   0.33\\
  492 &   161.69353 &    59.44222 &       0.760 &       0.282 &        1.36 &        0.42 &        0.58 &        0.22 &        0.18 &        0.76 &        1.93 &        0.50 &        0.57 &        0.08 &   0.07 &   0.27 &   2.53 &   0.77 &   0.20\\
  493 &   161.69381 &    59.21195 &       0.492 &       0.609 &        3.64 &        0.66 &        0.73 &        3.23 &        1.00 &        1.61 &        7.26 &        1.03 &        1.38 &        0.28 &   0.10 &   0.15 &   1.95 &   0.37 &   0.29\\
  494 &   161.69562 &    58.93841 &       0.466 &       0.225 &        7.50 &        0.88 &        0.93 &       10.33 &        1.84 &        2.41 &       17.70 &        1.75 &        1.93 &        0.39 &   0.08 &   0.10 &   1.66 &   0.19 &   0.21\\
  495 &   161.69684 &    59.36803 &       0.263 &       0.134 &        0.44 &        0.19 &        0.30 &        1.49 &        0.67 &        1.35 &        2.29 &        0.75 &        0.90 &        0.77 &   0.48 &   0.87 &   1.06 &   0.45 &   0.86\\
  496 &   161.69771 &    59.02276 &       0.513 &       0.188 &        1.04 &        0.29 &        0.38 &       31.20 &        4.04 &        4.91 &       28.35 &        3.63 &        3.88 &        4.32 &   1.31 &   1.70 &   0.08 &   0.34 &   0.26\\
  497 &   161.69820 &    58.91253 &       0.982 &       0.364 &        1.83 &        0.42 &        0.48 &        5.29 &        1.45 &        1.91 &        7.20 &        1.25 &        1.48 &        0.68 &   0.24 &   0.30 &   1.16 &   0.31 &   0.41\\
  498 &   161.69937 &    58.75779 &       0.171 &       0.107 &        1.27 &        0.40 &        0.54 &        4.58 &        1.68 &        2.05 &        4.75 &        1.10 &        1.79 &        0.81 &   0.39 &   0.50 &   1.03 &   0.35 &   0.57\\
  499 &   161.70019 &    59.01776 &       0.774 &       0.304 &        1.14 &        0.34 &        0.46 &        0.99 &        0.55 &        0.96 &        2.97 &        0.71 &        0.80 &        0.27 &   0.17 &   0.29 &   1.96 &   0.61 &   0.51\\
  500 &   161.70040 &    58.77576 &       0.298 &       0.121 &        1.21 &        0.39 &        0.80 &        0.91 &        0.83 &        1.08 &        2.32 &        0.67 &        1.26 &        0.25 &   0.24 &   0.33 &   2.05 &   0.72 &   0.69\\
  501 &   161.70547 &    59.36830 &       0.513 &       0.229 &        0.12 &        0.06 &        0.25 &        3.16 &        1.18 &        2.10 &        3.05 &        1.20 &        1.48 &        3.94 &   2.61 &   8.61 &   0.15 &   1.56 &   0.52\\
  502 &   161.70633 &    58.92563 &       0.658 &       0.364 &        4.58 &        0.70 &        0.82 &        4.40 &        1.26 &        1.67 &        9.35 &        1.22 &        1.49 &        0.30 &   0.10 &   0.12 &   1.90 &   0.31 &   0.28\\
  503 &   161.70955 &    59.29027 &       0.222 &       0.163 &        0.05 &        0.04 &        0.17 &       31.33 &        5.46 &        5.97 &       25.16 &        4.16 &        5.88 &       47.22 &  39.65 & 160.01 &  -2.40 &   4.56 &   1.82\\
  504 &   161.71068 &    59.17701 &       1.362 &       0.780 &        0.26 &        0.15 &        0.21 &        8.78 &        2.36 &        2.71 &        8.53 &        2.17 &        2.22 &        4.74 &   3.06 &   4.15 &  -0.01 &   0.83 &   0.61\\
  505 &   161.71264 &    58.67483 &       0.521 &       0.306 &        4.35 &        0.69 &        0.81 &        3.79 &        1.25 &        1.48 &        7.89 &        1.11 &        1.38 &        0.27 &   0.10 &   0.12 &   1.96 &   0.31 &   0.29\\
  506 &   161.71609 &    58.81412 &       0.332 &       0.065 &        0.23 &        0.13 &        0.23 &        2.61 &        0.98 &        1.74 &        3.73 &        1.07 &        1.42 &        1.96 &   1.31 &   2.31 &   0.55 &   0.46 &   0.65\\
  507 &   161.72052 &    58.72957 &       0.169 &       0.257 &        0.13 &        0.08 &        0.21 &        5.18 &        1.89 &        1.96 &        3.53 &        1.23 &        1.74 &        5.55 &   3.96 &   9.37 &  -0.17 &   1.30 &   0.79\\
  508 &   161.72068 &    59.43064 &       0.650 &       0.400 &        2.06 &        0.40 &        0.60 &        4.85 &        1.38 &        1.84 &        6.78 &        1.24 &        1.36 &        0.58 &   0.20 &   0.28 &   1.32 &   0.34 &   0.36\\
  509 &   161.72083 &    59.39664 &       0.464 &       0.229 &        0.09 &        0.08 &        0.15 &       11.02 &        2.47 &        3.97 &        8.98 &        2.26 &        3.31 &       12.80 &  11.78 &  21.36 &  -1.41 &   0.61 &   2.22\\
  510 &   161.72166 &    59.27249 &       0.443 &       0.271 &        0.06 &        0.05 &        0.19 &        5.19 &        1.81 &        2.55 &        5.80 &        1.71 &        2.69 &       10.73 &   9.57 &  36.67 &  -1.20 &   1.20 &   1.91\\
  511 &   161.72226 &    58.95976 &       0.837 &       0.379 &        1.93 &        0.41 &        0.64 &        2.46 &        1.04 &        1.31 &        4.05 &        0.82 &        1.12 &        0.36 &   0.17 &   0.23 &   1.71 &   0.42 &   0.49\\
  512 &   161.72739 &    58.96783 &       0.648 &       0.378 &        3.39 &        0.60 &        0.66  &$<$        7.97 &         -99 &         -99 &        7.94 &        1.26 &        1.59  &$<$        0.58 & -99.00\\
  513 &   161.72778 &    59.27574 &       0.283 &       0.298 &        0.25 &        0.13 &        0.29 &        0.43 &        0.39 &        0.70 &        1.22 &        0.45 &        0.66 &        0.46 &   0.47 &   0.91 &   1.53 &   0.86 &   1.28\\
  514 &   161.72822 &    59.24457 &       0.382 &       0.459 &        0.21 &        0.10 &        0.29 &        4.31 &        1.41 &        2.33 &        2.78 &        0.97 &        1.66 &        3.16 &   1.79 &   4.63 &   0.31 &   0.92 &   0.36\\
  515 &   161.72826 &    59.19306 &       0.497 &       0.469 &        4.58 &        0.65 &        0.81 &       10.51 &        2.17 &        2.42 &       14.84 &        1.84 &        1.96 &        0.57 &   0.14 &   0.17 &   1.34 &   0.24 &   0.24\\
  516 &   161.73022 &    58.64720 &       0.756 &       0.635 &        0.58 &        0.23 &        0.28 &        8.55 &        2.06 &        2.61 &        8.22 &        1.78 &        1.99 &        2.45 &   1.13 &   1.40 &   0.45 &   0.28 &   0.23\\
  517 &   161.73123 &    59.05038 &       0.174 &       0.075 &       33.44 &        1.76 &        1.80 &       99.55 &        6.25 &        6.87 &      132.13 &        5.39 &        5.61 &        0.69 &   0.05 &   0.06 &   1.14 &   0.06 &   0.08\\
  518 &   161.73572 &    59.35080 &       0.136 &       0.068 &        2.94 &        0.49 &        0.63 &        5.83 &        1.51 &        1.73 &        8.43 &        1.28 &        1.38 &        0.51 &   0.16 &   0.19 &   1.44 &   0.30 &   0.31\\
  519 &   161.73776 &    59.38896 &       0.356 &       0.156 &        0.55 &        0.19 &        0.41 &        3.51 &        1.22 &        2.09 &        5.04 &        1.35 &        1.55 &        1.26 &   0.62 &   1.19 &   0.69 &   0.24 &   0.53\\
  520 &   161.74549 &    58.99991 &       0.815 &       0.311 &        2.12 &        0.47 &        0.52 &        4.62 &        1.32 &        1.75 &        7.19 &        1.15 &        1.47 &        0.55 &   0.20 &   0.25 &   1.37 &   0.34 &   0.38\\
  521 &   161.74856 &    59.34565 &       0.140 &       0.068 &        3.96 &        0.61 &        0.71 &        4.95 &        1.21 &        1.75 &        8.65 &        1.17 &        1.34 &        0.36 &   0.10 &   0.14 &   1.73 &   0.28 &   0.29\\
  522 &   161.75090 &    59.31642 &       0.241 &       0.106 &        0.20 &        0.09 &        0.27  &$<$        2.62 &         -99 &         -99 &        0.82 &        0.60 &        0.70  &$<$        2.28 & -99.00\\
  523 &   161.75172 &    59.34610 &       0.154 &       0.165 &        0.26 &        0.11 &        0.27 &       11.42 &        2.42 &        3.35 &        5.77 &        1.73 &        2.03 &        5.82 &   2.69 &   6.31 &  -0.22 &   1.17 &   0.54\\
  524 &   161.75292 &    58.73609 &       0.494 &       0.139 &        0.21 &        0.11 &        0.24  &$<$        3.06 &         -99 &         -99 &        1.64 &        0.71 &        1.11  &$<$        2.44 & -99.00\\
  525 &   161.75340 &    58.83963 &       0.282 &       0.073 &        3.20 &        0.54 &        0.59 &        6.96 &        1.48 &        2.04 &       10.62 &        1.39 &        1.58 &        0.55 &   0.15 &   0.19 &   1.38 &   0.28 &   0.26\\
  526 &   161.75435 &    59.27799 &       0.211 &       0.095 &        1.68 &        0.39 &        0.44 &        7.68 &        1.55 &        2.38 &        9.29 &        1.48 &        1.74 &        0.97 &   0.30 &   0.39 &   0.87 &   0.20 &   0.31\\
  527 &   161.75483 &    59.31855 &       0.271 &       0.095 &        0.21 &        0.11 &        0.24 &        4.28 &        1.24 &        2.32 &        3.16 &        0.91 &        1.71 &        3.17 &   1.87 &   4.03 &   0.30 &   0.81 &   0.37\\
  528 &   161.75680 &    59.24286 &       0.414 &       0.305 &        0.96 &        0.24 &        0.42 &        6.01 &        1.59 &        2.07 &        6.42 &        1.19 &        1.76 &        1.23 &   0.45 &   0.69 &   0.69 &   0.14 &   0.36\\
  529 &   161.75723 &    59.11453 &       0.760 &       0.521 &        1.50 &        0.47 &        0.50 &        0.26 &        0.22 &        0.58 &        1.20 &        0.39 &        0.42 &        0.08 &   0.07 &   0.19 &   2.53 &   0.54 &   0.22\\
  530 &   161.75753 &    58.83951 &       0.416 &       0.169 &        0.44 &        0.22 &        0.30 &        0.22 &        0.18 &        0.74 &        0.96 &        0.39 &        0.43 &        0.18 &   0.18 &   0.63 &   2.23 &   1.21 &   0.52\\
  531 &   161.75775 &    59.28465 &       0.143 &       0.121 &        1.65 &        0.34 &        0.53 &        3.30 &        1.20 &        1.25 &        5.13 &        0.87 &        1.25 &        0.51 &   0.22 &   0.26 &   1.43 &   0.36 &   0.46\\
  532 &   161.75782 &    59.11042 &       0.563 &       0.345 &        2.27 &        0.43 &        0.55 &        4.88 &        1.29 &        1.68 &        7.90 &        1.22 &        1.37 &        0.54 &   0.18 &   0.23 &   1.38 &   0.32 &   0.33\\
  533 &   161.75782 &    59.41962 &       0.568 &       0.330 &        2.34 &        0.69 &        1.08 &        1.02 &        0.93 &        1.21 &        3.18 &        0.95 &        1.27 &        0.16 &   0.16 &   0.21 &   2.29 &   0.59 &   0.46\\
  534 &   161.75901 &    59.17276 &       0.802 &       0.542 &        0.39 &        0.15 &        0.34 &        1.24 &        0.73 &        1.02 &        2.25 &        0.60 &        1.05 &        0.72 &   0.50 &   0.86 &   1.11 &   0.49 &   1.01\\
  535 &   161.76677 &    58.88109 &       0.959 &       0.232 &        1.62 &        0.34 &        0.54 &        6.96 &        1.56 &        2.50 &        7.46 &        1.46 &        1.61 &        0.92 &   0.28 &   0.45 &   0.91 &   0.25 &   0.31\\
  536 &   161.76679 &    59.40866 &       0.527 &       0.354 &        0.20 &        0.18 &        0.33 &        8.76 &        3.05 &        5.21 &       10.13 &        2.98 &        4.69 &        5.82 &   5.58 &  10.10 &  -0.23 &   1.28 &   2.28\\
  537 &   161.76682 &    59.38654 &       0.232 &       0.096 &        4.68 &        0.67 &        0.77 &        6.63 &        1.37 &        2.13 &       11.59 &        1.37 &        1.63 &        0.40 &   0.10 &   0.14 &   1.64 &   0.25 &   0.26\\
  538 &   161.76813 &    59.40859 &       0.543 &       0.316  &$<$        0.34 &         -99 &         -99 &        5.44 &        2.37 &        3.67 &        5.46 &        2.14 &        2.65  &$>$        2.59 & -99.00\\
  539 &   161.77032 &    59.35826 &       0.088 &       0.049 &        7.08 &        0.79 &        0.93 &       10.27 &        1.80 &        2.34 &       17.56 &        1.74 &        1.83 &        0.40 &   0.08 &   0.11 &   1.62 &   0.18 &   0.21\\
  540 &   161.77044 &    59.05794 &       0.404 &       0.402 &        1.91 &        0.36 &        0.54 &        5.34 &        1.30 &        1.88 &        7.85 &        1.20 &        1.51 &        0.66 &   0.20 &   0.30 &   1.18 &   0.31 &   0.34\\
  541 &   161.77084 &    58.98011 &       1.014 &       0.521 &        1.52 &        0.46 &        0.53 &        0.47 &        0.26 &        0.97 &        1.88 &        0.52 &        0.60 &        0.13 &   0.08 &   0.27 &   2.40 &   0.74 &   0.23\\
  542 &   161.77107 &    59.12455 &       0.223 &       0.164 &        3.26 &        0.55 &        0.60 &       85.73 &        7.09 &        7.70 &       82.54 &        6.04 &        6.75 &        3.89 &   0.73 &   0.80 &   0.16 &   0.16 &   0.15\\
  543 &   161.77108 &    59.18537 &       0.954 &       0.681 &        1.05 &        0.30 &        0.40 &        9.02 &        2.30 &        2.35 &        9.87 &        1.70 &        2.21 &        1.59 &   0.61 &   0.73 &   0.62 &   0.15 &   0.23\\
  544 &   161.77348 &    58.75141 &       0.157 &       0.082 &        4.85 &        0.60 &        0.77 &       12.02 &        1.95 &        2.50 &       16.83 &        1.68 &        2.06 &        0.60 &   0.12 &   0.16 &   1.28 &   0.21 &   0.21\\
  545 &   161.77452 &    58.79512 &       0.314 &       0.116 &        0.44 &        0.16 &        0.29 &        4.58 &        1.58 &        1.64 &        4.50 &        1.21 &        1.39 &        1.87 &   0.95 &   1.41 &   0.56 &   0.28 &   0.35\\
  546 &   161.77875 &    58.86377 &       0.692 &       0.233 &        1.89 &        0.45 &        0.51  &$<$        3.45 &         -99 &         -99 &        4.06 &        0.84 &        1.15  &$<$        0.48 & -99.00\\
  547 &   161.77880 &    59.33647 &       0.148 &       0.149  &$<$        0.14 &         -99 &         -99 &        2.96 &        1.11 &        1.97 &        2.95 &        0.96 &        1.59  &$>$        3.34 & -99.00\\
  548 &   161.77886 &    59.24427 &       0.368 &       0.400 &        0.07 &        0.06 &        0.17 &        6.71 &        2.21 &        2.63 &        7.15 &        2.04 &        2.71 &       10.39 &   9.62 &  24.10 &  -1.14 &   0.90 &   2.21\\
  549 &   161.77899 &    59.16963 &       0.341 &       0.191 &       13.59 &        1.14 &        1.24 &       15.52 &        2.10 &        2.77 &       27.93 &        2.06 &        2.30 &        0.34 &   0.06 &   0.07 &   1.78 &   0.17 &   0.16\\
  550 &   161.77913 &    59.00383 &       0.712 &       0.472 &        0.66 &        0.23 &        0.32 &       30.29 &        4.09 &        5.40 &       29.58 &        3.94 &        4.50 &        6.08 &   2.17 &   3.04 &  -0.28 &   0.61 &   0.43\\
  551 &   161.78025 &    59.21416 &       0.391 &       0.287 &        5.75 &        0.74 &        0.97 &       11.29 &        2.03 &        2.95 &       18.03 &        1.95 &        2.43 &        0.51 &   0.11 &   0.16 &   1.44 &   0.27 &   0.20\\
  552 &   161.78045 &    59.38444 &       0.347 &       0.173 &        0.86 &        0.30 &        0.51 &        4.11 &        1.83 &        1.95 &        3.26 &        1.01 &        1.62 &        1.00 &   0.56 &   0.76 &   0.83 &   0.24 &   0.73\\
  553 &   161.78110 &    59.17942 &       0.685 &       0.389 &        1.38 &        0.31 &        0.50 &        8.64 &        1.79 &        2.77 &        9.79 &        1.76 &        1.93 &        1.23 &   0.38 &   0.59 &   0.69 &   0.12 &   0.28\\
  554 &   161.78111 &    59.30946 &       0.400 &       0.106 &        0.15 &        0.09 &        0.24 &        3.27 &        1.31 &        1.95 &        3.58 &        1.04 &        1.94 &        3.44 &   2.52 &   6.02 &   0.25 &   1.20 &   0.66\\
  555 &   161.78115 &    58.91178 &       0.995 &       0.300 &        0.44 &        0.21 &        0.35 &        0.25 &        0.21 &        0.85 &        0.88 &        0.35 &        0.53 &        0.20 &   0.19 &   0.69 &   2.18 &   1.24 &   0.55\\
  556 &   161.78240 &    59.41781 &       0.505 &       0.191 &        0.39 &        0.15 &        0.34 &        5.87 &        1.93 &        2.30 &        5.53 &        1.53 &        1.77 &        2.48 &   1.23 &   2.34 &   0.44 &   0.47 &   0.25\\
  557 &   161.78274 &    58.89440 &       0.743 &       0.268 &        2.39 &        0.43 &        0.57 &       11.61 &        2.14 &        2.82 &       12.83 &        1.88 &        2.03 &        1.01 &   0.26 &   0.34 &   0.82 &   0.15 &   0.27\\
  558 &   161.78362 &    58.64323 &       0.933 &       0.469 &        1.87 &        0.41 &        0.46 &       15.53 &        2.60 &        3.34 &       14.70 &        1.98 &        2.62 &        1.55 &   0.43 &   0.51 &   0.63 &   0.10 &   0.09\\
  559 &   161.78386 &    58.69912 &       0.483 &       0.416 &        1.85 &        0.47 &        0.53 &        0.81 &        0.41 &        0.93 &        2.85 &        0.63 &        0.71 &        0.16 &   0.09 &   0.19 &   2.29 &   0.55 &   0.27\\
  560 &   161.78723 &    59.08111 &       0.806 &       0.289 &        1.24 &        0.30 &        0.49 &        1.42 &        0.77 &        0.84 &        2.59 &        0.65 &        0.74 &        0.34 &   0.20 &   0.24 &   1.79 &   0.46 &   0.58\\
  561 &   161.78893 &    58.64536 &       0.676 &       0.467 &        3.18 &        0.55 &        0.60 &       12.67 &        2.30 &        2.76 &       13.93 &        1.72 &        2.22 &        0.87 &   0.22 &   0.25 &   0.96 &   0.25 &   0.24\\
  562 &   161.78898 &    58.80035 &       0.262 &       0.115 &        1.73 &        0.35 &        0.48 &        7.55 &        1.60 &        2.22 &        9.14 &        1.49 &        1.62 &        0.93 &   0.27 &   0.38 &   0.90 &   0.22 &   0.29\\
  563 &   161.79443 &    58.85748 &       0.517 &       0.251 &        2.86 &        0.53 &        0.71 &        1.03 &        0.42 &        1.08 &        3.49 &        0.63 &        0.83 &        0.14 &   0.06 &   0.15 &   2.35 &   0.45 &   0.19\\
  564 &   161.79875 &    58.82083 &       0.297 &       0.148 &        2.28 &        0.43 &        0.52 &        9.28 &        1.88 &        2.31 &       10.85 &        1.56 &        1.80 &        0.88 &   0.24 &   0.30 &   0.95 &   0.25 &   0.27\\
  565 &   161.79891 &    59.03465 &       0.321 &       0.230 &        5.52 &        0.72 &        0.82 &        9.23 &        1.87 &        2.08 &       14.89 &        1.67 &        1.77 &        0.45 &   0.11 &   0.12 &   1.54 &   0.20 &   0.23\\
  566 &   161.79906 &    59.15639 &       0.273 &       0.137 &       11.83 &        1.01 &        1.15 &       19.75 &        2.49 &        3.02 &       32.15 &        2.38 &        2.47 &        0.45 &   0.07 &   0.08 &   1.54 &   0.14 &   0.14\\
  567 &   161.80112 &    59.32180 &       0.000 &       0.232  &$<$        0.41 &         -99 &         -99 &        0.87 &        0.75 &        1.99 &        1.65 &        0.68 &        1.72  &$>$        0.54 & -99.00\\
  568 &   161.80227 &    59.30708 &       0.107 &       0.079 &        1.32 &        0.35 &        0.46 &        3.16 &        1.16 &        1.41 &        4.61 &        0.87 &        1.30 &        0.59 &   0.27 &   0.33 &   1.31 &   0.39 &   0.52\\
  569 &   161.80233 &    59.39647 &       0.118 &       0.052 &       10.58 &        0.99 &        1.14 &       16.47 &        2.56 &        2.77 &       27.54 &        2.27 &        2.37 &        0.42 &   0.08 &   0.08 &   1.58 &   0.14 &   0.17\\
  570 &   161.80574 &    59.28859 &       0.151 &       0.068 &        3.15 &        0.57 &        0.69 &        1.50 &        0.69 &        0.89 &        4.75 &        0.80 &        0.88 &        0.17 &   0.09 &   0.11 &   2.25 &   0.32 &   0.25\\
  571 &   161.80648 &    59.25031 &       0.093 &       0.075 &       22.03 &        1.44 &        1.54 &       30.79 &        3.32 &        3.50 &       52.98 &        2.88 &        3.22 &        0.39 &   0.05 &   0.05 &   1.65 &   0.10 &   0.12\\
  572 &   161.80663 &    59.14525 &       0.342 &       0.224 &        2.48 &        0.42 &        0.59 &        7.67 &        1.73 &        1.95 &       10.11 &        1.38 &        1.70 &        0.72 &   0.20 &   0.25 &   1.12 &   0.26 &   0.31\\
  573 &   161.80672 &    58.71093 &       0.682 &       0.385 &        0.18 &        0.13 &        0.19 &       12.60 &        2.61 &        4.04 &       10.28 &        2.59 &        2.95 &        8.38 &   6.11 &   9.25 &  -0.74 &   0.82 &   1.22\\
  574 &   161.80943 &    58.86533 &       0.720 &       0.257 &        1.18 &        0.30 &        0.44 &       13.29 &        2.59 &        3.15 &       12.06 &        1.96 &        2.51 &        1.98 &   0.63 &   0.87 &   0.54 &   0.17 &   0.13\\
  575 &   161.81107 &    58.76252 &       0.273 &       0.102 &        3.29 &        0.54 &        0.63 &        5.91 &        1.25 &        1.96 &        8.82 &        1.27 &        1.37 &        0.47 &   0.13 &   0.18 &   1.50 &   0.31 &   0.26\\
  576 &   161.81164 &    59.05681 &       0.399 &       0.443 &        1.05 &        0.34 &        0.57 &        1.95 &        0.88 &        1.77 &        3.20 &        0.91 &        1.21 &        0.49 &   0.27 &   0.51 &   1.48 &   0.65 &   0.65\\
  577 &   161.81217 &    58.80037 &       0.457 &       0.189 &        0.49 &        0.21 &        0.26 &        4.65 &        1.53 &        1.82 &        5.96 &        1.27 &        1.75 &        1.73 &   0.93 &   1.15 &   0.59 &   0.23 &   0.44\\
  578 &   161.81430 &    59.32040 &       0.102 &       0.067 &        0.68 &        0.29 &        0.36 &       19.79 &        3.49 &        5.05 &       17.23 &        3.31 &        3.65 &        4.22 &   1.93 &   2.49 &   0.10 &   0.50 &   0.39\\
  579 &   161.81445 &    59.16274 &       0.678 &       0.235 &        1.08 &        0.27 &        0.47 &        1.29 &        0.62 &        1.01 &        2.41 &        0.54 &        0.87 &        0.35 &   0.19 &   0.31 &   1.76 &   0.57 &   0.55\\
  580 &   161.81761 &    59.34980 &       0.253 &       0.126 &        1.34 &        0.44 &        0.61 &        3.12 &        1.36 &        2.11 &        4.48 &        1.13 &        1.65 &        0.58 &   0.31 &   0.47 &   1.33 &   0.54 &   0.67\\
  581 &   161.82608 &    59.05176 &       0.240 &       0.229 &        0.86 &        0.25 &        0.40 &        1.25 &        0.61 &        0.99 &        1.94 &        0.48 &        0.81 &        0.41 &   0.23 &   0.37 &   1.62 &   0.56 &   0.63\\
  582 &   161.82801 &    58.85538 &       0.674 &       0.309 &        2.29 &        0.51 &        0.57 &        1.63 &        0.71 &        1.10 &        4.34 &        0.73 &        1.03 &        0.24 &   0.12 &   0.17 &   2.07 &   0.46 &   0.34\\
  583 &   161.82808 &    59.02129 &       0.506 &       0.342 &        0.77 &        0.24 &        0.33 &       12.14 &        2.14 &        3.10 &       11.73 &        1.83 &        2.54 &        2.58 &   0.93 &   1.28 &   0.42 &   0.26 &   0.18\\
  584 &   161.82809 &    58.81608 &       0.463 &       0.146 &        2.72 &        0.55 &        0.61 &        4.66 &        1.19 &        2.05 &        7.45 &        1.18 &        1.50 &        0.46 &   0.15 &   0.23 &   1.53 &   0.37 &   0.33\\
  585 &   161.82851 &    58.99964 &       0.314 &       0.207 &       10.19 &        0.99 &        1.09 &        9.57 &        1.71 &        2.04 &       20.68 &        1.71 &        1.94 &        0.29 &   0.06 &   0.07 &   1.91 &   0.19 &   0.17\\
  586 &   161.83665 &    59.28864 &       0.182 &       0.126 &        1.64 &        0.34 &        0.52 &        4.75 &        1.17 &        1.97 &        6.37 &        1.05 &        1.49 &        0.68 &   0.22 &   0.36 &   1.16 &   0.37 &   0.36\\
  587 &   161.84176 &    58.70711 &       0.713 &       0.417 &        1.26 &        0.35 &        0.41 &        3.18 &        1.23 &        1.29 &        4.48 &        0.85 &        1.27 &        0.61 &   0.29 &   0.32 &   1.27 &   0.36 &   0.56\\
  588 &   161.84386 &    58.84265 &       0.465 &       0.154 &        6.92 &        0.79 &        0.89 &       12.69 &        2.14 &        2.53 &       19.88 &        1.94 &        2.04 &        0.48 &   0.10 &   0.11 &   1.49 &   0.19 &   0.18\\
  589 &   161.84453 &    58.71595 &       0.476 &       0.190 &        5.04 &        0.68 &        0.84 &        6.10 &        1.36 &        1.91 &       11.18 &        1.36 &        1.54 &        0.35 &   0.09 &   0.12 &   1.75 &   0.25 &   0.26\\
  590 &   161.84532 &    58.89162 &       1.330 &       0.448 &        0.08 &        0.06 &        0.25 &        0.09 &        0.09 &        0.58 &        1.20 &        0.45 &        0.65 &        0.35 &   0.46 &   2.52 &   1.74 &   1.38 &   1.32\\
  591 &   161.84673 &    58.78906 &       0.738 &       0.277 &        0.54 &        0.23 &        0.29 &        1.81 &        0.73 &        1.38 &        2.11 &        0.62 &        0.98 &        0.76 &   0.45 &   0.71 &   1.07 &   0.43 &   0.77\\
  592 &   161.84718 &    59.40702 &       0.439 &       0.173 &        1.33 &        0.32 &        0.52 &        2.03 &        0.70 &        1.51 &        3.16 &        0.67 &        1.05 &        0.42 &   0.18 &   0.35 &   1.59 &   0.53 &   0.46\\
  593 &   161.84759 &    59.37088 &       0.186 &       0.180 &        0.68 &        0.22 &        0.37 &        2.69 &        1.20 &        1.27 &        2.77 &        0.70 &        1.22 &        0.87 &   0.48 &   0.62 &   0.97 &   0.33 &   0.69\\
  594 &   161.84925 &    59.14429 &       0.343 &       0.200 &        0.53 &        0.23 &        0.28 &        3.82 &        1.18 &        1.90 &        5.16 &        1.26 &        1.43 &        1.38 &   0.72 &   1.01 &   0.66 &   0.20 &   0.53\\
  595 &   161.85122 &    59.20865 &       0.467 &       0.370 &        3.45 &        0.51 &        0.69 &       17.97 &        2.80 &        3.27 &       19.90 &        2.31 &        2.59 &        1.07 &   0.23 &   0.29 &   0.76 &   0.09 &   0.23\\
  596 &   161.85411 &    59.01934 &       0.473 &       0.281 &        1.30 &        0.29 &        0.47 &        5.74 &        1.40 &        2.03 &        6.45 &        1.28 &        1.42 &        0.94 &   0.31 &   0.47 &   0.89 &   0.24 &   0.35\\
  597 &   161.85575 &    58.98808 &       0.466 &       0.458 &        2.94 &        0.50 &        0.72 &        2.86 &        0.83 &        1.55 &        6.47 &        0.94 &        1.27 &        0.30 &   0.10 &   0.18 &   1.89 &   0.39 &   0.29\\
  598 &   161.85814 &    59.17385 &       0.286 &       0.138 &        8.33 &        0.89 &        0.94 &       14.03 &        2.02 &        2.71 &       23.00 &        1.94 &        2.20 &        0.45 &   0.08 &   0.10 &   1.54 &   0.17 &   0.16\\
  599 &   161.86191 &    59.31701 &       0.275 &       0.141 &        0.34 &        0.15 &        0.30  &$<$        0.62 &         -99 &         -99 &        1.04 &        0.42 &        0.62  &$<$        0.48 & -99.00\\
  600 &   161.86260 &    59.02548 &       0.384 &       0.274 &        1.41 &        0.31 &        0.49 &        3.78 &        1.07 &        1.64 &        5.00 &        0.94 &        1.24 &        0.64 &   0.23 &   0.35 &   1.22 &   0.38 &   0.38\\
  601 &   161.87087 &    59.09237 &       0.087 &       0.059 &       11.95 &        1.07 &        1.12 &       10.10 &        1.64 &        2.10 &       22.09 &        1.66 &        1.94 &        0.27 &   0.05 &   0.06 &   1.98 &   0.18 &   0.15\\
  602 &   161.87278 &    59.05213 &       0.208 &       0.268 &        0.43 &        0.20 &        0.26  &$<$        2.86 &         -99 &         -99 &        1.97 &        0.77 &        0.95  &$<$        1.29 & -99.00\\
  603 &   161.87557 &    58.71723 &       0.639 &       0.308 &        3.03 &        0.51 &        0.60 &       11.96 &        2.01 &        2.85 &       14.68 &        1.91 &        2.04 &        0.86 &   0.21 &   0.27 &   0.97 &   0.26 &   0.22\\
  604 &   161.87780 &    59.44953 &       0.934 &       0.495 &        0.19 &        0.13 &        0.20  &$<$        8.63 &         -99 &         -99 &        5.58 &        6.40 &        0.00  &$<$        5.97 & -99.00\\
  605 &   161.87907 &    59.42814 &       0.628 &       0.291 &        0.69 &        0.21 &        0.41 &        1.89 &        0.77 &        1.44 &        2.47 &        0.63 &        1.09 &        0.66 &   0.33 &   0.63 &   1.19 &   0.51 &   0.63\\
  606 &   161.87948 &    58.92823 &       0.951 &       0.471 &        0.52 &        0.23 &        0.25 &       13.78 &        2.74 &        3.34 &       12.19 &        2.25 &        2.71 &        3.92 &   0.22 &   0.33 &   0.16 &   0.07 &   0.04\\
  607 &   161.88224 &    59.40914 &       0.392 &       0.154 &        1.49 &        0.34 &        0.49 &        4.40 &        1.38 &        1.63 &        6.05 &        1.18 &        1.31 &        0.69 &   0.27 &   0.34 &   1.15 &   0.35 &   0.44\\
  608 &   161.88276 &    58.82668 &       0.816 &       0.520 &        1.29 &        0.39 &        0.45 &        4.48 &        1.73 &        1.81 &        5.49 &        1.14 &        1.76 &        0.78 &   0.38 &   0.42 &   1.05 &   0.35 &   0.58\\
  609 &   161.88326 &    59.33422 &       0.227 &       0.092 &        4.59 &        0.95 &        1.17  &$<$        2.22 &         -99 &         -99 &        5.76 &        1.07 &        1.58  &$<$        0.18 & -99.00\\
  610 &   161.88578 &    58.79174 &       0.990 &       0.243 &        1.23 &        0.33 &        0.42 &        4.24 &        1.19 &        1.84 &        5.22 &        1.13 &        1.26 &        0.78 &   0.30 &   0.43 &   1.06 &   0.36 &   0.44\\
  611 &   161.88719 &    59.16748 &       0.442 &       0.216 &        0.21 &        0.11 &        0.24 &        5.16 &        1.70 &        2.02 &        5.61 &        1.29 &        2.11 &        3.75 &   2.28 &   4.55 &   0.19 &   0.91 &   0.46\\
  612 &   161.88746 &    59.38206 &       0.281 &       0.121 &        0.38 &        0.16 &        0.29 &        3.50 &        1.15 &        1.89 &        3.84 &        1.00 &        1.49 &        1.67 &   0.87 &   1.56 &   0.60 &   0.31 &   0.43\\
  613 &   161.88940 &    59.35217 &       0.217 &       0.100 &        2.74 &        0.49 &        0.64 &        2.70 &        0.78 &        1.46 &        6.03 &        0.88 &        1.18 &        0.30 &   0.10 &   0.18 &   1.88 &   0.39 &   0.30\\
  614 &   161.89061 &    59.04169 &       0.327 &       0.160 &        1.64 &        0.42 &        0.54 &        0.36 &        0.20 &        0.75 &        1.79 &        0.38 &        0.59 &        0.10 &   0.06 &   0.21 &   2.48 &   0.60 &   0.17\\
  615 &   161.89193 &    58.71429 &       0.723 &       0.503 &        1.83 &        0.41 &        0.46  &$<$        8.85 &         -99 &         -99 &        5.58 &        1.13 &        1.54  &$<$        1.01 & -99.00\\
  616 &   161.89381 &    59.21118 &       0.954 &       0.467 &        0.97 &        0.31 &        0.36  &$<$        6.46 &         -99 &         -99 &        3.86 &        1.11 &        1.30  &$<$        1.29 & -99.00\\
  617 &   161.89971 &    59.09721 &       0.169 &       0.097 &        1.29 &        0.28 &        0.45 &        4.10 &        1.17 &        1.55 &        5.55 &        1.03 &        1.23 &        0.73 &   0.26 &   0.37 &   1.11 &   0.38 &   0.40\\
  618 &   161.90126 &    58.96821 &       0.968 &       0.548 &        1.80 &        0.44 &        0.50 &        5.20 &        1.28 &        2.16 &        6.64 &        1.18 &        1.55 &        0.68 &   0.24 &   0.34 &   1.16 &   0.35 &   0.39\\
  619 &   161.90322 &    59.06836 &       0.138 &       0.079 &        1.33 &        0.33 &        0.42 &       15.12 &        2.76 &        3.03 &       15.00 &        2.11 &        2.62 &        2.00 &   0.61 &   0.75 &   0.54 &   0.15 &   0.12\\
  620 &   161.90442 &    59.32797 &       0.211 &       0.108 &        0.66 &        0.20 &        0.39 &        1.71 &        0.70 &        1.31 &        2.01 &        0.66 &        0.79 &        0.63 &   0.32 &   0.61 &   1.24 &   0.55 &   0.62\\
  621 &   161.90504 &    59.30367 &       0.127 &       0.195 &        0.59 &        0.19 &        0.38  &$<$        1.99 &         -99 &         -99 &        1.30 &        0.49 &        0.87  &$<$        0.77 & -99.00\\
  622 &   161.90579 &    59.37734 &       0.214 &       0.182 &        1.46 &        0.32 &        0.50 &        3.73 &        1.16 &        1.59 &        4.81 &        0.98 &        1.20 &        0.62 &   0.24 &   0.34 &   1.25 &   0.38 &   0.42\\
  623 &   161.90872 &    59.02707 &       0.135 &       0.121 &        6.15 &        0.74 &        0.83 &       12.18 &        1.95 &        2.49 &       17.43 &        1.76 &        1.94 &        0.51 &   0.10 &   0.12 &   1.44 &   0.21 &   0.17\\
  624 &   161.90991 &    58.87900 &       0.595 &       0.423 &        4.01 &        0.69 &        0.78 &        2.48 &        1.02 &        1.08 &        6.50 &        1.04 &        1.07 &        0.21 &  28.51 & 209.28 &   2.14 &   9.16 &  83.52\\
  625 &   161.91161 &    58.83839 &       0.832 &       0.380 &        0.96 &        0.27 &        0.41 &        5.22 &        1.41 &        2.13 &        5.57 &        1.29 &        1.46 &        1.11 &   1.91 &   2.08 &   0.72 &   0.42 &   4.41\\
  626 &   161.91292 &    59.19493 &       0.653 &       0.386 &        5.23 &        0.67 &        0.88 &       16.17 &        2.59 &        3.30 &       21.31 &        2.36 &        2.50 &        0.71 &   0.15 &   0.19 &   1.12 &   0.19 &   0.22\\
  627 &   161.91421 &    58.70311 &       1.098 &       0.413 &        1.60 &        0.37 &        0.52 &        2.91 &        0.95 &        1.57 &        6.05 &        1.06 &        1.27 &        0.48 &   0.19 &   0.30 &   1.49 &   0.44 &   0.43\\
  628 &   161.91509 &    59.23380 &       0.773 &       0.374 &        1.44 &        0.34 &        0.57 &        1.09 &        0.64 &        0.89 &        2.79 &        0.68 &        0.77 &        0.25 &   0.16 &   0.23 &   2.04 &   0.54 &   0.46\\
  629 &   161.92386 &    59.33626 &       0.283 &       0.122 &        0.60 &        0.24 &        0.29 &        3.76 &        1.24 &        1.72 &        4.30 &        1.07 &        1.36 &        1.23 &   0.63 &   0.82 &   0.69 &   0.16 &   0.59\\
  630 &   161.93001 &    59.41114 &       0.559 &       0.255 &        1.98 &        0.44 &        0.55 &        4.53 &        1.35 &        1.82 &        5.89 &        1.17 &        1.30 &        0.57 &   0.21 &   0.28 &   1.34 &   0.35 &   0.39\\
  631 &   161.93130 &    59.31370 &       0.096 &       0.042 &       28.66 &        1.62 &        1.82 &       33.47 &        3.24 &        3.74 &       61.73 &        3.09 &        3.33 &        0.34 &   0.04 &   0.04 &   1.77 &   0.11 &   0.11\\
  632 &   161.93622 &    59.43041 &       0.818 &       0.279 &        3.42 &        0.65 &        0.87 &        3.61 &        1.10 &        2.14 &        7.36 &        1.25 &        1.61 &        0.32 &   0.11 &   0.20 &   1.83 &   0.42 &   0.33\\
  633 &   161.93683 &    59.09411 &       0.176 &       0.067 &        1.21 &        0.32 &        0.42 &        1.32 &        0.49 &        1.13 &        3.19 &        0.66 &        0.81 &        0.32 &   0.15 &   0.30 &   1.82 &   0.57 &   0.43\\
  634 &   161.94017 &    59.47282 &       1.172 &       0.343 &        1.90 &        0.38 &        0.57 &       18.47 &        3.00 &        3.84 &       19.36 &        2.71 &        2.91 &        1.75 &   0.45 &   0.64 &   0.59 &   0.13 &   0.09\\
  635 &   161.94115 &    59.43337 &       1.211 &       0.469 &        1.40 &        0.36 &        0.55  &$<$        5.86 &         -99 &         -99 &        3.85 &        1.16 &        1.34  &$<$        0.90 & -99.00\\
  636 &   161.94353 &    59.39784 &       0.810 &       0.330 &        0.16 &        0.10 &        0.21 &        5.56 &        2.03 &        2.11 &        4.89 &        1.29 &        2.29 &        4.90 &   3.70 &   6.70 &  -0.04 &   1.34 &   0.74\\
  637 &   161.94784 &    59.13585 &       0.272 &       0.124 &        1.72 &        0.38 &        0.48 &        2.43 &        0.80 &        1.32 &        3.92 &        0.73 &        0.97 &        0.39 &   0.16 &   0.24 &   1.64 &   0.42 &   0.42\\
  638 &   161.94846 &    59.09104 &       0.064 &       0.036 &        5.07 &        0.62 &        0.68 &       25.65 &        2.88 &        3.62 &       31.73 &        2.69 &        2.86 &        1.04 &   0.17 &   0.20 &   0.78 &   0.10 &   0.18\\
  639 &   161.94923 &    58.94985 &       1.093 &       0.497 &        0.87 &        0.28 &        0.47 &        0.28 &        0.24 &        0.63 &        1.09 &        0.38 &        0.45 &        0.13 &   0.05 &   0.18 &   2.39 &   0.52 &   0.15\\
  640 &   161.94944 &    59.33758 &       0.417 &       0.302 &        0.32 &        0.15 &        0.29 &        1.41 &        0.58 &        1.47 &        0.72 &        0.40 &        0.70 &        0.93 &   0.57 &   1.28 &   0.90 &   0.41 &   0.82\\
  641 &   161.94994 &    59.22637 &       0.523 &       0.291 &        2.01 &        0.40 &        0.60 &        3.54 &        1.23 &        1.48 &        5.57 &        1.07 &        1.18 &        0.47 &   0.19 &   0.24 &   1.51 &   0.38 &   0.43\\
  642 &   161.95019 &    59.07950 &       0.264 &       0.115 &        0.53 &        0.26 &        0.42 &        1.67 &        0.92 &        1.62 &        2.79 &        0.86 &        1.39 &        0.72 &   0.53 &   0.91 &   1.11 &   0.50 &   1.09\\
  643 &   161.95116 &    59.09294 &       0.162 &       0.086 &        0.88 &        0.26 &        0.35 &        1.93 &        0.77 &        1.15 &        2.45 &        0.57 &        0.91 &        0.55 &   0.27 &   0.40 &   1.37 &   0.48 &   0.59\\
  644 &   161.95118 &    59.34363 &       0.266 &       0.153 &        0.02 &        0.02 &        0.10 &       13.48 &        3.45 &        4.45 &       14.50 &        3.60 &        4.60 &       59.30 &  61.22 & 374.31 &  -2.74 &  10.67 &  11.11\\
  645 &   161.95309 &    59.39135 &       0.262 &       0.102 &        9.54 &        0.94 &        1.09 &       19.26 &        2.66 &        3.28 &       27.97 &        2.32 &        2.63 &        0.52 &   0.09 &   0.11 &   1.43 &   0.18 &   0.15\\
  646 &   161.95356 &    59.03560 &       0.280 &       0.201 &        0.54 &        0.19 &        0.32 &        3.28 &        1.21 &        1.47 &        3.53 &        0.89 &        1.30 &        1.20 &   0.61 &   0.89 &   0.70 &   0.18 &   0.60\\
  647 &   161.95666 &    58.81267 &       0.437 &       0.367 &        0.06 &        0.05 &        0.19 &        5.77 &        1.67 &        3.12 &        5.73 &        1.99 &        2.39 &       11.52 &   0.10 &   0.10 &  -1.36 &   0.02 &   0.02\\
  648 &   161.96159 &    59.09229 &       0.213 &       0.111 &        0.53 &        0.20 &        0.29 &        2.10 &        0.84 &        1.25 &        2.35 &        0.60 &        1.03 &        0.87 &   0.47 &   0.69 &   0.97 &   0.34 &   0.68\\
  649 &   161.96227 &    58.93202 &       0.360 &       0.175 &        8.62 &        0.90 &        1.05 &       16.01 &        2.38 &        2.98 &       25.44 &        2.18 &        2.48 &        0.49 &   0.09 &   0.11 &   1.48 &   0.18 &   0.16\\
  650 &   161.96273 &    58.98966 &       0.313 &       0.325 &        3.11 &        0.52 &        0.61 &        5.66 &        1.42 &        1.62 &        8.74 &        1.21 &        1.39 &        0.48 &   0.14 &   0.17 &   1.49 &   0.28 &   0.30\\
  651 &   161.96301 &    58.86113 &       0.309 &       0.227 &        2.26 &        0.48 &        0.53 &        5.41 &        1.50 &        1.74 &        8.05 &        1.27 &        1.48 &        0.59 &   0.21 &   0.23 &   1.30 &   0.29 &   0.37\\
  652 &   161.96447 &    58.81062 &       0.435 &       0.256 &        2.35 &        0.48 &        0.58 &        6.67 &        1.45 &        2.30 &       10.53 &        1.49 &        1.79 &        0.67 &   0.20 &   0.28 &   1.17 &   0.29 &   0.34\\
  653 &   161.96538 &    59.04217 &       0.301 &       0.296 &        0.37 &        0.16 &        0.25  &$<$        3.43 &         -99 &         -99 &        1.79 &        0.58 &        1.17  &$<$        1.68 & -99.00\\
  654 &   161.96731 &    59.26434 &       0.329 &       0.161 &        9.03 &        0.95 &        1.00 &       15.81 &        2.40 &        2.80 &       24.33 &        2.07 &        2.36 &        0.46 &   0.09 &   0.10 &   1.51 &   0.16 &   0.17\\
  655 &   161.96978 &    59.20682 &       0.286 &       0.229 &        0.70 &        0.26 &        0.31 &        5.03 &        1.58 &        1.86 &        5.64 &        1.34 &        1.52 &        1.38 &   0.67 &   0.80 &   0.66 &   0.16 &   0.46\\
  656 &   161.97706 &    59.00163 &       0.350 &       0.332 &        0.39 &        0.19 &        0.31 &        0.85 &        0.59 &        0.89 &        1.34 &        0.43 &        0.88 &        0.55 &   0.46 &   0.72 &   1.38 &   0.69 &   1.15\\
  657 &   161.97725 &    59.45315 &       1.335 &       0.330 &        2.00 &        0.41 &        0.64 &        5.31 &        1.35 &        2.33 &        6.69 &        1.36 &        1.51 &        0.64 &   0.21 &   0.35 &   1.22 &   0.38 &   0.35\\
  658 &   161.97832 &    59.13619 &       0.238 &       0.124 &        0.68 &        0.20 &        0.37 &        1.45 &        0.79 &        0.86 &        2.85 &        0.69 &        0.87 &        0.54 &   0.33 &   0.43 &   1.39 &   0.53 &   0.76\\
  659 &   161.98464 &    59.12749 &       0.336 &       0.104 &        0.11 &        0.10 &        0.13 &        2.67 &        0.92 &        1.98 &        2.89 &        0.94 &        1.56 &        3.69 &   3.60 &   5.18 &   0.20 &   1.04 &   2.28\\
  660 &   161.98681 &    58.89306 &       0.440 &       0.303 &        0.63 &        0.22 &        0.37 &        0.93 &        0.48 &        1.07 &        1.65 &        0.52 &        0.70 &        0.41 &   0.25 &   0.53 &   1.61 &   0.72 &   0.70\\
  661 &   161.98995 &    58.83665 &       0.704 &       0.274 &        0.83 &        0.24 &        0.45 &        1.46 &        0.71 &        1.15 &        2.04 &        0.61 &        0.82 &        0.46 &   0.53 &   0.75 &   1.51 &   0.82 &   1.44\\
  662 &   161.99051 &    58.83715 &       0.300 &       0.209 &        2.64 &        0.48 &        0.63 &        5.86 &        1.50 &        1.93 &        8.19 &        1.20 &        1.59 &        0.55 &   0.87 &   1.30 &   1.36 &   0.79 &   2.32\\
  663 &   161.99362 &    59.34696 &       0.718 &       0.292 &        1.08 &        0.28 &        0.47 &        2.46 &        0.79 &        1.61 &        3.40 &        0.82 &        1.04 &        0.57 &   0.23 &   0.45 &   1.34 &   0.53 &   0.45\\
  664 &   161.99423 &    59.26186 &       0.471 &       0.325 &        1.10 &        0.27 &        0.46 &        5.83 &        1.68 &        1.96 &        6.11 &        1.40 &        1.43 &        1.08 &   0.41 &   0.58 &   0.74 &   0.14 &   0.42\\
  665 &   161.99433 &    59.03686 &       0.407 &       0.164 &        0.11 &        0.06 &        0.23 &        0.64 &        0.39 &        1.06 &        1.35 &        0.50 &        0.90 &        1.15 &   0.94 &   3.05 &   0.71 &   0.61 &   1.46\\
  666 &   161.99518 &    59.18001 &       0.463 &       0.353 &        0.04 &        0.04 &        0.10 &        1.32 &        0.96 &        1.12 &        2.03 &        0.82 &        1.55 &        5.03 &   6.23 &  14.01 &  -0.07 &   1.52 &   6.33\\
  667 &   161.99537 &    58.85380 &       0.318 &       0.255 &        0.86 &        0.24 &        0.37 &        6.86 &        1.70 &        2.18 &        7.20 &        1.35 &        1.79 &        1.50 &   0.56 &   0.81 &   0.64 &   0.16 &   0.25\\
  668 &   161.99859 &    59.03537 &       0.321 &       0.165 &        0.70 &        0.23 &        0.38 &        0.64 &        0.45 &        0.68 &        1.08 &        0.38 &        0.53 &        0.28 &   0.22 &   0.34 &   1.93 &   0.68 &   0.64\\
  669 &   162.00040 &    58.93963 &       0.608 &       0.364 &        0.51 &        0.19 &        0.34 &        3.19 &        1.18 &        1.71 &        4.25 &        1.06 &        1.46 &        1.24 &   0.43 &   0.66 &   0.69 &   0.13 &   0.34\\
  670 &   162.00296 &    58.83595 &       0.134 &       0.080 &        5.93 &        0.67 &        0.85 &       14.11 &        2.15 &        2.71 &       20.39 &        1.99 &        2.09 &        0.59 &   0.11 &   0.14 &   1.31 &   0.20 &   0.19\\
  671 &   162.00397 &    59.15943 &       0.352 &       0.269 &        0.21 &        0.11 &        0.24 &        5.59 &        1.58 &        2.43 &        4.27 &        1.13 &        2.00 &        3.88 &   2.27 &   4.77 &   0.16 &   0.95 &   0.45\\
  672 &   162.00548 &    58.93987 &       0.571 &       0.300 &        2.05 &        0.44 &        0.55 &        4.79 &        1.30 &        1.96 &        7.57 &        1.21 &        1.55 &        0.58 &   0.65 &   1.06 &   1.32 &   0.71 &   1.66\\
  673 &   162.00616 &    59.35126 &       0.789 &       0.085 &        0.65 &        0.20 &        0.38  &$<$        5.39 &         -99 &         -99 &        2.47 &        0.86 &        1.22  &$<$        1.55 & -99.00\\
  674 &   162.01238 &    59.40946 &       0.468 &       0.254 &        1.69 &        0.45 &        0.52 &        1.12 &        0.66 &        0.91 &        3.27 &        0.74 &        0.83 &        0.22 &   0.14 &   0.19 &   2.11 &   0.52 &   0.42\\
  675 &   162.01283 &    59.32950 &       0.259 &       0.118 &       15.27 &        1.26 &        1.31 &       21.00 &        2.73 &        3.10 &       36.76 &        2.44 &        2.80 &        0.39 &   0.06 &   0.07 &   1.66 &   0.13 &   0.15\\
  676 &   162.01421 &    58.92982 &       0.165 &       0.082 &       22.44 &        1.51 &        1.56 &       24.63 &        2.78 &        3.30 &       47.78 &        2.78 &        2.86 &        0.33 &   0.04 &   0.05 &   1.81 &   0.12 &   0.12\\
  677 &   162.01716 &    59.16935 &       0.570 &       0.302 &        0.77 &        0.24 &        0.38 &        2.21 &        0.88 &        1.32 &        2.73 &        0.79 &        0.92 &        0.68 &   0.34 &   0.53 &   1.16 &   0.46 &   0.63\\
  678 &   162.01851 &    59.01263 &       0.216 &       0.204 &        0.92 &        0.29 &        0.34 &        6.21 &        1.59 &        2.05 &        7.39 &        1.47 &        1.63 &        1.31 &   0.53 &   0.65 &   0.68 &   0.13 &   0.38\\
  679 &   162.02368 &    58.85969 &       0.096 &       0.061 &        9.14 &        0.89 &        1.03 &       12.92 &        2.13 &        2.32 &       22.63 &        1.85 &        2.10 &        0.39 &   0.08 &   0.08 &   1.64 &   0.15 &   0.19\\
  680 &   162.02880 &    58.87952 &       0.235 &       0.161 &        1.04 &        0.30 &        0.39 &        2.37 &        0.82 &        1.41 &        3.25 &        0.73 &        1.02 &        0.57 &   0.25 &   0.40 &   1.34 &   0.48 &   0.51\\
  681 &   162.02940 &    58.93929 &       0.534 &       0.307 &        0.45 &        0.18 &        0.34 &        1.22 &        0.67 &        1.18 &        2.11 &        0.62 &        0.99 &        0.65 &  10.03 &  39.48 &   1.21 &   3.40 &  29.05\\
  682 &   162.02947 &    59.42744 &       1.195 &       0.540 &        0.89 &        0.26 &        0.41 &        4.85 &        1.60 &        1.90 &        5.37 &        1.11 &        1.72 &        1.11 &   0.49 &   0.67 &   0.72 &   0.14 &   0.54\\
  683 &   162.02972 &    58.80563 &       0.407 &       0.198 &        1.27 &        0.32 &        0.56 &        0.40 &        0.37 &        0.48 &        2.00 &        0.50 &        0.57 &        0.13 &   0.12 &   0.16 &   2.39 &   0.48 &   0.36\\
  684 &   162.03014 &    58.70683 &       0.411 &       0.282 &       17.52 &        1.33 &        1.53 &       13.12 &        2.09 &        2.45 &       31.03 &        2.20 &        2.31 &        0.25 &   0.04 &   0.05 &   2.05 &   0.15 &   0.13\\
  685 &   162.03114 &    59.21415 &       0.717 &       0.340 &        3.04 &        0.52 &        0.74 &        2.19 &        0.76 &        1.30 &        5.02 &        0.90 &        0.99 &        0.24 &   0.09 &   0.15 &   2.07 &   0.42 &   0.27\\
  686 &   162.03225 &    59.26124 &       1.087 &       0.433 &        0.26 &        0.14 &        0.25 &        4.34 &        1.51 &        2.14 &        3.04 &        0.99 &        1.64 &        2.73 &   1.79 &   2.97 &   0.39 &   0.59 &   0.49\\
  687 &   162.03265 &    58.70073 &       1.218 &       0.570 &        1.20 &        0.28 &        0.45 &       10.95 &        2.22 &        2.72 &       10.64 &        1.79 &        2.12 &        1.67 &   0.17 &   0.23 &   0.60 &   0.05 &   0.03\\
  688 &   162.03426 &    59.32076 &       0.658 &       0.345 &        0.86 &        0.25 &        0.40 &        5.41 &        1.55 &        2.05 &        6.26 &        1.27 &        1.73 &        1.24 &   0.51 &   0.74 &   0.69 &   0.15 &   0.41\\
  689 &   162.03732 &    59.33909 &       0.745 &       0.331 &        2.36 &        0.43 &        0.63 &        5.24 &        1.25 &        2.07 &        7.66 &        1.15 &        1.58 &        0.56 &   0.17 &   0.27 &   1.36 &   0.35 &   0.30\\
  690 &   162.03777 &    58.79595 &       0.230 &       0.200 &        1.90 &        0.38 &        0.52 &        6.62 &        1.67 &        1.90 &        8.76 &        1.38 &        1.61 &        0.78 &   0.25 &   0.31 &   1.05 &   0.32 &   0.35\\
  691 &   162.03807 &    59.25625 &       0.805 &       0.536 &        2.45 &        0.53 &        0.59 &        4.08 &        1.27 &        1.74 &        7.13 &        1.13 &        1.53 &        0.45 &   0.17 &   0.22 &   1.54 &   0.37 &   0.41\\
  692 &   162.04211 &    59.22668 &       0.634 &       0.266 &        3.37 &        0.53 &        0.68 &        6.15 &        1.55 &        1.76 &        9.40 &        1.30 &        1.49 &        0.48 &   0.14 &   0.17 &   1.49 &   0.28 &   0.29\\
  693 &   162.04297 &    59.42349 &       1.497 &       0.415 &        1.08 &        0.32 &        0.43 &        2.51 &        1.00 &        1.50 &        4.34 &        0.96 &        1.20 &        0.58 &   0.29 &   0.41 &   1.33 &   0.49 &   0.59\\
  694 &   162.04455 &    59.01048 &       0.227 &       0.142 &        9.99 &        0.93 &        1.13 &        7.07 &        1.49 &        1.67 &       17.37 &        1.50 &        1.70 &        0.24 &   0.05 &   0.06 &   2.08 &   0.18 &   0.16\\
  695 &   162.04826 &    59.23798 &       1.123 &       0.439 &        0.86 &        0.24 &        0.43 &        5.26 &        1.57 &        2.11 &        6.03 &        1.40 &        1.58 &        1.21 &   0.49 &   0.78 &   0.70 &   0.15 &   0.42\\
  696 &   162.04877 &    59.17967 &       0.184 &       0.053 &       25.78 &        1.61 &        1.71 &       22.25 &        2.51 &        3.17 &       49.11 &        2.67 &        2.90 &        0.27 &   0.04 &   0.04 &   1.96 &   0.12 &   0.10\\
  697 &   162.05065 &    58.99232 &       0.762 &       0.433 &        0.96 &        0.24 &        0.42 &        2.56 &        1.01 &        1.24 &        3.20 &        0.74 &        1.04 &        0.64 &   0.30 &   0.42 &   1.22 &   0.45 &   0.55\\
  698 &   162.05102 &    59.04933 &       0.268 &       0.239 &        0.45 &        0.18 &        0.27 &        4.10 &        1.35 &        1.60 &        4.08 &        1.05 &        1.35 &        1.67 &   0.87 &   1.19 &   0.60 &   0.24 &   0.42\\
  699 &   162.05365 &    58.90921 &       0.367 &       0.164 &        0.32 &        0.14 &        0.29 &        1.58 &        0.71 &        1.43 &        1.28 &        0.56 &        0.86 &        1.02 &   0.65 &   1.31 &   0.81 &   0.33 &   0.89\\
  700 &   162.05644 &    59.06140 &       0.246 &       0.091 &        1.34 &        0.34 &        0.44 &        1.88 &        0.75 &        1.12 &        2.80 &        0.66 &        0.83 &        0.39 &   0.19 &   0.27 &   1.65 &   0.46 &   0.51\\
  701 &   162.05775 &    58.78234 &       0.330 &       0.378 &        1.40 &        0.33 &        0.47 &        2.63 &        0.86 &        1.42 &        3.59 &        0.75 &        1.02 &        0.49 &   0.20 &   0.31 &   1.47 &   0.44 &   0.44\\
  702 &   162.05819 &    58.84325 &       0.108 &       0.071 &        4.02 &        0.55 &        0.73 &        7.60 &        1.44 &        2.15 &       11.42 &        1.43 &        1.52 &        0.49 &   0.11 &   0.17 &   1.47 &   0.28 &   0.22\\
  703 &   162.06159 &    59.06084 &       0.264 &       0.084 &        0.48 &        0.19 &        0.28 &        1.63 &        0.66 &        1.25 &        1.79 &        0.59 &        0.81 &        0.78 &   0.44 &   0.75 &   1.06 &   0.43 &   0.73\\
  704 &   162.06198 &    59.39384 &       0.866 &       0.570 &        1.80 &        0.41 &        0.59 &        6.28 &        1.54 &        2.61 &        7.67 &        1.53 &        1.69 &        0.78 &   0.26 &   0.41 &   1.05 &   0.35 &   0.37\\
  705 &   162.06389 &    58.77160 &       0.300 &       0.535 &        1.51 &        0.39 &        0.50 &        2.31 &        0.92 &        1.38 &        3.41 &        0.87 &        0.89 &        0.42 &   0.12 &   0.30 &   1.59 &   0.48 &   0.30\\
  706 &   162.06788 &    59.17916 &       0.497 &       0.295 &       11.16 &        3.45 &        5.55 &        0.00 &        0.00 &        0.06 &        0.04 &        0.01 &        0.01 &      -99.00 &   0.00 &   0.21 & -99.00 &   0.00 &   0.00\\
  707 &   162.06929 &    58.73347 &       0.480 &       0.600 &        0.46 &        0.17 &        0.30 &        6.26 &        1.81 &        2.10 &        6.38 &        1.52 &        1.72 &        2.32 &   0.51 &   0.75 &   0.47 &   0.15 &   0.10\\
  708 &   162.06992 &    59.30044 &       0.494 &       0.242 &        3.20 &        0.51 &        0.70 &       12.81 &        2.46 &        2.71 &       15.38 &        2.00 &        2.27 &        0.87 &   0.22 &   0.27 &   0.96 &   0.25 &   0.23\\
  709 &   162.07547 &    58.99822 &       0.604 &       0.416 &        4.46 &        0.76 &        0.82 &        0.77 &        0.42 &        0.74 &        4.15 &        0.68 &        0.73 &        0.08 &   0.05 &   0.08 &   2.53 &   0.23 &   0.14\\
  710 &   162.07732 &    58.75889 &       0.421 &       0.392 &        1.33 &        0.37 &        0.43 &        4.67 &        1.47 &        1.73 &        6.13 &        1.24 &        1.38 &        0.79 &   0.33 &   0.39 &   1.05 &   0.34 &   0.48\\
  711 &   162.07884 &    58.87794 &       0.227 &       0.096 &        1.82 &        0.44 &        0.56 &        0.90 &        0.50 &        0.87 &        2.79 &        0.63 &        0.71 &        0.18 &   0.11 &   0.18 &   2.24 &   0.52 &   0.32\\
  712 &   162.08032 &    58.77503 &       0.375 &       0.270 &        0.52 &        0.18 &        0.31 &        9.66 &        2.15 &        2.68 &       10.95 &        1.88 &        2.45 &        2.95 &   1.22 &   1.93 &   0.35 &   0.39 &   0.24\\
  713 &   162.08136 &    59.16027 &       0.343 &       0.279 &        0.44 &        0.16 &        0.29  &$<$        4.03 &         -99 &         -99 &        1.13 &        0.55 &        0.89  &$<$        1.68 & -99.00\\
  714 &   162.08250 &    59.15625 &       0.301 &       0.109 &        4.13 &        0.62 &        0.72 &        3.37 &        0.86 &        1.48 &        7.40 &        1.00 &        1.15 &        0.26 &   0.08 &   0.12 &   2.00 &   0.33 &   0.23\\
  715 &   162.08455 &    59.29939 &       1.491 &       0.603 &        0.97 &        0.27 &        0.47 &        2.67 &        1.10 &        1.49 &        2.92 &        0.91 &        0.97 &        0.66 &   0.33 &   0.49 &   1.19 &   0.48 &   0.62\\
  716 &   162.08477 &    58.84637 &       0.090 &       0.052 &        5.34 &        0.66 &        0.85 &        7.02 &        1.49 &        1.84 &       12.26 &        1.30 &        1.62 &        0.37 &   0.09 &   0.11 &   1.69 &   0.22 &   0.24\\
  717 &   162.08708 &    59.03494 &       0.428 &       0.261 &        0.44 &        0.21 &        0.23 &        5.75 &        1.73 &        2.02 &        3.85 &        1.04 &        1.57 &        2.24 &   1.28 &   1.41 &   0.49 &   0.28 &   0.38\\
  718 &   162.09218 &    58.79985 &       0.340 &       0.224 &        0.28 &        0.16 &        0.23  &$<$        2.91 &         -99 &         -99 &        1.53 &        0.62 &        1.17  &$<$        1.86 & -99.00\\
  719 &   162.09224 &    59.30250 &       0.755 &       0.276 &        4.70 &        0.72 &        0.74 &       17.28 &        2.79 &        3.28 &       20.79 &        2.20 &        2.74 &        0.82 &   0.18 &   0.20 &   1.02 &   0.21 &   0.21\\
  720 &   162.09447 &    59.25816 &       1.403 &       0.507 &        2.87 &        0.49 &        0.64 &        9.20 &        1.78 &        2.68 &       12.77 &        1.62 &        2.10 &        0.74 &   0.19 &   0.27 &   1.10 &   0.27 &   0.27\\
  721 &   162.10272 &    58.82236 &       0.089 &       0.066 &        4.37 &        0.57 &        0.75 &        7.38 &        1.59 &        1.78 &       11.57 &        1.40 &        1.49 &        0.45 &   0.11 &   0.13 &   1.54 &   0.23 &   0.24\\
  722 &   162.10601 &    59.19127 &       0.713 &       0.319 &        1.15 &        0.27 &        0.45 &        9.80 &        2.13 &        2.64 &        9.79 &        1.60 &        2.24 &        1.58 &   0.51 &   0.75 &   0.62 &   0.15 &   0.13\\
  723 &   162.10789 &    59.22729 &       0.849 &       0.357 &        1.66 &        0.43 &        0.49 &        1.86 &        0.86 &        1.11 &        4.20 &        0.84 &        1.02 &        0.33 &   0.18 &   0.22 &   1.80 &   0.43 &   0.51\\
  724 &   162.10916 &    59.01519 &       0.412 &       0.248 &        4.08 &        0.61 &        0.70 &        5.51 &        1.39 &        1.58 &        9.82 &        1.20 &        1.44 &        0.38 &   0.11 &   0.13 &   1.67 &   0.24 &   0.30\\
  725 &   162.11214 &    58.91070 &       0.259 &       0.134 &        1.02 &        0.26 &        0.39 &        6.03 &        1.35 &        2.17 &        5.10 &        1.01 &        1.53 &        1.18 &   0.95 &   1.36 &   0.70 &   0.27 &   1.36\\
  726 &   162.11257 &    58.81632 &       0.180 &       0.077 &        0.45 &        0.18 &        0.27 &        7.04 &        1.66 &        2.38 &        7.29 &        1.38 &        2.06 &        2.58 &   1.20 &   1.77 &   0.42 &   0.35 &   0.24\\
  727 &   162.11267 &    58.91097 &       0.283 &       0.134 &        0.23 &        0.13 &        0.22 &        3.94 &        1.37 &        1.94 &        5.86 &        1.35 &        1.91 &        2.75 &   1.80 &   2.99 &   0.39 &   0.60 &   0.49\\
  728 &   162.11979 &    58.86678 &       0.177 &       0.143 &        1.69 &        0.47 &        0.54 &        0.25 &        0.21 &        0.56 &        1.38 &        0.38 &        0.44 &        0.07 &   0.07 &   0.17 &   2.55 &   0.48 &   0.19\\
  729 &   162.12026 &    59.07559 &       0.342 &       0.176 &        0.12 &        0.07 &        0.25 &        0.94 &        0.65 &        0.99 &        0.63 &        0.44 &        0.66 &        1.46 &   1.30 &   3.42 &   0.65 &   0.68 &   1.64\\
  730 &   162.12257 &    59.21374 &       0.519 &       0.241 &        3.63 &        0.53 &        0.72 &       15.31 &        2.39 &        3.31 &       18.30 &        2.29 &        2.44 &        0.91 &   0.19 &   0.27 &   0.92 &   0.22 &   0.20\\
  731 &   162.12725 &    58.85719 &       0.259 &       0.163 &        0.18 &        0.08 &        0.25 &        4.17 &        1.21 &        2.26 &        3.00 &        1.10 &        1.34 &        3.47 &   1.90 &   5.09 &   0.24 &   1.02 &   0.38\\
  732 &   162.13168 &    58.87301 &       0.132 &       0.073 &        0.68 &        0.20 &        0.37 &        2.85 &        1.18 &        1.24 &        3.30 &        0.85 &        1.09 &        0.91 &   0.46 &   0.63 &   0.92 &   0.29 &   0.61\\
  733 &   162.13676 &    59.28782 &       0.739 &       0.394 &        7.53 &        0.85 &        1.00 &       19.25 &        2.77 &        3.44 &       26.93 &        2.42 &        2.78 &        0.62 &   0.11 &   0.14 &   1.25 &   0.18 &   0.19\\
  734 &   162.14459 &    58.93959 &       0.463 &       0.172 &        1.79 &        0.37 &        0.51 &        4.78 &        1.31 &        1.72 &        6.45 &        1.08 &        1.39 &        0.64 &   0.22 &   0.29 &   1.22 &   0.32 &   0.37\\
  735 &   162.14851 &    58.76799 &       0.355 &       0.195 &        0.41 &        0.17 &        0.31  &$<$        4.33 &         -99 &         -99 &        2.36 &        0.88 &        1.27  &$<$        1.87 & -99.00\\
  736 &   162.15035 &    59.20196 &       1.138 &       0.382 &        1.26 &        0.32 &        0.47 &        7.12 &        1.91 &        2.20 &        8.66 &        1.60 &        1.93 &        1.14 &   0.42 &   0.55 &   0.71 &   0.11 &   0.41\\
  737 &   162.15323 &    58.90419 &       0.163 &       0.065 &        3.82 &        0.56 &        0.70 &        5.04 &        1.19 &        1.70 &        9.40 &        1.12 &        1.44 &        0.37 &   0.10 &   0.14 &   1.69 &   0.27 &   0.28\\
  738 &   162.15341 &    58.94394 &       0.573 &       0.252 &        0.57 &        0.21 &        0.31 &        3.19 &        1.04 &        1.72 &        3.25 &        0.85 &        1.26 &        1.13 &   0.56 &   0.86 &   0.71 &   0.17 &   0.62\\
  739 &   162.15439 &    58.80919 &       0.360 &       0.129 &        0.42 &        0.18 &        0.29 &        2.14 &        0.99 &        1.27 &        2.88 &        0.73 &        1.27 &        1.04 &   0.66 &   0.94 &   0.78 &   0.24 &   0.89\\
  740 &   162.15765 &    58.73261 &       0.898 &       0.508 &        0.38 &        0.15 &        0.29 &        9.05 &        2.18 &        2.77 &        6.54 &        1.70 &        1.94 &        3.62 &   1.71 &   2.98 &   0.21 &   0.59 &   0.34\\
  741 &   162.15850 &    58.86853 &       0.286 &       0.099 &        0.54 &        0.19 &        0.32 &        1.60 &        0.60 &        1.38 &        2.07 &        0.58 &        0.90 &        0.69 &   0.35 &   0.72 &   1.15 &   0.49 &   0.63\\
  742 &   162.16225 &    59.01406 &       0.567 &       0.246 &        3.75 &        0.59 &        0.64 &       10.31 &        1.76 &        2.51 &       14.25 &        1.63 &        1.94 &        0.65 &   0.15 &   0.19 &   1.20 &   0.21 &   0.26\\
  743 &   162.16483 &    58.99261 &       0.890 &       0.510 &        2.23 &        0.43 &        0.58 &        3.14 &        1.09 &        1.31 &        5.68 &        1.00 &        1.10 &        0.39 &   0.16 &   0.19 &   1.64 &   0.34 &   0.42\\
  744 &   162.16828 &    59.17153 &       0.336 &       0.167 &        0.87 &        0.24 &        0.36 &       49.00 &        5.24 &        6.16 &       49.07 &        4.86 &        5.65 &        7.15 &   2.08 &   3.06 &  -0.49 &   0.61 &   0.42\\
  745 &   162.17225 &    59.04937 &       0.310 &       0.140 &       11.46 &        1.06 &        1.16 &       12.87 &        2.22 &        2.24 &       25.09 &        1.99 &        2.15 &        0.33 &   0.07 &   0.07 &   1.79 &   0.16 &   0.19\\
  746 &   162.17464 &    58.97059 &       0.524 &       0.172 &        6.89 &        0.78 &        0.99 &       10.97 &        2.03 &        2.44 &       17.65 &        1.75 &        2.03 &        0.43 &   0.09 &   0.11 &   1.57 &   0.19 &   0.21\\
  747 &   162.17894 &    59.05602 &       0.577 &       0.350 &        0.75 &        0.22 &        0.35 &       12.07 &        2.36 &        2.86 &       12.83 &        1.95 &        2.61 &        2.62 &   0.92 &   1.36 &   0.42 &   0.27 &   0.18\\
  748 &   162.18056 &    58.76109 &       0.883 &       0.302 &        0.42 &        0.18 &        0.28 &        2.61 &        1.04 &        1.56 &        3.74 &        0.94 &        1.38 &        1.23 &   1.09 &   1.73 &   0.69 &   0.35 &   1.67\\
  749 &   162.18082 &    59.05289 &       0.728 &       0.375 &        1.24 &        0.35 &        0.40  &$<$        4.93 &         -99 &         -99 &        4.19 &        0.93 &        1.32  &$<$        0.87 & -99.00\\
  750 &   162.18353 &    59.11833 &       0.594 &       0.260 &        2.44 &        0.48 &        0.58 &        3.03 &        0.84 &        1.52 &        5.39 &        0.84 &        1.17 &        0.36 &   0.12 &   0.20 &   1.73 &   0.37 &   0.34\\
  751 &   162.18869 &    58.96257 &       0.270 &       0.111 &        9.55 &        1.02 &        1.08 &       17.26 &        2.51 &        3.13 &       26.73 &        2.33 &        2.44 &        0.48 &   0.09 &   0.10 &   1.50 &   0.17 &   0.16\\
  752 &   162.19232 &    58.87953 &       0.170 &       0.224 &        2.34 &        0.55 &        0.69 &        0.42 &        0.23 &        0.88 &        2.32 &        0.54 &        0.61 &        0.08 & -99.00 & -99.00 &   2.52 &-289.97 &  -6.39\\
  753 &   162.19598 &    59.08201 &       0.196 &       0.085 &       25.42 &        1.58 &        1.68 &       21.34 &        2.61 &        2.78 &       47.12 &        2.60 &        2.75 &        0.27 &   0.04 &   0.04 &   1.98 &   0.11 &   0.11\\
  754 &   162.19854 &    59.09482 &       0.818 &       0.364 &        0.95 &        0.28 &        0.38 &        4.31 &        1.21 &        1.87 &        4.60 &        1.00 &        1.39 &        0.96 &   0.39 &   0.57 &   0.87 &   0.24 &   0.47\\
  755 &   162.20905 &    58.98577 &       0.643 &       0.237 &        2.55 &        0.45 &        0.59 &       10.56 &        2.10 &        2.56 &       13.13 &        1.68 &        2.18 &        0.89 &   0.24 &   0.30 &   0.94 &   0.24 &   0.25\\
  756 &   162.21557 &    58.74010 &       1.084 &       0.475 &        1.63 &        0.41 &        0.47 &       13.61 &        2.55 &        3.39 &       14.46 &        2.30 &        2.49 &        1.56 &   0.73 &   1.11 &   0.63 &   0.22 &   0.38\\
  757 &   162.21742 &    58.75600 &       0.679 &       0.342 &        2.66 &        0.61 &        1.00  &$<$        4.81 &         -99 &         -99 &        4.35 &        1.24 &        1.65  &$<$        0.48 & -99.00\\
  758 &   162.21829 &    58.93622 &       0.499 &       0.320 &        0.59 &        0.23 &        0.29 &        5.80 &        1.59 &        2.09 &        6.07 &        1.35 &        1.68 &        1.76 &   0.34 &   0.41 &   0.59 &   0.08 &   0.07\\
  759 &   162.21845 &    58.79483 &       0.317 &       0.170 &        2.27 &        0.42 &        0.56 &        5.03 &        1.16 &        1.89 &        6.82 &        1.03 &        1.40 &        0.56 &   0.16 &   0.25 &   1.36 &   0.33 &   0.29\\
  760 &   162.21974 &    59.00624 &       0.812 &       0.353 &        2.14 &        0.43 &        0.53 &       11.78 &        2.21 &        2.93 &       12.84 &        1.83 &        2.27 &        1.11 &   0.29 &   0.37 &   0.72 &   0.07 &   0.29\\
  761 &   162.22031 &    58.90160 &       0.159 &       0.065 &        4.38 &        0.64 &        0.69 &       10.33 &        1.76 &        2.52 &       14.39 &        1.70 &        1.81 &        0.58 &   0.13 &   0.17 &   1.32 &   0.23 &   0.22\\
\tableline
\end{tabular}
\end{small}
\footnotesize
\tablecomments{Table \ref{xcat table1} is presented in its entirety in the electronic edition. A portion is shown here for guidance regarding its form and content.}
\tablenotetext{a}{For sources detected in one band but not in the other, we list the upper limit to the flux in the undetected band and flag that flux with a $<$ symbol.}
\tablenotetext{b}{If the source was not detected in the $0.5-2~\rm keV$ ($2-8~\rm keV$) band we list the lower (upper) limit to the hardness ratio and flag the value with a $>$ ($<$) symbol.}
\tablenotetext{c}{If the source was detected in one band but not in the other, $\Gamma=-99$.}
\end{table}


==> tab5.tex <==
\begin{table}
\begin{small}
\caption{CLANS X-ray Catalog: Additional Source Properties}
\label{xcat table2}
\begin{tabular}{cccccccccccccc}
\tableline\tableline
Number & n$_{0.5-2~\rm keV}$ & $1\sigma_{low}$ & $1\sigma_{hi}$ & n$_{2-8~\rm keV}$ & $1\sigma_{low}$ & $1\sigma_{hi}$ & n$_{0.5-8~\rm keV}$ & $1\sigma_{low}$ & $1\sigma_{hi}$ & t$_{0.5-2~\rm keV}$ ($10^4$~s) & t$_{2-8~\rm keV}$ ($10^4$~s) & t$_{0.5-8~\rm keV}$ ($10^4$~s) & R$_{arcminutes}$\\
(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)&(11)&(12)&(13)&(14) \\
\tableline
   1 &  36.50 &   5.56 &   7.63 &  26.00 &   5.07 &   6.16 &  59.75 &   7.48 &   9.04 &   5.90 &   5.34 &   5.80 &    9.7\\
   2 &  83.75 &   8.90 &  10.45 &  29.75 &   5.20 &   6.78 & 112.50 &  10.12 &  12.16 &   6.47 &   6.26 &   6.40 &    6.8\\
   3 &   6.75 &   2.35 &   4.01 &   2.25 &   1.57 &   2.38 &   9.25 &   3.21 &   3.85 &   6.48 &   6.28 &   6.41 &    6.8\\
   4 &   5.75 &   2.15 &   3.83 &   0.75 &   0.62 &   2.54 &   7.50 &   2.28 &   4.44 &   2.71 &   2.62 &   2.65 &    7.2\\
   5 &  12.75 &   3.32 &   4.94 &  13.25 &   3.82 &   4.44 &  27.00 &   5.17 &   6.26 &   5.65 &   5.40 &   5.54 &    8.5\\
   6 &  11.00 &   3.28 &   4.41 &  11.00 &   3.28 &   4.41 &  23.00 &   4.77 &   5.86 &   6.27 &   6.07 &   6.20 &    7.8\\
   7 &   4.50 &   1.68 &   3.87 &  10.00 &   3.12 &   4.26 &  13.00 &   3.57 &   4.69 &   6.50 &   6.34 &   6.45 &    6.3\\
   8 &  20.00 &   4.44 &   5.54 &   8.75 &   2.71 &   4.35 &  31.00 &   5.55 &   6.62 &   6.10 &   5.91 &   6.02 &    6.9\\
   9 &   5.25 &   2.43 &   3.12 &   9.00 &   2.96 &   4.10 &  17.00 &   4.09 &   5.20 &   6.45 &   6.27 &   6.39 &    6.6\\
  10 &  10.75 &   3.03 &   4.66 &   3.00 &   1.66 &   2.91 &  14.00 &   3.71 &   4.83 &   6.65 &   6.49 &   6.61 &    5.5\\
  11 &   5.00 &   2.18 &   3.37 &  13.25 &   3.82 &   4.44 &  19.50 &   3.94 &   6.04 &   6.37 &   6.17 &   6.30 &    7.0\\
  12 &  30.00 &   5.45 &   6.53 &  13.00 &   3.57 &   4.69 &  41.50 &   5.96 &   8.03 &   6.48 &   6.37 &   6.30 &    5.3\\
  13 &  59.25 &   7.91 &   8.47 &  23.00 &   4.77 &   5.86 &  84.50 &   8.71 &  10.75 &   6.67 &   6.46 &   6.63 &    4.9\\
  14 &   9.75 &   2.87 &   4.51 &   9.75 &   2.87 &   4.51 &  22.00 &   4.66 &   5.76 &   6.71 &   6.54 &   6.67 &    4.7\\
  15 &  66.25 &   8.36 &   8.91 &  87.00 &   9.31 &  10.36 & 145.25 &  12.28 &  12.82 &   6.77 &   6.63 &   6.75 &    4.3\\
  16 &   6.00 &   2.40 &   3.58 &   5.00 &   2.18 &   3.37 &  10.25 &   3.37 &   4.01 &   6.82 &   6.61 &   6.76 &    4.4\\
  17 &  21.00 &   4.56 &   5.65 &  46.00 &   6.76 &   7.83 &  62.50 &   7.42 &   9.48 &   6.51 &   6.33 &   6.47 &    4.2\\
  18 & 150.25 &  12.49 &  13.02 & 100.00 &   9.99 &  11.03 & 249.75 &  15.55 &  17.08 &   6.60 &   6.44 &   6.47 &    7.1\\
  19 &  26.00 &   5.07 &   6.16 &  27.00 &   5.17 &   6.26 &  46.00 &   6.76 &   7.83 &   4.18 &   4.07 &   4.14 &    9.1\\
  20 &  35.50 &   5.48 &   7.55 &  75.75 &   8.45 &  10.00 & 109.00 &  10.43 &  11.47 &   6.53 &   6.31 &   6.46 &    5.6\\
  21 &   5.75 &   2.15 &   3.83 &  13.50 &   4.07 &   4.19 &  14.75 &   3.59 &   5.20 &   6.87 &   6.65 &   6.81 &    3.7\\
  22 &   4.50 &   1.68 &   3.87 &  11.00 &   3.28 &   4.41 &  14.50 &   3.34 &   5.45 &   5.92 &   5.77 &   5.88 &    4.3\\
  23 &   4.00 &   1.94 &   3.15 &  11.50 &   3.78 &   3.91 &  17.25 &   4.34 &   4.95 &   5.32 &   5.27 &   5.28 &    8.2\\
  24 &   2.00 &   1.32 &   2.63 &  25.50 &   4.57 &   6.66 &  27.25 &   5.42 &   6.01 &   6.88 &   6.80 &   6.87 &    4.7\\
  25 &  22.75 &   4.52 &   6.11 &   8.50 &   3.28 &   3.44 &  27.75 &   5.02 &   6.60 &   6.41 &   6.13 &   6.32 &    8.8\\
  26 &   4.00 &   1.94 &   3.15 &  18.75 &   4.08 &   5.68 &  27.75 &   5.02 &   6.60 &   5.55 &   5.45 &   5.50 &    7.9\\
  27 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   7.74 &   3.25 &   1.91 &   2.66 &   6.89 &   6.70 &   6.85 &    2.9\\
  28 &  13.00 &   3.57 &   4.69 &   0.75 &   0.62 &   2.54 &  17.00 &   4.09 &   5.20 &   6.70 &   6.54 &   6.67 &    3.7\\
  29 &   0.75 &   0.62 &   2.54 &   1.50 &   1.37 &   1.79 &   4.50 &   1.68 &   3.87 &   6.85 &   6.63 &   6.80 &    3.1\\
  30 & 167.00 &  12.91 &  13.95 &  68.00 &   8.23 &   9.28 & 230.25 &  15.41 &  15.94 &   5.90 &   5.90 &   5.95 &    7.3\\
  31 &   2.00 &   1.32 &   2.63 &   9.25 &   3.21 &   3.85 &  11.25 &   3.53 &   4.16 &   6.86 &   6.63 &   6.81 &    3.0\\
  32 &   4.00 &   1.94 &   3.15 &  10.00 &   3.12 &   4.26 &  14.00 &   3.71 &   4.83 &   3.84 &   3.62 &   3.78 &    7.0\\
  33 &  56.25 &   7.72 &   8.28 &  60.75 &   7.54 &   9.10 & 117.25 &  11.06 &  11.60 &   5.59 &   5.49 &   5.57 &    7.9\\
  34 &   0.00 &   0.00 &   1.66 &   9.75 &   2.87 &   4.51 &  12.25 &   3.68 &   4.30 &   6.95 &   6.73 &   6.90 &    2.4\\
  35 &  13.75 &   3.46 &   5.08 &  16.25 &   4.22 &   4.83 &  28.00 &   5.27 &   6.35 &   6.50 &   6.48 &   6.51 &    4.5\\
  36 &  16.50 &   3.59 &   5.70 &  28.00 &   5.27 &   6.35 &  38.50 &   6.64 &   6.72 &   6.24 &   5.95 &   6.12 &   10.4\\
  37 &   2.75 &   1.41 &   3.16 &   8.00 &   2.78 &   3.94 &  10.50 &   2.78 &   4.91 &   7.05 &   6.82 &   7.00 &    1.8\\
  38 &   6.25 &   2.65 &   3.33 &   2.25 &   1.57 &   2.38 &   8.50 &   2.46 &   4.60 &   5.90 &   5.64 &   5.84 &    3.6\\
  39 &  21.75 &   4.41 &   6.01 &  11.25 &   3.53 &   4.16 &  37.25 &   6.31 &   6.88 &   7.08 &   6.85 &   7.03 &    1.7\\
  40 &  14.25 &   3.96 &   4.58 &  10.75 &   3.03 &   4.66 &  25.50 &   4.57 &   6.66 &   6.05 &   5.95 &   6.02 &    6.6\\
  41 &   2.75 &   1.41 &   3.16 &   2.75 &   1.41 &   3.16 &   8.75 &   2.71 &   4.35 &   6.99 &   6.75 &   6.93 &    2.0\\
  42 &  15.00 &   3.84 &   4.95 &   6.00 &   2.40 &   3.58 &  22.25 &   4.91 &   5.51 &   6.82 &   6.53 &   6.74 &    1.6\\
  43 &   0.00 &   0.00 &   1.66 &   5.00 &   2.18 &   3.37 &   4.50 &   1.68 &   3.87 &   7.04 &   7.11 &   7.08 &    2.0\\
  44 &  24.75 &   4.72 &   6.31 &   7.25 &   2.85 &   3.51 &  33.00 &   5.72 &   6.80 &   7.07 &   6.79 &   7.01 &    1.2\\
  45 &  35.50 &   5.48 &   7.55 &  30.00 &   5.45 &   6.53 &  60.00 &   7.73 &   8.79 &   5.89 &   5.80 &   5.86 &    7.4\\
  46 &  42.75 &   6.29 &   7.86 &  34.50 &   5.39 &   7.47 &  69.25 &   8.54 &   9.09 &   6.59 &   6.55 &   6.63 &    1.9\\
  47 &  20.50 &   4.06 &   6.15 &  19.50 &   3.94 &   6.04 &  35.00 &   5.89 &   6.97 &   5.32 &   5.23 &   5.28 &    8.4\\
  48 &  44.00 &   6.61 &   7.68 &  18.25 &   4.46 &   5.07 &  57.75 &   7.35 &   8.91 &   5.95 &   5.91 &   6.02 &    6.0\\
  49 &   2.25 &   1.57 &   2.38 &   6.75 &   2.35 &   4.01 &  10.00 &   3.12 &   4.26 &   6.93 &   6.86 &   6.92 &    4.2\\
  50 &  53.00 &   7.26 &   8.32 &  30.25 &   5.70 &   6.28 &  75.25 &   8.90 &   9.45 &   6.13 &   6.06 &   6.11 &    6.0\\
  51 &   5.50 &   1.90 &   4.08 &  24.00 &   4.87 &   5.96 &  28.25 &   5.52 &   6.10 &   6.13 &   5.98 &   6.09 &    6.3\\
  52 &   8.00 &   2.78 &   3.94 &  19.00 &   4.33 &   5.43 &  25.00 &   4.97 &   6.06 &   6.14 &   5.98 &   6.09 &    6.3\\
  53 &  91.75 &   9.33 &  10.87 &  53.00 &   7.26 &   8.32 & 138.25 &  11.99 &  12.52 &   6.50 &   6.30 &   6.42 &    8.3\\
  54 & 815.00 &  28.54 &  29.56 & 436.25 &  21.12 &  21.65 &1240.00 &  35.21 &  36.22 &   7.11 &   6.82 &   7.04 &    0.9\\
  55 &  25.25 &   5.22 &   5.81 &  11.00 &   3.28 &   4.41 &  33.25 &   5.97 &   6.55 &   7.05 &   6.99 &   7.06 &    3.2\\
  56 &  97.75 &   9.64 &  11.18 &  34.75 &   5.64 &   7.22 & 134.25 &  11.82 &  12.35 &   4.25 &   4.03 &   4.19 &    2.7\\
  57 &  68.25 &   8.48 &   9.03 &  22.75 &   4.52 &   6.11 &  86.00 &   9.26 &  10.31 &   5.70 &   5.73 &   5.70 &    8.9\\
  58 &   0.00 &   0.00 &   1.07 &  13.25 &   3.82 &   4.44 &  17.00 &   4.09 &   5.20 &   6.71 &   6.65 &   6.74 &    3.5\\
  59 &  56.75 &   7.28 &   8.84 &  11.00 &   3.28 &   4.41 &  69.00 &   8.29 &   9.34 &   5.62 &   5.54 &   5.60 &    6.8\\
  60 &  19.75 &   4.19 &   5.79 &   6.75 &   2.35 &   4.01 &  26.00 &   5.07 &   6.16 &   6.55 &   6.17 &   6.36 &    6.1\\
  61 &  23.75 &   4.62 &   6.21 &  17.00 &   4.09 &   5.20 &  35.50 &   5.48 &   7.55 &   6.04 &   5.87 &   5.97 &    7.4\\
  62 &  10.00 &   3.12 &   4.26 &   5.00 &   2.18 &   3.37 &  15.75 &   3.72 &   5.33 &   5.61 &   5.61 &   5.47 &    6.5\\
  63 &   6.00 &   2.40 &   3.58 &   1.50 &   1.37 &   1.79 &   8.25 &   3.03 &   3.69 &   7.11 &   6.82 &   7.05 &    0.5\\
  64 &   2.50 &   1.82 &   2.13 &   9.25 &   3.21 &   3.85 &  15.50 &   4.34 &   4.45 &   6.47 &   6.18 &   6.35 &    6.9\\
  65 &  14.25 &   3.96 &   4.58 &   6.25 &   2.65 &   3.33 &  22.25 &   4.91 &   5.51 &   6.24 &   6.14 &   6.22 &    5.2\\
  66 &  10.75 &   3.03 &   4.66 &   4.50 &   1.68 &   3.87 &  15.50 &   3.47 &   5.58 &   6.92 &   6.81 &   6.90 &    4.7\\
  67 &   8.50 &   2.46 &   4.60 &  17.75 &   3.96 &   5.57 &  24.50 &   4.47 &   6.56 &   5.81 &   5.78 &   5.88 &    5.2\\
  68 &   7.75 &   2.53 &   4.19 &  18.75 &   4.08 &   5.68 &  25.50 &   4.57 &   6.66 &   5.77 &   5.77 &   5.76 &    5.7\\
  69 &  48.75 &   6.73 &   8.29 &  30.25 &   5.70 &   6.28 &  79.50 &   8.43 &  10.48 &   5.99 &   5.77 &   6.12 &    6.6\\
  70 &  28.50 &   4.86 &   6.94 &   5.75 &   2.15 &   3.83 &  36.50 &   5.56 &   7.63 &   6.32 &   6.23 &   6.30 &    4.9\\
  71 &  42.00 &   6.46 &   7.53 &  14.50 &   4.21 &   4.33 &  54.50 &   6.90 &   8.96 &   5.02 &   5.02 &   5.11 &    5.0\\
  72 &   6.00 &   2.40 &   3.58 &   0.00 &   0.00 &   9.02 &   7.50 &   2.28 &   4.44 &   7.05 &   6.99 &   7.11 &    2.8\\
  73 &   4.50 &   1.68 &   3.87 &   1.25 &   1.12 &   2.04 &   4.50 &   1.68 &   3.87 &   6.32 &   6.23 &   6.31 &    4.5\\
  74 &  25.25 &   5.22 &   5.81 &  24.50 &   5.37 &   5.46 &  45.50 &   6.26 &   8.33 &   5.69 &   5.62 &   5.65 &    6.8\\
  75 &   0.25 &   0.25 &   1.58 &   2.75 &   1.41 &   3.16 &   4.50 &   1.68 &   3.87 &   6.07 &   5.99 &   6.04 &    7.7\\
  76 &  21.00 &   4.56 &   5.65 &  12.75 &   3.32 &   4.94 &  33.00 &   5.72 &   6.80 &   5.92 &   5.78 &   5.88 &    6.8\\
  77 &   4.50 &   1.68 &   3.87 &   0.00 &   0.00 &   6.33 &   5.75 &   2.15 &   3.83 &   5.92 &   5.83 &   5.81 &    4.2\\
  78 &  26.75 &   4.92 &   6.51 &   6.75 &   2.35 &   4.01 &  34.50 &   5.39 &   7.47 &   6.46 &   6.28 &   6.43 &    6.3\\
  79 &  30.75 &   5.30 &   6.87 &  10.00 &   3.12 &   4.26 &  45.00 &   6.69 &   7.76 &   5.87 &   5.81 &   5.86 &    4.6\\
  80 &   0.00 &   0.00 &   1.83 &   8.25 &   3.03 &   3.69 &   9.00 &   2.96 &   4.10 &   5.21 &   5.15 &   5.23 &    4.8\\
  81 &   6.25 &   2.65 &   3.33 &  16.00 &   3.97 &   5.08 &  19.25 &   4.58 &   5.18 &   5.89 &   5.90 &   5.86 &    5.2\\
  82 &   8.75 &   2.71 &   4.35 &  16.00 &   3.97 &   5.08 &  21.00 &   4.56 &   5.65 &   6.25 &   5.92 &   6.28 &    7.2\\
  83 &  66.75 &   7.92 &   9.47 &  29.25 &   5.61 &   6.19 &  98.25 &  10.14 &  10.68 &   6.57 &   6.36 &   6.50 &    7.6\\
  84 &   5.00 &   2.18 &   3.37 &  11.25 &   3.53 &   4.16 &  12.50 &   3.07 &   5.19 &   7.05 &   7.03 &   7.09 &    1.7\\
  85 &   4.50 &   1.68 &   3.87 &  11.00 &   3.28 &   4.41 &  13.00 &   3.57 &   4.69 &   6.21 &   6.18 &   6.21 &    6.4\\
  86 &  13.75 &   3.46 &   5.08 &  62.75 &   7.67 &   9.23 &  78.75 &   8.62 &  10.17 &   6.49 &   6.25 &   6.40 &    6.9\\
  87 &   7.50 &   2.28 &   4.44 &   0.00 &   0.00 &   5.80 &   8.50 &   2.46 &   4.60 &   5.91 &   5.96 &   5.91 &    4.7\\
  88 &   7.00 &   2.60 &   3.76 &   0.00 &   0.00 &  10.20 &   8.00 &   2.78 &   3.94 &   2.93 &   2.82 &   2.89 &    7.8\\
  89 &   4.50 &   1.68 &   3.87 &   4.75 &   1.93 &   3.62 &   4.25 &   2.19 &   2.90 &   6.42 &   6.30 &   6.41 &    3.5\\
  90 &  18.00 &   4.21 &   5.32 &   9.25 &   3.21 &   3.85 &  24.25 &   5.12 &   5.71 &   6.10 &   5.96 &   6.06 &    5.4\\
  91 &  10.75 &   3.03 &   4.66 &   4.50 &   2.44 &   2.65 &  15.50 &   4.34 &   4.45 &   6.09 &   5.80 &   5.92 &    6.9\\
  92 &   5.00 &   2.18 &   3.37 &   2.25 &   1.57 &   2.38 &  11.00 &   3.28 &   4.41 &   6.99 &   6.80 &   6.93 &    3.2\\
  93 &  86.75 &   9.06 &  10.61 &  34.50 &   5.39 &   7.47 & 119.75 &  10.69 &  12.23 &   6.33 &   6.01 &   6.19 &    7.9\\
  94 &  19.25 &   4.58 &   5.18 &   7.75 &   2.53 &   4.19 &  28.50 &   4.86 &   6.94 &   5.96 &   5.97 &   6.00 &    4.0\\
  95 &  15.00 &   3.84 &   4.95 &   6.50 &   2.10 &   4.26 &  23.00 &   4.77 &   5.86 &   5.88 &   5.97 &   5.95 &    4.0\\
  96 &  10.50 &   2.78 &   4.91 &   0.25 &   0.25 &   1.58 &  13.86 &   3.57 &   4.97 &   5.52 &   5.47 &   5.51 &    6.5\\
  97 &   8.75 &   2.71 &   4.35 &   4.00 &   1.94 &   3.15 &  13.50 &   3.21 &   5.33 &   6.67 &   6.63 &   6.70 &    3.1\\
  98 & 285.25 &  17.12 &  17.65 & 138.00 &  11.74 &  12.77 & 422.50 &  20.06 &  22.08 &   6.45 &   6.31 &   6.43 &    3.1\\
  99 &   9.75 &   2.87 &   4.51 &  12.50 &   3.07 &   5.19 &  22.75 &   4.52 &   6.11 &   6.29 &   6.29 &   6.30 &    5.8\\
 100 &   5.75 &   2.15 &   3.83 &  10.50 &   2.78 &   4.91 &  12.75 &   3.32 &   4.94 &   6.30 &   6.06 &   6.15 &    4.6\\
 101 &  13.29 &   3.86 &   4.41 &   3.25 &   1.91 &   2.66 &  17.50 &   3.71 &   5.82 &   6.21 &   6.17 &   6.20 &    6.6\\
 102 &  28.25 &   5.52 &   6.10 &   6.00 &   2.40 &   3.58 &  38.50 &   5.72 &   7.80 &   7.00 &   7.00 &   7.05 &    2.8\\
 103 &  16.75 &   3.84 &   5.45 &   1.75 &   1.07 &   2.88 &  19.50 &   3.94 &   6.04 &   6.48 &   6.34 &   6.46 &    2.9\\
 104 &   0.75 &   0.62 &   2.54 &   5.50 &   2.68 &   2.87 &   7.00 &   2.60 &   3.76 &   6.37 &   6.27 &   6.36 &    3.1\\
 105 &   2.50 &   1.16 &   3.41 &  13.25 &   3.82 &   4.44 &  10.50 &   2.78 &   4.91 &   5.81 &   5.64 &   5.73 &    7.7\\
 106 &   4.00 &   1.94 &   3.15 &  15.25 &   4.09 &   4.70 &  16.50 &   3.59 &   5.70 &   6.96 &   6.99 &   7.02 &    2.8\\
 107 &   1.50 &   1.37 &   1.79 &   3.00 &   1.66 &   2.91 &   4.25 &   2.19 &   2.90 &   6.53 &   6.41 &   6.52 &    2.3\\
 108 &   8.50 &   2.46 &   4.60 &  16.50 &   3.59 &   5.70 &  25.50 &   4.57 &   6.66 &   5.87 &   5.69 &   5.79 &    7.5\\
 109 &  18.50 &   3.83 &   5.93 &   6.57 &   2.17 &   4.19 &  21.50 &   4.16 &   6.26 &   5.88 &   5.68 &   5.79 &    7.3\\
 110 &  38.00 &   6.14 &   7.22 &  13.00 &   3.57 &   4.69 &  50.75 &   6.87 &   8.44 &   6.46 &   6.36 &   6.46 &    2.4\\
 111 &  35.25 &   6.14 &   6.72 &  17.50 &   3.71 &   5.82 &  52.75 &   7.01 &   8.57 &   6.56 &   6.45 &   6.55 &    2.0\\
 112 &  12.75 &   3.32 &   4.94 &   2.86 &   1.52 &   3.05 &  18.86 &   4.19 &   5.57 &   5.75 &   5.69 &   5.82 &    6.8\\
 113 &   5.00 &   2.18 &   3.37 &  41.50 &   5.96 &   8.03 &  45.25 &   6.94 &   7.51 &   5.51 &   5.46 &   5.54 &    6.5\\
 114 &  65.75 &   7.86 &   9.41 &  25.75 &   4.82 &   6.41 &  95.50 &   9.29 &  11.33 &   6.35 &   6.03 &   6.20 &    7.8\\
 115 &  61.50 &   7.36 &   9.41 &  34.00 &   5.81 &   6.88 &  95.00 &   9.73 &  10.78 &   5.76 &   5.61 &   5.68 &    7.7\\
 116 &  16.00 &   3.97 &   5.08 &  33.50 &   5.31 &   7.38 &  47.00 &   6.84 &   7.90 &   6.53 &   6.60 &   6.58 &    3.3\\
 117 &   4.50 &   1.68 &   3.87 &   6.25 &   2.65 &   3.33 &  10.00 &   3.12 &   4.26 &   6.23 &   6.28 &   6.25 &    4.2\\
 118 &  14.00 &   3.71 &   4.83 &   0.00 &   0.00 &  16.03 &  17.00 &   4.09 &   5.20 &   5.93 &   5.71 &   5.83 &    6.9\\
 119 &   0.75 &   0.62 &   2.54 &   6.50 &   2.90 &   3.08 &  11.50 &   2.93 &   5.05 &   6.32 &   6.16 &   6.29 &    3.3\\
 120 &   5.00 &   2.18 &   3.37 &   5.25 &   2.43 &   3.12 &  13.75 &   3.46 &   5.08 &   5.76 &   5.70 &   5.75 &    6.8\\
 121 & 173.25 &  13.39 &  13.93 &  73.00 &   8.53 &   9.58 & 243.75 &  15.36 &  16.89 &   5.63 &   5.55 &   5.70 &    7.2\\
 122 &  15.25 &   4.09 &   4.70 &   6.25 &   2.65 &   3.33 &  18.50 &   3.83 &   5.93 &   3.46 &   3.23 &   3.34 &    5.1\\
 123 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &  18.78 &   5.00 &   2.18 &   3.37 &   5.85 &   5.72 &   5.79 &    7.0\\
 124 &   9.00 &   2.96 &   4.10 &   9.50 &   2.62 &   4.76 &  18.75 &   4.08 &   5.68 &   5.76 &   5.60 &   5.62 &    1.6\\
 125 &  35.75 &   5.73 &   7.30 &   6.75 &   2.35 &   4.01 &  41.75 &   6.21 &   7.78 &   6.17 &   6.16 &   6.08 &    6.7\\
 126 &  16.00 &   3.97 &   5.08 &  32.50 &   5.22 &   7.30 &  46.50 &   6.34 &   8.40 &   6.45 &   6.45 &   6.47 &    4.4\\
 127 &  13.75 &   3.46 &   5.08 &   0.00 &   0.00 &  22.41 &  14.50 &   3.34 &   5.45 &   6.03 &   5.93 &   5.99 &    8.5\\
 128 &  54.00 &   7.33 &   8.39 &  33.75 &   5.56 &   7.13 &  87.00 &   9.31 &  10.36 &   6.37 &   6.13 &   6.32 &    2.8\\
 129 &   6.00 &   2.40 &   3.58 &   2.50 &   1.16 &   3.41 &   5.75 &   2.15 &   3.83 &   5.66 &   5.83 &   5.75 &    4.0\\
 130 &  25.75 &   4.82 &   6.41 &  21.75 &   4.41 &   6.01 &  45.75 &   6.51 &   8.08 &   6.72 &   6.65 &   6.71 &    5.5\\
 131 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   8.91 &   2.25 &   1.57 &   2.38 &   6.46 &   6.25 &   6.42 &    2.1\\
 132 &   5.00 &   2.18 &   3.37 &   0.75 &   0.62 &   2.54 &   5.75 &   2.15 &   3.83 &   3.91 &   3.73 &   3.88 &    3.7\\
 133 &   1.00 &   0.87 &   2.29 &   5.00 &   2.18 &   3.37 &   9.00 &   2.96 &   4.10 &   5.84 &   6.01 &   6.13 &    3.7\\
 134 &  10.25 &   3.37 &   4.01 &   6.25 &   2.65 &   3.33 &  17.50 &   3.71 &   5.82 &   5.04 &   4.85 &   4.97 &    3.0\\
 135 &   7.50 &   2.28 &   4.44 &  22.25 &   4.91 &   5.51 &  31.75 &   5.38 &   6.96 &   6.19 &   5.97 &   6.11 &    5.5\\
 136 & 342.75 &  18.26 &  19.79 & 134.75 &  11.36 &  12.90 & 469.50 &  21.17 &  23.19 &   5.71 &   5.58 &   5.71 &    6.6\\
 137 &   6.25 &   2.65 &   3.33 &   3.25 &   1.91 &   2.66 &   7.25 &   2.85 &   3.51 &   6.44 &   6.42 &   6.47 &    4.9\\
 138 &  30.75 &   5.30 &   6.87 &  10.25 &   3.37 &   4.01 &  40.00 &   6.30 &   7.37 &   6.20 &   5.84 &   6.04 &    9.0\\
 139 &  10.00 &   3.12 &   4.26 &  17.00 &   4.09 &   5.20 &  24.50 &   4.47 &   6.56 &   6.08 &   5.82 &   5.99 &    3.0\\
 140 &   7.50 &   2.28 &   4.44 &   3.25 &   1.91 &   2.66 &  11.00 &   3.28 &   4.41 &   5.89 &   5.75 &   5.82 &    6.5\\
 141 &  12.00 &   3.43 &   4.55 &   4.75 &   1.93 &   3.62 &  15.25 &   4.09 &   4.70 &   6.61 &   6.71 &   6.68 &    2.5\\
 142 & 180.50 &  12.94 &  14.98 &  57.50 &   7.10 &   9.16 & 235.00 &  15.32 &  16.35 &   6.56 &   6.40 &   6.52 &    6.9\\
 143 &  21.75 &   4.41 &   6.01 &   1.25 &   1.12 &   2.04 &  27.25 &   5.42 &   6.01 &   6.06 &   5.87 &   5.97 &    3.2\\
 144 &   6.50 &   2.10 &   4.26 &  22.50 &   4.27 &   6.36 &  26.50 &   4.67 &   6.76 &   6.11 &   5.91 &   6.03 &    5.6\\
 145 &  94.25 &   9.93 &  10.48 &  46.50 &   6.34 &   8.40 & 140.00 &  11.82 &  12.86 &   5.87 &   5.71 &   5.82 &    6.0\\
 146 &   7.50 &   2.28 &   4.44 &   0.00 &   0.00 &  12.24 &  11.25 &   3.53 &   4.16 &   5.87 &   5.95 &   5.99 &    4.6\\
 147 &  11.75 &   3.18 &   4.80 &   7.75 &   2.53 &   4.19 &  16.00 &   3.97 &   5.08 &   6.68 &   6.67 &   6.70 &    5.1\\
 148 &  54.25 &   7.58 &   8.14 &  19.00 &   4.33 &   5.43 &  73.25 &   8.78 &   9.33 &   6.60 &   6.38 &   6.56 &    0.1\\
 149 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   7.33 &   6.25 &   2.65 &   3.33 &   4.97 &   4.80 &   4.93 &    0.5\\
 150 &   0.00 &   0.00 &   1.83 &  12.57 &   3.14 &   5.12 &  11.25 &   3.53 &   4.16 &   6.13 &   5.96 &   6.06 &    5.3\\
 151 &  22.00 &   4.66 &   5.76 &  32.50 &   5.22 &   7.30 &  49.75 &   6.80 &   8.37 &   5.87 &   5.74 &   5.87 &    5.6\\
 152 &  49.50 &   6.55 &   8.62 &  14.25 &   3.96 &   4.58 &  63.75 &   7.73 &   9.29 &   6.07 &   5.93 &   6.02 &    3.4\\
 153 &  41.75 &   6.21 &   7.78 &  21.75 &   4.41 &   6.01 &  60.75 &   7.54 &   9.10 &   6.12 &   5.98 &   6.04 &    4.0\\
 154 &   0.00 &   0.00 &   2.34 &  11.50 &   3.78 &   3.91 &  11.25 &   3.53 &   4.16 &   6.52 &   6.52 &   6.55 &    3.7\\
 155 &   4.00 &   1.94 &   3.15 &   2.75 &   1.41 &   3.16 &   5.00 &   2.18 &   3.37 &   6.53 &   6.39 &   6.48 &    2.8\\
 156 &  66.75 &   7.92 &   9.47 &  27.25 &   5.42 &   6.01 &  93.25 &   9.88 &  10.43 &   6.38 &   6.45 &   6.45 &    1.8\\
 157 &   5.50 &   1.90 &   4.08 &   4.00 &   1.94 &   3.15 &   6.25 &   2.65 &   3.33 &   6.52 &   6.52 &   6.55 &    3.7\\
 158 &  11.50 &   2.93 &   5.05 &  13.50 &   4.07 &   4.19 &  22.50 &   4.27 &   6.36 &   6.55 &   6.39 &   6.51 &    6.8\\
 159 &  17.50 &   3.71 &   5.82 &  12.25 &   3.68 &   4.30 &  26.75 &   4.92 &   6.51 &   6.31 &   6.34 &   6.32 &    3.0\\
 160 &   3.25 &   1.91 &   2.66 &   9.43 &   3.39 &   3.68 &  10.50 &   2.78 &   4.91 &   4.22 &   4.23 &   4.21 &    1.3\\
 161 &  10.00 &   3.12 &   4.26 &  12.00 &   3.43 &   4.55 &  20.75 &   4.31 &   5.90 &   6.68 &   6.58 &   6.69 &    0.8\\
 162 &  16.25 &   4.22 &   4.83 &   0.75 &   0.62 &   2.54 &  19.50 &   3.94 &   6.04 &   5.36 &   5.16 &   5.13 &    6.6\\
 163 &  70.75 &   8.16 &   9.71 &  37.75 &   5.89 &   7.47 & 105.75 &  10.03 &  11.58 &   5.64 &   5.39 &   5.52 &   10.6\\
 164 &  14.75 &   3.59 &   5.20 &   8.25 &   3.03 &   3.69 &  25.25 &   5.22 &   5.81 &   5.58 &   5.32 &   5.42 &    8.5\\
 165 &  54.50 &   6.90 &   8.96 &  10.50 &   3.62 &   3.76 &  63.25 &   8.17 &   8.73 &   6.58 &   6.30 &   6.47 &    6.7\\
 166 &   2.00 &   1.32 &   2.63 &   0.25 &   0.25 &   1.58 &   4.25 &   2.19 &   2.90 &   6.52 &   6.52 &   6.55 &    3.6\\
 167 &   6.00 &   2.40 &   3.58 &   1.25 &   1.12 &   2.04 &  10.75 &   3.03 &   4.66 &   3.00 &   2.86 &   2.90 &    1.0\\
 168 &   4.00 &   1.94 &   3.15 &   4.75 &   1.93 &   3.62 &   8.75 &   2.71 &   4.35 &   2.31 &   2.56 &   2.53 &    1.0\\
 169 &  33.25 &   5.97 &   6.55 &  24.75 &   4.72 &   6.31 &  58.25 &   7.85 &   8.41 &   6.56 &   6.50 &   6.56 &    6.3\\
 170 &  17.50 &   3.71 &   5.82 &  33.00 &   5.72 &   6.80 &  51.75 &   6.94 &   8.50 &   6.17 &   6.03 &   6.12 &    4.2\\
 171 &   8.75 &   2.71 &   4.35 &   3.00 &   1.66 &   2.91 &  12.75 &   3.32 &   4.94 &   5.69 &   5.68 &   5.84 &    3.6\\
 172 & 319.50 &  17.38 &  19.41 & 128.75 &  11.10 &  12.64 & 442.50 &  20.54 &  22.56 &   6.25 &   6.11 &   6.19 &    5.1\\
 173 &   2.00 &   1.32 &   2.63 &   7.50 &   2.28 &   4.44 &   6.50 &   2.90 &   3.08 &   6.51 &   6.63 &   6.63 &    1.8\\
 174 &   0.25 &   0.25 &   1.58 &  13.50 &   3.21 &   5.33 &   9.75 &   2.87 &   4.51 &   6.52 &   6.64 &   6.60 &    2.0\\
 175 &  27.75 &   5.02 &   6.60 &   8.50 &   2.46 &   4.60 &  40.00 &   6.30 &   7.37 &   6.02 &   5.92 &   5.97 &    4.4\\
 176 &   6.75 &   2.35 &   4.01 &   0.00 &   0.00 &   6.80 &   8.25 &   3.03 &   3.69 &   6.22 &   6.24 &   6.26 &    1.3\\
 177 &  19.50 &   3.94 &   6.04 &  16.50 &   3.59 &   5.70 &  39.00 &   6.22 &   7.30 &   6.26 &   6.09 &   6.20 &    3.7\\
 178 &  48.75 &   6.73 &   8.29 &   9.00 &   2.96 &   4.10 &  60.50 &   7.29 &   9.35 &   6.46 &   6.30 &   6.42 &    7.4\\
 179 &  43.25 &   6.79 &   7.36 &  19.75 &   4.19 &   5.79 &  64.00 &   7.98 &   9.04 &   5.90 &   5.74 &   5.82 &    8.2\\
 180 &   7.75 &   2.53 &   4.19 &   1.50 &   0.82 &   3.13 &  10.50 &   2.78 &   4.91 &   4.27 &   4.24 &   4.26 &    4.0\\
 181 &   6.75 &   2.35 &   4.01 &   3.75 &   1.69 &   3.40 &   7.25 &   2.85 &   3.51 &   6.71 &   6.61 &   6.71 &    1.7\\
 182 &  27.50 &   4.77 &   6.85 &  40.25 &   6.55 &   7.12 &  62.25 &   8.11 &   8.66 &   6.30 &   6.13 &   6.29 &    4.0\\
 183 &   6.75 &   2.35 &   4.01 &   8.50 &   2.46 &   4.60 &  11.75 &   3.18 &   4.80 &   6.47 &   6.38 &   6.44 &    3.0\\
 184 &   6.25 &   2.65 &   3.33 &   2.75 &   1.41 &   3.16 &  14.25 &   3.96 &   4.58 &   6.43 &   6.34 &   6.41 &    7.4\\
 185 &   1.00 &   0.87 &   2.29 &  11.50 &   2.93 &   5.05 &  13.25 &   3.82 &   4.44 &   6.53 &   6.63 &   6.61 &    2.6\\
 186 &  11.00 &   3.28 &   4.41 &   0.00 &   0.00 &  15.51 &   9.00 &   2.96 &   4.10 &   6.22 &   6.11 &   6.17 &    7.4\\
 187 &  15.75 &   3.72 &   5.33 &   4.75 &   1.93 &   3.62 &  23.25 &   5.02 &   5.61 &   5.90 &   5.56 &   5.68 &    7.4\\
 188 & 553.00 &  23.51 &  24.53 & 298.50 &  16.78 &  18.81 & 831.00 &  28.82 &  29.84 &   5.91 &   5.71 &   5.81 &    7.6\\
 189 &  13.25 &   3.82 &   4.44 &   5.50 &   1.90 &   4.08 &  22.25 &   4.91 &   5.51 &   5.81 &   5.64 &   5.72 &    7.8\\
 190 &  11.75 &   3.18 &   4.80 &   0.00 &   0.00 &   7.49 &  15.25 &   4.09 &   4.70 &   6.46 &   6.49 &   6.51 &    3.4\\
 191 &   9.75 &   2.87 &   4.51 &   0.00 &   0.00 &   6.86 &  10.75 &   3.03 &   4.66 &   5.32 &   5.15 &   5.23 &    4.1\\
 192 &  13.75 &   3.46 &   5.08 &   5.75 &   2.15 &   3.83 &  20.00 &   4.44 &   5.54 &   5.98 &   5.77 &   5.89 &    5.4\\
 193 &   6.00 &   2.40 &   3.58 &   8.25 &   3.03 &   3.69 &  13.75 &   3.46 &   5.08 &   6.07 &   5.89 &   6.00 &    4.7\\
 194 &   3.50 &   1.44 &   3.65 &   5.00 &   2.18 &   3.37 &   9.50 &   2.62 &   4.76 &   6.07 &   5.89 &   6.00 &    4.7\\
 195 &  21.50 &   4.16 &   6.26 &  23.00 &   4.77 &   5.86 &  43.00 &   6.54 &   7.61 &   5.67 &   5.44 &   5.59 &    5.7\\
 196 &   6.71 &   2.31 &   4.05 &   3.75 &   1.69 &   3.40 &  10.86 &   3.14 &   4.55 &   5.95 &   5.74 &   5.87 &    5.5\\
 197 &   2.50 &   1.16 &   3.41 &   7.75 &   2.53 &   4.19 &   9.50 &   2.62 &   4.76 &   6.18 &   6.00 &   6.11 &    3.7\\
 198 &  14.00 &   3.71 &   4.83 &  12.00 &   3.43 &   4.55 &  25.00 &   4.97 &   6.06 &   5.62 &   5.38 &   5.41 &    6.0\\
 199 &   3.75 &   1.69 &   3.40 &   2.50 &   1.82 &   2.13 &   6.50 &   2.10 &   4.26 &   2.57 &   2.35 &   2.38 &    3.0\\
 200 &  88.50 &   8.92 &  10.97 &  24.25 &   5.12 &   5.71 & 113.25 &  10.87 &  11.41 &   6.41 &   6.32 &   6.38 &    4.0\\
 201 &  16.50 &   3.59 &   5.70 &   7.00 &   2.60 &   3.76 &  24.00 &   4.87 &   5.96 &   5.75 &   5.55 &   5.65 &    6.8\\
 202 &  28.29 &   5.55 &   6.07 &  28.50 &   5.77 &   5.85 &  54.29 &   7.62 &   8.11 &   5.98 &   5.80 &   5.89 &    6.7\\
 203 &  41.75 &   6.21 &   7.78 &  22.75 &   4.52 &   6.11 &  63.50 &   7.48 &   9.54 &   6.44 &   6.56 &   6.52 &    3.2\\
 204 &  68.00 &   8.23 &   9.28 &  27.75 &   5.02 &   6.60 &  97.75 &   9.64 &  11.18 &   6.24 &   6.21 &   6.23 &    5.6\\
 205 &  40.86 &   6.24 &   7.60 &  26.50 &   4.67 &   6.76 &  66.29 &   8.39 &   8.88 &   6.00 &   5.83 &   5.91 &    6.5\\
 206 &  69.00 &   8.29 &   9.34 &  22.50 &   4.27 &   6.36 &  86.75 &   9.06 &  10.61 &   6.39 &   6.21 &   6.33 &    2.1\\
 207 &   4.25 &   2.19 &   2.90 &   2.75 &   1.41 &   3.16 &  11.75 &   3.18 &   4.80 &   5.01 &   4.91 &   4.90 &    7.7\\
 208 &   7.29 &   2.88 &   3.48 &  13.29 &   3.86 &   4.41 &  19.29 &   4.62 &   5.15 &   6.24 &   6.20 &   6.25 &    5.8\\
 209 &   7.50 &   2.28 &   4.44 &   8.43 &   3.21 &   3.51 &  15.75 &   3.72 &   5.33 &   6.24 &   6.19 &   6.24 &    5.8\\
 210 &  11.50 &   2.93 &   5.05 &   0.00 &   0.00 &  11.76 &  14.00 &   3.71 &   4.83 &   5.54 &   5.45 &   5.53 &    6.1\\
 211 &  65.00 &   8.05 &   9.10 &  69.00 &   8.29 &   9.34 & 131.00 &  11.43 &  12.47 &   5.62 &   5.38 &   5.57 &    9.4\\
 212 &   8.50 &   2.46 &   4.60 &   7.00 &   2.60 &   3.76 &  14.50 &   3.34 &   5.45 &   6.38 &   6.42 &   6.43 &    4.0\\
 213 &   1.25 &   1.12 &   2.04 &   0.00 &   0.00 &  10.16 &   1.25 &   1.12 &   2.04 &   5.84 &   5.71 &   5.79 &    5.4\\
 214 &  63.00 &   7.92 &   8.98 &  79.50 &   8.43 &  10.48 & 143.50 &  11.49 &  13.53 &   5.68 &   5.43 &   5.58 &    9.4\\
 215 &  10.50 &   2.78 &   4.91 &  12.00 &   3.43 &   4.55 &  21.75 &   4.41 &   6.01 &   5.95 &   5.78 &   5.86 &    7.8\\
 216 & 146.00 &  12.07 &  13.11 &  39.75 &   6.05 &   7.62 & 183.75 &  13.31 &  14.84 &   6.07 &   6.01 &   6.04 &    4.4\\
 217 &  17.25 &   4.34 &   4.95 &   7.00 &   2.60 &   3.76 &  22.25 &   4.91 &   5.51 &   5.60 &   5.47 &   5.52 &    7.2\\
 218 &   5.00 &   2.18 &   3.37 &   7.25 &   2.85 &   3.51 &  12.75 &   3.32 &   4.94 &   6.32 &   6.12 &   6.26 &    2.4\\
 219 &   7.00 &   2.60 &   3.76 &  13.50 &   3.21 &   5.33 &  16.50 &   3.59 &   5.70 &   5.93 &   5.49 &   5.71 &    8.9\\
 220 &  23.25 &   5.02 &   5.61 &  13.25 &   3.82 &   4.44 &  35.00 &   5.89 &   6.97 &   6.03 &   5.88 &   5.99 &    7.5\\
 221 &  57.50 &   7.10 &   9.16 &  17.50 &   3.71 &   5.82 &  73.00 &   8.53 &   9.58 &   6.09 &   5.84 &   5.99 &    4.4\\
 222 &  10.25 &   3.37 &   4.01 &  13.00 &   3.57 &   4.69 &  20.25 &   4.69 &   5.29 &   6.20 &   6.06 &   6.14 &    5.7\\
 223 &  72.25 &   8.72 &   9.27 &  11.25 &   3.53 &   4.16 &  83.25 &   9.35 &   9.89 &   5.98 &   5.82 &   5.93 &    7.1\\
 224 &  20.75 &   4.31 &   5.90 &   8.00 &   2.78 &   3.94 &  28.75 &   5.11 &   6.69 &   3.73 &   3.54 &   3.65 &    5.3\\
 225 &   1.75 &   1.07 &   2.88 &   7.00 &   2.60 &   3.76 &   7.25 &   2.85 &   3.51 &   6.45 &   6.23 &   6.39 &    1.2\\
 226 &  19.25 &   4.58 &   5.18 &  33.75 &   5.56 &   7.13 &  52.25 &   7.44 &   8.00 &   6.29 &   6.34 &   6.34 &    5.0\\
 227 &   4.50 &   1.68 &   3.87 &   2.75 &   1.41 &   3.16 &   9.50 &   2.62 &   4.76 &   6.02 &   5.92 &   5.98 &    5.1\\
 228 &   6.75 &   2.35 &   4.01 &   0.00 &   0.00 &  11.06 &   4.75 &   1.93 &   3.62 &   6.12 &   5.98 &   6.05 &    5.4\\
 229 &  41.75 &   6.21 &   7.78 &  21.75 &   4.41 &   6.01 &  66.00 &   8.11 &   9.16 &   6.14 &   5.92 &   6.04 &    5.8\\
 230 &   3.75 &   1.69 &   3.40 &  12.00 &   3.43 &   4.55 &  15.75 &   3.72 &   5.33 &   6.04 &   6.10 &   6.10 &    1.8\\
 231 &   4.00 &   1.94 &   3.15 &  13.25 &   3.82 &   4.44 &  19.00 &   4.33 &   5.43 &   6.23 &   6.15 &   6.15 &    5.4\\
 232 &  31.25 &   5.80 &   6.37 &  15.50 &   4.34 &   4.45 &  47.50 &   6.41 &   8.47 &   6.21 &   5.94 &   6.12 &    3.2\\
 233 & 172.75 &  12.89 &  14.43 &  58.75 &   7.41 &   8.97 & 229.00 &  15.12 &  16.15 &   6.17 &   5.96 &   6.08 &    5.5\\
 234 &  18.50 &   3.83 &   5.93 &   6.00 &   2.40 &   3.58 &  24.00 &   4.87 &   5.96 &   4.95 &   4.65 &   4.82 &    4.5\\
 235 &  12.75 &   3.32 &   4.94 &   6.25 &   2.65 &   3.33 &  19.75 &   4.19 &   5.79 &   5.97 &   5.77 &   5.90 &    7.9\\
 236 &   2.50 &   1.16 &   3.41 &   9.75 &   2.87 &   4.51 &  11.50 &   2.93 &   5.05 &   5.71 &   5.35 &   5.54 &    5.2\\
 237 &   7.50 &   2.28 &   4.44 &   0.75 &   0.62 &   2.54 &   8.00 &   2.78 &   3.94 &   6.18 &   5.97 &   6.08 &    5.5\\
 238 &   3.00 &   1.66 &   2.91 &   7.00 &   2.60 &   3.76 &   9.75 &   2.87 &   4.51 &   6.27 &   6.36 &   6.33 &    4.6\\
 239 &  17.71 &   3.93 &   5.60 &   0.75 &   0.62 &   2.54 &  22.43 &   5.09 &   5.33 &   4.78 &   4.78 &   4.69 &    8.3\\
 240 &  28.00 &   5.27 &   6.35 &  11.25 &   3.53 &   4.16 &  39.43 &   6.65 &   6.87 &   5.88 &   5.67 &   5.79 &    8.0\\
 241 &   6.25 &   2.65 &   3.33 &   0.50 &   0.37 &   2.79 &   2.00 &   1.32 &   2.63 &   6.08 &   5.94 &   5.94 &    5.4\\
 242 &  67.50 &   7.73 &   9.78 &  30.50 &   5.95 &   6.03 &  99.50 &   9.49 &  11.53 &   5.68 &   5.51 &   5.61 &    6.4\\
 243 &   0.00 &   0.00 &   2.34 &   6.25 &   2.65 &   3.33 &   8.75 &   2.71 &   4.35 &   5.85 &   5.68 &   5.77 &    5.1\\
 244 &  25.00 &   4.97 &   6.06 &  20.75 &   4.31 &   5.90 &  39.00 &   6.22 &   7.30 &   6.50 &   6.52 &   6.52 &    2.3\\
 245 &  17.71 &   3.93 &   5.60 &   0.00 &   0.00 &  29.78 &  23.14 &   4.91 &   5.72 &   5.69 &   5.45 &   5.54 &    8.4\\
 246 & 116.00 &  10.76 &  11.80 &  52.00 &   7.19 &   8.25 & 164.75 &  12.59 &  14.12 &   6.21 &   6.27 &   6.26 &    5.4\\
 247 &   0.50 &   0.37 &   2.79 &  30.00 &   5.45 &   6.53 &  26.25 &   5.32 &   5.91 &   5.83 &   5.60 &   5.72 &    7.1\\
 248 &  12.75 &   3.32 &   4.94 &   1.75 &   1.07 &   2.88 &  16.25 &   4.22 &   4.83 &   6.39 &   6.11 &   6.28 &    2.7\\
 249 &  15.00 &   3.84 &   4.95 &   0.00 &   0.00 &  21.44 &  16.50 &   4.47 &   4.58 &   5.27 &   5.11 &   5.27 &    8.4\\
 250 &   1.50 &   1.37 &   1.79 &   0.00 &   0.00 &  17.88 &   2.75 &   1.41 &   3.16 &   5.90 &   5.79 &   5.84 &    6.4\\
 251 &  90.00 &   9.47 &  10.52 &  21.50 &   4.16 &   6.26 & 119.50 &  10.44 &  12.48 &   4.81 &   4.77 &   4.88 &    9.6\\
 252 &  10.00 &   3.12 &   4.26 &   0.00 &   0.00 &  11.16 &  11.25 &   3.53 &   4.16 &   5.71 &   5.50 &   5.61 &    5.5\\
 253 &  28.50 &   4.86 &   6.94 &  13.50 &   3.21 &   5.33 &  39.25 &   6.47 &   7.05 &   5.69 &   5.62 &   5.67 &    6.5\\
 254 &   0.50 &   0.50 &   1.33 &  14.50 &   3.34 &   5.45 &  13.25 &   3.82 &   4.44 &   6.11 &   5.99 &   5.97 &    3.1\\
 255 &  59.50 &   7.23 &   9.29 &  74.75 &   8.40 &   9.95 & 131.50 &  10.98 &  13.02 &   5.75 &   5.51 &   5.65 &    5.9\\
 256 &  44.67 &   6.36 &   8.09 &  25.00 &   4.97 &   6.06 &  66.00 &   8.11 &   9.16 &   6.12 &   6.17 &   6.16 &    6.0\\
 257 &  24.25 &   5.12 &   5.71 &  24.00 &   4.87 &   5.96 &  43.25 &   6.79 &   7.36 &   5.95 &   5.75 &   5.87 &    3.4\\
 258 &  12.50 &   3.07 &   5.19 &   2.50 &   1.16 &   3.41 &  14.50 &   3.34 &   5.45 &   6.33 &   6.15 &   6.25 &    4.1\\
 259 &  10.50 &   2.78 &   4.91 &   7.75 &   2.53 &   4.19 &  17.50 &   3.71 &   5.82 &   6.34 &   6.15 &   6.26 &    3.7\\
 260 &  11.00 &   3.28 &   4.41 &  12.00 &   3.43 &   4.55 &  23.25 &   5.02 &   5.61 &   5.82 &   5.60 &   5.71 &    9.0\\
 261 &  14.50 &   3.34 &   5.45 &   7.00 &   2.60 &   3.76 &  23.75 &   4.62 &   6.21 &   6.52 &   6.40 &   6.47 &    1.8\\
 262 &  44.75 &   6.44 &   8.01 &  45.00 &   6.69 &   7.76 &  84.75 &   8.96 &  10.50 &   5.67 &   5.59 &   5.55 &    9.3\\
 263 &  65.67 &   7.78 &   9.50 &  52.00 &   7.19 &   8.25 & 119.00 &  10.90 &  11.94 &   6.10 &   6.14 &   6.14 &    6.1\\
 264 &  30.75 &   5.30 &   6.87 &  25.00 &   4.97 &   6.06 &  52.25 &   7.44 &   8.00 &   5.63 &   5.46 &   5.54 &    8.1\\
 265 &  38.00 &   6.14 &   7.22 &  82.50 &   8.60 &  10.64 & 120.50 &  10.49 &  12.53 &   5.66 &   5.37 &   5.51 &   10.5\\
 266 & 200.75 &  13.92 &  15.45 &  67.75 &   7.98 &   9.53 & 270.75 &  16.20 &  17.73 &   5.81 &   5.54 &   5.69 &    7.2\\
 267 &  36.25 &   6.23 &   6.80 &  10.57 &   2.85 &   4.84 &  49.75 &   6.80 &   8.37 &   5.76 &   5.53 &   5.63 &    9.3\\
 268 &  19.50 &   3.94 &   6.04 &  15.25 &   4.09 &   4.70 &  31.00 &   5.55 &   6.62 &   6.05 &   6.09 &   6.09 &    6.3\\
 269 &  18.75 &   4.08 &   5.68 &  39.50 &   5.80 &   7.87 &  56.25 &   7.72 &   8.28 &   6.25 &   6.06 &   6.17 &    4.1\\
 270 & 190.75 &  13.56 &  15.09 &  65.25 &   8.30 &   8.85 & 256.25 &  16.24 &  16.77 &   5.68 &   5.69 &   5.69 &    6.5\\
 271 &   1.50 &   0.82 &   3.13 &   0.00 &   0.00 &   7.91 &   2.00 &   1.32 &   2.63 &   5.60 &   5.84 &   5.79 &    4.1\\
 272 &   9.75 &   2.87 &   4.51 &   3.75 &   1.69 &   3.40 &  15.25 &   4.09 &   4.70 &   6.42 &   6.45 &   6.45 &    1.8\\
 273 &  29.75 &   5.20 &   6.78 &  34.25 &   6.06 &   6.63 &  62.50 &   7.42 &   9.48 &   5.90 &   5.69 &   5.81 &    8.4\\
 274 &   3.25 &   1.91 &   2.66 &   6.50 &   2.10 &   4.26 &   8.00 &   2.78 &   3.94 &   6.22 &   6.16 &   6.20 &    3.9\\
 275 &   4.00 &   1.94 &   3.15 &   8.00 &   2.78 &   3.94 &   8.00 &   2.78 &   3.94 &   4.75 &   4.68 &   4.72 &    3.6\\
 276 &   6.50 &   2.10 &   4.26 &  12.50 &   3.07 &   5.19 &  15.00 &   3.84 &   4.95 &   6.44 &   6.21 &   6.35 &    2.9\\
 277 &  14.50 &   3.34 &   5.45 &   9.25 &   3.21 &   3.85 &  21.75 &   4.41 &   6.01 &   6.40 &   6.36 &   6.37 &    4.0\\
 278 &  58.25 &   7.85 &   8.41 &  24.00 &   4.87 &   5.96 &  78.50 &   8.37 &  10.42 &   6.05 &   5.86 &   5.95 &    5.7\\
 279 & 292.25 &  17.33 &  17.86 & 151.75 &  12.07 &  13.60 & 441.75 &  20.77 &  22.29 &   5.97 &   5.88 &   5.96 &    3.3\\
 280 &   6.75 &   2.35 &   4.01 &   7.50 &   2.28 &   4.44 &   8.75 &   2.71 &   4.35 &   6.28 &   6.18 &   6.15 &    4.4\\
 281 &   4.75 &   1.93 &   3.62 &   0.00 &   0.00 &   5.27 &   4.50 &   1.68 &   3.87 &   5.26 &   4.91 &   4.93 &    5.3\\
 282 &   9.75 &   2.87 &   4.51 &  21.25 &   4.81 &   5.40 &  27.75 &   5.02 &   6.60 &   5.61 &   5.49 &   5.58 &    8.8\\
 283 &  26.25 &   5.32 &   5.91 &  10.50 &   3.62 &   3.76 &  38.75 &   5.97 &   7.55 &   6.01 &   6.00 &   5.97 &    3.0\\
 284 &   6.25 &   2.65 &   3.33 &  56.25 &   7.72 &   8.28 &  57.50 &   7.10 &   9.16 &   6.09 &   5.86 &   5.98 &    7.2\\
 285 &   9.75 &   2.87 &   4.51 &   4.50 &   1.68 &   3.87 &  16.75 &   3.84 &   5.45 &   5.98 &   5.77 &   5.88 &    8.0\\
 286 &   6.50 &   2.10 &   4.26 &   4.25 &   2.19 &   2.90 &  11.25 &   3.53 &   4.16 &   2.92 &   2.72 &   2.81 &    6.5\\
 287 &   3.75 &   1.69 &   3.40 &  13.50 &   3.21 &   5.33 &  17.25 &   4.34 &   4.95 &   5.78 &   5.60 &   5.70 &    5.2\\
 288 &   9.75 &   2.87 &   4.51 &  22.75 &   4.52 &   6.11 &  27.00 &   5.17 &   6.26 &   6.20 &   6.23 &   6.22 &    3.3\\
 289 & 102.75 &   9.89 &  11.43 &  37.00 &   6.06 &   7.13 & 139.00 &  11.78 &  12.82 &   6.09 &   5.94 &   6.04 &    6.1\\
 290 &  10.00 &   3.12 &   4.26 &  11.75 &   3.18 &   4.80 &  20.00 &   4.44 &   5.54 &   5.99 &   6.02 &   6.03 &    3.4\\
 291 &  13.75 &   3.46 &   5.08 &  11.75 &   3.18 &   4.80 &  25.50 &   4.57 &   6.66 &   5.89 &   5.63 &   5.76 &    7.0\\
 292 &   1.75 &   1.07 &   2.88 &   6.50 &   2.10 &   4.26 &   5.75 &   2.15 &   3.83 &   6.36 &   6.14 &   6.27 &    2.6\\
 293 &   8.50 &   3.28 &   3.44 &   1.00 &   0.87 &   2.29 &  16.25 &   4.22 &   4.83 &   5.85 &   5.82 &   5.88 &    8.0\\
 294 &   3.25 &   1.91 &   2.66 &   0.00 &   0.00 &  28.55 &   5.00 &   2.18 &   3.37 &   5.97 &   5.80 &   5.88 &    7.5\\
 295 &  15.75 &   3.72 &   5.33 &  12.25 &   3.68 &   4.30 &  29.25 &   5.61 &   6.19 &   5.88 &   5.40 &   5.69 &    7.2\\
 296 &  17.50 &   3.71 &   5.82 &  10.50 &   3.62 &   3.76 &  25.00 &   4.97 &   6.06 &   5.91 &   5.54 &   5.71 &    7.3\\
 297 &   8.50 &   2.46 &   4.60 &   9.50 &   2.62 &   4.76 &  19.25 &   4.58 &   5.18 &   5.82 &   5.62 &   5.68 &    6.8\\
 298 & 484.00 &  21.99 &  23.01 & 176.25 &  13.51 &  14.04 & 662.00 &  25.72 &  26.74 &   6.18 &   5.93 &   6.00 &    1.7\\
 299 &  60.50 &   7.29 &   9.35 &  35.75 &   5.73 &   7.30 &  92.75 &   9.38 &  10.93 &   6.37 &   6.29 &   6.32 &    4.7\\
 300 & 162.50 &  12.26 &  14.29 &  50.00 &   7.05 &   8.12 & 213.00 &  14.59 &  15.62 &   6.16 &   6.00 &   6.08 &    6.2\\
 301 &  26.00 &   5.07 &   6.16 &  16.75 &   3.84 &   5.45 &  39.50 &   5.80 &   7.87 &   6.10 &   5.96 &   6.02 &    6.5\\
 302 &  13.75 &   3.46 &   5.08 &  25.00 &   4.97 &   6.06 &  39.00 &   6.22 &   7.30 &   6.25 &   6.29 &   6.28 &    3.7\\
 303 &   8.50 &   2.46 &   4.60 &   5.25 &   2.43 &   3.12 &  12.00 &   3.43 &   4.55 &   6.49 &   6.47 &   6.48 &    3.3\\
 304 &  27.00 &   5.17 &   6.26 &  24.75 &   4.72 &   6.31 &  51.75 &   6.94 &   8.50 &   5.35 &   5.11 &   5.22 &    8.3\\
 305 &   4.50 &   1.68 &   3.87 &   4.43 &   2.37 &   2.73 &   5.25 &   2.43 &   3.12 &   4.39 &   4.17 &   4.30 &    4.0\\
 306 &   9.75 &   2.87 &   4.51 &  10.25 &   3.37 &   4.01 &  15.25 &   4.09 &   4.70 &   5.18 &   4.89 &   5.04 &    7.9\\
 307 & 103.25 &  10.39 &  10.93 &  48.00 &   6.91 &   7.97 & 151.25 &  12.53 &  13.06 &   5.95 &   5.62 &   5.80 &    3.7\\
 308 &  51.25 &   7.37 &   7.94 &  40.25 &   6.55 &   7.12 &  87.50 &   8.87 &  10.91 &   5.85 &   5.63 &   5.73 &    7.2\\
 309 &  26.50 &   4.67 &   6.76 &   6.25 &   2.65 &   3.33 &  32.25 &   5.88 &   6.46 &   5.77 &   5.74 &   5.68 &    3.7\\
 310 &   4.50 &   1.68 &   3.87 &   1.75 &   1.07 &   2.88 &   9.50 &   2.62 &   4.76 &   6.16 &   6.14 &   6.16 &    5.0\\
 311 &   8.00 &   2.78 &   3.94 &   3.50 &   2.16 &   2.41 &  10.75 &   3.03 &   4.66 &   6.20 &   5.94 &   6.12 &    5.8\\
 312 &  20.25 &   4.69 &   5.29 &  13.00 &   3.57 &   4.69 &  35.75 &   5.73 &   7.30 &   6.21 &   6.19 &   6.20 &    3.1\\
 313 &  77.71 &   8.53 &  10.15 &  45.14 &   6.83 &   7.61 & 117.00 &  10.81 &  11.85 &   5.99 &   5.82 &   5.90 &    8.0\\
 314 & 147.14 &  12.26 &  13.01 &  48.25 &   7.16 &   7.72 & 191.43 &  14.24 &  14.41 &   6.02 &   5.85 &   5.93 &    8.1\\
 315 &   8.50 &   2.46 &   4.60 &  14.75 &   3.59 &   5.20 &  14.75 &   3.59 &   5.20 &   6.11 &   5.93 &   6.01 &    5.0\\
 316 &   7.75 &   2.53 &   4.19 &   5.00 &   2.18 &   3.37 &   9.25 &   3.21 &   3.85 &   6.32 &   6.18 &   6.28 &    4.8\\
 317 &   6.00 &   2.40 &   3.58 &  10.75 &   3.03 &   4.66 &  14.50 &   3.34 &   5.45 &   5.61 &   5.58 &   5.84 &    4.7\\
 318 &  31.75 &   5.38 &   6.96 &   8.75 &   2.71 &   4.35 &  42.50 &   6.04 &   8.11 &   6.28 &   6.13 &   6.21 &    4.5\\
 319 &  20.00 &   4.44 &   5.54 &   8.75 &   2.71 &   4.35 &  26.75 &   4.92 &   6.51 &   6.57 &   6.57 &   6.57 &    2.3\\
 320 &   4.75 &   1.93 &   3.62 &   7.00 &   2.60 &   3.76 &  10.00 &   3.12 &   4.26 &   6.43 &   6.35 &   6.39 &    4.1\\
 321 &   4.75 &   1.93 &   3.62 &   2.50 &   1.82 &   2.13 &   5.50 &   2.68 &   2.87 &   5.87 &   5.74 &   5.80 &    6.7\\
 322 &   8.75 &   2.71 &   4.35 &   6.75 &   2.35 &   4.01 &  16.00 &   3.97 &   5.08 &   5.86 &   5.73 &   5.79 &    6.8\\
 323 &   1.75 &   1.07 &   2.88 &   2.00 &   1.32 &   2.63 &   6.00 &   2.40 &   3.58 &   6.49 &   6.27 &   6.39 &    2.5\\
 324 &   3.50 &   2.16 &   2.41 &   4.25 &   2.19 &   2.90 &   5.50 &   2.68 &   2.87 &   6.39 &   6.21 &   6.30 &    4.9\\
 325 &  17.50 &   3.71 &   5.82 &   4.25 &   2.19 &   2.90 &  23.00 &   4.77 &   5.86 &   5.84 &   5.64 &   5.72 &    7.1\\
 326 & 112.00 &  10.57 &  11.61 &   0.75 &   0.62 &   2.54 & 108.25 &  10.63 &  11.17 &   6.01 &   5.83 &   5.91 &    7.6\\
 327 &  12.25 &   3.68 &   4.30 &   7.75 &   2.53 &   4.19 &  16.75 &   3.84 &   5.45 &   6.41 &   6.22 &   6.32 &    4.6\\
 328 &   9.25 &   3.21 &   3.85 &   7.25 &   2.85 &   3.51 &  15.25 &   4.09 &   4.70 &   4.53 &   4.40 &   4.47 &    5.2\\
 329 &  13.75 &   3.46 &   5.08 &  33.43 &   6.15 &   6.37 &  47.50 &   6.41 &   8.47 &   6.57 &   6.56 &   6.57 &    1.8\\
 330 &   4.00 &   1.94 &   3.15 &  20.00 &   4.44 &   5.54 &  20.00 &   4.44 &   5.54 &   6.00 &   5.92 &   5.98 &    4.3\\
 331 &   4.75 &   1.93 &   3.62 &  13.43 &   4.00 &   4.26 &  16.25 &   4.22 &   4.83 &   4.40 &   4.44 &   4.34 &    2.0\\
 332 &  10.25 &   3.37 &   4.01 &   5.75 &   2.15 &   3.83 &  12.50 &   3.07 &   5.19 &   5.53 &   5.31 &   5.37 &    5.2\\
 333 &  10.50 &   2.78 &   4.91 &   5.50 &   1.90 &   4.08 &  10.25 &   3.37 &   4.01 &   5.91 &   5.77 &   5.85 &    7.5\\
 334 &   0.00 &   0.00 &   1.07 &  10.00 &   3.12 &   4.26 &  10.75 &   3.03 &   4.66 &   6.44 &   6.34 &   6.39 &    3.9\\
 335 &  26.25 &   5.32 &   5.91 &   8.00 &   2.78 &   3.94 &  37.25 &   6.31 &   6.88 &   5.60 &   5.43 &   5.51 &    6.2\\
 336 &  71.25 &   8.66 &   9.21 &  25.75 &   4.82 &   6.41 &  99.25 &  10.19 &  10.73 &   5.99 &   5.77 &   5.87 &    9.2\\
 337 &   0.50 &   0.37 &   2.79 &   8.50 &   2.46 &   4.60 &  11.25 &   3.53 &   4.16 &   5.98 &   5.99 &   6.07 &    6.9\\
 338 &   5.75 &   2.15 &   3.83 &   0.00 &   0.00 &  15.99 &   9.00 &   2.96 &   4.10 &   6.00 &   5.97 &   5.99 &    6.2\\
 339 &   3.75 &   1.69 &   3.40 &   6.50 &   2.10 &   4.26 &   7.75 &   2.53 &   4.19 &   5.88 &   5.74 &   5.82 &    4.9\\
 340 &  18.00 &   4.21 &   5.32 &   7.25 &   2.85 &   3.51 &  24.25 &   5.12 &   5.71 &   5.77 &   5.52 &   5.67 &    8.9\\
 341 &  53.00 &   7.26 &   8.32 &  30.25 &   5.70 &   6.28 &  84.75 &   8.96 &  10.50 &   6.49 &   6.50 &   6.51 &    2.0\\
 342 &   8.00 &   2.78 &   3.94 &   5.00 &   2.18 &   3.37 &  12.50 &   3.07 &   5.19 &   6.43 &   6.26 &   6.34 &    3.2\\
 343 &  81.14 &   9.13 &   9.89 &  36.57 &   5.63 &   7.56 & 108.14 &  10.52 &  11.28 &   5.84 &   5.59 &   5.71 &    7.7\\
 344 &  14.50 &   3.34 &   5.45 &   3.00 &   1.66 &   2.91 &  19.00 &   4.33 &   5.43 &   6.47 &   6.46 &   6.48 &    2.6\\
 345 &   8.75 &   2.71 &   4.35 &   0.00 &   0.00 &  17.28 &   5.25 &   2.43 &   3.12 &   5.96 &   5.93 &   5.94 &    6.2\\
 346 &  44.43 &   7.04 &   7.25 &  92.71 &   9.34 &  10.96 & 130.43 &  11.82 &  12.00 &   5.83 &   5.58 &   5.71 &    7.8\\
 347 &  68.75 &   8.04 &   9.59 &  34.25 &   6.06 &   6.63 & 104.75 &   9.98 &  11.53 &   6.28 &   6.23 &   6.27 &    3.4\\
 348 &  67.50 &   7.73 &   9.78 &  30.00 &   5.45 &   6.53 &  96.75 &   9.59 &  11.13 &   6.37 &   6.32 &   6.36 &    3.7\\
 349 &   8.50 &   2.46 &   4.60 &   2.00 &   1.32 &   2.63 &  12.25 &   3.68 &   4.30 &   6.57 &   6.41 &   6.50 &    2.5\\
 350 &  48.75 &   6.73 &   8.29 &  19.75 &   4.19 &   5.79 &  68.00 &   8.23 &   9.28 &   6.55 &   6.29 &   6.47 &    2.6\\
 351 & 602.00 &  24.53 &  25.55 & 169.75 &  12.78 &  14.31 & 762.50 &  27.12 &  29.13 &   5.81 &   5.75 &   5.79 &    7.1\\
 352 &  79.71 &   8.64 &  10.27 &  22.00 &   4.66 &   5.76 & 102.71 &   9.85 &  11.47 &   5.98 &   5.81 &   5.90 &    6.1\\
 353 &   5.75 &   2.15 &   3.83 &   3.75 &   1.69 &   3.40 &  13.25 &   3.82 &   4.44 &   5.84 &   5.78 &   5.81 &    7.1\\
 354 &  12.75 &   3.32 &   4.94 &   2.25 &   1.57 &   2.38 &  19.25 &   4.58 &   5.18 &   5.85 &   5.78 &   5.82 &    7.4\\
 355 &  10.75 &   3.03 &   4.66 &   9.75 &   2.87 &   4.51 &  17.25 &   4.34 &   4.95 &   6.17 &   6.10 &   6.14 &    4.6\\
 356 &  19.57 &   4.02 &   5.97 &   4.50 &   2.44 &   2.65 &  23.71 &   4.59 &   6.25 &   4.98 &   4.80 &   4.93 &    6.1\\
 357 &   1.00 &   0.87 &   2.29 &   4.00 &   1.94 &   3.15 &   5.75 &   2.15 &   3.83 &   2.94 &   2.84 &   2.91 &    2.8\\
 358 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   5.07 &   3.75 &   1.69 &   3.40 &   6.61 &   6.39 &   6.53 &    2.3\\
 359 &  18.50 &   3.83 &   5.93 &   0.00 &   0.00 &  23.52 &  16.75 &   3.84 &   5.45 &   6.03 &   5.82 &   5.92 &    9.1\\
 360 &  38.25 &   6.39 &   6.97 &  42.50 &   6.04 &   8.11 &  79.75 &   8.68 &  10.23 &   5.93 &   5.67 &   5.81 &    6.3\\
 361 &  18.00 &   4.21 &   5.32 &   0.25 &   0.25 &   1.58 &  20.25 &   4.69 &   5.29 &   6.27 &   6.38 &   6.26 &    3.4\\
 362 &   8.00 &   2.78 &   3.94 &  17.25 &   4.34 &   4.95 &  25.25 &   5.22 &   5.81 &   6.33 &   6.15 &   6.23 &    4.2\\
 363 &  37.00 &   6.06 &   7.13 &   0.25 &   0.25 &   1.58 &  41.50 &   6.88 &   6.95 &   6.07 &   5.75 &   5.83 &    7.9\\
 364 &   0.75 &   0.62 &   2.54 &   8.00 &   2.78 &   3.94 &   6.50 &   2.10 &   4.26 &   6.02 &   5.85 &   5.96 &    3.1\\
 365 &   1.75 &   1.07 &   2.88 &   9.75 &   2.87 &   4.51 &  10.25 &   3.37 &   4.01 &   6.29 &   6.22 &   6.27 &    4.5\\
 366 &  41.75 &   6.21 &   7.78 &  19.25 &   4.58 &   5.18 &  61.75 &   7.61 &   9.16 &   2.36 &   2.42 &   2.32 &    7.6\\
 367 &   5.75 &   2.15 &   3.83 &   8.50 &   2.46 &   4.60 &  10.00 &   3.12 &   4.26 &   5.70 &   5.52 &   5.60 &    8.0\\
 368 &   7.25 &   2.85 &   3.51 &  17.00 &   4.09 &   5.20 &  19.50 &   3.94 &   6.04 &   6.30 &   6.04 &   6.18 &    7.0\\
 369 &  52.50 &   6.76 &   8.82 &  18.75 &   4.08 &   5.68 &  67.25 &   8.42 &   8.97 &   6.22 &   6.03 &   6.11 &    5.0\\
 370 &  38.75 &   5.97 &   7.55 &  22.50 &   4.27 &   6.36 &  63.25 &   8.17 &   8.73 &   5.84 &   5.72 &   5.88 &    7.6\\
 371 &  10.50 &   2.78 &   4.91 &   8.50 &   3.28 &   3.44 &  14.00 &   3.71 &   4.83 &   6.46 &   6.22 &   6.36 &    2.9\\
 372 &   8.25 &   3.03 &   3.69 &   8.50 &   2.46 &   4.60 &  15.50 &   3.47 &   5.58 &   6.14 &   5.92 &   6.02 &    5.7\\
 373 &   6.75 &   2.35 &   4.01 &   1.75 &   1.07 &   2.88 &   8.00 &   2.78 &   3.94 &   6.09 &   5.89 &   5.98 &    7.8\\
 374 &   4.00 &   1.94 &   3.15 &   5.75 &   2.15 &   3.83 &   9.75 &   2.87 &   4.51 &   6.45 &   6.17 &   6.34 &    3.0\\
 375 &   0.00 &   0.00 &   1.07 &   7.25 &   2.85 &   3.51 &   9.00 &   2.96 &   4.10 &   6.51 &   6.26 &   6.42 &    2.4\\
 376 &  76.00 &   8.70 &   9.75 & 101.00 &  10.04 &  11.08 & 176.50 &  12.79 &  14.83 &   6.39 &   6.13 &   6.27 &    6.2\\
 377 &   2.75 &   1.41 &   3.16 &   1.00 &   0.87 &   2.29 &   6.25 &   2.65 &   3.33 &   6.69 &   6.43 &   6.60 &    1.0\\
 378 &  14.25 &   3.96 &   4.58 &   5.75 &   2.15 &   3.83 &  23.25 &   5.02 &   5.61 &   6.39 &   6.22 &   6.30 &    6.0\\
 379 &  15.75 &   3.72 &   5.33 &   5.00 &   2.18 &   3.37 &  19.75 &   4.19 &   5.79 &   6.19 &   6.20 &   6.19 &    4.6\\
 380 &   4.00 &   1.94 &   3.15 &   5.75 &   2.15 &   3.83 &   6.25 &   2.65 &   3.33 &   6.08 &   6.11 &   6.14 &    1.6\\
 381 &  15.00 &   3.84 &   4.95 &   5.50 &   1.90 &   4.08 &  21.75 &   4.41 &   6.01 &   3.46 &   3.45 &   3.46 &    1.1\\
 382 &  16.75 &   3.84 &   5.45 &   8.75 &   2.71 &   4.35 &  26.25 &   5.32 &   5.91 &   5.82 &   5.51 &   5.66 &    6.2\\
 383 &   4.00 &   1.94 &   3.15 &  21.75 &   4.41 &   6.01 &  24.00 &   4.87 &   5.96 &   6.16 &   6.16 &   6.16 &    4.7\\
 384 &   6.25 &   2.65 &   3.33 &   2.75 &   1.41 &   3.16 &  13.25 &   3.82 &   4.44 &   6.02 &   5.87 &   5.95 &    5.9\\
 385 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   4.14 &   6.00 &   2.40 &   3.58 &   3.04 &   3.11 &   3.12 &    2.3\\
 386 &  26.50 &   4.67 &   6.76 &   8.00 &   2.78 &   3.94 &  36.50 &   5.56 &   7.63 &   6.12 &   5.88 &   5.99 &    9.4\\
 387 & 169.50 &  12.53 &  14.56 &  63.25 &   8.17 &   8.73 & 227.25 &  15.31 &  15.84 &   6.19 &   5.92 &   6.12 &    5.5\\
 388 &   7.25 &   2.85 &   3.51 &   1.25 &   1.12 &   2.04 &  11.00 &   3.28 &   4.41 &   6.23 &   6.03 &   6.12 &    5.5\\
 389 &  11.75 &   3.18 &   4.80 &   8.00 &   2.78 &   3.94 &  18.50 &   3.83 &   5.93 &   5.84 &   5.81 &   5.81 &    5.2\\
 390 &  68.75 &   8.04 &   9.59 &  35.75 &   5.73 &   7.30 & 100.50 &   9.54 &  11.58 &   3.34 &   3.19 &   3.27 &    6.4\\
 391 &  41.75 &   6.21 &   7.78 &  25.25 &   5.22 &   5.81 &  61.75 &   7.61 &   9.16 &   5.88 &   5.64 &   5.75 &    6.2\\
 392 &   9.50 &   2.62 &   4.76 &   0.00 &   0.00 &   8.54 &  12.25 &   3.68 &   4.30 &   6.51 &   6.40 &   6.45 &    4.9\\
 393 &   2.00 &   1.32 &   2.63 &  14.75 &   3.59 &   5.20 &  19.25 &   4.58 &   5.18 &   6.37 &   6.22 &   6.29 &    5.7\\
 394 &   6.75 &   2.35 &   4.01 &   5.00 &   2.18 &   3.37 &  10.75 &   3.03 &   4.66 &   6.71 &   6.71 &   6.71 &    2.4\\
 395 &   7.00 &   2.60 &   3.76 &   0.75 &   0.62 &   2.54 &  14.50 &   3.34 &   5.45 &   5.98 &   5.81 &   5.89 &    7.3\\
 396 &  27.50 &   4.77 &   6.85 &  19.50 &   3.94 &   6.04 &  42.25 &   6.71 &   7.28 &   6.24 &   5.99 &   6.11 &    5.7\\
 397 & 115.00 &  10.71 &  11.75 &  33.75 &   5.56 &   7.13 & 143.75 &  11.74 &  13.28 &   5.05 &   4.98 &   5.08 &    5.2\\
 398 &   3.75 &   1.69 &   3.40 &  14.00 &   3.71 &   4.83 &  14.50 &   3.34 &   5.45 &   6.58 &   6.38 &   6.49 &    4.6\\
 399 &   7.71 &   2.50 &   4.22 &   4.50 &   2.44 &   2.65 &  10.71 &   2.99 &   4.70 &   6.04 &   6.01 &   6.02 &    5.7\\
 400 &  33.25 &   5.97 &   6.55 &   3.25 &   1.91 &   2.66 &  38.00 &   6.14 &   7.22 &   6.20 &   5.98 &   6.08 &    8.9\\
 401 &   7.75 &   2.53 &   4.19 &   0.50 &   0.50 &   1.33 &   8.00 &   2.78 &   3.94 &   6.13 &   5.89 &   6.01 &    7.3\\
 402 &   5.00 &   2.18 &   3.37 &  10.25 &   3.37 &   4.01 &  16.50 &   3.59 &   5.70 &   5.74 &   5.63 &   5.70 &    5.1\\
 403 &  21.50 &   4.16 &   6.26 &  10.75 &   3.03 &   4.66 &  31.00 &   5.55 &   6.62 &   6.53 &   6.35 &   6.44 &    4.5\\
 404 &   0.00 &   0.00 &   1.83 &  43.25 &   6.79 &   7.36 &  39.75 &   6.05 &   7.62 &   5.87 &   5.66 &   5.94 &    5.6\\
 405 &  25.25 &   5.22 &   5.81 &  17.00 &   4.09 &   5.20 &  43.50 &   6.11 &   8.18 &   6.61 &   6.52 &   6.56 &    5.2\\
 406 &  25.75 &   4.82 &   6.41 &  11.00 &   3.28 &   4.41 &  33.50 &   5.31 &   7.38 &   6.61 &   6.44 &   6.53 &    3.9\\
 407 &   9.00 &   2.96 &   4.10 &   0.75 &   0.62 &   2.54 &  11.00 &   3.28 &   4.41 &   6.54 &   6.35 &   6.46 &    4.2\\
 408 &  38.25 &   6.39 &   6.97 &  11.86 &   3.28 &   4.70 &  50.50 &   6.62 &   8.69 &   6.40 &   6.20 &   6.30 &    5.9\\
 409 &   5.00 &   2.18 &   3.37 &   2.00 &   1.32 &   2.63 &  11.00 &   3.28 &   4.41 &   6.37 &   6.27 &   6.26 &    1.5\\
 410 &   9.75 &   2.87 &   4.51 &   0.00 &   0.00 &   6.91 &  11.25 &   3.53 &   4.16 &   6.70 &   6.49 &   6.61 &    3.6\\
 411 & 171.00 &  13.07 &  14.10 &  65.25 &   8.30 &   8.85 & 231.25 &  15.44 &  15.97 &   6.39 &   6.20 &   6.31 &    3.5\\
 412 &  55.75 &   7.22 &   8.78 &  16.75 &   3.84 &   5.45 &  71.50 &   7.97 &  10.02 &   5.80 &   5.60 &   5.73 &    8.7\\
 413 &   7.25 &   2.85 &   3.51 &   6.50 &   2.10 &   4.26 &  13.75 &   3.46 &   5.08 &   6.09 &   5.97 &   6.01 &    5.6\\
 414 &  87.75 &   9.12 &  10.66 &  61.50 &   7.36 &   9.41 & 151.25 &  12.53 &  13.06 &   6.63 &   6.65 &   6.65 &    2.2\\
 415 &  13.75 &   3.46 &   5.08 &   8.25 &   3.03 &   3.69 &  23.75 &   4.62 &   6.21 &   6.70 &   6.60 &   6.55 &    4.0\\
 416 &   0.00 &   0.00 &   1.83 &  14.00 &   3.71 &   4.83 &  11.75 &   3.18 &   4.80 &   6.68 &   6.58 &   6.65 &    1.9\\
 417 &  44.00 &   6.61 &   7.68 &  15.25 &   4.09 &   4.70 &  59.25 &   7.91 &   8.47 &   5.81 &   5.56 &   5.68 &    6.9\\
 418 &   7.00 &   2.60 &   3.76 &   1.00 &   0.87 &   2.29 &  11.00 &   3.28 &   4.41 &   6.55 &   6.38 &   6.46 &    3.4\\
 419 &   0.00 &   0.00 &   1.07 &  20.25 &   4.69 &   5.29 &  19.50 &   3.94 &   6.04 &   6.66 &   6.53 &   6.60 &    2.5\\
 420 &   6.00 &   2.40 &   3.58 &   2.00 &   1.32 &   2.63 &   7.50 &   2.28 &   4.44 &   6.47 &   6.28 &   6.36 &    4.1\\
 421 &   3.75 &   1.69 &   3.40 &   1.25 &   1.12 &   2.04 &   5.25 &   2.43 &   3.12 &   6.70 &   6.39 &   6.61 &    3.0\\
 422 &  13.00 &   3.57 &   4.69 &   7.25 &   2.85 &   3.51 &  23.00 &   4.77 &   5.86 &   6.14 &   5.94 &   6.03 &    2.6\\
 423 &  42.25 &   6.71 &   7.28 &  12.25 &   3.68 &   4.30 &  54.50 &   6.90 &   8.96 &   6.48 &   6.28 &   6.38 &    4.5\\
 424 &  22.75 &   4.52 &   6.11 &   0.00 &   0.00 &   1.83 &  26.25 &   5.32 &   5.91 &   6.59 &   6.61 &   6.61 &    2.7\\
 425 &  11.50 &   2.93 &   5.05 &  51.00 &   7.12 &   8.19 &  56.25 &   7.72 &   8.28 &   5.85 &   5.77 &   5.81 &    7.3\\
 426 &  40.00 &   6.30 &   7.37 &  19.50 &   4.83 &   4.93 &  60.25 &   7.98 &   8.54 &   5.45 &   5.23 &   5.35 &    8.3\\
 427 &  26.50 &   4.67 &   6.76 &  23.50 &   4.37 &   6.46 &  46.00 &   6.76 &   7.83 &   4.93 &   4.73 &   4.79 &    6.4\\
 428 &   1.75 &   1.07 &   2.88 &   7.00 &   2.60 &   3.76 &   7.75 &   2.53 &   4.19 &   5.65 &   5.51 &   5.56 &    7.3\\
 429 &   3.75 &   1.69 &   3.40 &   1.75 &   1.07 &   2.88 &   6.75 &   2.35 &   4.01 &   3.74 &   3.71 &   3.73 &    3.4\\
 430 &  44.50 &   6.19 &   8.26 &   6.75 &   2.35 &   4.01 &  54.25 &   7.58 &   8.14 &   4.66 &   4.52 &   4.48 &    5.4\\
 431 &  84.50 &   8.71 &  10.75 &  51.50 &   6.69 &   8.75 & 134.25 &  11.82 &  12.35 &   6.20 &   5.97 &   6.07 &    9.1\\
 432 &  41.00 &   6.38 &   7.45 &  17.00 &   4.09 &   5.20 &  56.50 &   7.03 &   9.09 &   5.86 &   5.76 &   5.81 &    7.7\\
 433 &   0.50 &   0.37 &   2.79 &   8.50 &   2.46 &   4.60 &   7.25 &   2.85 &   3.51 &   5.93 &   5.73 &   5.90 &    4.1\\
 434 &  28.50 &   4.86 &   6.94 &  22.00 &   4.66 &   5.76 &  51.00 &   7.12 &   8.19 &   5.97 &   5.77 &   5.88 &    7.2\\
 435 &   0.50 &   0.50 &   1.33 &   0.50 &   0.37 &   2.79 &   3.50 &   1.44 &   3.65 &   6.53 &   6.57 &   6.56 &    3.0\\
 436 &   7.75 &   2.53 &   4.19 &  10.75 &   3.03 &   4.66 &  20.00 &   4.44 &   5.54 &   6.59 &   6.36 &   6.50 &    3.5\\
 437 &  54.00 &   7.33 &   8.39 &  22.50 &   4.27 &   6.36 &  75.25 &   8.90 &   9.45 &   5.55 &   5.53 &   5.57 &    5.3\\
 438 &  44.14 &   6.76 &   7.54 &  19.00 &   4.33 &   5.43 &  61.00 &   7.79 &   8.85 &   5.48 &   5.19 &   5.39 &    7.3\\
 439 &   3.75 &   1.69 &   3.40 &   0.75 &   0.62 &   2.54 &   8.50 &   2.46 &   4.60 &   6.59 &   6.62 &   6.55 &    4.2\\
 440 &  25.50 &   4.57 &   6.66 &  13.25 &   3.82 &   4.44 &  39.25 &   6.47 &   7.05 &   5.27 &   5.33 &   5.35 &    7.8\\
 441 &  11.00 &   3.28 &   4.41 &  23.75 &   4.62 &   6.21 &  27.50 &   4.77 &   6.85 &   6.64 &   6.53 &   6.58 &    5.3\\
 442 &  12.00 &   3.43 &   4.55 &  19.00 &   4.33 &   5.43 &  27.75 &   5.02 &   6.60 &   5.31 &   5.39 &   5.36 &    2.9\\
 443 &  28.86 &   5.22 &   6.59 &  30.71 &   5.26 &   6.91 &  53.00 &   7.26 &   8.32 &   5.98 &   5.77 &   5.89 &    7.1\\
 444 &  11.75 &   3.18 &   4.80 &   3.00 &   1.66 &   2.91 &  17.25 &   4.34 &   4.95 &   5.93 &   5.81 &   5.79 &    3.1\\
 445 &  12.25 &   3.68 &   4.30 &  30.75 &   5.30 &   6.87 &  38.50 &   5.72 &   7.80 &   6.31 &   6.10 &   6.19 &    5.3\\
 446 &  18.50 &   3.83 &   5.93 &   7.00 &   2.60 &   3.76 &  24.25 &   5.12 &   5.71 &   6.76 &   6.71 &   6.73 &    3.9\\
 447 &   5.75 &   2.15 &   3.83 &   2.00 &   1.32 &   2.63 &   9.00 &   2.96 &   4.10 &   6.70 &   6.48 &   6.61 &    2.6\\
 448 &  25.75 &   4.82 &   6.41 &  17.75 &   3.96 &   5.57 &  42.25 &   6.71 &   7.28 &   6.66 &   6.42 &   6.57 &    2.9\\
 449 &  32.25 &   5.88 &   6.46 &  15.50 &   3.47 &   5.58 &  49.25 &   7.23 &   7.79 &   6.04 &   5.69 &   5.90 &    5.7\\
 450 &  14.00 &   3.71 &   4.83 &   7.75 &   2.53 &   4.19 &  18.00 &   4.21 &   5.32 &   6.04 &   5.91 &   5.98 &    6.0\\
 451 &  14.25 &   3.96 &   4.58 &   7.25 &   2.85 &   3.51 &  17.00 &   4.09 &   5.20 &   5.95 &   5.82 &   5.89 &    6.5\\
 452 & 101.50 &   9.59 &  11.63 &  25.75 &   4.82 &   6.41 & 129.25 &  11.60 &  12.14 &   6.43 &   6.45 &   6.44 &    4.0\\
 453 &  67.75 &   7.98 &   9.53 &  24.75 &   4.72 &   6.31 &  94.25 &   9.93 &  10.48 &   6.82 &   6.79 &   6.80 &    3.3\\
 454 &  42.25 &   6.71 &   7.28 &  20.50 &   4.06 &   6.15 &  67.00 &   8.17 &   9.22 &   6.12 &   5.92 &   6.04 &    5.8\\
 455 &  64.75 &   7.80 &   9.35 &   9.00 &   2.96 &   4.10 &  77.25 &   9.01 &   9.56 &   5.33 &   5.13 &   5.21 &    8.4\\
 456 &  63.75 &   7.73 &   9.29 &  10.75 &   3.03 &   4.66 &  74.50 &   8.15 &  10.20 &   6.64 &   6.63 &   6.78 &    2.5\\
 457 &  95.25 &   9.98 &  10.53 &  40.00 &   6.30 &   7.37 & 136.50 &  11.19 &  13.23 &   5.56 &   5.35 &   5.40 &    6.5\\
 458 &  11.43 &   3.71 &   3.98 &   9.57 &   2.69 &   4.69 &  20.29 &   4.73 &   5.26 &   4.28 &   4.13 &   4.22 &    6.8\\
 459 &  63.25 &   8.17 &   8.73 &  11.75 &   3.18 &   4.80 &  78.00 &   8.82 &   9.87 &   5.08 &   4.90 &   5.00 &    9.3\\
 460 &  19.50 &   3.94 &   6.04 &  13.25 &   3.82 &   4.44 &  35.50 &   5.48 &   7.55 &   5.65 &   5.37 &   5.50 &    7.7\\
 461 &  62.75 &   7.67 &   9.23 &  32.50 &   5.22 &   7.30 &  91.00 &   9.53 &  10.57 &   6.35 &   6.31 &   6.33 &    5.1\\
 462 &  25.50 &   4.57 &   6.66 &   7.50 &   3.10 &   3.26 &  33.50 &   5.31 &   7.38 &   5.85 &   5.62 &   5.79 &    8.3\\
 463 &   7.75 &   2.53 &   4.19 &   2.00 &   1.32 &   2.63 &   9.00 &   2.96 &   4.10 &   5.91 &   5.72 &   5.85 &    5.6\\
 464 &  14.00 &   3.71 &   4.83 &   5.00 &   2.18 &   3.37 &  17.75 &   3.96 &   5.57 &   6.50 &   6.31 &   6.40 &    6.7\\
 465 &   1.00 &   0.87 &   2.29 &   9.00 &   2.96 &   4.10 &   8.00 &   2.78 &   3.94 &   6.92 &   6.92 &   6.92 &    2.3\\
 466 &   8.50 &   2.46 &   4.60 &   9.25 &   3.21 &   3.85 &  17.75 &   3.96 &   5.57 &   6.31 &   6.28 &   6.29 &    5.1\\
 467 &  34.00 &   5.81 &   6.88 &  18.25 &   4.46 &   5.07 &  52.00 &   7.19 &   8.25 &   6.20 &   6.07 &   6.15 &    6.6\\
 468 &  17.75 &   3.96 &   5.57 &  12.50 &   3.07 &   5.19 &  31.00 &   5.55 &   6.62 &   6.21 &   6.17 &   6.11 &    5.3\\
 469 &  29.50 &   4.95 &   7.03 &   6.75 &   2.35 &   4.01 &  38.50 &   5.72 &   7.80 &   6.42 &   6.40 &   6.37 &    6.0\\
 470 &   4.50 &   1.68 &   3.87 &   1.75 &   1.07 &   2.88 &   6.50 &   2.10 &   4.26 &   5.93 &   5.76 &   5.79 &    5.8\\
 471 &  19.25 &   4.58 &   5.18 &  14.50 &   3.34 &   5.45 &  31.25 &   5.80 &   6.37 &   6.26 &   6.11 &   6.21 &    4.5\\
 472 &  20.50 &   4.06 &   6.15 &  16.50 &   4.47 &   4.58 &  36.00 &   5.98 &   7.05 &   6.21 &   5.99 &   6.09 &    9.1\\
 473 &  49.25 &   7.23 &   7.79 &  39.50 &   6.72 &   6.80 &  93.25 &   9.88 &  10.43 &   5.79 &   5.56 &   5.69 &    7.4\\
 474 & 162.25 &  12.97 &  13.50 &  52.00 &   7.19 &   8.25 & 212.50 &  14.09 &  16.12 &   6.14 &   5.88 &   6.00 &    6.8\\
 475 &   7.00 &   2.60 &   3.76 &   0.00 &   0.00 &   5.74 &   9.25 &   3.21 &   3.85 &   6.93 &   6.93 &   6.93 &    2.1\\
 476 &  33.25 &   5.97 &   6.55 &  11.00 &   3.28 &   4.41 &  47.50 &   6.41 &   8.47 &   6.07 &   5.99 &   6.02 &    9.4\\
 477 &   7.25 &   2.85 &   3.51 &   4.50 &   2.44 &   2.65 &  12.75 &   3.32 &   4.94 &   6.08 &   5.83 &   5.89 &    5.4\\
 478 &  16.00 &   3.97 &   5.08 &  12.50 &   3.07 &   5.19 &  27.86 &   5.12 &   6.49 &   5.63 &   5.57 &   5.58 &    9.5\\
 479 &  10.50 &   2.78 &   4.91 &  10.50 &   2.78 &   4.91 &  17.50 &   3.71 &   5.82 &   6.18 &   6.03 &   6.12 &    4.5\\
 480 &  30.50 &   5.05 &   7.12 &  15.50 &   4.34 &   4.45 &  49.00 &   6.98 &   8.04 &   6.22 &   5.96 &   6.17 &    3.1\\
 481 &   5.57 &   1.97 &   4.00 &  14.29 &   3.99 &   4.54 &  14.86 &   3.70 &   5.10 &   5.80 &   5.55 &   5.69 &    7.3\\
 482 & 102.75 &   9.89 &  11.43 &  44.00 &   6.61 &   7.68 & 146.50 &  11.61 &  13.65 &   5.85 &   5.63 &   5.76 &    6.8\\
 483 &   4.75 &   1.93 &   3.62 &   4.00 &   1.94 &   3.15 &  10.25 &   3.37 &   4.01 &   3.78 &   3.68 &   3.71 &    0.6\\
 484 &   6.75 &   2.35 &   4.01 &   6.75 &   2.35 &   4.01 &  13.00 &   3.57 &   4.69 &   6.21 &   6.10 &   6.09 &    5.9\\
 485 &   9.50 &   2.62 &   4.76 &  29.00 &   5.36 &   6.44 &  36.25 &   6.23 &   6.80 &   6.22 &   6.06 &   6.16 &    4.2\\
 486 &  16.50 &   3.59 &   5.70 &  21.25 &   4.81 &   5.40 &  32.50 &   5.22 &   7.30 &   6.21 &   6.18 &   6.19 &    5.7\\
 487 &  31.50 &   5.13 &   7.21 &  37.50 &   5.64 &   7.72 &  69.50 &   7.85 &   9.90 &   5.81 &   5.60 &   5.70 &    9.6\\
 488 &  12.75 &   3.32 &   4.94 &  25.25 &   5.22 &   5.81 &  35.00 &   5.89 &   6.97 &   6.33 &   6.15 &   6.27 &    3.6\\
 489 &   6.00 &   2.40 &   3.58 &   2.00 &   1.32 &   2.63 &  11.25 &   3.53 &   4.16 &   6.91 &   6.64 &   6.91 &    2.1\\
 490 &  12.50 &   3.07 &   5.19 &  17.50 &   3.71 &   5.82 &  28.75 &   5.11 &   6.69 &   6.07 &   5.99 &   6.02 &    9.6\\
 491 &  13.75 &   3.46 &   5.08 &  17.00 &   4.09 &   5.20 &  29.00 &   5.36 &   6.44 &   5.95 &   5.91 &   5.75 &    5.6\\
 492 &  10.00 &   3.12 &   4.26 &   0.75 &   0.62 &   2.54 &  16.25 &   4.22 &   4.83 &   5.79 &   5.53 &   5.68 &    7.3\\
 493 &  32.25 &   5.88 &   6.46 &   8.75 &   2.71 &   4.35 &  42.50 &   6.04 &   8.11 &   5.59 &   5.45 &   5.53 &    8.2\\
 494 &  76.25 &   8.95 &   9.50 &  28.75 &   5.11 &   6.69 & 102.00 &  10.09 &  11.13 &   6.07 &   5.92 &   6.00 &    7.7\\
 495 &   5.00 &   2.18 &   3.37 &   3.75 &   1.69 &   3.40 &  10.25 &   3.37 &   4.01 &   6.23 &   6.07 &   6.17 &    3.9\\
 496 &  13.00 &   3.57 &   4.69 &  55.75 &   7.22 &   8.78 &  64.25 &   8.23 &   8.79 &   6.13 &   6.09 &   6.10 &    6.1\\
 497 &  20.25 &   4.69 &   5.29 &  13.00 &   3.57 &   4.69 &  33.00 &   5.72 &   6.80 &   6.13 &   5.79 &   5.96 &    8.0\\
 498 &  10.00 &   3.12 &   4.26 &   8.25 &   3.03 &   3.69 &  14.50 &   3.34 &   5.45 &   4.29 &   4.39 &   4.30 &    1.8\\
 499 &  11.00 &   3.28 &   4.41 &   3.00 &   1.66 &   2.91 &  19.25 &   4.58 &   5.18 &   6.13 &   6.09 &   6.10 &    6.2\\
 500 &   6.50 &   2.10 &   4.26 &   1.50 &   1.37 &   1.79 &   8.50 &   2.46 &   4.60 &   3.46 &   3.25 &   3.34 &    1.2\\
 501 &   1.50 &   0.82 &   3.13 &   5.75 &   2.15 &   3.83 &   7.25 &   2.85 &   3.51 &   6.25 &   6.09 &   6.19 &    3.7\\
 502 &  42.00 &   6.46 &   7.53 &  12.00 &   3.43 &   4.55 &  54.75 &   7.15 &   8.71 &   5.73 &   5.54 &   5.62 &    8.4\\
 503 &   0.75 &   0.62 &   2.54 &  35.25 &   6.14 &   6.72 &  30.50 &   5.05 &   7.12 &   5.96 &   5.94 &   6.25 &    4.0\\
 504 &   3.25 &   1.91 &   2.66 &  15.25 &   4.09 &   4.70 &  18.50 &   4.71 &   4.82 &   6.09 &   6.03 &   6.05 &    9.3\\
 505 &  39.00 &   6.22 &   7.30 &  10.25 &   3.37 &   4.01 &  46.75 &   6.59 &   8.15 &   5.67 &   5.42 &   5.57 &    6.5\\
 506 &   3.00 &   1.66 &   2.91 &   5.75 &   2.15 &   3.83 &  12.00 &   3.43 &   4.55 &   6.56 &   6.40 &   6.48 &    2.6\\
 507 &   1.75 &   1.07 &   2.88 &   9.50 &   3.46 &   3.60 &   8.00 &   2.78 &   3.94 &   6.73 &   6.57 &   6.70 &    3.5\\
 508 &  21.50 &   4.16 &   6.26 &  12.00 &   3.43 &   4.55 &  32.25 &   5.88 &   6.46 &   5.90 &   5.67 &   5.81 &    6.3\\
 509 &   1.25 &   1.12 &   2.04 &  15.50 &   3.47 &   5.58 &  13.75 &   3.46 &   5.08 &   6.13 &   5.94 &   6.06 &    4.5\\
 510 &   0.75 &   0.62 &   2.54 &   8.00 &   2.78 &   3.94 &   9.75 &   2.87 &   4.51 &   6.34 &   6.31 &   6.33 &    4.6\\
 511 &  17.50 &   3.71 &   5.82 &   6.25 &   2.65 &   3.33 &  21.75 &   4.41 &   6.01 &   5.46 &   5.34 &   5.49 &    7.7\\
 512 &  34.25 &   6.06 &   6.63 &   0.00 &   0.00 &  20.84 &  36.75 &   5.81 &   7.38 &   5.70 &   5.62 &   5.65 &    7.6\\
 513 &   2.75 &   1.41 &   3.16 &   1.25 &   1.12 &   2.04 &   7.00 &   2.60 &   3.76 &   6.37 &   6.34 &   6.36 &    4.3\\
 514 &   2.50 &   1.16 &   3.41 &   7.75 &   2.53 &   4.19 &   6.75 &   2.35 &   4.01 &   5.85 &   5.75 &   5.82 &    6.0\\
 515 &  45.75 &   6.51 &   8.08 &  25.25 &   5.22 &   5.81 &  68.25 &   8.48 &   9.03 &   5.65 &   5.48 &   5.57 &    8.9\\
 516 &   7.25 &   2.85 &   3.51 &  17.00 &   4.09 &   5.20 &  23.25 &   5.02 &   5.61 &   6.30 &   6.04 &   6.17 &    8.3\\
 517 & 371.25 &  19.50 &  20.03 & 245.75 &  15.43 &  16.95 & 601.00 &  24.51 &  25.53 &   2.92 &   2.90 &   2.92 &    7.4\\
 518 &  32.75 &   5.47 &   7.05 &  16.25 &   4.22 &   4.83 &  46.25 &   7.01 &   7.58 &   6.40 &   6.23 &   6.35 &    2.4\\
 519 &   5.50 &   1.90 &   4.08 &   6.75 &   2.35 &   4.01 &  15.25 &   4.09 &   4.70 &   5.23 &   5.11 &   5.17 &    3.9\\
 520 &  22.25 &   4.91 &   5.51 &  12.00 &   3.43 &   4.55 &  35.75 &   5.73 &   7.30 &   5.98 &   5.89 &   5.93 &    7.7\\
 521 &  42.00 &   6.46 &   7.53 &  14.75 &   3.59 &   5.20 &  54.00 &   7.33 &   8.39 &   6.41 &   6.26 &   6.35 &    1.9\\
 522 &   2.50 &   1.16 &   3.41 &   0.00 &   0.00 &   7.80 &   2.50 &   1.82 &   2.13 &   6.50 &   6.34 &   6.46 &    2.1\\
 523 &   3.50 &   1.44 &   3.65 &  19.75 &   4.19 &   5.79 &  12.25 &   3.68 &   4.30 &   6.45 &   6.26 &   6.39 &    1.8\\
 524 &   2.75 &   1.41 &   3.16 &   0.00 &   0.00 &   7.91 &   5.00 &   2.18 &   3.37 &   6.68 &   6.62 &   6.66 &    3.9\\
 525 &  37.25 &   6.31 &   6.88 &  19.75 &   4.19 &   5.79 &  58.00 &   7.60 &   8.66 &   6.62 &   6.42 &   6.51 &    4.5\\
 526 &  20.25 &   4.69 &   5.29 &  19.50 &   3.94 &   6.04 &  39.00 &   6.22 &   7.30 &   6.42 &   6.41 &   6.42 &    3.8\\
 527 &   2.75 &   1.41 &   3.16 &   8.50 &   2.46 &   4.60 &   8.50 &   2.46 &   4.60 &   6.52 &   6.35 &   6.48 &    1.9\\
 528 &  11.50 &   2.93 &   5.05 &  14.00 &   3.71 &   4.83 &  23.50 &   4.37 &   6.46 &   6.25 &   6.17 &   6.21 &    5.8\\
 529 &  12.43 &   3.86 &   4.13 &   1.00 &   0.87 &   2.29 &  11.43 &   3.71 &   3.98 &   6.47 &   6.47 &   6.47 &    6.7\\
 530 &   4.25 &   2.19 &   2.90 &   0.75 &   0.62 &   2.54 &   7.43 &   3.03 &   3.33 &   6.61 &   6.41 &   6.50 &    4.6\\
 531 &  18.50 &   3.83 &   5.93 &   9.50 &   3.46 &   3.60 &  28.50 &   4.86 &   6.94 &   6.45 &   6.45 &   6.46 &    3.4\\
 532 &  25.86 &   4.93 &   6.30 &  14.00 &   3.71 &   4.83 &  43.14 &   6.68 &   7.46 &   6.49 &   6.49 &   6.48 &    6.7\\
 533 &   9.75 &   2.87 &   4.51 &   1.50 &   1.37 &   1.79 &  11.00 &   3.28 &   4.41 &   2.88 &   2.72 &   2.83 &    5.3\\
 534 &   4.50 &   1.68 &   3.87 &   3.25 &   1.91 &   2.66 &  10.50 &   2.78 &   4.91 &   6.26 &   6.25 &   6.24 &    7.9\\
 535 &  17.50 &   3.71 &   5.82 &  15.50 &   3.47 &   5.58 &  28.25 &   5.52 &   6.10 &   5.79 &   5.57 &   5.67 &    6.8\\
 536 &   1.25 &   1.12 &   2.04 &   6.75 &   2.35 &   4.01 &   9.75 &   2.87 &   4.51 &   3.01 &   2.79 &   2.89 &    4.6\\
 537 &  49.00 &   6.98 &   8.04 &  18.50 &   3.83 &   5.93 &  67.75 &   7.98 &   9.53 &   6.23 &   5.95 &   6.13 &    3.3\\
 538 &   0.00 &   0.00 &   2.34 &   5.00 &   2.18 &   3.37 &   7.25 &   2.85 &   3.51 &   3.07 &   2.82 &   2.96 &    4.6\\
 539 &  76.75 &   8.51 &  10.06 &  29.75 &   5.20 &   6.78 & 106.25 &  10.53 &  11.08 &   6.43 &   6.20 &   6.38 &    1.8\\
 540 &  22.50 &   4.27 &   6.36 &  14.75 &   3.59 &   5.20 &  39.75 &   6.05 &   7.62 &   6.55 &   6.48 &   6.51 &    6.7\\
 541 &  12.25 &   3.68 &   4.30 &   1.50 &   0.82 &   3.13 &  14.25 &   3.96 &   4.58 &   5.86 &   5.72 &   5.79 &    8.7\\
 542 &  37.25 &   6.31 &   6.88 & 146.00 &  12.07 &  13.11 & 179.75 &  13.16 &  14.69 &   5.64 &   5.68 &   5.64 &    6.4\\
 543 &  12.00 &   3.43 &   4.55 &  18.50 &   4.71 &   4.82 &  30.75 &   5.30 &   6.87 &   5.90 &   5.72 &   5.81 &    9.1\\
 544 &  57.50 &   7.10 &   9.16 &  34.75 &   5.64 &   7.22 &  90.50 &   9.03 &  11.07 &   6.66 &   6.66 &   6.66 &    3.8\\
 545 &   5.75 &   2.15 &   3.83 &  10.50 &   3.62 &   3.76 &  15.25 &   4.09 &   4.70 &   6.77 &   6.61 &   6.71 &    3.5\\
 546 &  19.25 &   4.58 &   5.18 &   0.00 &   0.00 &   9.11 &  20.75 &   4.31 &   5.90 &   5.90 &   5.67 &   5.77 &    6.1\\
 547 &   0.00 &   0.00 &   1.79 &   5.75 &   2.15 &   3.83 &   7.75 &   2.53 &   4.19 &   6.51 &   6.28 &   6.44 &    0.9\\
 548 &   1.00 &   0.87 &   2.29 &  10.25 &   3.37 &   4.01 &  12.00 &   3.43 &   4.55 &   6.29 &   6.21 &   6.25 &    5.5\\
 549 & 141.00 &  11.86 &  12.90 &  47.50 &   6.41 &   8.47 & 177.75 &  13.08 &  14.62 &   5.38 &   5.05 &   5.20 &    7.3\\
 550 &   8.00 &   2.78 &   3.94 &  47.50 &   6.41 &   8.47 &  56.00 &   7.47 &   8.53 &   5.69 &   5.82 &   5.97 &    8.3\\
 551 &  52.50 &   6.76 &   8.82 &  25.50 &   4.57 &   6.66 &  76.50 &   8.26 &  10.31 &   5.25 &   5.04 &   4.90 &    7.3\\
 552 &   6.75 &   2.35 &   4.01 &   6.50 &   2.90 &   3.08 &   8.75 &   2.71 &   4.35 &   4.16 &   4.01 &   4.17 &    3.1\\
 553 &  15.50 &   3.47 &   5.58 &  18.50 &   3.83 &   5.93 &  33.25 &   5.97 &   6.55 &   5.86 &   5.67 &   5.77 &    7.6\\
 554 &   1.75 &   1.07 &   2.88 &   6.00 &   2.40 &   3.58 &   8.50 &   2.46 &   4.60 &   5.99 &   5.97 &   5.88 &    1.7\\
 555 &   4.00 &   1.94 &   3.15 &   0.75 &   0.62 &   2.54 &   6.00 &   2.40 &   3.58 &   6.04 &   5.71 &   5.86 &    8.6\\
 556 &   4.50 &   1.68 &   3.87 &  10.25 &   3.37 &   4.01 &  14.25 &   3.96 &   4.58 &   5.80 &   5.33 &   5.66 &    5.0\\
 557 &  27.75 &   5.02 &   6.60 &  26.75 &   4.92 &   6.51 &  49.25 &   7.23 &   7.79 &   6.17 &   5.87 &   6.01 &    7.7\\
 558 &  22.25 &   4.91 &   5.51 &  32.75 &   5.47 &   7.05 &  47.50 &   6.41 &   8.47 &   6.14 &   5.84 &   5.96 &    9.1\\
 559 &  17.25 &   4.34 &   4.95 &   2.75 &   1.41 &   3.16 &  22.25 &   4.91 &   5.51 &   6.46 &   6.30 &   6.39 &    6.2\\
 560 &  13.50 &   3.21 &   5.33 &   4.50 &   2.44 &   2.65 &  17.25 &   4.34 &   4.95 &   6.63 &   6.59 &   6.61 &    5.8\\
 561 &  36.25 &   6.23 &   6.80 &  30.00 &   5.45 &   6.53 &  57.50 &   7.10 &   9.16 &   6.14 &   5.85 &   6.01 &    9.0\\
 562 &  21.75 &   4.41 &   6.01 &  19.75 &   4.19 &   5.79 &  40.25 &   6.55 &   7.12 &   6.74 &   6.55 &   6.63 &    4.0\\
 563 &  25.75 &   4.82 &   6.41 &   3.50 &   1.44 &   3.65 &  27.75 &   5.02 &   6.60 &   6.40 &   6.14 &   6.26 &    6.1\\
 564 &  28.00 &   5.27 &   6.35 &  24.00 &   4.87 &   5.96 &  48.00 &   6.91 &   7.97 &   6.61 &   6.41 &   6.50 &    4.8\\
 565 &  58.00 &   7.60 &   8.66 &  26.25 &   5.32 &   5.91 &  83.25 &   9.35 &   9.89 &   6.14 &   6.21 &   6.15 &    6.6\\
 566 & 130.75 &  11.18 &  12.72 &  58.75 &   7.41 &   8.97 & 189.25 &  13.99 &  14.52 &   6.47 &   6.49 &   6.47 &    6.4\\
 567 &   0.00 &   0.00 &   1.83 &   1.00 &   0.87 &   2.29 &   3.50 &   1.44 &   3.65 &   2.54 &   2.59 &   2.51 &    0.8\\
 568 &  14.00 &   3.71 &   4.83 &   8.25 &   3.03 &   3.69 &  22.50 &   4.27 &   6.36 &   5.96 &   5.98 &   5.98 &    1.7\\
 569 & 108.75 &  10.18 &  11.72 &  44.25 &   6.86 &   7.43 & 152.25 &  12.57 &  13.10 &   6.06 &   5.81 &   5.95 &    3.7\\
 570 &  30.00 &   5.45 &   6.53 &   5.25 &   2.43 &   3.12 &  37.25 &   6.31 &   6.88 &   6.52 &   6.54 &   6.54 &    2.8\\
 571 & 234.00 &  15.29 &  16.32 &  90.25 &   9.72 &  10.27 & 319.50 &  17.38 &  19.41 &   6.34 &   6.24 &   6.30 &    5.1\\
 572 &  29.50 &   4.95 &   7.03 &  21.25 &   4.81 &   5.40 &  49.75 &   6.80 &   8.37 &   6.55 &   6.59 &   6.56 &    5.8\\
 573 &   2.25 &   1.57 &   2.38 &  18.50 &   3.83 &   5.93 &  17.25 &   4.34 &   4.95 &   5.82 &   5.71 &   5.77 &    6.1\\
 574 &  13.75 &   3.46 &   5.08 &  26.00 &   5.07 &   6.16 &  34.75 &   5.64 &   7.22 &   5.96 &   5.70 &   5.82 &    6.8\\
 575 &  37.00 &   6.06 &   7.13 &  17.50 &   3.71 &   5.82 &  51.25 &   7.37 &   7.94 &   6.53 &   6.53 &   6.53 &    4.7\\
 576 &   7.75 &   2.53 &   4.19 &   3.75 &   1.69 &   3.40 &  12.00 &   3.43 &   4.55 &   4.27 &   4.26 &   4.26 &    5.6\\
 577 &   6.25 &   2.65 &   3.33 &  10.25 &   3.37 &   4.01 &  19.75 &   4.19 &   5.79 &   6.61 &   6.25 &   6.37 &    4.7\\
 578 &   6.25 &   2.65 &   3.33 &  26.50 &   4.67 &   6.76 &  29.25 &   5.61 &   6.19 &   4.51 &   4.54 &   4.53 &    0.9\\
 579 &  11.50 &   2.93 &   5.05 &   4.00 &   1.94 &   3.15 &  15.50 &   3.47 &   5.58 &   6.48 &   6.49 &   6.47 &    6.2\\
 580 &   9.00 &   2.96 &   4.10 &   5.00 &   2.18 &   3.37 &  13.75 &   3.46 &   5.08 &   3.79 &   3.66 &   3.73 &    0.9\\
 581 &   9.75 &   2.87 &   4.51 &   4.00 &   1.94 &   3.15 &  12.50 &   3.07 &   5.19 &   6.75 &   6.84 &   6.79 &    5.3\\
 582 &  22.25 &   4.91 &   5.51 &   5.00 &   2.18 &   3.37 &  29.50 &   4.95 &   7.03 &   6.31 &   6.01 &   6.14 &    6.8\\
 583 &  10.00 &   3.12 &   4.26 &  26.50 &   4.67 &   6.76 &  34.50 &   5.39 &   7.47 &   6.53 &   6.71 &   6.55 &    6.5\\
 584 &  26.25 &   5.32 &   5.91 &  11.50 &   2.93 &   5.05 &  36.75 &   5.81 &   7.38 &   5.63 &   5.40 &   5.47 &    5.5\\
 585 & 106.00 &  10.28 &  11.33 &  31.00 &   5.55 &   6.62 & 139.75 &  11.57 &  13.11 &   6.52 &   6.56 &   6.46 &    7.4\\
 586 &  18.50 &   3.83 &   5.93 &  12.50 &   3.07 &   5.19 &  30.50 &   5.05 &   7.12 &   6.25 &   6.20 &   6.24 &    2.9\\
 587 &  14.25 &   3.96 &   4.58 &   8.50 &   3.28 &   3.44 &  22.50 &   4.27 &   6.36 &   6.32 &   6.17 &   6.25 &    7.1\\
 588 &  76.00 &   8.70 &   9.75 &  35.00 &   5.89 &   6.97 & 109.25 &  10.68 &  11.22 &   6.36 &   6.10 &   6.21 &    6.7\\
 589 &  50.75 &   6.87 &   8.44 &  17.75 &   3.96 &   5.57 &  67.00 &   8.17 &   9.22 &   6.11 &   6.09 &   6.05 &    6.8\\
 590 &   0.75 &   0.62 &   2.54 &   0.25 &   0.25 &   1.58 &   7.00 &   2.60 &   3.76 &   6.05 &   5.72 &   5.87 &    8.7\\
 591 &   6.25 &   2.65 &   3.33 &   4.75 &   1.93 &   3.62 &   9.75 &   2.87 &   4.51 &   6.36 &   6.33 &   6.34 &    5.7\\
 592 &  13.50 &   3.21 &   5.33 &   5.50 &   1.90 &   4.08 &  17.50 &   3.71 &   5.82 &   6.01 &   5.83 &   5.92 &    4.5\\
 593 &   7.75 &   2.53 &   4.19 &   6.50 &   2.90 &   3.08 &  11.50 &   2.93 &   5.05 &   6.16 &   5.97 &   6.05 &    2.5\\
 594 &   6.25 &   2.65 &   3.33 &   8.75 &   2.71 &   4.35 &  18.25 &   4.46 &   5.07 &   6.11 &   6.20 &   6.25 &    4.7\\
 595 &  39.50 &   5.80 &   7.87 &  41.00 &   6.38 &   7.45 &  74.00 &   8.59 &   9.64 &   6.05 &   5.87 &   5.96 &    7.6\\
 596 &  15.50 &   3.47 &   5.58 &  14.75 &   3.59 &   5.20 &  27.25 &   5.42 &   6.01 &   6.36 &   6.45 &   6.38 &    6.0\\
 597 &  28.50 &   4.86 &   6.94 &   8.50 &   2.46 &   4.60 &  40.50 &   5.88 &   7.95 &   6.04 &   6.04 &   6.02 &    7.6\\
 598 &  92.25 &   9.83 &  10.37 &  41.50 &   5.96 &   8.03 & 134.75 &  11.36 &  12.90 &   6.48 &   6.46 &   6.46 &    5.7\\
 599 &   3.75 &   1.69 &   3.40 &   0.00 &   0.00 &   1.83 &   6.00 &   2.40 &   3.58 &   6.48 &   6.51 &   6.51 &    2.0\\
 600 &  16.50 &   3.59 &   5.70 &  10.75 &   3.03 &   4.66 &  25.75 &   4.82 &   6.41 &   6.50 &   6.62 &   6.53 &    5.6\\
 601 & 130.25 &  11.64 &  12.18 &  34.75 &   5.64 &   7.22 & 163.50 &  12.30 &  14.33 &   6.92 &   6.88 &   6.92 &    3.2\\
 602 &   5.25 &   2.43 &   3.12 &   0.00 &   0.00 &   7.44 &   7.25 &   2.85 &   3.51 &   6.30 &   6.48 &   6.35 &    4.2\\
 603 &  35.00 &   5.89 &   6.97 &  29.50 &   4.95 &   7.03 &  62.25 &   8.11 &   8.66 &   6.24 &   6.09 &   6.16 &    7.6\\
 604 &   2.25 &   1.57 &   2.38 &   0.00 &   0.00 &  19.92 &   0.00 &   0.00 &  11.72 &   5.66 &   5.44 &   5.56 &    7.2\\
 605 &   7.50 &   2.28 &   4.44 &   4.75 &   1.93 &   3.62 &  11.50 &   2.93 &   5.05 &   6.07 &   5.87 &   5.97 &    6.0\\
 606 &  21.75 &   4.41 &   6.01 &  15.50 &   3.47 &   5.58 &  29.25 &   5.61 &   6.19 &   5.88 &   5.78 &   5.88 &    8.9\\
 607 &  16.75 &   3.84 &   5.45 &  11.25 &   3.53 &   4.16 &  28.25 &   5.52 &   6.10 &   6.19 &   6.03 &   6.12 &    5.0\\
 608 &  12.25 &   3.68 &   4.30 &   8.50 &   3.28 &   3.44 &  18.50 &   3.83 &   5.93 &   5.17 &   4.59 &   4.68 &    7.3\\
 609 &  23.00 &   4.77 &   5.86 &   0.00 &   0.00 &   6.14 &  23.50 &   4.37 &   6.46 &   3.43 &   3.49 &   3.41 &    2.3\\
 610 &  14.00 &   3.71 &   4.83 &  10.75 &   3.03 &   4.66 &  23.25 &   5.02 &   5.61 &   6.21 &   6.13 &   6.16 &    6.9\\
 611 &   2.75 &   1.41 &   3.16 &  10.25 &   3.37 &   4.01 &  14.50 &   3.34 &   5.45 &   6.62 &   6.58 &   6.61 &    4.9\\
 612 &   4.75 &   1.93 &   3.62 &   7.75 &   2.53 &   4.19 &  12.75 &   3.32 &   4.94 &   6.37 &   6.23 &   6.30 &    3.7\\
 613 &  28.75 &   5.11 &   6.69 &   8.50 &   2.46 &   4.60 &  40.50 &   5.88 &   7.95 &   6.54 &   6.42 &   6.48 &    2.7\\
 614 &  15.00 &   3.84 &   4.95 &   1.50 &   0.82 &   3.13 &  17.50 &   3.71 &   5.82 &   6.92 &   7.08 &   6.98 &    4.3\\
 615 &  21.25 &   4.81 &   5.40 &   0.00 &   0.00 &  21.41 &  21.75 &   4.41 &   6.01 &   6.17 &   6.01 &   6.09 &    8.1\\
 616 &  11.25 &   3.53 &   4.16 &   0.00 &   0.00 &  14.99 &  13.25 &   3.82 &   4.44 &   6.02 &   5.79 &   5.92 &    7.2\\
 617 &  16.50 &   3.59 &   5.70 &  12.00 &   3.43 &   4.55 &  29.00 &   5.36 &   6.44 &   7.01 &   7.00 &   7.03 &    2.3\\
 618 &  18.25 &   4.46 &   5.07 &  12.50 &   3.07 &   5.19 &  28.75 &   5.11 &   6.69 &   5.61 &   5.66 &   5.63 &    8.2\\
 619 &  16.00 &   3.97 &   5.08 &  32.25 &   5.88 &   6.46 &  46.75 &   6.59 &   8.15 &   6.16 &   6.22 &   6.32 &    2.8\\
 620 &   7.50 &   2.28 &   4.44 &   4.75 &   1.93 &   3.62 &  10.25 &   3.37 &   4.01 &   6.36 &   6.43 &   6.41 &    3.0\\
 621 &   6.50 &   2.10 &   4.26 &   0.00 &   0.00 &   6.74 &   5.75 &   2.15 &   3.83 &   6.06 &   6.06 &   6.09 &    3.5\\
 622 &  16.50 &   3.59 &   5.70 &  10.00 &   3.12 &   4.26 &  24.00 &   4.87 &   5.96 &   6.33 &   6.21 &   6.24 &    3.9\\
 623 &  69.00 &   8.29 &   9.34 &  35.75 &   5.73 &   7.30 &  98.00 &   9.89 &  10.93 &   6.45 &   6.56 &   6.51 &    4.8\\
 624 &   0.50 &   0.37 &   2.79 &  18.50 &   3.83 &   5.93 &  21.75 &   4.41 &   6.01 &   6.13 &   6.06 &   6.15 &    7.1\\
 625 &   6.50 &   2.90 &   3.08 &  25.00 &   4.97 &   6.06 &  29.00 &   5.36 &   6.44 &   6.18 &   6.06 &   6.18 &    7.1\\
 626 &  52.50 &   6.76 &   8.82 &  35.75 &   5.73 &   7.30 &  85.25 &   9.46 &  10.00 &   5.52 &   5.26 &   5.33 &    6.0\\
 627 &  16.75 &   3.84 &   5.45 &   7.75 &   2.53 &   4.19 &  32.00 &   5.63 &   6.71 &   6.07 &   5.88 &   5.97 &    9.1\\
 628 &  13.50 &   3.21 &   5.33 &   3.25 &   1.91 &   2.66 &  18.25 &   4.46 &   5.07 &   6.06 &   5.88 &   5.99 &    6.9\\
 629 &   7.25 &   2.85 &   3.51 &   9.00 &   2.96 &   4.10 &  16.00 &   3.97 &   5.08 &   6.28 &   6.33 &   6.32 &    3.6\\
 630 &  20.00 &   4.44 &   5.54 &  11.00 &   3.28 &   4.41 &  27.25 &   5.42 &   6.01 &   5.72 &   5.54 &   5.59 &    5.9\\
 631 & 295.50 &  16.70 &  18.72 & 101.75 &   9.84 &  11.38 & 389.75 &  19.49 &  21.01 &   6.28 &   6.33 &   6.31 &    4.0\\
 632 &  24.75 &   4.72 &   6.31 &   7.50 &   2.28 &   4.44 &  31.75 &   5.38 &   6.96 &   4.47 &   4.26 &   4.22 &    6.9\\
 633 &  14.00 &   3.71 &   4.83 &   4.50 &   1.68 &   3.87 &  23.00 &   4.77 &   5.86 &   7.09 &   7.05 &   7.10 &    1.1\\
 634 &  20.50 &   4.06 &   6.15 &  34.75 &   5.64 &   7.22 &  54.25 &   7.58 &   8.14 &   5.53 &   5.35 &   5.41 &    9.2\\
 635 &  12.71 &   3.28 &   4.98 &   0.00 &   0.00 &  13.24 &  12.29 &   3.71 &   4.27 &   4.89 &   4.46 &   4.74 &    7.2\\
 636 &   2.00 &   1.32 &   2.63 &   9.50 &   3.46 &   3.60 &  10.50 &   2.78 &   4.91 &   6.16 &   5.97 &   6.06 &    5.6\\
 637 &  20.00 &   4.44 &   5.54 &   7.75 &   2.53 &   4.19 &  25.75 &   4.82 &   6.41 &   6.92 &   6.79 &   6.89 &    2.3\\
 638 &  68.14 &   8.37 &   9.14 &  70.50 &   7.91 &   9.96 & 142.14 &  12.05 &  12.80 &   7.10 &   7.04 &   7.11 &    0.9\\
 639 &  18.00 &   4.21 &   5.32 &   1.50 &   0.82 &   3.13 &  20.25 &   4.69 &   5.29 &   5.98 &   5.91 &   6.00 &    7.8\\
 640 &   3.75 &   1.69 &   3.40 &   3.50 &   1.44 &   3.65 &   3.00 &   1.66 &   2.91 &   6.20 &   6.23 &   6.22 &    4.3\\
 641 &  20.50 &   4.06 &   6.15 &   9.25 &   3.21 &   3.85 &  29.25 &   5.61 &   6.19 &   5.93 &   5.74 &   5.86 &    7.7\\
 642 &   4.00 &   1.94 &   3.15 &   3.00 &   1.66 &   2.91 &   8.75 &   2.71 &   4.35 &   4.14 &   4.29 &   4.20 &    1.4\\
 643 &  11.00 &   3.28 &   4.41 &   6.00 &   2.40 &   3.58 &  14.57 &   3.41 &   5.38 &   7.10 &   7.04 &   7.10 &    0.8\\
 644 &   0.25 &   0.25 &   1.58 &  15.00 &   3.84 &   4.95 &  16.00 &   3.97 &   5.08 &   6.03 &   6.11 &   5.95 &    4.4\\
 645 &  97.75 &   9.64 &  11.18 &  48.75 &   6.73 &   8.29 & 138.75 &  11.53 &  13.07 &   5.88 &   5.67 &   5.78 &    5.6\\
 646 &   6.75 &   2.35 &   4.01 &   8.25 &   3.03 &   3.69 &  13.75 &   3.46 &   5.08 &   6.49 &   6.62 &   6.54 &    3.9\\
 647 &  35.14 &   6.04 &   6.83 &   7.50 &   3.10 &   3.26 &  43.43 &   6.97 &   7.18 &   5.80 &   5.83 &   5.87 &    6.4\\
 648 &   7.00 &   2.60 &   3.76 &   6.00 &   2.40 &   3.58 &  11.50 &   2.93 &   5.05 &   7.11 &   7.04 &   7.11 &    0.5\\
 649 &  86.75 &   9.06 &  10.61 &  41.75 &   6.21 &   7.78 & 130.75 &  11.18 &  12.72 &   5.82 &   5.78 &   5.83 &    6.8\\
 650 &  36.00 &   5.98 &   7.05 &  17.25 &   4.34 &   4.95 &  52.00 &   7.19 &   8.25 &   6.71 &   6.73 &   6.71 &    6.6\\
 651 &  24.25 &   5.12 &   5.71 &  14.25 &   3.96 &   4.58 &  40.00 &   6.30 &   7.37 &   6.05 &   6.04 &   6.10 &    5.4\\
 652 &  24.00 &   4.87 &   5.96 &  16.50 &   3.59 &   5.70 &  47.86 &   6.77 &   8.12 &   5.66 &   5.81 &   5.88 &    6.2\\
 653 &   5.00 &   2.18 &   3.37 &   0.00 &   0.00 &   9.59 &   6.50 &   2.10 &   4.26 &   6.89 &   7.05 &   6.92 &    3.4\\
 654 &  94.25 &   9.93 &  10.48 &  43.00 &   6.54 &   7.61 & 131.75 &  11.23 &  12.77 &   6.07 &   5.97 &   6.04 &    6.5\\
 655 &   8.25 &   3.03 &   3.69 &  11.25 &   3.53 &   4.16 &  19.25 &   4.58 &   5.18 &   6.12 &   6.05 &   6.03 &    6.5\\
 656 &   4.00 &   1.94 &   3.15 &   2.25 &   1.57 &   2.38 &   6.50 &   2.10 &   4.26 &   5.85 &   6.02 &   5.80 &    5.9\\
 657 &  18.50 &   3.83 &   5.93 &  11.50 &   2.93 &   5.05 &  26.25 &   5.32 &   5.91 &   5.17 &   5.04 &   4.97 &    8.8\\
 658 &   8.50 &   2.46 &   4.60 &   4.50 &   2.44 &   2.65 &  17.00 &   4.09 &   5.20 &   7.09 &   6.98 &   7.04 &    2.2\\
 659 &   1.50 &   1.37 &   1.79 &   5.50 &   1.90 &   4.08 &   7.75 &   2.53 &   4.19 &   6.86 &   6.81 &   6.82 &    1.7\\
 660 &   6.75 &   2.35 &   4.01 &   2.75 &   1.41 &   3.16 &  10.00 &   3.12 &   4.26 &   6.36 &   6.33 &   6.41 &    5.0\\
 661 &   7.75 &   2.53 &   4.19 &   8.25 &   3.03 &   3.69 &  11.75 &   3.18 &   4.80 &   6.47 &   6.42 &   6.52 &    4.8\\
 662 &   4.25 &   2.19 &   2.90 &   5.75 &   2.15 &   3.83 &   8.00 &   2.78 &   3.94 &   6.48 &   6.43 &   6.52 &    4.8\\
 663 &  11.50 &   2.93 &   5.05 &   6.50 &   2.10 &   4.26 &  17.00 &   4.09 &   5.20 &   6.03 &   6.03 &   6.03 &    5.7\\
 664 &  12.50 &   3.07 &   5.19 &  13.25 &   3.82 &   4.44 &  22.50 &   5.16 &   5.26 &   5.99 &   5.86 &   5.94 &    7.2\\
 665 &   1.50 &   0.82 &   3.13 &   1.75 &   1.07 &   2.88 &   5.75 &   2.15 &   3.83 &   7.00 &   7.11 &   7.05 &    3.8\\
 666 &   0.50 &   0.50 &   1.33 &   2.50 &   1.82 &   2.13 &   4.75 &   1.93 &   3.62 &   6.71 &   6.66 &   6.67 &    4.9\\
 667 &  10.75 &   3.03 &   4.66 &  16.00 &   3.97 &   5.08 &  25.75 &   4.82 &   6.41 &   6.49 &   6.42 &   6.53 &    4.4\\
 668 &   7.75 &   2.53 &   4.19 &   2.25 &   1.57 &   2.38 &   8.00 &   2.78 &   3.94 &   6.97 &   7.10 &   7.04 &    3.9\\
 669 &  10.75 &   3.03 &   4.66 &  11.75 &   3.18 &   4.80 &  20.25 &   4.69 &   5.29 &   5.91 &   5.83 &   5.93 &    6.2\\
 670 &  68.50 &   7.79 &   9.84 &  39.75 &   6.05 &   7.62 & 109.25 &  10.68 &  11.22 &   6.51 &   6.46 &   6.56 &    4.5\\
 671 &   2.75 &   1.41 &   3.16 &  10.75 &   3.03 &   4.66 &  10.50 &   2.78 &   4.91 &   6.37 &   6.41 &   6.37 &    3.7\\
 672 &   5.75 &   2.15 &   3.83 &   7.00 &   2.60 &   3.76 &  14.86 &   3.70 &   5.10 &   5.92 &   5.82 &   5.94 &    6.1\\
 673 &   7.50 &   2.28 &   4.44 &   0.00 &   0.00 &  15.32 &   8.00 &   2.78 &   3.94 &   5.98 &   5.96 &   5.97 &    6.1\\
 674 &  15.25 &   4.09 &   4.70 &   3.25 &   1.91 &   2.66 &  21.25 &   4.81 &   5.40 &   5.91 &   5.66 &   5.78 &    7.7\\
 675 & 153.25 &  12.61 &  13.14 &  59.00 &   7.66 &   8.72 & 211.50 &  14.05 &  16.08 &   6.00 &   5.97 &   5.99 &    6.3\\
 676 & 228.25 &  15.34 &  15.87 &  73.75 &   8.34 &   9.89 & 304.25 &  17.68 &  18.20 &   6.25 &   6.18 &   6.28 &    5.5\\
 677 &   8.75 &   2.71 &   4.35 &   6.00 &   2.40 &   3.58 &  13.25 &   3.82 &   4.44 &   6.32 &   6.39 &   6.31 &    4.4\\
 678 &  11.25 &   3.53 &   4.16 &  15.00 &   3.84 &   4.95 &  27.25 &   5.42 &   6.01 &   6.35 &   6.47 &   6.40 &    5.4\\
 679 & 100.75 &   9.79 &  11.33 &  39.25 &   6.47 &   7.05 & 142.75 &  11.70 &  13.23 &   6.57 &   6.48 &   6.61 &    3.5\\
 680 &  12.00 &   3.43 &   4.55 &   6.75 &   2.35 &   4.01 &  17.75 &   3.96 &   5.57 &   6.53 &   6.49 &   6.59 &    3.5\\
 681 &   0.75 &   0.62 &   2.54 &   8.50 &   2.46 &   4.60 &   9.25 &   3.21 &   3.85 &   6.22 &   6.12 &   6.24 &    5.6\\
 682 &   9.75 &   2.87 &   4.51 &  10.25 &   3.37 &   4.01 &  18.50 &   3.83 &   5.93 &   5.77 &   5.47 &   5.61 &    8.7\\
 683 &  11.50 &   2.93 &   5.05 &   1.50 &   1.37 &   1.79 &  17.25 &   4.34 &   4.95 &   6.54 &   6.61 &   6.63 &    4.8\\
 684 & 162.57 &  12.33 &  14.22 &  39.00 &   6.22 &   7.30 & 203.14 &  14.38 &  15.13 &   5.99 &   5.86 &   5.98 &    9.9\\
 685 &  28.50 &   4.86 &   6.94 &   6.75 &   2.35 &   4.01 &  33.25 &   5.97 &   6.55 &   6.09 &   6.05 &   6.00 &    7.1\\
 686 &   3.00 &   1.66 &   2.91 &   8.00 &   2.78 &   3.94 &   7.75 &   2.53 &   4.19 &   5.87 &   5.73 &   5.81 &    8.2\\
 687 &  27.71 &   4.98 &   6.64 &  15.00 &   3.84 &   4.95 &  40.57 &   5.95 &   7.88 &   5.96 &   5.81 &   5.93 &   10.3\\
 688 &   9.75 &   2.87 &   4.51 &  12.00 &   3.43 &   4.55 &  21.75 &   4.41 &   6.01 &   5.93 &   5.88 &   5.91 &    7.0\\
 689 &  24.50 &   4.47 &   6.56 &  13.50 &   3.21 &   5.33 &  37.50 &   5.64 &   7.72 &   5.90 &   5.84 &   5.87 &    7.0\\
 690 &  21.75 &   4.41 &   6.01 &  17.25 &   4.34 &   4.95 &  40.00 &   6.30 &   7.37 &   6.25 &   6.32 &   6.35 &    5.1\\
 691 &  23.25 &   5.02 &   5.61 &  10.00 &   3.12 &   4.26 &  34.57 &   5.47 &   7.40 &   5.55 &   5.34 &   5.32 &    8.5\\
 692 &  36.75 &   5.81 &   7.38 &  17.25 &   4.34 &   4.95 &  52.00 &   7.19 &   8.25 &   6.33 &   6.20 &   6.24 &    7.9\\
 693 &  11.00 &   3.28 &   4.41 &   6.00 &   2.40 &   3.58 &  20.00 &   4.44 &   5.54 &   5.75 &   5.46 &   5.60 &    8.9\\
 694 & 103.50 &   9.69 &  11.73 &  24.25 &   5.12 &   5.71 & 128.75 &  11.10 &  12.64 &   6.74 &   6.72 &   6.69 &    5.8\\
 695 &   9.50 &   2.62 &   4.76 &  11.00 &   3.28 &   4.41 &  20.25 &   4.69 &   5.29 &   5.75 &   5.52 &   5.65 &    9.4\\
 696 & 256.00 &  15.99 &  17.02 &  69.50 &   7.85 &   9.90 & 328.75 &  17.88 &  19.41 &   6.29 &   6.26 &   6.29 &    5.4\\
 697 &  11.50 &   2.93 &   5.05 &   7.25 &   2.85 &   3.51 &  16.75 &   3.84 &   5.45 &   6.67 &   6.59 &   6.62 &    6.8\\
 698 &   6.00 &   2.40 &   3.58 &  10.25 &   3.37 &   4.01 &  15.00 &   3.84 &   4.95 &   6.90 &   7.04 &   6.98 &    3.8\\
 699 &   3.75 &   1.69 &   3.40 &   3.75 &   1.69 &   3.40 &   5.00 &   2.18 &   3.37 &   6.19 &   6.06 &   6.15 &    3.8\\
 700 &  15.00 &   3.84 &   4.95 &   6.00 &   2.40 &   3.58 &  18.00 &   4.21 &   5.32 &   6.66 &   6.80 &   6.72 &    3.4\\
 701 &  15.75 &   3.72 &   5.33 &   7.75 &   2.53 &   4.19 &  20.75 &   4.31 &   5.90 &   6.51 &   6.54 &   6.58 &    5.4\\
 702 &  46.50 &   6.34 &   8.40 &  22.50 &   4.27 &   6.36 &  67.25 &   8.42 &   8.97 &   6.68 &   6.57 &   6.72 &    2.7\\
 703 &   6.00 &   2.40 &   3.58 &   4.75 &   1.93 &   3.62 &   9.00 &   2.96 &   4.10 &   6.89 &   7.03 &   6.97 &    3.6\\
 704 &  16.75 &   3.84 &   5.45 &  12.50 &   3.07 &   5.19 &  27.25 &   5.42 &   6.01 &   5.06 &   4.82 &   4.94 &    8.5\\
 705 &   7.75 &   2.53 &   4.19 &   1.00 &   0.87 &   2.29 &   9.25 &   3.21 &   3.85 &   6.45 &   6.47 &   6.52 &    5.9\\
 706 &   8.75 &   2.71 &   4.35 &   0.00 &   0.00 &   1.83 &  12.75 &   3.32 &   4.94 &   6.45 &   6.39 &   6.40 &    5.6\\
 707 &  14.50 &   3.34 &   5.45 &  24.00 &   4.87 &   5.96 &  35.00 &   5.89 &   6.97 &   6.22 &   6.17 &   6.24 &    8.1\\
 708 &  33.50 &   5.31 &   7.38 &  29.25 &   5.61 &   6.19 &  59.00 &   7.66 &   8.72 &   5.65 &   5.65 &   5.60 &    8.3\\
 709 &  37.25 &   6.31 &   6.88 &   3.00 &   1.66 &   2.91 &  40.25 &   6.55 &   7.12 &   6.53 &   6.47 &   6.59 &    6.8\\
 710 &  14.25 &   3.96 &   4.58 &  11.25 &   3.53 &   4.16 &  26.25 &   5.32 &   5.91 &   5.82 &   5.83 &   5.96 &    6.5\\
 711 &  17.00 &   4.09 &   5.20 &   3.00 &   1.66 &   2.91 &  21.25 &   4.81 &   5.40 &   6.37 &   6.26 &   6.39 &    2.0\\
 712 &   6.75 &   2.35 &   4.01 &  20.00 &   4.44 &   5.54 &  30.75 &   5.30 &   6.87 &   6.50 &   6.53 &   6.57 &    5.6\\
 713 &   5.75 &   2.15 &   3.83 &   0.00 &   0.00 &  14.68 &   4.00 &   1.94 &   3.15 &   6.77 &   6.77 &   6.75 &    5.0\\
 714 &  44.00 &   6.61 &   7.68 &  11.50 &   2.93 &   5.05 &  54.00 &   7.33 &   8.39 &   6.80 &   6.80 &   6.77 &    4.8\\
 715 &   9.57 &   2.69 &   4.69 &   6.14 &   2.54 &   3.43 &  12.43 &   3.86 &   4.13 &   5.49 &   5.38 &   5.44 &    8.7\\
 716 &  57.50 &   7.10 &   9.16 &  22.00 &   4.66 &   5.76 &  79.50 &   8.43 &  10.48 &   6.47 &   6.62 &   6.67 &    1.9\\
 717 &   5.50 &   2.68 &   2.87 &  12.25 &   3.68 &   4.30 &  11.75 &   3.18 &   4.80 &   6.39 &   6.36 &   6.45 &    5.2\\
 718 &   3.25 &   1.91 &   2.66 &   0.00 &   0.00 &   7.86 &   4.75 &   1.93 &   3.62 &   5.99 &   6.04 &   6.14 &    4.0\\
 719 &  47.43 &   7.27 &   7.47 &  38.00 &   6.14 &   7.22 &  79.50 &   8.43 &  10.48 &   5.47 &   5.37 &   5.42 &    8.9\\
 720 &  30.75 &   5.30 &   6.87 &  21.50 &   4.16 &   6.26 &  54.50 &   6.90 &   8.96 &   4.96 &   4.77 &   4.87 &    9.9\\
 721 &  50.50 &   6.62 &   8.69 &  23.25 &   5.02 &   5.61 &  72.25 &   8.72 &   9.27 &   6.76 &   6.89 &   6.89 &    2.7\\
 722 &  13.50 &   3.21 &   5.33 &  21.00 &   4.56 &   5.65 &  31.50 &   5.13 &   7.21 &   6.06 &   5.96 &   5.98 &    6.9\\
 723 &  16.25 &   4.22 &   4.83 &   5.25 &   2.43 &   3.12 &  25.00 &   4.97 &   6.06 &   5.98 &   5.83 &   5.89 &    8.7\\
 724 &  45.00 &   6.69 &   7.76 &  17.25 &   4.34 &   4.95 &  62.75 &   7.67 &   9.23 &   6.61 &   6.64 &   6.62 &    6.6\\
 725 &   6.00 &   2.40 &   3.58 &  11.00 &   3.28 &   4.41 &  10.75 &   3.03 &   4.66 &   6.52 &   6.30 &   6.52 &    3.0\\
 726 &   6.00 &   2.40 &   3.58 &  15.75 &   3.72 &   5.33 &  22.50 &   4.27 &   6.36 &   6.74 &   6.87 &   6.87 &    2.9\\
 727 &   3.00 &   1.66 &   2.91 &   8.00 &   2.78 &   3.94 &  16.75 &   3.84 &   5.45 &   6.52 &   6.31 &   6.52 &    3.0\\
 728 &  14.25 &   3.96 &   4.58 &   1.00 &   0.87 &   2.29 &  14.25 &   3.96 &   4.58 &   6.75 &   6.61 &   6.79 &    0.6\\
 729 &   1.50 &   0.82 &   3.13 &   2.25 &   1.57 &   2.38 &   2.25 &   1.57 &   2.38 &   6.43 &   6.59 &   6.50 &    4.8\\
 730 &  39.50 &   5.80 &   7.87 &  34.50 &   5.39 &   7.47 &  67.25 &   8.42 &   8.97 &   5.84 &   5.62 &   5.47 &    8.3\\
 731 &   2.50 &   1.16 &   3.41 &   8.50 &   2.46 &   4.60 &   8.25 &   3.03 &   3.69 &   6.78 &   6.65 &   6.82 &    0.5\\
 732 &   8.50 &   2.46 &   4.60 &   7.50 &   3.10 &   3.26 &  15.00 &   3.84 &   4.95 &   6.74 &   6.55 &   6.76 &    0.6\\
 733 &  74.75 &   8.40 &   9.95 &  44.75 &   6.44 &   8.01 & 117.75 &  10.60 &  12.14 &   5.56 &   5.38 &   5.47 &   10.5\\
 734 &  20.75 &   4.31 &   5.90 &  13.00 &   3.57 &   4.69 &  32.75 &   5.47 &   7.05 &   6.46 &   6.34 &   6.44 &    4.6\\
 735 &   4.75 &   1.93 &   3.62 &   0.00 &   0.00 &   9.11 &   7.00 &   2.60 &   3.76 &   5.91 &   5.90 &   5.86 &    5.7\\
 736 &  13.75 &   3.46 &   5.08 &  15.25 &   4.09 &   4.70 &  29.00 &   5.36 &   6.44 &   5.71 &   5.58 &   5.51 &    8.2\\
 737 &  42.75 &   6.29 &   7.86 &  15.75 &   3.72 &   5.33 &  61.50 &   7.36 &   9.41 &   6.72 &   6.61 &   6.74 &    2.5\\
 738 &   7.00 &   2.60 &   3.76 &   7.75 &   2.53 &   4.19 &  12.75 &   3.32 &   4.94 &   6.43 &   6.32 &   6.43 &    4.9\\
 739 &   5.00 &   2.18 &   3.37 &   5.25 &   2.43 &   3.12 &  11.50 &   2.93 &   5.05 &   6.26 &   6.29 &   6.34 &    3.3\\
 740 &   4.75 &   1.93 &   3.62 &  17.00 &   4.09 &   5.20 &  16.25 &   4.22 &   4.83 &   6.25 &   6.18 &   6.27 &    7.9\\
 741 &   6.75 &   2.35 &   4.01 &   4.50 &   1.68 &   3.87 &  10.75 &   3.03 &   4.66 &   6.89 &   6.64 &   6.82 &    0.8\\
 742 &  43.25 &   6.79 &   7.36 &  28.50 &   4.86 &   6.94 &  71.75 &   8.22 &   9.77 &   6.40 &   6.46 &   6.44 &    7.8\\
 743 &  23.75 &   4.62 &   6.21 &   9.25 &   3.21 &   3.85 &  34.25 &   6.06 &   6.63 &   6.35 &   6.28 &   6.32 &    7.8\\
 744 &  11.75 &   3.18 &   4.80 &  82.75 &   8.85 &  10.39 &  96.75 &   9.59 &  11.13 &   6.46 &   6.37 &   6.39 &    7.4\\
 745 & 117.00 &  10.81 &  11.85 &  38.50 &   6.64 &   6.72 & 159.00 &  12.60 &  13.63 &   6.25 &   6.20 &   6.28 &    6.8\\
 746 &  68.50 &   7.79 &   9.84 &  29.00 &   5.36 &   6.44 &  96.75 &   9.59 &  11.13 &   5.85 &   5.73 &   5.94 &    6.6\\
 747 &   9.75 &   2.87 &   4.51 &  26.00 &   5.07 &   6.16 &  37.57 &   5.72 &   7.64 &   6.51 &   6.63 &   6.56 &    6.9\\
 748 &   5.75 &   2.15 &   3.83 &  13.25 &   3.82 &   4.44 &  19.25 &   4.58 &   5.18 &   6.40 &   6.36 &   6.46 &    6.3\\
 749 &  14.25 &   3.96 &   4.58 &   0.00 &   0.00 &  15.18 &  17.71 &   3.93 &   5.60 &   6.18 &   6.31 &   6.16 &    7.0\\
 750 &  26.00 &   5.07 &   6.16 &   9.50 &   2.62 &   4.76 &  34.50 &   5.39 &   7.47 &   6.44 &   6.58 &   6.49 &    6.6\\
 751 &  91.25 &   9.78 &  10.32 &  43.75 &   6.36 &   7.93 & 136.25 &  11.90 &  12.44 &   5.54 &   5.59 &   5.74 &    6.2\\
 752 &   0.00 &   0.00 &   1.83 &   4.50 &   1.68 &   3.87 &   6.50 &   2.10 &   4.26 &   6.00 &   5.94 &   5.99 &    2.0\\
 753 & 258.00 &  16.05 &  17.08 &  70.25 &   8.60 &   9.15 & 328.00 &  18.10 &  19.13 &   6.45 &   6.58 &   6.50 &    7.0\\
 754 &  11.00 &   3.28 &   4.41 &  10.75 &   3.03 &   4.66 &  18.75 &   4.08 &   5.68 &   6.19 &   6.29 &   6.23 &    7.0\\
 755 &  28.75 &   5.11 &   6.69 &  25.00 &   4.97 &   6.06 &  53.50 &   6.83 &   8.89 &   6.19 &   6.02 &   6.13 &    7.7\\
 756 &   5.00 &   2.18 &   3.37 &   6.00 &   2.40 &   3.58 &  13.75 &   3.46 &   5.08 &   6.25 &   6.09 &   6.24 &    7.8\\
 757 &  14.50 &   3.34 &   5.45 &   0.00 &   0.00 &   8.91 &  12.00 &   3.43 &   4.55 &   3.16 &   3.06 &   3.11 &    6.9\\
 758 &   6.25 &   2.65 &   3.33 &   2.50 &   1.82 &   2.13 &   9.50 &   2.62 &   4.76 &   6.11 &   6.04 &   6.10 &    5.1\\
 759 &  25.75 &   4.82 &   6.41 &  14.50 &   3.34 &   5.45 &  37.50 &   5.64 &   7.72 &   6.45 &   6.54 &   6.59 &    4.8\\
 760 &  24.00 &   4.87 &   5.96 &  25.75 &   4.82 &   6.41 &  45.75 &   6.51 &   8.08 &   5.65 &   5.77 &   5.66 &    9.0\\
 761 &  49.25 &   7.23 &   7.79 &  28.50 &   4.86 &   6.94 &  75.25 &   8.90 &   9.45 &   6.35 &   6.32 &   6.39 &    3.5\\
\tableline
\end{tabular}
\end{small}
\footnotesize
\end{table}

